Finite-Cliquewidth Sets of Existential Rules: Toward a General Criterion for Decidable yet Highly Expressive Querying

In our pursuit of generic criteria for decidable ontology-based querying, we introduce 'finite-cliquewidth sets' (FCS) of existential rules, a model-theoretically defined class of rule sets, inspired by the cliquewidth measure from graph theory. By a generic argument, we show that FCS ensures decidability of entailment for a sizable class of queries (dubbed 'DaMSOQs') subsuming conjunctive queries (CQs). The FCS class properly generalizes the class of finite-expansion sets (FES), and for signatures of arity at most 2, the class of bounded-treewidth sets (BTS). For higher arities, BTS is only indirectly subsumed by FCS by means of reification. Despite the generality of FCS, we provide a rule set with decidable CQ entailment (by virtue of first-order-rewritability) that falls outside FCS, thus demonstrating the incomparability of FCS and the class of finite-unification sets (FUS). In spite of this, we show that if we restrict ourselves to single-headed rule sets over signatures of arity at most 2, then FCS subsumes FUS.

==> ICDT 2023 Updated LaTeXFiles/appendices/fo-well-decoration.tex <==
\section{Definition of $\Phi_\mathrm{well}$ (\NoCaseChange{\cref{sec:cwdef}})}

Recall that a decorated tree $\mathcal{T}$ is called a \emph{well-decorated tree} \iffi
\begin{itemize}
\item for every null $s \in \{0,1\}^*$, $\mathcal{T}$ contains exactly one fact $\mathrm{Dec}(s)$ with  $\mathrm{Dec} \in \decorum$,
\item for every $\const{c}\in \mathrm{Cnst}$, $\mathcal{T}$ contains at most one fact of the form $\pred{c}_k(s)$,
%%%
%% THE FOLLOWING MODIFICATION WAS PLAIN WRONG AND HAS BEEN REVERTED -- DO NOT REINTRODUCE!!!
%%
%% \item for every null $s \in \{0,1\}^*$ and every $c\in \mathrm{Cnst}$, $\mathcal{T}$ contains at most one fact of the form $c_k(s)$;
%%
%% NOTE THAT CONSTANTS NEED TO BE UNIQUE ACROSS THE WHOLE MODEL!!!
%%%
\item if $\pred{Add}_{\rpred,\vk}(s) \in \mathcal{T}$ or $\pred{Recolor}_{k\to k'}(s) \in \mathcal{T}$,
       then $\pred{Void}(s0)\not\in \mathcal{T}$ and $\pred{Void}(s1) \in \mathcal{T}$,
\item if $\oplus(s) \in \mathcal{T}$, then $\pred{Void}(s0),\pred{Void}(s1) \not\in \mathcal{T}$,
\item if $\pred{Void}(s) \in \mathcal{T}$ or $\pred{c}_k(s) \in \mathcal{T}$, then  $\pred{Void}(s0),\pred{Void}(s1) \in \mathcal{T}$.
%\item if $\pred{Recolor}_{k\to k'}(s) \in \mathcal{T}$\!, $\pred{Add}_{\rpred,k,k'}(s) \in \mathcal{T}$\!, or $\pred{Add}_{\rpred,k}(s) \in \mathcal{T}$\!, then $\pred{Void}(s0)\not\in \mathcal{T}$ and $\pred{Void}(s1) \in \mathcal{T}$.

\end{itemize}

Here, fixing $\cols$, $\Sigma$, and $\mathrm{Cnst}$,  we will define a first-order sentence $\Phi_\mathrm{well}$ such that for any $(\cols,\mathrm{Cnst},\Sigma)$-decorated tree $\mathcal{T}$, $\mathcal{T}$ is well-decorated \ifandonlyif $\mathcal{T} \models \Phi_\mathrm{well}$. 

Let us denote $\decorum$ with $\Gamma$ and we write $\varphi^i_{\pred{Void}}(x)$ to abbreviate $\exists z (\pred{Succ}_i(x,z) \wedge \pred{Void}(z))$. 
Consider the following (where $\pred{c} \in \mathrm{Cnst}$, $\pred{d} \in \mathrm{Cnst} \cup\{\pred{*}\}$):
\begin{align*}
    \Phi^{\mathrm{funct}} &= \forall{x} \bigvee_{\mathrm{Dec} \in \Gamma}\Big( \mathrm{Dec}(x) \wedge \scaleobj{0.8}{\bigwedge_{\scaleobj{1.25}{\mathrm{Dec}' \in \Gamma \setminus \{\mathrm{Dec}\}}}} \neg\mathrm{Dec}'(x) \Big)\\ 
    %
    \Phi^{\mathrm{unique}}_{\pred{c}_k} &=  \forall{xy}\; \pred{c}_k(x) \Rightarrow (\pred{c}_k(y) \Rightarrow x = y) \wedge \bigwedge_{k'\in \cols\setminus\{k\}}\neg\pred{c}_{k'}(y)\\
\end{align*}
\begin{align*}
    %
    \Phi_{\pred{d}_k} &=  & \forall{x}\; \pred{d}_k(x) & \Rightarrow \ \ \varphi^0_{\pred{Void}}(x) \wedge \varphi^1_{\pred{Void}}(x)\\
    %
    \Phi_{\pred{Add}_{\rpred,\vk}} &= & \forall{x}\; \pred{Add}_{\rpred,\vk}(x) & \Rightarrow \neg \varphi^0_{\pred{Void}}(x) \wedge \varphi^1_{\pred{Void}}(x)\\
    %
    \Phi_{\pred{Recolor}_{k\to k'}} &= & \forall{x}\; \pred{Recolor}_{k\to k'}(x) & \Rightarrow \neg \varphi^0_{\pred{Void}}(x) \wedge \varphi^1_{\pred{Void}}(x)\\
    %
    \Phi_{\oplus} &= & \forall{x}\; \oplus(x) & \Rightarrow \neg \varphi^0_{\pred{Void}}(x) \wedge \neg\varphi^1_{\pred{Void}}(x)\\
    %
    \Phi_{\pred{Void}} &= &\forall{x}\; \pred{Void}(x) & \Rightarrow \ \ \varphi^0_{\pred{Void}}(x) \wedge \varphi^1_{\pred{Void}}(x)\\
\end{align*}
%
Then we let 
$$
\Phi_\mathrm{well} = 
\Phi^{\mathrm{funct}} \wedge 
\hspace{-3ex}\bigwedge_{\hspace{3ex}\pred{c}_k\in \Gamma,\,\pred{c} \in \mathrm{Cnst}}\hspace{-3ex} \Phi^{\mathrm{unique}}_{\pred{c}_k} \wedge 
\bigwedge_{\mathrm{Dec}\in \Gamma} \Phi_{\mathrm{Dec}}.
$$
%$$\Phi_{\mathrm{Dec}}
%    \bigwedge_{\pred{c}_k\in \Gamma} \Phi_{\pred{c}_k}
%    \bigwedge_{\pred{Add}_{\rpred,\vk} \in \Gamma} \Phi_{\pred{Add}_{\rpred,\vk}}
%    \bigwedge_{\pred{Recolor}_{k\to k'} \in \Gamma} \Phi_{k\to k'} \wedge
%    \Phi_{\oplus} \wedge
%    \Phi_{\pred{Void}} $$

==> ICDT 2023 Updated LaTeXFiles/appendices/multihead-full.tex <==
\section{Extended Version of \NoCaseChange{\cref{sec:higher-arity}}}\label{appendix:higher-arity}

We will now prove \cref{thm:higher-arity} implying that for multi-headed rules, $\fus$ is no longer subsumed by $\fcs$. To this end, we exhibit a $\fus$ rule set which may unavoidably lead to universal models of infinite cliquewidth. 

We let $\sigi = \set{\hpred, \vpred}$ with $\hpred$ and $\vpred$ being binary predicates. Let us define $\rsgrid$ to be the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} & \top & \rightarrow \exists x \; (\hpred(x,x) \land \vpred (x,x)) \\[0.5ex]
\text{(grow)} & \top & \rightarrow \exists y \exists y'\; (\hpred(x,y) \land \vpred (x,y')) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists y' \; (\hpred(x',y') \land \vpred(y,y'))
\end{array}
$$

We make use of $\rsgrid$ to establish \cref{thm:higher-arity}, whose proof is split into two parts. First, we provide a database $\dbg$ to form a knowledge base $(\dbg, \rsg)$ for which no universal model of finite cliquewidth exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\subsection{$\rsgrid$ is not a finite-cliquewidth set}

We devote this section to establishing the subsequent lemma, which is sufficient to conclude \cref{lem:no-universal-model-cw}.

\begin{lemma}\label{lem:no-universal-model-cw-intermediate}
Let $\const{a}$ be a constant and let $\dbg = \set{\top(\const{a})}$ be a database. Then, no universal model of finite cliquewidth exists for $\kbaseg$.
\end{lemma}


With the aim of establishing the lemma above, we define the instance $\ginf$ below, where $\const{a}$ is a constant and $x_{i,j}$ and $y$ are nulls for $i,j \in \mathbb{N}$. To provide the reader with further intuition, a graphical depiction of $\ginf$ is given in \cref{fig:ginf}.
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{img/ginf.pdf}
%    \vspace{-1ex}
%    \caption{ The instance $\ginf$.}
%    \label{fig:ginf}
%\end{figure}
%
\begin{eqnarray*}
\ginf & = & \{\top(\const{a}),\hpred(\const{a},x_{1,0}),\vpred(\const{a},x_{0,1}),\hpred(y,y),\vpred(y,y)\} \\
 & & \cup \big\{\hpred(x_{i,j},x_{i+1,j}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} \\
 & & \cup \big\{\vpred(x_{i,j},x_{i,j+1}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} 
\end{eqnarray*}


%\begin{figure}[H]
%    \centering
%    \includegraphics[width=\linewidth]{img/ginf.pdf}
%    \caption{ The instance $\ginf$.}
%    \label{fig:ginf}
%\end{figure}

It is straightforward to show that $\ginf$ serves as a model of $\kbaseg$, and a routine exercise to prove that $\ginf$ is universal. Hence, we have the following:

\begin{observation}\label{obs:ginf-is-universal-model}
$\ginf$ is a universal model of $\kbaseg$.
\end{observation}

%\begin{proof} Let $\model = (\dom,\inter)$ be any model of $\kbaseg$. Then, it follows that (i) $\inter(a) \in \inter(\origin)$, (ii) there exists some $d_{0} \in \dom$ such that $d \in \inter[d/x](\hpred) \cap \inter[d/x](\vpred)$, (iii) for any $d_{1} \in \dom$, there exist $d_{2}, d_{3} \in \dom$ such that $(\inter(d_{1})\inter(d_{2}) \in \inter(\hpred)$ and $(\inter(d_{1})\inter(d_{3}) \in \inter(\vpred)$, and (iv) for any $d_{4}, d_{5}, d_{6} \in \dom$, if $(d_{4},d_{5}) \in \inter(\hpred)$ and $(d_{4},d_{6}) \in \inter(\vpred)$, then there exists a $d_{7} \in \dom$ such that 
%\end{proof}


%It is well known~\cite{} that all grid like structures have infinite cliquewidth. 
%\thomas{The original proof for (undirected!) grids w.r.t. cliquewidth was done in \cite[\thm~4]{GolumbicRot99}, where grids are considered as (undirected) graphs. We probably(?) should be ``careful'' here since we have two types of edges and are in the directed setting. It's not that it wouldn't work or anything... But we probably should make a short argument why it does hold here.}

%It is well known that infinite grids over a signature consisting of single binary relation have infinite cliquewidth (see \cite[\thm~4]{GolumbicRot99} for the reference). Consider the following:

%It is known that \thomas{Change to finite!} infinite grids constructed over a signature with a single binary relation have infinite cliquewidth~\cite[\thm~4]{GolumbicRot99}. By making use of this fact, and the subsequent two claims, we can prove \cref{fact:grid-has-unbounded-cw} below.

It is known that the cliquewidth of an $n \times n$ grid tends to infinity as $n$ tends to infinity~\cite[\thm~4]{GolumbicRot99}, entailing that any infinite grid will have an infinite cliquewidth since the cliquewidth of any instance bounds the cliquewidth of any induced sub-instance from above. By making use of this fact, along with the subsequent two, we can prove \cref{fact:grid-has-unbounded-cw} below.

\begin{fact}
        Let $\sig$ be a binary signature, $\epred$ be a binary predicate, 
        $\inst$ be an instance over $\sig$, and $\inst' = \set{\epred(t,t') \ | \ \rpred(t,t') \in \inst, \rpred \in \sig}$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}

    
\begin{fact}
        Let $\sig$ be a signature consisting of a single binary predicate $\epred$, let $\inst$ be an instance over $\sig$, and let $\inst' = \set{\epred(t',t) \ | \ \epred(t,t') \in \inst} \cup \inst$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}



\begin{observation}\label{fact:grid-has-unbounded-cw}
$\ginf$ has an infinite cliquewidth.
\end{observation}
\begin{proof} The observation follows from the previous two facts, the fact that infinite grids have infinite cliquewidth, and the fact that adding a set of the form $\{\hpred(y, y), \vpred(y, y) \}$ with $\const{a}$ a constant and $y$ a null to any instance does not lower its cliquewidth.
\end{proof}

We now leverage the above result to demonstrate that {\em every} universal model of $\kbaseg$ has an infinite cliquewidth. Observe that if we consider any homomorphism from $\ginf$ to itself, then (i) the null $y$ must be mapped to itself as no other terms are associated with loops, and (ii) the constant $a$ must be mapped to itself, thus anchoring the image of $\ginf$ under the homomorphism at the origin of the grid shown in \cref{fig:ginf}, thus ensuring that each term of the grid will map to itself accordingly. It follows that any homomorphism from $\ginf$ to itself will be the identity function, giving rise to the following observation.

\begin{observation}\label{obs:identity}
If $h: \ginf \to \ginf$ is a homomorphism then $h$ is the identity.
\end{observation}

We now make use of the above observation to show that every universal model of $\kbaseg$ contains a sub-instance that is isomorphic to $\ginf$, thus ensuring that every universal model of $\kbaseg$ is of infinite cliquewidth (by \cref{fact:grid-has-unbounded-cw} and the fact that the cliquewidth of an instance is greater than or equal to the cliquewidth of any induced sub-instance). From this lemma, we may conclude  \cref{lem:no-universal-model-cw-intermediate} and thus \cref{lem:no-universal-model-cw}.

\begin{lemma}
Every universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$.
\end{lemma}

\begin{proof}
Let $\unimod$ be a universal model of $\kbaseg$. As $\ginf$ is a universal model (by \cref{obs:ginf-is-universal-model} above), we know that two homomorphisms $h\colon \ginf \to \unimod$ and $h'\colon \unimod \to \ginf$ exist between $\unimod$ and $\ginf$. Let us consider the homomorphism $h' \circ h$. By \cref{obs:identity}, the homomorphism $h'\circ h$ is the identity on $\ginf$, implying that $h$ is injective. Furthermore, $h$ is reflective, and hence, constitutes an embedding. To show this, suppose that $\rpred\in\sigi$ and let $\vt$ be a tuple of length $\arity{\rpred}$ from $\ginf$. If $\rpred(h(\vt))$ holds in $\unimod$ , then $\rpred((h' \circ h)(\vt))$ holds in $\ginf$, but since $h'\circ h$ is the identity on $\ginf$, we immediately obtain that $\rpred(\vt)$  holds in $\ginf$. Finally, note that the image of $\ginf$ under $h$ serves as the induced sub-instance of $\unimod$ that is isomorphic to $\ginf$, completing the proof.
\end{proof}



\subsection{$\rsgrid$ is a finite-unification set}

As we have now shown that $\rsgrid$ is not a finite-cliquewidth set, we focus our attention on demonstrating \cref{lem:rsg-is-fus}, which is restated below, and from which we may conclude the final main result (\cref{thm:higher-arity}).

\begin{customlem}{\ref{lem:rsg-is-fus}}
$\rsg$ is $\fus$.
\end{customlem}

As the rule $(loop)$ is a member of $\rsg$, every BCQ that is free of constants can be trivially re-written, implying the following:

\begin{observation}\label{obs:bcq-no-const-trivial}
Every BCQ that is free of constants is FO-rewritable with respect to $\rsg$.
\end{observation}

%\piotr{Here is a link for Xrewrite \url{https://arxiv.org/pdf/1405.2848.pdf}}

Showing that a provided rule set is $\fus$ is a notoriously difficult task.\footnote{This should not be too surprising however, as being $\fus$ is an undecidable property~\cite{BagLecMugSal11}.} To this end, we hand-tailor a rewriting algorithm to be used for the proof of~\cref{lem:rsg-is-fus}. However, one can refer to existing rewriting algorithms, e.g., XRewrite~\cite{GotOrsPie14}, for additional intuition. Finally, it is important to note that the proof closely follows the ideas provided in \cite{OstMarCarRud22}.


\subsection{Necessary definitions}

%As we are considering a binary signature, we will treat queries as graphs with the company of standard graph theoretic notions. \thomas{Does this suffice or would Reviewer 2 state: ``The term \emph{graph} has not been defined. Suggest strong reject.''?}

%Since each CQ can be viewed as an instance, and each instance can be viewed as a structure (see \tim{Sect ?}), we will hereafter interpret queries as their corresponding structures. Moreover, we note that since the signature $\sigi$ contains only binary predicates, we can view queries as directed, binary graphs.

We first introduce special queries, referred to as \emph{marked queries}, which are queries supplemented with a set of markings, the significance of which, is to keep track of what terms of the CQs are mapped to constants in a given database throughout the course of rewriting. A marked CQ is defined to be a pair $(q, M)$ where $q$ is a CQ and the set of markings $M$ is a subset of terms (i.e., variables and constants) of $q$. Given an instance $\inst$ we say that $\inst \models (q,M)$ $\iffi$ there exists a homomorphism $h$ mapping $q$ to $\inst$ such that for every term $t$ of $q$ we have $t \in M$ $\iffi$ $h(t)$ is a constant in $\inst$.

We now make a useful observation, which follows by considering the structures that arise when applying the rules from $\rsgrid$ to any given database. Afterward, we show that marked queries take on a special form when interpreted on the instance $\sg$, where $\db$ is an arbitrary database.

\begin{observation}\label{obs:buildup-for-properly-marked-chase}
Let $\db$ be a database. Then,
\begin{itemize}
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom of $\sg$ and $t'\in \adom{\db}$, then $t\in \adom{\db}$,
    \item if there is a cycle $C \subseteq \sg$ that contains at least one constant, then $C \subseteq \db$,
    \item if $\rpred(t_1,t'), \rpred(t_2,t') \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1\in  \adom{\db}$, then $t_2\in  \adom{\db}$,
    \item if $\rpred(\const{a},t), \rpred(\const{b},t) \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $\const{a}\neq \const{b}$ are constants, then $t$ is a constant.
\end{itemize}
\end{observation}

Keeping the above observation in mind, we define the notion of a {\em properly marked CQ}.

\begin{definition}\label{def:properly-marked}
A marked CQ $(q, M)$ is {\em properly marked} when:
\begin{itemize}
    \item if $\const{a}$ is a constant in $q$, then $\const{a} \in M$,
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom in $q$ and $t' \in M$, then $t \in M$,
    \item if there is a cycle $C$ in $q$ that contains at least one constant, then all terms of $C$ are contained in $M$,
    \item if $\rpred(t_1,t')$ and $\rpred(t_2,t')$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1 \in M$, then $t_2 \in M$,
    \item if $\rpred(\const{a},t)$ and $\rpred(\const{b},t)$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $\const{a}\neq \const{b}$ are constants, then $t \in M$.\defend
\end{itemize}
\end{definition}

\begin{observation}\label{obs:query-extendable-properly-marked}
If $\sg \models q$, then there exists a set of markings $M$ such that $(q,M)$ is properly marked and $\sg \models (q,M)$.
\end{observation}

\begin{proof} Suppose that $\sg \models q$. Then, we know that a homomorphism $h$ exists mapping terms from $q$ into $\sg$. Let $M$ be the set of terms from $q$ such that $h(t)$ is mapped to a constant in $\sg$. One can readily check if $(q,M)$ is properly marked, and if not, add the terms from $q$ to $M$ accordingly until a properly marked CQ $(q,M')$ is constructed such that $\sg \models (q,M)$.
\end{proof}

From \cref{obs:buildup-for-properly-marked-chase} and \cref{def:properly-marked} we immediately conclude the following:

\begin{corollary}
Let $(q, M)$ be a marked query, and $\db$ be any database. If $\sg \models \mq$, then $\mq$ is properly marked.
\end{corollary}

Let us refer to a marked CQ $(q, M)$ as {\em alive} given that it is properly marked and $M$ does not contain all terms of $q$. In the case where every term of a properly marked CQ is marked, we refer to the CQ as {\em dead}.

To prove~\cref{lem:rsg-is-fus} it suffices to prove the following lemma, which we direct our attention to in the subsequent section. 

\begin{lemma}\label{lem:rsg-is-fus-reformulated}
For any properly marked CQ $(q, \prmark)$ there exists a set of dead queries $\fcn{rew}(q,\prmark)$ such that for any database $\db$ the following holds: 
\begin{center}
$\sg \models (q,\prmark)$ \ $\iffi$ \ $\exists{Q' \in \fcn{rew}(q, \prmark)}, \db \models Q'.$
\end{center}
\end{lemma}

\subsection{Rewriting Alive Queries}

We begin this section by proving the following lemma, which will later prove useful in rewriting queries relative to $\rsgrid$.

\begin{lemma}\label{lem:exists-maximal}
%For every alive CQ there exists at least one variable with no out-going edges.
If a marked CQ $(q,\prmark)$ is alive, then there exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{lemma}
\begin{proof} Let the marked CQ $(q,\prmark)$ be alive. Then, by the definition above, we know that there exists a set of terms in $q$ that are not a members of $M$. Since $(q,\prmark)$ is properly marked, by \cref{def:properly-marked}, we know that all such terms are not constants, and hence, all such terms must be variables. Let us refer to all such terms as \emph{unmarked variables}. If we consider the sub-instance of the CQ induced by all unmarked variables, we can see that (i) it forms a directed acyclic graph as all cycles of the CQ must be in $M$ by \cref{def:properly-marked}, which (ii) is non-empty as $(q,\prmark)$ is alive. Hence, there must exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$, which corresponds to a sink in the directed acyclic graph described above.
\end{proof}

We will refer to unmarked variables -- such as those described in the above proof -- which possess no out-going edges, as {\em maximal}. These maximal variables will be used to initiate our rewriting process. 

\begin{lemma}\label{lem:maximal-cases}
Let $x$ be a maximal variable of an alive CQ $(q, \prmark)$. Then, one of the following holds:
\begin{enumerate}
    \item \label{lem:maximal-cases-one} $x$ occurs in exactly one atom  $\rpred(t,x)$, with $\rpred\in \{\hpred,\vpred\}$ for some term $t$ of $q$,
    \item \label{lem:maximal-cases-two} $x$ occurs in exactly two atoms $\hpred(t_{\hpred},x)$ and $\vpred(t_{\vpred},x)$ for some terms $t_{\hpred},t_{\vpred}$ of $q$,
    \item \label{lem:maximal-cases-three} there exist at least two distinct terms $t\neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are atoms of $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{enumerate}
\end{lemma}

%Now, in the light~\cref{lem:maximal-cases} we will present four operations that when combined will compute rewritings required by \cref{lem:rsg-is-fus-reformulated}.

\medskip
\noindent
{\bf Rewriting Operations.}
We now make use of~\cref{lem:maximal-cases} to define three operations that compute rewritings. When exhaustively applied to a query, we obtain the rewritings required by \cref{lem:rsg-is-fus-reformulated}. Given an alive CQ $(q, \prmark)$ we define the following three operations:

\begin{definition}[$\cutop$]\label{def:cut}
Let $x$ be a maximal variable of $(q, \prmark)$ satisfying case \ref{lem:maximal-cases-one} of \cref{lem:maximal-cases}, i.e., $x$ occurs in exactly one atom $\rpred(t,x)$ of $q$ with $\rpred\in \{\hpred, \vpred\}$. Then, letting $\query = \query' \cup \{\rpred(t,x)\}$, we define
\[
  \ \ \ \ \cutop((q,\prmark), \set{x}) =
  \begin{cases}
     (q' \cup \{\top(\const{c})\}, \prmark)  & \text{if $t$ is a constant $\const{c}$} \\[-1ex]
      & \text{not occurring in $\query'$;}\ \ \ \ \ \ \\
     (q', \prmark) & \text{otherwise.}\defend
  \end{cases}
\]
%Then, $\cutop((q,\prmark), \set{x}) = (q', \prmark)$, where $q'$ is the sub-query of $q$ with the atom containing $x$ removed.
\end{definition}


\begin{definition}[$\reduceop$]\label{def:reduce}
Let $x, t_{\hpred}$, and $t_{\vpred}$ be as in case \ref{lem:maximal-cases-two} of \cref{lem:maximal-cases}, meaning that there exist two atoms of the form $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ in $q$. We define $q'$ to be the same as $q$, but where $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ are replaced by $\hpred(x', t_{\vpred})$ and $\vpred(x', t_{\hpred})$, and where $x'$ is fresh. We now %by replacing $\hpred(t_{\hpred}, x),\vpred(t_{\vpred}, x)$ with $\hpred(x', t_{\vpred}), \vpred(x', t_{\hpred})$, where $x'$ is a fresh variable. 
 define $\reduceop((q,\prmark), \set{x}) = \set{ (q', \prmark), (q', \prmark \cup \set{x'})}$.\defend
\end{definition}

\begin{definition}[$\mergeop$]\label{def:merge}
Let $x, t$, and $t'$ be as in case \ref{lem:maximal-cases-three} of \cref{lem:maximal-cases}. We let $q'$ be obtained from $q$ by replacing all occurrences of $t$ in $q$ with $t'$ and define $\mergeop((q, \prmark), \set{x, t, t'}) = (q' \cup \{\top(t)\}, \prmark)$.\defend
\end{definition}

Let us briefly describe how rewritings are computed by means of the above operations. %First, when given a CQ $q$ that is satisfied on $\sg$, we extend the CQ to a properly marked CQ $(q,M)$, which can always be accomplished by \cref{obs:query-extendable-properly-marke}.  
 Given an alive CQ $(q,M)$, we know that one of the three rewriting operations will be applicable (by \cref{lem:maximal-cases}), which we note, may return a \emph{set} of rewritings if the $\reduceop$ operation is applied. We ultimately obtain the set $\fcn{rew}(q, \prmark)$ of rewritings of $(q,\prmark)$ by sequentially applying the three rewriting operations to all alive queries within the set of rewritings, until all marked queries in the set are dead, at which point, the rewriting process terminates. As shown below, we can always apply a rewriting operation to a CQ if it is alive (i.e., rewriting is complete), and also, applying such an operation preserves satisfaction on $\sg$ (i.e., rewriting is sound). %We note that the soundness proofs can be found in \cref{appendix:higher-arity}.

\begin{observation}[Completeness]\label{obs:high-completeness}
If a CQ is alive then at least one of above operations can be applied to it.
\end{observation}
\begin{proof}
Follows from~\cref{def:cut,def:reduce,def:merge}, and~\cref{lem:maximal-cases}.
\end{proof}

Let us now prove the soundness of the above operations:

\begin{lemma}[Soundness --- $\cutop$]\label{lem:high-soundness-cut}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x$ is as in \cref{def:cut}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \cutop(\mquery, \set{x}).$$
\end{lemma}

\begin{proof} Let $\mquery = (\query,\prmark)$ be an alive CQ and $\cutop(\mquery, \set{x}) = (q',M)$. The forward direction is trivial. For the backward direction, assume that $\sg \models \cutop(\mquery, \set{x})$. By our assumption, there exists a homormorphism $h$ from $\query'$ into $\sg$ such that for all terms $t$ in $\query'$, $t \in M$ \iffi $h(t)$ is a constant in $\sg$. Since the $\cutop$ operation was applied, we know that there exists exactly one atom of the from $\rpred(t,x)$ in $\query$ with $\rpred\in \{\hpred,\vpred\}$ and $x$ a maximal variable. We have two cases to consider: either (i) the term $t$ exists in $\query'$, or (ii) the term $t$ does not exist in $\query'$.

(i) Suppose that the term $t$ exists in $\query'$. Then, $h$ maps $t$ to some element $t'$ of $\sg$. Based on the functionality of the rules in $\rsgrid$, one can see that for every term $t''$ in $\sg$ and $\ppred \in \{\hpred,\vpred\}$, there exists a null $y$ such that $\ppred(t'',y) \in \sg$. Therefore, there exists a null $y$ such that $\rpred(t',y) \in \sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for all terms $s \neq x$ in $\query$ and $h'(x) = y$. It follows that $h'$ is a homomorphism from $\query$ to $\sg$, and thus $\sg \models \query$.

To complete the proof of this case, it suffices to show that for all terms $t$ in $\query$ that $t \in M$ \iffi $h'(t)$ is a constant in $\sg$. If we consider only the terms $s \neq x$ in $\query$, then the above equivalence holds as $h'(s) = h(s)$ for all such terms and we know that for all terms $s$ in $\query'$ that $s \in M$ \iffi $h(s)$ is a constant in $\sg$. The above equivalence also holds for the maximal variable $x$ since $x \not\in M$ and $h'(x) = y$ maps to a null (and not a constant) in $\sg$. This completes the proof of this case.

(ii) Suppose that the term $t$ does not exist in $\query'$. We know that either (a) the term $t$ is a constant $\const{c}$, or (b) the term $t$ is a variable $y$. We prove both cases below.

(a) Assume that $t$ is a constant $\const{c}$. If $\const{c}$ does not occur in the database $\db$, then $\sg \not\models \cutop(\mquery, \set{x})$, contrary to our assumption. Hence, we may assume that $\const{c}$ occurs in $\db$. By the (grow) rule in $\rsgrid$, we know that for the constant $\const{c}$ in $\db$, there exists a null $z$ such that $\rpred(\const{c},z) \in \sg$. Let us extend the homomorphism $h$ to a homomorphism $h'$ such that $h'(s) = h(s)$ for $s \neq x$ and $h'(x) = z$. It is straightforward to show that $h'$ is a homomorphism from $\query$ to $\sg$, and showing that for all terms $t'$ in $\query$ we have $t' \in M$ \iffi $h'(t')$ is a constant in $\sg$ is argued similarly as in case (i) above.

(b) Assume that $t$ is a variable $y$. Based on the (loop) rule in $\rsgrid$, we know that there exists a null $z$ such that $\rpred(z,z) \in \sg$. Let us now extend the homomorphism $h$ to a homomorphism $h'$ such that $h'(s) = h(s)$ for $s \not\in\{y,x\}$ and $h'(y) = h'(x) = z$. It is straightforward to show that $\sg \models \mquery$ by making use of $h'$.
\end{proof}


\begin{lemma}[Soundness --- $\reduceop$]\label{lem:high-soundness-reduce}
Let $\db$ be a database and let $Q$ be an alive CQ. If $x$ is as in \cref{def:reduce} and $\reduceop(\mquery, \set{x}) = \set{\mquery_{1}, \mquery_{2}}$, then
$$\sg \models \mquery \ \text{\iffi} \ \exists i \in \{1,2\}, \sg \models \mquery_{i}.$$
\end{lemma}

\begin{proof} Let $Q = (\query,M)$ and $\mquery_{i} = (\query',M_{i})$ with $i \in \{1,2\}$. 

For the forward direction, suppose that $\sg \models \mquery$. It follows that there exists a homomorphism $h$ such that $h$ maps $\query$ to $\sg$ and for all terms $t$ in $\query$, $t \in M$ \iffi $h(t)$ is a constant in $\sg$. By our assumption that $\reduceop$ was applied, we know that there exist two atoms of the form $\hpred(t_{\hpred},x)$ and $\vpred(t_{\vpred},x)$ in $\query$ with $x$ maximal and $x$ occurring in no other atoms of $\query$. We have two cases to consider: either (i) both $t_{\hpred}$ and $t_{\vpred}$ are constants, or (ii) at least one term is not a constant. We argue each case accordingly.

(i) Observe that if both $t_{\hpred}$ and $t_{\vpred}$ are constants, then since $\mquery$ is properly marked, we know that $x \in M$ by \cref{def:properly-marked}. However, this contradicts our assumption that $x$ is maximal, and so, this case cannot occur.

(ii) In the alternative case, by the functionality of the Skolem chase (see~\cref{sec:preliminaries}), the fact that our rule set is $\rsgrid$, and since one term maps to a null in $\sg$ via $h$, we know that the (grid) rule must have been applied for $\hpred(h(t_{\hpred}),h(x))$ and $\vpred(h(t_{\vpred}),h(x))$ to occur in $\sg$. It follows that for some term $t$, $\hpred(t,h(t_{\vpred}))$ and $\vpred(t,h(t_{\hpred}))$ must occur in $\sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for each term $s \neq x$ in $\query$ and $h'(x') = t$. Then, we have that $\sg \models \query'$. Note that if $t$ is a null, then $\sg \models Q_{1}$ and if $t$ is a constant, then $\sg \models Q_{2}$, thus showing the desired conclusion.

Let us now show the backward direction and assume that there exists an $i \in \{1,2\}$ such that $\sg \models \mquery_{i}$. We have that $\sg \models \query'$, meaning that there exists a homomorphism $h$ mapping $\query'$ into $\sg$. Due to the fact that $\reduceop$ was applied, it follows that there exist atoms $\hpred(x',t_{\vpred})$ and $\vpred(x',t_{\hpred})$ in $\query'$ that are mapped into $\sg$, that is to say, $\hpred(h(x'),h(t_{\vpred})),\vpred(h(x'),h(t_{\hpred})) \in \sg$. By the (grid) rule and the functionality of the Skolem chase, there exists a null $y$ such that $\hpred(h(t_{\hpred}),y),\vpred(h(t_{\vpred}),y) \in \sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for all terms $s \neq x'$ in $\query'$ and $h'(x) = y$. Then, $h'$ is a homomorphism from $\query$ to $\sg$ and it is straightforward to show that for all terms $t'$ in $\query$, $t' \in M$ \iffi $h'(t')$ maps to a constant in $\sg$.
\end{proof}


\begin{lemma}[Soundness --- $\mergeop$]\label{lem:high-soundness-merge}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x, t$, and $t'$ are as in \cref{def:merge}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \mergeop(\mquery, \set{x, t, t'}).$$
\end{lemma}

\begin{proof} Let $Q = (\query,M)$, $\mergeop(\mquery, \set{x, t, t'}) = (\query',M )$, $\rpred \in \{\hpred, \vpred\}$, and $\query' = \query'' \cup \{\top(t)\}$.

For the forward direction, assume that $\sg \models \mquery$. It follows that there exists a homomorphism $h$ such that $h$ maps $\query$ into $\sg$ and for all terms $s$ in $\query$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$. Also, since $\mergeop$ was applied, we know that there are at least two terms $t \neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are in $\query$ and that $t'$ was substituted for $t$ in $\query$ to obtain $\query'$. Hence, $\rpred(h(t),h(x)), \rpred(h(t'),h(x)) \in \sg$, however, since we are using rules from $\rsgrid$ and by the functionality of the Skolem chase (see~\cref{sec:preliminaries}), it must be the case that either (i) $h(t)$, $h(x)$, and $h(t')$ all occur in $\db$, or (ii) $h(t) = h(x) = h(t') = y$ with $y$ the null generated by the (loop) rule. In case (i), $h(x)$ will be a constant as all terms of $\db$ are constants, meaning that $x$ will not be maximal, in contradiction to our assumption. Let us consider case (ii) then. %We define the homomorphism $h'$ to be the homomorphism $h$ restricted to the terms of $\query'$. Note that in case (ii), the entire connected component of $\query$ containing $t$, $x$, and $t'$ is mapped to $y$ via $h$, meaning that the entire connected component of $\query'$ containing $x$ and $t'$ will be mapped to $y$ as well. The remaining connected components of $\query'$ will be mapped by $h'$ just as they are mapped by $h$, showing that $h'$ serves a homomorphism from $\query'$ to $\sg$. Last, we must show that for all terms $s'$ in $\query'$, $s' \in M$ \iffi $h'(s')$ is a constant in $\sg$, however, this follows from the fact that for all terms $s$ in $\query$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$, the fact that $t \not\in M$ (as it is mapped to the null $y$ via $h$), and the fact that $t$ is not in the domain of $h'$, so it cannot be mapped to a constant in $\sg$ by $h'$.
 Note that in case (ii), the entire connected component of $\query$ containing $t$, $x$, and $t'$ is mapped to $y$ via $h$, meaning that the entire connected component of $\query'$ containing $x$ and $t'$ will be mapped to $y$ via $h$ as well. If we restrict our attention to the remaining connected components of $\query'$, then we can see that $h$ maps all such components homomorphically into $\sg$, showing that $h$ serves a homomorphism from $\query'$ to $\sg$. Last, we must show that for all terms $s'$ in $\query'$, $s' \in M$ \iffi $h(s')$ is a constant in $\sg$, however, this follows from the fact that $\query$ and $\query'$ have the same set of terms.

For the backward direction, suppose that $\sg \models \mergeop(\mquery, \set{x, t, t'})$. Then, there exists a homomorphism $h$ such that $h$ maps $\query'$ into $\sg$ and for all terms $s$ in $\query'$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$. In addition, as $\mergeop$ was applied, there are at least two terms $t \neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are in $\query$ with $t'$ substituted for $t$ in $\query$ to obtain $\query'$. Let us define a homomorphism $h'$ such that $h'(s) = s$ for all terms $s \neq t$ and $h'(t) = t'$. Then, $h'$ is a homomorphism from $\query$ to $\query'$, and since $h$ is a homomorphism from $\query'$ to $\sg$, we have that $h \circ h'$ is a homomorphism from $\query'$ to $\sg$. To finish the proof of the backward direction, we need to show that for all terms $s'$ in $\query$, $s' \in M$ \iffi $(h \circ h')(s')$ is a constant in $\sg$. %; however, this follows from the definition of $h'$ and the fact that for all terms $s$ in $\query'$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$

Let $s'$ be a term in $\query$. Suppose that $s' \in M$. Then, if $s' \neq t$, we have that $h(s')$ is a constant in $\sg$, and since $h(s') = (h \circ h')(s')$, it follows that $(h \circ h')(s')$ is a constant in $\sg$. If $s' = t$, then by \cref{def:properly-marked}, $t' \in M$, from which it follows that $h(t') = (h \circ h')(t)$ is a constant in $\sg$. Let us now suppose that $(h \circ h')(s')$ is a constant in $\sg$. If $s' \neq t$, then $(h \circ h')(s') = h(s')$ is a constant in $\sg$, implying that $s' \in M$; however, if $s' = t$, then $(h \circ h')(s') = (h \circ h')(t) = h(t')$ is a constant in $\sg$, implying that $t' \in M$, so by \cref{def:properly-marked}, $t \in M$ as well.
\end{proof}


\medskip
\noindent
{\bf Termination.}
Given two queries $\mquery$ and $\mquery'$, we write $\mquery \stepop \mquery'$ \iffi $\mquery'$ can be obtained from $\mquery$ by applying $\reduceop$, $\cutop$, or $\mergeop$. We let $\stepop^*$ denote the transitive closure of $\stepop$.


%\begin{observation}\label{obs:limit-on-variables}
%Let $\mquery$ and $\mquery'$ be two marked queries. If $\mquery \stepop \mquery'$ then $|\varset(\mquery)| \geq |\varset(\mquery')|$.
%\end{observation}

\begin{lemma}[Termination]\label{lem:termination}
For any properly marked CQ $\mquery$ the set of properly marked queries $\set{Q' \;|\; \mquery \stepop^* \mquery'}$ is finite.
\end{lemma}

\begin{proof} Observe that $\cutop$ deletes the only atom containing the considered maximal variable and $\mergeop$ reduces the number of atoms containing the considered maximal variable. Moreover, neither $\cutop$ nor $\mergeop$ introduce converging atoms of the form $\hpred(t_{1},t)$ and $\vpred(t_{2},t)$ when applied. Since the operation $\reduceop$ reduces the number of such converging atoms in a properly marked CQ as well, and since all such operations either preserve or decrease the number of terms occurring the query, it follows that the rewriting process will eventually terminate. 
\end{proof}

By \cref{obs:high-completeness} (Completeness), \cref{lem:high-soundness-cut,lem:high-soundness-reduce,lem:high-soundness-merge} (Soundness), and \cref{lem:termination} (Termination), we may conclude~\cref{lem:rsg-is-fus-reformulated}, thus completing the proof of \cref{lem:rsg-is-fus}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Comment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

% here - 001
\section{Proofs for \NoCaseChange{\cref{sec:higher-arity}}}%\label{appendix:higher-arity}

\begin{customlem}{\ref{lem:high-soundness-cut}}[Soundness --- $\cutop$]
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x$ is as in \cref{def:cut}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \cutop(\mquery, \set{x}).$$
\end{customlem}

\begin{proof} Let $\mquery = (\query,\prmark)$ be an alive CQ and $\cutop(\mquery, \set{x}) = (q',M)$. The forward direction is trivial, so we focus on the backward direction and assume that $\sg \models \cutop(\mquery, \set{x})$. By our assumption, there exists a homormorphism $h$ from $\query'$ into $\sg$ such that for all terms $t$ in $\query'$, $t \in M$ \iffi $h(t)$ is a constant in $\sg$. Since the $\cutop$ operation was applied, we know that there exists exactly one atom of the from $\rpred(t,x)$ in $\query$ with $\rpred\in \{\hpred,\vpred\}$ and $x$ a maximal variable. We have two cases to consider: either (i) the term $t$ exists in $\query'$, or (ii) the term $t$ does not exist in $\query'$.

(i) Suppose that the term $t$ exists in $\query'$. Then, $h$ maps $t$ to some element $t'$ of $\sg$. Based on the functionality of the rules in $\rsgrid$, one can see that for every term $t''$ in $\sg$ and $\ppred \in \{\hpred,\vpred\}$, there exists a null $y$ such that $\ppred(t'',y) \in \sg$. Therefore, there exists a null $y$ such that $\rpred(t',y) \in \sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for all terms $s \neq x$ in $\query$ and $h'(x) = y$. It follows that $h'$ is a homomorphism from $\query$ to $\sg$, and thus $\sg \models \query$.

To complete the proof of this case, it suffices to show that for all terms $t$ in $\query$ that $t \in M$ \iffi $h'(t)$ is a constant in $\sg$. If we consider only the terms $s \neq x$ in $\query$, then the above equivalence holds as $h'(s) = h(s)$ for all such terms and we know that for all terms $s$ in $\query'$ that $s \in M$ \iffi $h(s)$ is a constant in $\sg$. The above equivalence also holds for the maximal variable $x$ since $x \not\in M$ and $h'(x) = y$ maps to a null (and not a constant) in $\sg$. This completes the proof of this case.

(ii) Suppose that the term $t$ does not exist in $\query'$. We know that either (a) the term $t$ is a constant $c$, or (b) the term $t$ is a variable $y$. We prove both cases below.

(a) Assume that $t$ is a constant $c$. If $c$ does not occur in the database $\db$, then $\sg \not\models \cutop(\mquery, \set{x})$, contrary to our assumption. Hence, we may assume that $c$ occurs in $\db$. By the (grow) rule in $\rsgrid$, we know that for the constant $c$ in $\db$, there exists a null $z$ such that $\rpred(c,z) \in \sg$. Let us extend the homomorphism $h$ to a homomorphism $h'$ such that $h'(s) = h(s)$ for $s \neq x$ and $h'(x) = z$. It is straightforward to show that $h'$ is a homomorphism from $\query$ to $\sg$, and showing that for all terms $t'$ in $\query$ we have $t' \in M$ \iffi $h'(t')$ is a constant in $\sg$ is argued similarly as in case (i) above.

(b) Assume that $t$ is a variable $y$. Based on the (loop) rule in $\rsgrid$, we know that there exists a null $z$ such that $\rpred(z,z) \in \sg$. Let us now extend the homomorphism $h$ to a homomorphism $h'$ such that $h'(s) = h(s)$ for $s \not\in\{y,x\}$ and $h'(y) = h'(x) = z$. It is straightforward to show that $\sg \models \mquery$ by making use of $h'$.
\end{proof}


\begin{customlem}{\ref{lem:high-soundness-reduce}}[Soundness --- $\reduceop$]
Let $\db$ be a database and let $Q$ be an alive CQ. If $x$ is as in \cref{def:reduce} and $\reduceop(\mquery, \set{x}) = \set{\mquery_{1}, \mquery_{2}}$, then
$$\sg \models \mquery \ \text{\iffi} \ \exists i \in \{1,2\}, \sg \models \mquery_{i}.$$
\end{customlem}

\begin{proof} Let $Q = (\query,M)$ and $\mquery_{i} = (\query',M_{i})$ with $i \in \{1,2\}$. 

For the forward direction, suppose that $\sg \models \mquery$. It follows that there exists a homomorphism $h$ such that $h$ maps $\query$ to $\sg$ and for all terms $t$ in $\query$, $t \in M$ \iffi $h(t)$ is a constant in $\sg$. By our assumption that $\reduceop$ was applied, we know that there exist two atoms of the form $\hpred(t_{\hpred},x)$ and $\vpred(t_{\vpred},x)$ in $\query$ with $x$ maximal and $x$ occurring in no other atoms of $\query$. We have two cases to consider: either (i) both $t_{\hpred}$ and $t_{\vpred}$ are constants, or (ii) at least one term is not a constant. We argue each case accordingly.

(i) Observe that if both $t_{\hpred}$ and $t_{\vpred}$ are constants, then since $\mquery$ is properly marked, we know that $x \in M$ by \cref{def:properly-marked}. However, this contradicts our assumption that $x$ is maximal, and so, this case cannot occur.

(ii) In the alternative case, by the functionality of the Skolem chase (see~\cref{sec:preliminaries}), the fact that our rule set is $\rsgrid$, and since one term maps to a null in $\sg$ via $h$, we know that the (grid) rule must have been applied for $\hpred(h(t_{\hpred}),h(x))$ and $\vpred(h(t_{\vpred}),h(x))$ to occur in $\sg$. It follows that for some term $t$, $\hpred(t,h(t_{\vpred}))$ and $\vpred(t,h(t_{\hpred}))$ must occur in $\sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for each term $s \neq x$ in $\query$ and $h'(x') = t$. Then, we have that $\sg \models \query'$. Note that if $t$ is a null, then $\sg \models Q_{1}$ and if $t$ is a constant, then $\sg \models Q_{2}$, thus showing the desired conclusion.

Let us now show the backward direction and assume that there exists an $i \in \{1,2\}$ such that $\sg \models \mquery_{i}$. We have that $\sg \models \query'$, meaning that there exists a homomorphism $h$ mapping $\query'$ into $\sg$. Due to the fact that $\reduceop$ was applied, it follows that there exist atoms $\hpred(x',t_{\vpred})$ and $\vpred(x',t_{\hpred})$ in $\query'$ that are mapped into $\sg$, that is to say, $\hpred(h(x'),h(t_{\vpred})),\vpred(h(x'),h(t_{\hpred})) \in \sg$. By the (grid) rule and the functionality of the Skolem chase, there exists a null $y$ such that $\hpred(h(t_{\hpred}),y),\vpred(h(t_{\vpred}),y) \in \sg$. Let us define the homomorphism $h'$ such that $h'(s) = h(s)$ for all terms $s \neq x'$ in $\query'$ and $h'(x) = y$. Then, $h'$ is a homomorphism from $\query$ to $\sg$ and it is straightforward to show that for all terms $t'$ in $\query$, $t' \in M$ \iffi $h'(t')$ maps to a constant in $\sg$.
\end{proof}



\begin{customlem}{\ref{lem:high-soundness-merge}}[Soundness --- $\mergeop$]
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x, t$, and $t'$ are as in \cref{def:merge}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \mergeop(\mquery, \set{x, t, t'}).$$
\end{customlem}
\begin{proof} Let $Q = (\query,M)$, $\mergeop(\mquery, \set{x, t, t'}) = (\query',M )$, $\rpred \in \{\hpred, \vpred\}$, and $\query' = \query'' \cup \{\top(t)\}$.

For the forward direction, assume that $\sg \models \mquery$. It follows that there exists a homomorphism $h$ such that $h$ maps $\query$ into $\sg$ and for all terms $s$ in $\query$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$. Also, since $\mergeop$ was applied, we know that there are at least two terms $t \neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are in $\query$ and that $t'$ was substituted for $t$ in $\query$ to obtain $\query'$. Hence, $\rpred(h(t),h(x)), \rpred(h(t'),h(x)) \in \sg$, however, since we are using rules from $\rsgrid$ and by the functionality of the Skolem chase (see~\cref{sec:preliminaries}), it must be the case that either (i) $h(t)$, $h(x)$, and $h(t')$ all occur in $\db$, or (ii) $h(t) = h(x) = h(t') = y$ with $y$ the null generated by the (loop) rule. In case (i), $h(x)$ will be a constant as all terms of $\db$ are constants, meaning that $x$ will not be maximal, in contradiction to our assumption. Let us consider case (ii) then. %We define the homomorphism $h'$ to be the homomorphism $h$ restricted to the terms of $\query'$. Note that in case (ii), the entire connected component of $\query$ containing $t$, $x$, and $t'$ is mapped to $y$ via $h$, meaning that the entire connected component of $\query'$ containing $x$ and $t'$ will be mapped to $y$ as well. The remaining connected components of $\query'$ will be mapped by $h'$ just as they are mapped by $h$, showing that $h'$ serves a homomorphism from $\query'$ to $\sg$. Last, we must show that for all terms $s'$ in $\query'$, $s' \in M$ \iffi $h'(s')$ is a constant in $\sg$, however, this follows from the fact that for all terms $s$ in $\query$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$, the fact that $t \not\in M$ (as it is mapped to the null $y$ via $h$), and the fact that $t$ is not in the domain of $h'$, so it cannot be mapped to a constant in $\sg$ by $h'$.
 Note that in case (ii), the entire connected component of $\query$ containing $t$, $x$, and $t'$ is mapped to $y$ via $h$, meaning that the entire connected component of $\query'$ containing $x$ and $t'$ will be mapped to $y$ via $h$ as well. If we restrict our attention to the remaining connected components of $\query'$, then we can see that $h$ maps all such components homomorphically into $\sg$, showing that $h$ serves a homomorphism from $\query'$ to $\sg$. Last, we must show that for all terms $s'$ in $\query'$, $s' \in M$ \iffi $h(s')$ is a constant in $\sg$, however, this follows from the fact that $\query$ and $\query'$ have the same set of terms.

For the backward direction, suppose that $\sg \models \mergeop(\mquery, \set{x, t, t'})$. Then, there exists a homomorphism $h$ such that $h$ maps $\query'$ into $\sg$ and for all terms $s$ in $\query'$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$. In addition, as $\mergeop$ was applied, there are at least two terms $t \neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are in $\query$ with $t'$ substituted for $t$ in $\query$ to obtain $\query'$. Let us define a homomorphism $h'$ such that $h'(s) = s$ for all terms $s \neq t$ and $h'(t) = t'$. Then, $h'$ is a homomorphism from $\query$ to $\query'$, and since $h$ is a homomorphism from $\query'$ to $\sg$, we have that $h \circ h'$ is a homomorphism from $\query'$ to $\sg$. To finish the proof of the backward direction, we need to show that for all terms $s'$ in $\query$, $s' \in M$ \iffi $(h \circ h')(s')$ is a constant in $\sg$. %; however, this follows from the definition of $h'$ and the fact that for all terms $s$ in $\query'$, $s \in M$ \iffi $h(s)$ is a constant in $\sg$

Let $s'$ be a term in $\query$. Suppose that $s' \in M$. Then, if $s' \neq t$, we have that $h(s')$ is a constant in $\sg$, and since $h(s') = (h \circ h')(s')$, it follows that $(h \circ h')(s')$ is a constant in $\sg$. If $s' = t$, then by \cref{def:properly-marked}, $t' \in M$, from which it follows that $h(t') = (h \circ h')(t)$ is a constant in $\sg$. Let us now suppose that $(h \circ h')(s')$ is a constant in $\sg$. If $s' \neq t$, then $(h \circ h')(s') = h(s')$ is a constant in $\sg$, implying that $s' \in M$; however, if $s' = t$, then $(h \circ h')(s') = (h \circ h')(t) = h(t')$ is a constant in $\sg$, implying that $t' \in M$, so by \cref{def:properly-marked}, $t \in M$ as well.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Comment End
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

==> ICDT 2023 Updated LaTeXFiles/appendices/reification/reify-i.tex <==
%\subsection{Reification preserves finite width - Instance wise}
\subsection{$\tw{\instance} \in \mathbb{N}$ implies $\tw{\fcn{reify}(\instance)}\in \mathbb{N}$ and $\cw{\fcn{reify}(\instance)}\in \mathbb{N}$.}




Let $\Sigma$ be a finite signature, $\inst$ an instance over $\Sigma$, $T = (V, E)$ a tree decomposition of $\inst$ of width $n$, and denote by $\inst_{\ge 3} \subseteq \inst$ the sub-instance of $\inst$ consisting of all atoms over $\Sigma_{\ge 3}$ from $\inst$. Define $\reify{T}$ to be a pair $(V', E')$ consisting of:
\begin{itemize}
    \item Let $V'$ contain the sets $X'$ obtained in the following way: For $X \in V$ of the original tree decomposition, let \[ X' = X \cup \{ u_{\alpha} \mid \alpha \in \inst_{\ge 3}[X] \} \] (where $\inst_{\ge 3}[X]$ denotes the induced sub-instance of $\inst_{\ge 3}$ with active domain $X$). This gives rise to a bijection $V \to V', X\mapsto X'$, which we will use implicitly in the following.
    \item $E' = \{ (X_1', X_2') \in V' \times V' \mid (X_1, X_2)\in E \}$
\end{itemize}

\begin{observation}\label{obs:reify-tree-ftw}
    Let $\Sigma$ be a finite signature, $\inst$ an instance over $\Sigma$ of finite treewidth, and $T = (V, E)$ a tree decomposition of $\inst$ of width $n$. Then $\reify{T}$ is a tree decomposition of $\reify{\inst}$ of finite width.
\end{observation}
\begin{proof}
    Let $\inst$ be an instance of treewidth $n$ and $T=(V,E)$ a tree decomposition with width $n$. $\reify{T} = (V', E')$ is a tree decomposition of $\reify{\inst}$:
    \begin{itemize}
        \item We will establish that $\bigcup_{X'\in V'}X' = \adom{\reify{\inst}}$. By definition each $X'\in V'$ is a subset of $\adom{\reify{\inst}}$, which shows the $\subseteq$ inclusion. On the other hand, let $t\in\adom{\reify{\inst}}$. If $t\in \adom{\inst}$, then there exists an $X\in V$ such that $t\in X$ and hence by definition of $\reify{T}$, the node $X'$ in $\reify{T}$ corresponding to $X$ contains $t$. So assume $t\not\in\adom{\inst}$. Then, there exists an atom $\alpha\in \inst$ such that $t = u_{\alpha}$. Furthermore, there exists an $X\in V$ such that every term of $\alpha$ is contained in $X$. By construction this means that $u_{\alpha}\in X'$, where $X'$ is the node in $\reify{T}$ corresponding to node $X$. We obtain thus the inclusion $\supseteq$ and hence have shown the claim.
        \item Let $\rpred(t_1, \ldots, t_n)\in \reify{\inst}$. In order to show that this implies $t_{1}, \ldots, t_{n} \in X'$ for some $X'\in V'$, we discuss two cases: Either %$\rpred\in \Sigma_{1}\cup\Sigma_{2}$ 
        $\rpred\in \Sigma_{\leq2}$ or $\rpred\in \Sigma^{\mathrm{rf}}\setminus \Sigma_{\leq2}$ (which means that %$n\le 2$). 
        $n = 2$). In the former case, there exists an $X\in V$ such that $t_{1}, \ldots, t_{n}\in X$, and hence (by definition) $t_{1}, \ldots, t_{n}\in X'$, the corresponding node of $X$ in $\reify{T}$. In the latter case, there exists an atom $\alpha\in\inst$ and a null $u_{\alpha}$ such that %$\rpred(t_{1}, u_{\alpha})$
         $\rpred(t_1, \ldots, t_n)$ is of the form $\rpred(t_{1}, u_{\alpha})$. By definition, the node $X'$ in $\reify{T}$ corresponding to $X$ contains not just $t_{1}$, but $u_{\alpha}$ as well. Hence, the claim follows.
        \item Last, we show that for every $t\in \adom{\reify{\inst}}$ the subgraph of $\reify{T}$ induced by all nodes $X'$ containing $t$ is connected. Again, we have two cases: Either $t\in \adom{\inst}$ or $t\not\in\adom{\inst}$ with $t\in \adom{\reify{\inst}}$. The former case is immediate by the definition of $\reify{T}$, so we focus on the latter case, and assume that $t = u_{\alpha}$ for some  %$\alpha(t_{1}, \ldots, t_{n})\in \inst$. 
        $\alpha \in \inst$. By the definition of $\reify{T}$, $u_{\alpha}$ is in exactly those $X'\in V'$ for which the corresponding $X\in V$ contains all of $t_{1}, \ldots, t_{n}$. By $T$ being a tree decomposition, the set of all those $X$ induces a connected subgraph of $T$. By the definition of $\reify{T}$, the nodes of $\reify{T}$ are connected in exactly the same way in $E'$ as their corresponding nodes in $T$; hence, we immediately obtain that all $X'\in V'$ containing $t$ induce a connected subgraph of $\reify{T}$.
    \end{itemize}
    This establishes, that $\reify{T}$ is a tree decomposition of $\reify{\inst}$.
    
    Last, it is clear that $\reify{T}$ has a width of at most $n + K$ where $K$ is the maximal number of atoms over $\Sigma_{\ge 3}$ using elements from a set of cardinality $n+1$, as this constitutes the maximal amount of ``reification-nulls'' introduced in a node $X'$ in $\reify{T}$ in comparison to the corresponding node $X$ in $T$.
\end{proof}
\begin{corollary}\label{cor:reify-i}
    Let $\Sigma$ be a finite signature. If $\inst$ over $\Sigma$ has finite treewidth, then $\tw{\reify{\inst}}$ and $\cw{\reify{\inst}}$ are finite.
\end{corollary}
\begin{proof}
    Since $\inst$ has finite treewidth, there is a tree decomposition $T = (V, E)$ of $\inst$. Then, $\reify{T}$ is a tree decomposition of $\reify{I}$ of finite width. This implies finite treewidth and, by \cref{thm:tree-width-implies-clique-width}, finite cliquewidth of $\reify{I}$.
\end{proof}

==> ICDT 2023 Updated LaTeXFiles/appendices/reification/reify-ii.tex <==
%\subsection{Reification preserves finite-width sets - Ruleset-wise}
\subsection{If $\ruleset$ is $\bts$, then $\fcn{reify}(\ruleset)$ is $\bts$ and $\fcs$.}

\begin{comment}
--- OBSOLETE ---
\begin{observation}\label{obs:pseudoreified}
    Let $\Sigma$ be a signature and $\inst$ an instance over the reified signature $\Sigma^{\mathrm{rf}}$. Furthermore let $\ruleset$ be a set of rules over $\Sigma$. Then there exists a unique and maximal sub-instance $\inst_{\mathrm{prf}}$ (up to isomorphy) of $\inst$ such that:
    
    For every $\rpred\in \Sigma_{\ge 3}$, if $\rpred_i(t{}, t_i) \in \inst_{\mathrm{prf}}$ for some $t{}, t_{i} \in \adom{\inst_{\mathrm{prf}}}$ and $1\le i \le \arity{\rpred}$, then there exist $t_{j}\in \adom{\inst_{\mathrm{prf}}}$ such that $\rpred_{j}(t{}, t_{j})\in \inst_{\mathrm{prf}}$ for every $1\le j\le \arity{\rpred}$.
    
    Furthermore, $\adom{\inst_{\mathrm{prf}}} = \adom{\inst}$ and for every $\rho \in \reify{\ruleset}$, $(\rho, h)$ is a trigger of $\inst_{\mathrm{prf}}$ if and only if it is a trigger of $\inst$. 
\end{observation}
\begin{proof}
    In order to obtain $\inst_{\mathrm{prf}}$ we prune away all those atoms from $\inst$ that are of the form $\rpred_{i}(t{}, t_{i})$ for some $\rpred\in\Sigma_{\ge 3}$ and $1\le i \le \arity{\rpred}$ such that there is at least one $j$ with $1 \le j \le \arity{\rpred}$ and no $t_{j}\in \adom{\inst}$ with $\rpred_{j}(t{}, t_{j})\in \inst$.
    
    As we tacitly assume that in any instance each term satisfies $\top$ vacuously, we might now obtain (more) isolated terms in $\inst_{\mathrm{prf}}$ but do not lose any from $\inst$, as the tacit assumption of $\top$ holding universally is carried over.
    
    
    Last, we have two cases:
    
    If $\rho\in\ruleset$, note that $\rho$ makes only use of atoms over $\Sigma_{1}\cup \Sigma_{2}$. As for every such atom $\alpha$ it holds by construction that $\alpha\in\inst$ if and only if $\alpha \in \inst_{\mathrm{prf}}$ we conclude the follwing: For every trigger $(\rho, h)$ of $\inst$ the homomorphism $h$ maps the body of $\rho$ homomorphically to $\inst_{\mathrm{prf}}$ and hence $(\rho, h)$ is a trigger of $\inst_{\mathrm{prf}}$. Moreover, for every trigger $(\rho, h)$ of $\inst_{\mathrm{prf}}$, since $\inst_{\mathrm{prf}} \subseteq \inst$ we obtain $h$ being also a homomorphism to $\inst$, hence $(\rho, h)$ is a trigger of $\inst$.
    
    %then by construction $(\rho, h)$ is is a trigger on $\inst_{\mathrm{prf}}$ if and only if it is one on $\inst$. \sebastian{Too unspecific, use triggers/hopmomorphisms and describe what exactly that means.}
    
    So suppose $\rho = \reify{\rho_{\mathrm{urf}}}$ is obtained by reification for some $\rho_{\mathrm{urf}}\in\ruleset$. Then every atom $\alpha = \rpred(x_1, \ldots, x_n)$ with $\rpred \in \Sigma_{\ge 3}$ from the body of $\rho_{\mathrm{urf}}$ will be exchanged by the conjunction $\bigwedge_{1\le i\le n}\rpred_{i}(u_{\alpha}, x_{i})$ for some fresh variable $u_{\alpha}$ in the reification process to obtain $\rho = \reify{\rho_{\mathrm{urf}}}$.
    Let $(\rho, h)$ be a trigger of $\inst$. Since the body of $\rho$ contains an atom of the form $\rpred_{i}(u_{\alpha}, x_{i})$ if and only if it contains all such atoms for $1 \le i \le \arity{\rpred}$, the homomorphism $h$ to $\inst$ is also one to $\inst_{\mathrm{prf}}$. Hence $(\rho, h)$ is also a trigger of $\inst_{\mathrm{prf}}$. Conversely, suppose $(\rho, h)$ is also a trigger of $\inst_{\mathrm{prf}}$. Since $\inst_{\mathrm{prf}}\subseteq \inst$ it follows that $h$ being a homomorphism from the body of $\rho$ to $\inst_{\mathrm{prf}}$ is also a homomorphism to $\inst$. This means that $(\rho, h)$ is also a trigger of $\inst$.
    
    %It is now obvious by definition of $\inst_{\mathrm{prf}}$ that $\rho$ is applicable in $\inst$ if and only if it is applicable in $\inst_{\mathrm{prf}}$ on the exact same terms. \sebastian{Same as before: too unspecific.}
\end{proof}

--- NOT obsolete ---
\end{comment}

\begin{lemma}\label{lem:reify-ii}
    If $\ruleset$ is $\bts$, then $\reify{\ruleset}$ is $\bts$ and $\fcs$.
\end{lemma}


%%%%%
% Old
%%%%%
\begin{comment}
\begin{proof}
    Let $\db$ be a database (hence finite) over $\Sigma^{\mathrm{rf}}$. In a first step we decompose $\db$ into two parts, $\db = \db_{\mathrm{prf}}\uplus\db_{\mathrm{dw}}$. By \cref{obs:pseudoreified} we note that all the rules from $\reify{\ruleset}$ fire on $\db$ if and only if they fire on $\db_{\mathrm{prf}}$. \sebastian{This is even more unspecific: ``firing on sth.'' is not defined at all.} Also, as will be important later on, note that $\adom{\db} = \adom{\db_{\mathrm{prf}}}$ by the same \cref{obs:pseudoreified}.
    
    We introduce $\ruleset_{\mathrm{purf}}$ as the set of rules of the following form: \[ \rho_{\rpred} = \big( \bigwedge_{1 \le i \le \arity{\rpred}} \rpred_{i}(x, y_{i}) \big) \rightarrow \rpred(y_{1}, \ldots, y_{\arity{\rpred}}) \] for every $\rpred \in\Sigma_{\ge 3}$. $\ruleset_{\mathrm{purf}}$ is a purely datalog rule set and does not introduce any new nulls if applied. We now define $\db'$ to be the restriction of $\sa{(\db_{\mathrm{prf}}, \ruleset_{\mathrm{purf}})}$ to the signature $\Sigma$.
    \sebastian{Actually, $\ksat{1}{...}$ is enough, but no harm done.}

    Since $\ruleset$ is $\bts$ there exists a universal model $\unimod$ of $(\db', \ruleset)$ that has finite treewidth $n$. Let $T = (V,E)$ be a tree decomposition of $\unimod$ of width $n$.
    $\reify{\unimod}\cup \db_{\mathrm{dw}}$ is clearly a model of $(\db, \reify{\ruleset})$. \sebastian{Why ``clearly''??? This requires a detailed argument! In fact the statement is wrong. Consider $\db=\{\rpred_1(a,b),\rpred_2(a,c),\rpred_3(a,a)\}$ and $\ruleset=\{\rpred(x,y,z)\to\ppred(x)\}$.} Furthermore, as $\db_{\mathrm{dw}}$ is finite, $\reify{T}$ has finite treewidth and is a tree decomposition of $\reify{\unimod}$ (see \cref{obs:reify-tree-ftw}) we can conclude that $\reify{\unimod}\cup \db_{\mathrm{dw}}$ has finite treewidth (for an upper approximation add every term from $\db_{\mathrm{dw}}$ to every node of $\reify{T}$).
    
    To prove universality of $\reify{\unimod}\cup \db_{\mathrm{dw}}$ let $\inst$ be some instance satisfying $(\db, \reify{\ruleset})$. As for $\db$ we decompose $\inst$ into the disjoint union $\inst = \inst_{\mathrm{prf}}\cup \inst_{\mathrm{dw}}$ (see \cref{obs:pseudoreified}). Furthermore, let $\inst'$ be the restriction of $\sa{(\inst_{\mathrm{prf}}, \ruleset_{\mathrm{purf}})}$ to the signature $\Sigma$. The following properties hold:
    \begin{enumerate}
        \item\label{item:reifybttsfcs1} $\inst'$ satisfies $(\db', \ruleset)$,
        \item\label{item:reifybttsfcs2} $\db_{\mathrm{prf}}\subseteq \inst_{\mathrm{prf}}$, and
        \item\label{item:reifybttsfcs3} $\db_{\mathrm{dw}}\subseteq \inst_{\mathrm{dw}}$.
    \end{enumerate}
    
     Because of \cref{item:reifybttsfcs1} and $\unimod$ being a universal model, there exists a homomorphism $h'\colon \unimod \to \inst'$. $h'$ can now be extended to a homomorphism $h''\colon \reify{\unimod}\to \inst_{\mathrm{prf}}$ in the following way: Observe that for every atom using $\rpred\in\Sigma_{\ge 3}$ of the form \[ \alpha = \rpred(t_{1}, \ldots, t_{\arity{\rpred}})\in \unimod \] we have \[ \rpred_{1}(u_{\alpha}, t_{1}), \ldots, \rpred_{\arity{\rpred}}(u_{\alpha}, t_{\arity{\rpred}})\in\reify{\unimod} \, . \] Furthermore, since $h'$ is a homomorphism, it holds that \[ h(\alpha) = \rpred(h(t_{1}), \ldots, h(t_{\arity{\rpred}}))\in \inst'\, , \] hence there exists a $t^{\ast}\in\adom{\inst_{\mathrm{prf}}}$ such that \[ \rpred_{1}(t^{\ast}, t_{1}), \ldots, \rpred_{\arity{\rpred}}(t^{\ast}, t_{\arity{\rpred}}) \in \inst_{\mathrm{prf}} \, . \] Taking an arbitrary such $t^{\ast}$ we define $u_{\alpha}^{h'} := t^{\ast}$. Then \[ h''(x) = \begin{cases} h'(x) & \text{if } x\in\adom{\unimod} \\ u_{\alpha}^{h'} & \text{if } x = u_{\alpha} \text{ for some } \alpha \in\unimod \end{cases} \] is a homomorphism.
     
     Lastly, we extend $h''$ to a homomorphism $h\colon \reify{\unimod}\uplus  \db_{\mathrm{dw}} \to \inst$. The trick here is that every term in $\adom{\db_{\mathrm{dw}}}$ is by construction already in $\db'$ (albeit possibly isolated) of which $\unimod$ is a model (and thus $h$ has the same domain and codomain as $h''$). By this and the fact that terms from $\db'$ are constants, we ensure with \cref{item:reifybttsfcs3} that $h$ is homomorphism.

    In conclusion, $\reify{\unimod}\cup\db_{\mathrm{dw}}$ is a universal model with finite treewidth of $(\db, \reify{\ruleset})$. As $\db$ was an arbitrary database over $\Sigma^{\mathrm{rf}}$ we obtain that $\reify{\ruleset}$ is $\bts$ and by \cref{thm:tree-width-implies-clique-width} this implies that $\reify{\ruleset}$ is also $\fcs$, finishing the proof.
\end{proof}
\end{comment}

%%%%%
% New
%%%%%
\begin{proof}
%\sebastian{Don't jump right in, explain what you are doing: ``Let $\ruleset$ be a $\bts$ ruleset. We now show that $\reify{\ruleset}$ is $\bts$, by showing that for every database $\db$...''}
    Let $\ruleset$ be a $\bts$ rule set. We will show that $\reify{\ruleset}$ is also $\bts$. To this end, we let $\db$ be an arbitrary database over $\Sigma^{\mathrm{rf}}$ and show in the following that $(\db,\reify{\ruleset})$ has a universal model of finite treewidth. 

%    Let $\db' = \db_{{\leq}2} \cup \db_{{\geq}3}$, where $\db_{{\leq}2}=\{\rpred(\vt)\in \db \mid \arity{\rpred} \leq 2\}$ and $\db_{{\geq}3}$ denotes the database defined by 
%    $$
%    \big\{ \rpred(t_{1}, \ldots, t_{\arity{\rpred}}) \mid \{ \rpred_{i}(t, t_{i}) \mid 3 \le i \le \arity{\rpred} \} \subseteq \db , t\in \adom{\db} \big\}.
%    $$

    From $\db$, we obtain the database $\db' = \fcn{dereify}(\db)$ over the original signature $\Sigma$, defined to consist of
    \begin{itemize}
        \item every atom $\rpred(\vt)$ from $\db$ with $\arity{\rpred}\leq 2$ and
        \item each atom $\rpred(t_{1}, \ldots, t_{\arity{\rpred}})$ with ${\arity{\rpred}}\geq 3$ for which there exists some $t\in \adom{\db}$ such that $\{ \rpred_{i}(t, t_{i}) \mid 1 \le i \le \arity{\rpred}\} \subseteq \db$.
    \end{itemize}
    Intuitively, $\fcn{dereify}$ constitutes the ``best effort'' of reconstructing the original database from some ``imperfectly reified'' one.    

%    We introduce $\ruleset_{\mathrm{purf}}$ as the set of rules of the following form: \[ \rho_{\rpred} = \big( \bigwedge_{1 \le i \le \arity{\rpred}} \rpred_{i}(x, y_{i}) \big) \rightarrow \rpred(y_{1}, \ldots, y_{\arity{\rpred}}) \] for every $\rpred \in\Sigma_{\ge 3}$. $\ruleset_{\mathrm{purf}}$ is a purely datalog rule set and does not introduce any new nulls if applied. We now define $\db'$ to be the restriction of $\ksat{1}{(\db, \ruleset_{\mathrm{purf}})}$ to the signature $\Sigma$.

    Since $\ruleset$ is $\bts$ there exists a universal model $\unimod$ of $(\db', \ruleset)$ that has finite treewidth $n$. Let $T = (V,E)$ be a tree decomposition of $\unimod$ of width $n$.

    Next, we will show that $\reify{\unimod}\cup \db$ is a model of $(\db, \reify{\ruleset})$.
    As $\db \subseteq \reify{\unimod}\cup \db$, it remains to be shown that $\reify{\ruleset}$ is satisfied in $\reify{\unimod}\cup \db$. 
%    
    Let $\rho \in \reify{\ruleset}$ be a rule of the form 
    \[ \rho = \forall\vx\vy\phi(\vx, \vy) \rightarrow \exists\vz \psi(\vy, \vz)\] 
    and let $\rho_{\mathrm{urf}}\in\ruleset$ be the rule for which $\rho = \reify{\rho_{\mathrm{urf}}}$. We will denote by $\vu$ the variables from $\vx$ that are introduced by the reification.
    Last, let $h$ be a homomorphism mapping $\body(\rho)$ to $\reify{\unimod}\cup \db$. We will use $v$ and $v_{i}$ to denote variables from $\vx\vy$. 
    %in order to first talk about arbitrary body variables and secondly distinguish the choice of index from the index $x^{\ast}_{i}$ would have if it where part of $\vx$. 
    %Similarly, $\vx_{\body}'$ will signify a sequence of variables from $\vx$ or $\vy$ which does not need to be equal to $\vx$ itself.
    
    Note that if for $\rpred\in\Sigma_{\ge 3}$ and $1\le i \le \arity{\rpred}$ an atom of the form $\rpred_{i}(u, v{})$ from $\body(\rho)$ is mapped via $h$ to $\reify{\unimod}\cup \db$, then %there are the following cases for the mapping itself:
    one of the two holds:
    \begin{itemize}
        \item If $h(u)$ is a constant, then $h(v)$ is a constant. We may conclude this from the following argument: Since $\reify{\unimod}$ has appearances of atoms of the form $\ppred_{k}(u_{\beta}, t)$ for $u_{\beta}$ being a null, $h$ can only map $\rpred_{i}(u, v{})$ to $\db$. But then, since $\db$ is a database and contains only constants as terms, $h(v{})$ has to be a constant as well.
        \item If $h(u)$ is not a constant, then no restrictions are imposed on $h(v{})$. More precisely, $h$ would map $\rpred_{i}(u, v{})$ into $\reify{\unimod}$.
    \end{itemize}
    
    We differentiate several cases in which $h$ maps the atoms of $\body(\rho)$ to $\reify{\unimod}\cup \db$:
    \begin{enumerate}
        \item\label{item:reify-ii-1} Suppose $h$ maps the atom $\alpha$ from $\body(\rho)$ into $\reify{\unimod}\setminus \db$. If  $\alpha$ is an atom over $\Sigma_{\le 2}$, then $h$ will map it not only to $\reify{\unimod}$, but also to $\unimod$ by the definition of reification. Therefore, we suppose that $\alpha$ is an atom over $\Sigma_{\ge 3}$. Then, it is part of the conjunction in $\body(\rho)$ consisting of the ``complete set'' of atoms of the form $\rpred_{i}(u, v{}_i)$ (with $1\le i \le \arity{\rpred}$) which are mapped to $\rpred_{i}(h(u), h(v{}_{i}))\in \reify{\unimod}$ such that there is an atom $\beta = \rpred(h(v{}_{1}), \ldots, h(v{}_{\arity{\rpred}}))\in \unimod$ and $h(u)=u_{\beta}$. 

        
        \item\label{item:reify-ii-2} Suppose $h$ maps the atom $\alpha$ from $\body(\rho)$ into $\db$. Hence, $\alpha$ is of the form $\rpred(\vvv)$, where either (1) $\rpred\in\Sigma_{\le 2}$ or (2) $\rpred\in\Sigma^{\mathrm{rf}}$. Since $\db$ restricted to the signature $\Sigma_{\le 2}$ is a sub-instance of $\db'$, $\alpha$ is mapped via $h$ to $\db'$ in case (1). In case (2), there exists an atom $\beta = \rpred(h(v{}_{1}), \ldots, h(v{}_{\arity{\rpred}}))$ in $\body(\rho_{\mathrm{urf}})$ such that $\alpha = \rpred_{i}(u_{\beta}, v{}_{i}) \in \reify{\beta}$. As $\rho = \reify{\rho_{\mathrm{urf}}}$, the conjunction 
        \[ \reify{\beta} = \bigwedge_{1\le i \le \arity{\rpred}}\rpred_{i}(u_{\beta}, v{}_{i})\] 
        appears in $\body(\rho)$. Furthermore, since $h(u_{\beta})$ is a constant appearing in $\db$, and the whole of $\body(\rho)$ is mapped into $\db$, we know that each $h(v{}_{i})$ is a constant, and hence, every $\rpred_{i}(u_{\beta}, v{}_{i})$ is mapped into $\db$. Consequently, $\beta$ is mapped via $h$ to an atom of $\db'$, and in the case of $\alpha$ being an atom over $\Sigma^{\mathrm{rf}}$, it is also part of a conjunction $\bigwedge_{1\le i \le \arity{\rpred}}\rpred_{i}(u_{\beta}, v{}_{i})$, which is the same as $\reify{\beta}$, and which constitutes a ``full set'' of $\Sigma^{\mathrm{rf}}$ atoms holding that are mapped atom by atom to $\db$. Also, note that by construction, $\beta \in \db'$. %This will be of use later on, \sebastian{Don't give previews, stick to the line of argumentation strictly chronologically.} when we are reintroducing the unreified atoms in order to make use of $\unimod$ being a model of $(\db, \reify{\ruleset})$.
        
        
\end{enumerate}
    
    Putting all of this together, we obtain the following: Every atom over $\Sigma_{\le 2}$ is mapped by $h$ either into $\db$ or into $\reify{\unimod}$. In the former case, each atom over $\Sigma_{\le 2}$ is also mapped to $\db'$, as we are not dealing with predicates introduced by reification. In the latter case, by the definition of reification, it follows that each atom is actually mapped to $\unimod$.
    Atoms over $\Sigma^{\mathrm{rf}}$ (meaning that they are of the form $\rpred_{i}(u, v_{i})$ for $\rpred\in\Sigma_{\ge 3}$) are dealt with in two cases: The first is when $h(u)$ is a constant. Then, they are mapped into $\db$ (meaning that $h(v{}_{i})$ is a constant), so by \cref{item:reify-ii-2}, we know that the whole conjunction $\bigwedge_{1\le i \le \arity{\rpred}}\rpred_{i}(u, v{}_{i})$ of $\rho$ is mapped to $\db$. Furthermore, by the same token, we know that $\rpred(h(v{}_{1}), \ldots, h(v{}_{\arity{\rpred}})) \in \db'$.
    For the second case (meaning that $h(u)$ is a null) note that first it is mapped to $\reify{\unimod}$ and by \cref{item:reify-ii-1} we obtain an analogous result where we know that the whole conjunction $\bigwedge_{1\le i \le \arity{\rpred}}\rpred_{i}(u, v{}_{i})$ of $\rho$ is mapped to $\reify{\unimod}$. Furthermore, by the same token, we know that $\rpred(h(v{}_{1}), \ldots, h(v{}_{\arity{\rpred}})) \in \unimod$.
    This implies that the body of $\rho_{\mathrm{urf}}$ is mapped into $\unimod$ (note that $\db'\subseteq \unimod$ as $\unimod$ is a model of $\db'$) by $h$. %$h|_{(\vx\cup\vy)\setminus \vu}$ (which is the homomorphism $h$ restricted to only map variables from $\vx$ to terms in $\unimod$).\sebastian{Here, it seems $\vx$ are just the body variables of $\rho$}
    Since $\unimod$ is a model of $(\db', \ruleset)$, $\head(\rho_{\mathrm{urf}})$ is mapped into $\unimod$ by a homomorphism $h_{\mathrm{head}}$ extending $h$ mapping $\vz$ to $\vt$, componentwise, for a tuple of terms $\vt$ from $\unimod$.
    Then, by reifying again, we obtain by \cref{fact:reification-homm} that $\reify{h_{\mathrm{head}}}$ is a homomorphism that maps $\reify{\head(\rho_{\mathrm{urf}})}$ to $\reify{\unimod}$. Note that, by the definition of reification for rules, $\reify{\head(\rho_{\mathrm{urf}})} = \head(\rho)$. 
    Consequently, $\rho$ is satisfied in $\reify{\unimod}\cup\db$.
    
    Additionally, as $\db$ is finite and since $\reify{T}$ is a tree decomposition of $\reify{\unimod}$ of finite width (see \cref{obs:reify-tree-ftw}), we can conclude that $\reify{\unimod}\cup \db$ has finite treewidth (a witnessing tree decomposition can be obtained from $\reify{T}$ by adding every term from $\db$ to every node).
    
    To prove universality of $\reify{\unimod}\cup \db$, we consider an arbitrary instance $\inst$ over $\Sigma^\mathrm{rf}$ satisfying $(\db, \reify{\ruleset})$ and show the existence of a homomorphism $h^\mathrm{univ}$ from $\reify{\unimod}\cup \db$ into $\inst$. 
    Let $\inst' = \fcn{dereify}(\inst)$, that is, $\inst'$ is obtained from $\inst$ in the same way $\db'$ was obtained from $\db$. 
%    The following properties hold:
%    \begin{enumerate}%[(a)]
%        \item\label{item:reifybttsfcs1} $\inst'$ satisfies $(\db', \ruleset)$ \sebastian{WHY??? Argument/reference missing!} and
%        \item\label{item:reifybttsfcs2} $\db\subseteq \inst$.
%    \end{enumerate}
    
%    Note that first $\db \subseteq \inst$. Secondly, 
    We next show Claim~${\dag}$: $\inst'$ satisfies $(\db', \ruleset)$. Because $\db\subseteq \inst$, we immediately obtain $\db'\subseteq \inst'$. It remains to show that $\ruleset$ is satisfied in $\inst'$. For this suppose that $\rho \in\ruleset$ of the form \[ \forall\vx\vy \phi(\vx, \vy) \rightarrow \exists\vz\psi(\vy, \vz) \] 
    and $h$ is a homomorphism mapping $\body(\rho)$ to $\inst'$. Similar to before, $v{}$ or $v{}_{i}$ will signify variables from $\vx\vy$. Furthermore, let 
    \[ \reify{\rho} = \forall\vx\vu\vy\,\reify{\phi}(\vx, \vu, \vy) \rightarrow \exists\vz\vu'\,\reify{\psi}(\vy, \vz, \vu'), \] 
    where we explicitly mention the nulls introduced by the reification of $\rho$, namely $\vu$ and $\vu'$. 
    For each atom of $\body(\rho)$, there are two possibilities: Either the atom is over $\Sigma_{\le 2}$, or it is over $\Sigma_{\ge 3}$. 
    $h$ (and any extension of it) already maps atoms from the first case directly into $\inst$. 
    For the second case, let $\alpha$ be such an atom from $\body(\rho)$. 
    We know by the definition of $\inst'$ that any atom of the form $\rpred(t_{1}, \ldots, t_{\arity{\rpred}})\in\inst'$ corresponds to $\{\rpred_{1}(t{}, t_{1}), \ldots, \rpred_{\arity{\rpred}}(t{}, t_{\arity{\rpred}})\}\subseteq \inst$ for some $t{}\in\adom{\inst}$. 
    In this case, we extend $h$ to a homomorphism $h^{\alpha}$ by mapping $u_{\alpha}$ to $t{}$. Since $u_{\alpha}$ appears only in the conjunction $\bigwedge_{1\le i \le \arity{\rpred}}\rpred_{i}(u_{\alpha}, v{}_{i})$ in $\body(\reify{\rho})$, $h^{\alpha}$ is a partial homomorphism from $\body(\reify{\rho})$ into $\inst$.
    In this way we extend $h$ successively to a homomorphism $h^{\ast}$ mapping all of $\body(\reify{\rho})$ into $\inst$. As $\inst$ satisfies $(\db, \reify{\ruleset})$, it also satisfies $\reify{\rho}$. Consequently, there is an extension $h^{\ast}_{\mathrm{head}}$ of $h^{\ast}$ mapping $\head(\reify{\rho})$ to $\inst$.
    Concerning the atoms appearing in $\head(\reify{\rho})$ we again have two cases: Either, an atom $\beta$ is over $\Sigma_{\le 2}$ or it is over $\Sigma_{2}^{\mathrm{rf}}$. In the former case, $h^{\ast}_{\mathrm{head}}$ maps $\beta$ into $\inst'$. 
    Note that in this case $\beta$ is an atom from $\head(\rho)$. 
    In the latter case, observe that $\beta$ is a conjunct of a conjunction of the form $\bigwedge_{1\le i \le \arity{\ppred}}\ppred_{i}(u_{\gamma}, z^{\ast}_{i})$ in $\head(\reify{\rho})$ for an atom $\gamma = \ppred(z^{\ast}_{1}, \ldots, z^{\ast}_{\arity{\ppred}})\in \head(\rho)$. 
    This conjunction is mapped via $h^{\ast}_{\mathrm{head}}$ into $\inst$ and by construction, $\gamma$ is mapped by the same homomorphism $h^{\ast}_{\mathrm{head}}$ into $\inst'$.
    It follows that $\head(\rho)$ is mapped by $h^{\ast}_{\mathrm{head}}$ to $\inst'$. 
    As $h$ was an arbitrary homomorphism mapping $\body(\rho)$ into $\inst'$, we have shown that $\inst'$ satisfies $\rho$. And since $\rho$ is an arbitrary rule from $\ruleset$, $\inst'$ satisfies $\ruleset$, establishing Claim~${\dag}$.
    
    
%    We proceed by constructing a homomorphism from $\reify{\unimod}\cup \db$ into $\inst'$. 
    Because of Claim~${\dag}$ and $\unimod$ being a universal model of $(\db',\ruleset)$, there exists a homomorphism $h'\colon \unimod \to \inst'$, which we extend to a homomorphism $h^\mathrm{univ}\colon \reify{\unimod}\to \inst$ in the following way: Observe that for every atom using $\rpred\in\Sigma_{\ge 3}$ of the form 
    \[ \alpha = \rpred(t_{1}, \ldots, t_{\arity{\rpred}})\in \unimod \] 
    we have 
    \[ \rpred_{1}(u_{\alpha}, t_{1}), \ldots, \rpred_{\arity{\rpred}}(u_{\alpha}, t_{\arity{\rpred}})\in\reify{\unimod} \, . \] 
    Moreover, since $h'$ is a homomorphism, it holds that 
    \[ h'(\alpha) = \rpred(h'(t_{1}), \ldots, h'(t_{\arity{\rpred}}))\in \inst'\, , \] 
    %\sebastian{What the heck is $h$ in this equation? Do you mean $h'$???}
    hence there exists a $t{}\in\adom{\inst}$ such that 
    \[ \rpred_{1}(t{}, t_{1}), \ldots, \rpred_{\arity{\rpred}}(t{}, t_{\arity{\rpred}}) \in \inst \, . \] 
    Taking an arbitrary such $t{}$, we let $u_{\alpha}^{h'} = t{}$. Then, $h^\mathrm{univ}$ defined by 
    \[ h^\mathrm{univ}(x) = \begin{cases} h'(x) & \text{if } x\in\adom{\unimod} \\ u_{\alpha}^{h'} & \text{if } x = u_{\alpha} \text{ for some } \alpha \in\unimod \end{cases} \] 
    is a homomorphism.
    We conclude by arguing that $h^\mathrm{univ}$ also serves as a homomorphism from $\reify{\unimod}\cup \db$ into $\inst$. Note that every term in $\adom{\db}$ is already in $\db'$ by construction (albeit, the term is possibly isolated, only occurring in the context of $\top$) of which $\unimod$ is a model (and thus $h$ has the same domain and codomain as $h^\mathrm{univ}$). From this insight, together with the fact that $\db\subseteq \inst$ (due to $\inst$ being a model of $(\db,\reify{\ruleset})$), and the fact that the terms from $\db'$ are constants, the claimed correspondence holds.

    In summary, $\reify{\unimod}\cup\db$ is a universal model of $(\db, \reify{\ruleset})$ with finite treewidth. As $\db$ was assumed to be an arbitrary database over $\Sigma^{\mathrm{rf}}$, we obtain that $\reify{\ruleset}$ is $\bts$, and by \cref{thm:tree-width-implies-clique-width}, this implies that $\reify{\ruleset}$ is also $\fcs$, completing the proof.
\end{proof}

==> ICDT 2023 Updated LaTeXFiles/appendices/reification/reify-iii.tex <==
\subsection{\large $(\database,\ruleset) \models (\mathfrak{q},\Xi)$ \iffi $(\fcn{reify}(\database), \fcn{reify}(\ruleset)) \models \fcn{reify}((\mathfrak{q},\Xi))$}

\newcommand{\damsoq}{(\mathfrak{q},\Xi)}
\newcommand{\rdamsoq}{(\reify{\mathfrak{q}},\reify{\Xi})}
\newcommand{\daq}{\mathfrak{q}}
\newcommand{\rsdaq}{\rs_{\daq}}
\newcommand{\rdaq}{\reify{\mathfrak{q}}}
\newcommand{\msoq}{\Xi}
\newcommand{\msoqv}{\msoq(\vX, \vx)}
\newcommand{\rmsoq}{\reify{\Xi}}
\newcommand{\msoqq}{\Xi(\vX, \vx)}
\newcommand{\rmsoqq}{\reify{\Xi(\vX, \vx)}}
\newcommand{\kbs}{\db, \rs}
\newcommand{\kbr}{\reify{\db}, \reify{\rs}}
\newcommand{\ch}{\sat{\db, \rs}}
\newcommand{\reipm}[1]{#1^{+}}
\newcommand{\instp}{\reipm{\inst}}
%\newcommand{\instp}[1]{\reipm{\inst}}

Let us begin by stating the following observation and fact:

\begin{fact}\label{fact:reify-iii-1}
For a given datalog query $\daq$, a database $\db$, and a rule set $\rs$, the following are equivalent:
\begin{itemize}
    \item $(\kbs) \models \daq$.
    \item $\sat{\kbs} \models \daq$.
    \item $\sat{\sat{\kbs}, \rsdaq} \models \goal$.
\end{itemize}
\end{fact}

\begin{fact}\label{fact:reify-iii-2}
For a given datalog query $\daq$, a database $\db$, and a rule set $\rs$, the following are equivalent:
\begin{itemize}
    \item  $\sat{\kbr} \models \rdaq.$ 
    \item  $\sat{\reify\db, \reify\rs \cup \reify{\rs_{\daq}}} \models \goal.$
\end{itemize}
\end{fact}

\newcommand{\siff}[1]{{\stackrel{\textrm{\cref{#1}}\ \ }{\hfill\iff}} &}
\newcommand{\ssiff}[1]{{\stackrel{#1\ \ }{\hfill\iff}} &}

\begin{lemma}\label{lem:reify-iii-lem-1}
For a given datalog query $\daq$, a database $\db$, and a rule set $\rs$, the following holds:
$$(\kbs) \models \daq \iff (\kbr) \models \rdaq$$
\end{lemma}
\begin{proof}
\begin{align*}
                        & \hspace{-8ex} (\kbs) \models \daq \\
                        \iff & \ch \models \daq \\
\siff{fact:reify-iii-1}    \sat{\ch, \rsdaq} \models \goal\\
\ssiff{\goal \in \sig_0}  \reify{\sat{\ch, \rsdaq}} \models \goal\\
\siff{cor:reify-iv}        \sat{\reify{\ch}, \reify{\rsdaq}} \models \goal\\
\siff{cor:reify-iv}        \sat{\sat{\kbr}, \reify{\rsdaq}} \models \goal\\
%\ssiff{\mathrm{Cor.~\ref{cor:reify-iv}}}        \sat{\reify{\ch}, \reify{\rsdaq}} \models \goal\\
%\ssiff{\mathrm{Cor.~\ref{cor:reify-iv}}}        \sat{\sat{\kbr}, \reify{\rsdaq}} \models \goal\\
\siff{fact:reify-iii-2}    \sat{\kbr} \models \rdaq\\
\siff{fact:reify-iii-1}    (\kbr) \models \rdaq
\end{align*}

\vspace{-4ex}
\end{proof}

\begin{definition}\label{def:reify-iii-reipm}
For an instance $\inst$, let us define the following: $$\reipm{\inst} = \set{\top(u_\alpha) \;|\; \alpha \in \inst} \cup \inst.$$

\vspace{-4ex}~\defend
\end{definition}

\begin{fact}\label{fact:reify-iii-3}
For every instance $\inst$, $\adom{\reipm{\inst}} = \adom{\reify{\inst}}$.
\end{fact}

\begin{observation}\label{obs:reify-iii-hom-closed}
For every DaMSOQ $\damsoq$ and every instance $\inst$ we have:
$$\inst \models \damsoq \iff \reipm{\inst} \models \damsoq$$
\end{observation}
\begin{proof}
Recall that every DaMSOQ is closed under homomorphisms.\\
$(\Leftarrow)$ Note that there exists a homomorphism from $\reipm{\inst}$ to $\inst$.\\
$(\Rightarrow)$ Note that $\inst \subset \reipm{\inst}$.
\end{proof}


\begin{lemma}\label{lem:reify-iii-mso-instp}
If $\msoq$ be an MSO formula and $\inst$ be an instance, then
$$\reipm{\inst} \models \msoq \iff \reify{\inst} \models \reify{\msoq}.$$
\end{lemma}
\begin{proof}

We prove the lemma by induction on the structure of $\msoq=\msoqv$, with the following thesis: For every 
assignment $\mu$ that maps variables from $\vx$ to terms from $\adom{\reipm{\inst}}$ and set variables from $\VX$ to subsets of $\adom{\reipm{\inst}}$ holds
%$$\forall{\vX, \vx}\;\; \reipm{\inst} \models \msoqv \iff \reify{\inst} \models \reify{\msoqv}.$$
$$\reipm{\inst}, \mu \models \msoqv \iff \reify{\inst}, \mu \models \reify{\msoqv}.$$

For the base case, let us assume that $\msoqv$ is atomic. Then, there are three cases to consider:
\begin{itemize}
    \item $\msoqv = \pred{R}(\vx)$ with $\arity{\pred{R}} > 2$. Then, letting $\vx = x_1, \ldots, x_n$, we have $\reify{\msoqv}=\reify{\pred{R}(\vx)} = \exists{y} \bigwedge_{1 \leq i \leq n} \pred{R}_i(y, x_i)$. 
    Now, we note that $\alpha = \pred{R}(\mu(x_1), \ldots, \mu(x_n)) \in \reipm{\inst}$ holds by the definition of $\reify{\cdot}$ \iffi $\reify{\alpha} = \bigwedge_{1 \leq i \leq n} \pred{R}_i(u_\alpha, \mu(x_i)) \in \reify{\inst}$.
    \item $\msoqv = \pred{R}(\vx)$, where $\arity{\pred{R}} \leq 2$. This case trivially follows since $\reify{\pred{R}(\vx)} = \pred{R}(\vx)$ and $\reify{\inst}$ coincides with $\reipm{\inst}$ on atoms of low arity.
    \item $\msoqv = X(x)$, where $X$ is a second-order variable. This case follows as $\reify{X(x)} = X(x)$.
\end{itemize}

The cases for the Boolean connectives are trivial. Therefore, we prove one of the quantifier cases and note that all other cases are shown in a similar fashion.
Assume $\msoqv = \forall{y}\; \msoq'(\vX, \vx, y)$. 
            By induction hypothesis, we know that for every 
            %$\vT \subseteq \adom{\reipm{\inst}}^{|\vT|}, 
            $t' \in \adom{\reipm{\inst}}$, 
            %and  $\vt \in \adom{\instp}^{|\vt|}$, 
            we have:
            \begin{align*}
            & \instp,\mu\cup\{y \mapsto t'\}\models \msoq'(\vX, \vx, y) \iff\\[-0.8ex] 
            & \ \ \ \ \reify{\inst},\mu\cup\{y \mapsto t'\} \models \reify{\msoq'(\vX, \vx, y)}.
            \end{align*}
            From this and \cref{fact:reify-iii-3}  we may conclude that the thesis holds for $\msoqv = \forall{y}\; \msoq'(\vX, \vx, y)$.
%
%\begin{itemize}
%\item $\msoqv = \forall{y}\; \msoq'(\vX, \vx, y)$. This case is analogous.
%\item $\msoqv = \exists{Y}\; \msoq'(\vX, \vx, Y)$. This case is analogous.
%\item $\msoqv = \forall{Y}\; \msoq'(\vX, \vx, Y)$. This case is analogous.
%\end{itemize}
\end{proof}

Finally, combining \cref{cor:reify-iv}, \cref{lem:reify-iii-lem-1}, \cref{obs:reify-iii-hom-closed}, and \cref{lem:reify-iii-mso-instp}, we obtain the following corollary:

\begin{corollary}\label{cor:reify-iii}
For every DaMSOQ $\damsoq$, every database $\db$, and every rule set $\rs$, we have:
$$(\kbs) \models \damsoq \!\iff\! (\kbr) \models \rdamsoq.$$
\end{corollary}
\begin{proof}
From \cref{lem:reify-iii-lem-1} we know that:
$$(\kbs) \models \daq \iff (\kbr) \models \rdaq.$$
Moreover, by \cref{obs:reify-iii-hom-closed} and \cref{lem:reify-iii-mso-instp}, we obtain:
\begin{align*}
    &\hspace{-8ex} (\kbs) \models \msoq\\        
\ssiff{\text{$\msoq$ is hom. closed}} \sat{\db, \rs} \models \msoq\\
\siff{obs:reify-iii-hom-closed} \reipm{(\sat{\db, \rs})} \models \msoq\\
\siff{lem:reify-iii-mso-instp}  \reify{\sat{\db, \rs}} \models \rmsoq\\
\siff{cor:reify-iv}             (\kbr) \models \rmsoq
\end{align*}

\vspace{-4ex}
\end{proof}


==> ICDT 2023 Updated LaTeXFiles/appendices/reification/reify-iv.tex <==



\subsection{$\sat{\hspace{-0.3mm}\fcn{reify}(\instance),\!\fcn{reify}(\ruleset)\hspace{-0.3mm}} \equiv \fcn{reify}(\sat{\instance\!,\hspace{-0.3mm}\ruleset})$}


\newcommand{\homfrom}{h_{\leftarrow}}
\newcommand{\homto}{h_\to}
\newcommand{\homtop}{h'_\to}

%\sebastian{We need to go back to isomorphism (which is also what the proof does anyways), equality doesn't really hold. Do not use $\equiv$, rather use words, or $\cong$ (to be introduced locally).}

%\begin{definition}
%Let $\alpha$ be any atom then with $\reifynew{\alpha}$ we will mean the newly introduced term.
%\end{definition}

\begin{definition}\label{def:reify-hom-to}
Let $h$ be a homomorphism from some instance $\inst$ to other instance $\inst'$. We let $\reify{h}$ denote the following homomorphism from $\reify{\inst}$ to $\reify{\inst'}$:
%
$$ \reify{h}(x) = \begin{cases}
\homm(x)\;&\text{if $x \in \termset(\inst)$},\\
u_{h(\alpha)}\;&\text{if $x$ = $u_{\alpha}$},
 \text{where $\alpha$ is an atom of $\inst$}.\ \ \ 
\end{cases}
$$

\vspace{-4ex}
~\defend
\end{definition}

\begin{fact}\label{fact:reification-homm}
If $\homm$ is a homomorphism from $\inst$ to $\inst'$, then $\reify{\homm}$ is a homomorphism from $\reify{\inst}$ to $\reify{\inst'}$.
\end{fact}

\begin{definition}\label{def:reify-hom-from}
Let $\inst$ and $\inst'$ be instances and let $h$ be a homomorphism from $\reify{\inst}$ to $\reify{\inst'}$. We let $\reifym{h}$ denote the function $t \mapsto \homm(t)$ from $\inst$ to $\inst'$, i.e. the restriction of $h$ to elements of $\adom{\inst}$.
\defend
\end{definition}


\begin{fact}\label{fact:reification-homm-two}
If $\homm$ is a homomorphism from $\reify{\inst}$ to $\reify{\inst'}$, then $\reifym{\homm}$ is a homomorphism from $\inst$ to $\inst'$.
\end{fact}

\begin{observation}\label{obs:reification-bijection}
Given two instances $\inst$ and $\inst'$ and two sets of homomorphisms $H = \set{h : \inst \to \inst'}$ and $H' = \set{h : \reify{\inst} \to \reify{\inst'}}$, the function $\reify{\cdot}$ is a bijection from $H$ to $H'$.
\end{observation}
\begin{proof}
Follows from \cref{def:reify-hom-to} and \cref{def:reify-hom-from}.
\end{proof}

We now prove the following statement by induction on $n$: For every instance $\inst$ and every rule set $\ruleset$, 
$$
\pn{n}.
$$
%\sebastian{This is using formal notation where none is defined (we haven't defined quantification over instances or rule sets). Use verbal descriptions. Also, $\inst$ and $\ruleset$ can be fixed upfront and do not need to go into the statement. I also would prefer not to use $P(n)$ just call it the induction statement.}

\textit{Base case.} We note that the base case for $n = 0$ is trivial since
$$
\pnl{0} = \reify{\inst} = \pnr{0}.
$$
Hence, we show the case for $n = 1$, that is, we show that
$$
\pnl{1} \equiv \pnr{1}.
$$
We define two homomorphisms: (i) $\homto$ from $\pnl{1}$ to $\pnr{1}$ and (ii) $\homfrom$ from $\pnr{1}$ to $\pnl{1}$. For any term $t$ in $\reify{\inst}$ we set $\homto(t) = t = \homfrom(t)$. By \cref{obs:reification-bijection}, we know that any trigger $\tau = (\rho, \homm)$ in $(\inst, \ruleset)$ is mirrored in $(\reify{\inst}, \reify{\ruleset})$ by $\tau' = (\reify{\rho}, \reify{\homm})$. Moreover, we know that both $\tau$ and $\tau'$ are satisfied in $\pnl{1}$ and $\pnr{1}$  by the homomorphisms $\homm'_l : \head(\rho) \to \ksat{1}{\inst, \rs}$ and $\homm_r : \head(\reify{\rho}) \to \pnr{1}$, respectively. Let $\homm_l = \reify{\homm'_l}$ be a homomorphism from $\head(\reify{\rho})$ to $\pnl{1}$.

Let us assume that an application of $\tau$ resulted in the creation of a new atom $\pred{R}_i(t,u)$ in $\pnl{1}$ (after reification). Let $\pred{R}_i(x,v_u)$ be the respective atom of the head of $\reify{\rho}$. Then, we set $\homto(u) = \homm_r(v_u)$, and if $x$ is existentially quantified, we set $\homto(t) = \homm_r(x)$. 

Let us assume that an application of $\tau'$ resulted in the creation of a new atom $\pred{R}_i(t,u)$ in $\pnr{1}$. Let $\pred{R}_i(x,v_u)$ be the respective atom of the head of $\reify{\rho}$. Then, we set $\homfrom(u) = \homm_l(v_u)$, and if $x$ is existentially quantified, we set $\homfrom(t) = \homm_l(x)$. 


\begin{comment}
% old version just in case
First we will construct homomorphism $\homto$ from $\pnl{1}$ to $\pnr{1}$. For any term $t$ in $\reify{\inst}$ we set $\homto(t) = t$.
Let $\alpha$ be a new atom in $\ksat{1}{\inst, \ruleset}$ created from application of some trigger $(\rho, \homm)$. Let $\homm'$ be the homomorphism from the atom $\beta$ appearing in the head of $\rho$ that is responsible for creation of $\alpha$.
%\sebastian{Doesn't always exist: $\head(\rho)$ can contain several atoms!!!}
Intuitively speaking we will set $\homto(\reify{\alpha}) = \reify{\homm'}(\head(\reify{\rho}))$. To properly construct $\homto$, we take an existentially quantified variable $x$ of $\rho$ appearing in $\beta$. Note that $x$ is unchanged in $\reify{\rho}$. Thus $\homm'(x) = \reify{\homm'}(x)$, and so we set $\homto(\homm'(x)) = \homm'(x)$. We set $\homto(u_\alpha)$ to $\reify{\homm'}(x_\alpha)$ where $x_\alpha$ is the new existentially quantified variable in the head of $\reify{\rho}$. 
From \cref{obs:reification-bijection} we know that $(\reify{\rho}, \reify{\homm})$ is a trigger in $(\reify{\inst}, \reify{\ruleset})$, thus we know that $\homto$ is a homomorphism.
%
Now, we will construct homomorphism $\homfrom$ from\\ $\pnr{1}$ to $\pnl{1}$. 
Let $\pred{R}(t,u)$ be a new atom in $\pnl{1}$ created from application of some trigger $(\reify{\rho}, \homm)$. Let $\pred{R}(x,u_\beta)$ be the atom appearing in the head of $\rho$ that is responsible for creation of $\pred{R}(t,u)$, where $\beta$ is an atom of $\head(\rho)$ such that $\pred{R}(x,u_\beta) \in \reify{\beta}$. Let $\homm'$ be the homomorphism from $\pred{R}(x,u_\beta)$ to $\pred{R}(t,u)$.
If $x$ is an existential variable we note that $x$ is unchanged in $\reify{\rho}$ when compared to $\rho$. Thus $\homm'(x) = \reifym{\homm'}(x)$, and so we set $\homfrom(t) = \homm'(x)$. 
When $x$ is not an existentially quantified variable, the value of $\homfrom(t)$ is already set.
From \cref{obs:reification-bijection} we know that $(\reifym{\homm}, \rho)$ is a trigger in $(\reify{\inst}, \reify{\ruleset})$ and so there exists a homomorphism $\homm''$ from $\beta$ to some atom $\alpha$ in $\pnl{1}$ such that $\homm''(x) = \reifym{\homm}(x)$ for every frontier variable. We set $\homfrom(u) = u_\alpha$. Recall, as noted before, that $(\rho, \reifym{\homm})$ is a trigger in $(\inst, \ruleset)$. Thus we know that $\homfrom$ is a homomorphism.
\end{comment}

\textit{Inductive step.} Now, given a natural number $n$, we will prove the claim for $n+ 1$, assuming that it holds for every natural number $i \leq n$.
\begin{align*}
\pnl{n + 1} =&\; \reify{\ksat{1}{\ksat{n}{\inst, \ruleset}, \ruleset}} \\
            \equiv&\; \ksat{1}{\reify{\ksat{n}{\inst, \ruleset}}, \reify{\ruleset}}\\
            \equiv&\; \ksat{1}{\ksat{n}{\reify{\inst}, \reify{\ruleset}}, \reify{\ruleset}}\\
            %=&\; \ksat{1}{\pnr{n}. \reify{\ruleset}}\\
            =&\; \pnr{n + 1}
\end{align*}
Therefore, we may conclude the following: %\sebastian{Same here don't use formal quantifiers in undefined ways, just start the statement along the lines ``For every instance $\inst$ and rule set $\ruleset$...}
\begin{corollary}\label{cor:reify-iv}
For every instance $\inst$ and every rule set $\ruleset$,
$$
\pn{\infty}.
$$
\end{corollary}
\begin{proof}
\begin{align*}
\pnl{\infty} =&\; \reify{\bigcup_{i\in\mathbb{N}} \ksat{i}{\inst, \ruleset}}\\
            =&\; \bigcup_{i\in\mathbb{N}} \pnl{i}\\
            \equiv&\; \bigcup_{i\in\mathbb{N}} \pnr{i}\\
            =&\; \pnr{\infty}
\end{align*}
\end{proof}

==> ICDT 2023 Updated LaTeXFiles/appendices/reify.tex <==
\section{Justification of \Cref{ex:badnewsternary} (\NoCaseChange{\cref{sec:cw-vs-tw}})}\label{app:example-15-justification}

To provide some insight into why $\inst_\mathrm{tern}$ from \Cref{ex:badnewsternary} does not have finite cliquewidth, first observe that the instance has the structure of the natural number line, but with an additional term (viz. $-1$) that stands in a ternary relation with each natrual number and its successor. We will argue that no coloring $\coloring$ exists such that $(\inst_{\mathrm{tern}},\coloring)$ is isomorphic to a colored instance represented by some well-decorated tree $\mathcal{T}$. For a contradiction, let us suppose the contrary. Then, we may assume w.l.o.g. that some node $s$ in $\mathcal{T}$ is decorated with $-1_k(s)$ (if $-1$ is assumed to be a null, introduced by a node $\const{*}_k(s)$, then an almost identical argument can be given). Now, we know that at some node $s'$ along the path from $s$ to the root $\varepsilon$ of $\mathcal{T}$ a disjoint union will occur introducing an infinite amount of pairs of consecutive natural numbers. In order for the ternary edges to be added between $-1$ and each pair of consecutive natural numbers, an infinite number of $\pred{Add}_{\rpred,\vk}$ operations are required. However, since only a finite number of operations can be performed after the introduction of $-1$ (as only a finite number of nodes exist between $s$ and the root $\varepsilon$ of $\mathcal{T}$), all such ternary edges cannot be added, showing that for all colorings $\coloring$, $(\inst_{\mathrm{tern}},\coloring)$ is not isomorphic to a colored instance represented by some well-decorated tree. Concomitantly, the rule set $\ruleset_\mathrm{tern} = \{ \rpred(v,x,y) \to \exists z \rpred(v,y,z) \}$ is $\bts$, but not $\fcs$.  


\section{Properties of Reification (\NoCaseChange{\cref{sec:cw-vs-tw}})}

\newcommand{\reify}[1]{\fcn{reify}(#1)}
\newcommand{\reifym}[1]{\fcn{reify}^{-1}(#1)}
\newcommand{\homm}{h}
\newcommand{\reifynew}[1]{\fcn{new}(\reify{#1})}
\newcommand{\newreify}[1]{\reifynew{#1}}
\newcommand{\pn}[1]{\reify{\ksat{#1}{\inst, \ruleset}} \equiv \ksat{#1}{\reify{\inst}, \reify{\ruleset}}}
\newcommand{\pnl}[1]{\reify{\ksat{#1}{\inst, \ruleset}}}
\newcommand{\pnr}[1]{\ksat{#1}{\reify{\inst}, \reify{\ruleset}}}

%%%%%%%%%%%%
%  Reification (i)
%%%%%%%%%%%%
\input{appendices/reification/reify-i}


%%%%%%%%%%%%
%  Reification (iv)
%%%%%%%%%%%%
\input{appendices/reification/reify-iv}

%%%%%%%%%%%%
%  Reification (ii)
%%%%%%%%%%%%
\input{appendices/reification/reify-ii}




%%%%%%%%%%%%
%  Reification (iii)
%%%%%%%%%%%%
\input{appendices/reification/reify-iii}

==> ICDT 2023 Updated LaTeXFiles/appendices/tree-width-clique-proof-simplified.tex <==
\begin{proof}
Let $T = (V,E)$ be a tree-decomposition of $\inst$ witnessing that $\inst$ has a treewidth of $k$. 
Then, countability of $\inst$ implies countability (and thus countable degree) of $(V,E)$.

Therefore, $(V,E)$ can be oriented (by repeated introduction of $E$-neighboring copies of nodes) and transformed into a full binary tree $T'=(V',E',\termset)$ with $V'= \{0,1\}^*$, $E'= \{(s,s0), (s,s1) \mid s\in\{0,1\}^*\}$, and $\termset:V'\to 2^{\adom{\inst}}$, which inherits all tree decomposition properties from $T$. The moderate reformulation using the $\termset$ function is necessary due to the introduction of node copies containing identical sets of terms.

Let $\fcn{slot}: \adom{\inst} \to \{0,\ldots,k\}$ be a function that satisfies $\fcn{slot}(t_1)\neq \fcn{slot}(t_2)$ for any $t_1\neq t_2$ with $\{t_1,t_2\} \subseteq \termset(s)$ for some $s\in V'$; note that the existence of such a function is guaranteed by the treewidth bound of $T'$ inherited from $T$. Moreover, for each domain element $t\in \adom{\inst}$ let $\fcn{pivot}(t)$ denote the node $s \in V'$ with $t \in \termset(s)$ that is closest to the root of $T'$.
%
For each atom $\rpred(t_1,t_2) \in \inst$, one of the following three statements must hold for $T'$:

\begin{itemize}
    \item $\fcn{pivot}(t_1) = \fcn{pivot}(t_2)$, denoted $t_1 \approx t_2$,
    \item $\fcn{pivot}(t_1)$ is an ancestor of $\fcn{pivot}(t_2)$, denoted $t_1 \prec t_2$,
    \item $\fcn{pivot}(t_2)$ is an ancestor of $\fcn{pivot}(t_1)$, denoted $t_2 \prec t_1$.
\end{itemize}

Let now the finite set $\cols$ of colors consist of pairs $(j,S)$ with $0\leq j\leq k$ and $S$ being a subset of
$$ 
\{ \rpred(\downarrow) \mid \rpred \in \Sigma_1 \} \cup \{ \rpred(\downarrow,i), \rpred(i,\downarrow), \rpred(\downarrow,\downarrow) \mid \rpred \in \Sigma_2, 0\leq i\leq k\}.
$$

Let us provide a description of the process transforming~$T'$ into a $(\cols,\mathrm{Cnst},\Sigma)$–well-decorated infinite binary tree representing $\inst$. For a node $s$ of $T'$, we define $\fcn{tf}(s)$ as follows:

\begin{itemize}
\item Take a fresh node $v$, decorate it with $\oplus$, and set its two children to be $\fcn{tf}(s0)$ and $\fcn{tf}(s1)$ with $s0$ and $s1$ the two children of $s$ in $T'$. Set $v$ to be the {\em current root} of the transformation.
\item Next, go through all $t \in \adom{\inst}$ with $\fcn{pivot}(t)=s$, which we assume are in ascending order by $\fcn{slot}(t)$ (there are at most $k+1$ of such terms) and do the following:
    \begin{enumerate}
    \item Take a fresh node $v'$, decorate it with $\oplus$, and set its children to be the current root and a fresh node decorated with $t_{(j,S)}$ if $t \in \mathrm{Cnst}$, or $\const{*}_{(j,S)}$ otherwise, where $j = \fcn{slot}(t)$ and $S$ contains:
        \begin{itemize}
        \item[$\circ$] all $\rpred(\downarrow)$ with $\rpred(t) \in \inst$ and all $\rpred(\downarrow,\downarrow)$ with $\rpred(t,t) \in \inst$, 
        \item[$\circ$] all $\rpred(\downarrow,i)$ with $\rpred(t,t') \in \inst$ for some $t' \in \adom{\inst}$ with $\fcn{slot}(t')=i$ and where $t'\prec t$ or ($t'\approx t$ and $i>j$), and
        \item[$\circ$] all $\rpred(i,\downarrow)$ with $\rpred(t',t) \in \inst$ for some $t' \in \adom{\inst}$ with $\fcn{slot}(t')=i$ and where $t'\prec t$ or ($t'\approx t$ and $i>j$).
        \end{itemize}
    \item Build a chain $P$ of nodes decorated with $\pred{Add}$ and $\pred{Recolor}$ predicates to reflect the following set of operations:
        \begin{itemize}
        \item[$\circ$] for every color $(j,S)$, for which $S$ contains some $\rpred(\downarrow)$, perform $\fcn{Add}_{\rpred,(j,S)}$ and then $\fcn{Recolor}_{(j,S)\to(j,S \setminus \{\rpred(\downarrow)\})}$,
        \item[$\circ$] for every color $(j,S)$ such that $S$ contains some $\rpred(\downarrow,\downarrow)$, perform $\fcn{Add}_{\rpred,(j,S),(j,S)}$ and then $\fcn{Recolor}_{(j,S)\to(j,S \setminus \{\rpred(\downarrow,\downarrow)\})}$,
        \item[$\circ$] for any two colors $(j,S)$ and $(i,S')$, for which $S'$ contains some $\rpred(\downarrow,j)$, perform $\fcn{Add}_{\rpred,(i,S'),(j,S)}$ and immediately afterward perform $\fcn{Recolor}_{(i,S')\to(i,S' \setminus \{\rpred(\downarrow,j)\})}$,
        \item[$\circ$] for any two colors $(j,S)$ and $(i,S')$, for which $S'$ contains some $\rpred(j,\downarrow)$, perform $\fcn{Add}_{\rpred,(j,S),(i,S')}$ and immediately afterward perform $\fcn{Recolor}_{(i,S')\to(i,S' \setminus \{\rpred(\downarrow,j)\})}$.
        \end{itemize}
    \item Set the current root to be the highest node of $P$ and set $v'$ to be the child of the lowest node of $P$.
    \end{enumerate}
\end{itemize}

To obtain $\fcn{tf}(s)$, take the resulting decorated tree and extend the resulting tree to a full binary one by adding missing elements and decorating them with $\pred{Void}$.

Finally, take the root $\varepsilon$ of $T'$, obtain $\fcn{tf}(\varepsilon)$, add on top nodes decorated with $\pred{Add}_\rpred$ for all nullary predicates $\rpred \in \Sigma$ with $\rpred \in \inst$ (in arbitrary order), again 
add missing nodes, and decorate them with $\pred{Void}$.
The resulting $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated tree represents $\inst$.
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% Comment SEBASTIAN'S ORIGINAL VERSION
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{proof} (Sketch)
Let $T = (V,E)$ be a tree-decomposition of $\inst$ witnessing that $\inst$ has a treewidth of $k$.
Then, countability of $\inst$ implies countability (and thus countable degree) of $(V,E)$.
Therefore, $(V,E)$ can be oriented and (by repeated introduction of $E$-neighboring copies of nodes) turned into a(n incomplete) binary tree $T'=(V',E',\termset)$ with $V'\subseteq \{0,1\}^*$ prefix-closed, $E'= \{(s,s0), (s,s1) \mid s\in\{0,1\}^*\} \cap V'\times V'$, and $\termset:V'\to 2^{\adom{\inst}}$ which inherits all tree decomposition properties from $T$.
Let $\mathrm{slot}: \adom{\inst} \to \{0,\ldots,k\}$ be a function that satisfies $\mathrm{slot}(t_1)\neq \mathrm{slot}(t_2)$ for any $t_1\neq t_2$ with $\{t_1,t_2\} \subseteq \termset(v)$ for some $v\in V'$; existence is guaranteed by the treewidth bound of $T$.
Moreover, for each domain element $t\in \adom{\inst}$ let $\mathrm{pivot}(t)$ denote the node $v \in V$ with $t \in \termset(v)$ that is closest to the root of $T'$.
%For each atom $R(\vt)$ from $\inst$, let $$
For each atom $R(t_1,t_2)$ from $\inst$ one of the three holds in $T'$:

\begin{itemize}
    \item $\mathrm{pivot}(t_1) = \mathrm{pivot}(t_2)$, denoted $t_1 \approx t_2$,
    \item $\mathrm{pivot}(t_1)$ is an ancestor of $\mathrm{pivot}(t_2)$, denoted $t_1 \prec t_2$,
    \item $\mathrm{pivot}(t_2)$ is an ancestor of $\mathrm{pivot}(t_1)$, denoted $t_2 \prec t_1$.
\end{itemize}

Let now the finite set $\cols$ of colors consist of pairs $(j,S)$ with $0\leq j\leq k$ and $S$ being a subset of
$$ 
\{ R(\downarrow) \mid R \in \Sigma_1 \} \cup \{ R(\downarrow,i), R(i,\downarrow), R(\downarrow,\downarrow) \mid R \in \Sigma_2, 0\leq i\leq k\}.
$$

Intuitively, now, a $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated infinite binary tree representing $\inst$ can be obtained from $T'$ by 
\begin{enumerate}
    \item independently transforming every node $v$ of $T'$ into a connected assortment of nodes indicating a sequence of instructions (while preserving the ``outer'' parent and child connections of $v$) and
    \item afterwards completing the decorated (but incomplete) binary tree thus obtained by adding all missing elements (including the successor relationships) and declaring them $\mathrm{Void}$.  
\end{enumerate}
In the node-wise transformation, every node $v$ of $T'$ will be substituted by the tree-shaped instruction set advising (bottom-up) the following actions:
\begin{itemize}
\item if $v$ has no children, introduce a complete infinite binary tree, entirely decorated with $\oplus$,
\item if $v$ has one child, introduce an $\oplus$-decorated node with $\szero$ linking to the only child and $\sone$ linking to a complete infinite binary tree, entirely decorated with $\oplus$,
\item if $v$ has two children, introduce an $\oplus$-decorated node linking down to either child via $\szero$ and $\sone$, respectively,
\item next, go through all $t \in \adom{\inst}$ with $\mathrm{pivot}(t)=v$, ordered ascendingly by $\mathrm{slot}(t)$ (there are at most $k+1$ of such terms) and
\begin{itemize}
\item take $\oplus$ of the current state and  a new ``side leaf node'' decorated by $t_{(j,S)}$ (if $t \in \mathrm{Cnst}$) or $\ast_{(j,S)}$ (otherwise), where $j = \mathrm{slot}(t)$ and $S$ contains
\begin{itemize}
\item all $R(\downarrow)$ with $R(t) \in \inst$ and all $R(\downarrow,\downarrow)$ with $R(t,t) \in \inst$,  
\item all $R(\downarrow,i)$ with $R(t,t') \in \inst$ for some $t' \in \adom{\inst}$ with $\mathrm{slot}(t')=i$ and where $t'\prec t$ or ($t'\approx t$ and $i>j$), and
\item all $R(i,\downarrow)$ with $R(t',t) \in \inst$ for some $t' \in \adom{\inst}$ with $\mathrm{slot}(t')=i$ and where $t'\prec t$ or ($t'\approx t$ and $i>j$).
\end{itemize}
\item for every color $(j,S)$, for which $S$ contains some $R(\downarrow)$, perform $\mathrm{Add}_{R,(j,S)}$ and then $\mathrm{Recolor}_{(j,S)\to(j,S \setminus \{R(\downarrow)\})}$
\item for every color $(j,S)$, for which $S$ contains some $R(\downarrow,\downarrow)$, perform $\mathrm{Add}_{R,(j,S),(j,S)}$ and then $\mathrm{Recolor}_{(j,S)\to(j,S \setminus \{R(\downarrow,\downarrow)\})}$
\item for any two colors $(j,S)$ and $(i,S')$, for which $S'$ contains some $R(\downarrow,j)$, perform $\mathrm{Add}_{R,(i,S'),(j,S)}$ and right afterwards  $\mathrm{Recolor}_{(i,S')\to(i,S' \setminus \{R(\downarrow,j)\})}$
\item for any two colors $(j,S)$ and $(i,S')$, for which $S'$ contains some $R(j,\downarrow)$, perform $\mathrm{Add}_{R,(j,S),(i,S')}$ and right afterwards $\mathrm{Recolor}_{(i,S')\to(i,S' \setminus \{R(\downarrow,j)\})}$
\end{itemize}
\end{itemize}



\end{proof}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% Comment
%%%%%%%%%%%%%%%%%%%%%%%%


==> ICDT 2023 Updated LaTeXFiles/binary-case.tex <==

\subsection{The Case of Single-Headed Rules}\label{sec:binary}

In this section, we establish \cref{thm:binary}. To this end, let a binary signature $\sig$, a finite unification set $\ruleset$ of single-headed rules over $\sig$, and a database $\database$ over $\sig$ be arbitrary but fixed for the remainder of the section. \prm{Hence, we will often conveniently}\pin{We will} abbreviate $\sat{\database,\ruleset}$ by $\sa$.
Noting that $\sa$ is a universal model, \cref{thm:binary} is an immediate consequence of the following lemma, which we are going to establish in this section.

\begin{lemma}\label{lem:binary-main}
%There exists an $n \in \mathbb{N}$ s.t. $\cw{\sat{\ruleset, \database}} \leq n$. 
%$\sat{\database,\ruleset}$ has finite cliquewidth.
$\sa$ has finite cliquewidth.
\end{lemma}
%

\msubsection{Looking past datalog}
Let $\se \subseteq \sa$ be the instance containing the \emph{existential atoms} of $\sa$, that is, the atoms derived via the non-datalog rules of $\ruleset$. We show that $\se$ forms a \emph{typed polyforest}, meaning that $\se$ can be viewed as a directed graph where
(i) edges are typed with binary predicates from $\sig$ and (ii) when disregarding the orientation of the edges, the graph forms a forest.
This implies that $\se$ has treewidth $1$. A tree decomposition of $\se$ can be extended into a finite-width tree decomposition of $\db \cup \se$ by adding  the finite set $\adom{\db}$ to every node. 
%
In the sequel, we use $\db \cup \se$ as a basis, to which, in a very controlled manner, we then add the ``missing'' non-existential atoms derived via datalog rules. Thereby, $\ruleset$ being $\fus$ will be of great help.

%%%COMMENT%%%
\begin{comment}
\tim{Concerning the sentence: ``If $\sa$ can be derived in multiple ways, we fix a single derivation sequence to determine which atoms are existential.'' which was the second sentence above. Isn't it enough to observe that the atom contains at least one null without consulting a derivation? Since databases only contain constants, we should immediately be able to conclude that any atom with a null was derived via a non-datalog rule. Perhaps we should delete this sentence then, if you agree.}
\piotr{No :) Consider the following rule set $R=$ \begin{itemize}
    \item $A(x) \to \exists{y} E(x,y)$
    \item $A(x) \to \exists{y} F(x,y)$
    \item $E(x,y) \to F(x,y)$
    \item $F(x,y) \to E(x,y)$
\end{itemize}
And the following instance $\set{A(a), E(a,t), F(a, t)} = 
\sat{R, \set{A(a)}}$ there is no way to determine which atom is datalog and which is existential. As a matter of fact, the result of the restricted chase very much depends on the order of rule application. Consider $\set{A(a), E(a, t) F(a, t), E(a, t'), F(a, t')}$. We should discuss that somewhere in the paper as well.
}
\end{comment}
%%%COMMENT%%%




\begin{comment}
\begin{corollary}\label{cor:skeleton-has-bounded-cw}
%The cliquewidth of $\struc^{\se}$ is bounded.
 The cliquewidth of $\se$ is bounded.
\end{corollary}

\begin{proof} %Let $\inst = \se \setminus \db$ and define $\struc^{\inst} = (\sdom^{\inst}, \srel^{\inst})$. 
 By \cref{obs:sate-is-forest}, we know that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest of bounded degree, and by \cref{obs:trees_cw_le3}, we know %$\cw{\struc^{\inst}} \le 2 \cdot |\sig| + 2$
 $\cw{\se \setminus \database} \le 2 \cdot |\sig| + 2$. For some set of typed polytrees in the typed polyforest %$\struc^{\inst}$
 $\se \setminus \database$ (of which there are only finitely many), each has a unique term (which we call a \emph{connection element}) that is connected to a term of $\db$ in %$\struc^{\se}$ 
 $\se$ (which we call a \emph{connection root}). Let $n$ be the number of connection elements in %$\struc^{\inst}$ 
 $\se \setminus \database$ and define the set $\cols_{1} = \{m \in \mathbb{N} \ | \ m \leq n\}$ of colors, which we assume w.l.o.g. to be fresh. Observe that if we additionally extend the set of colors $\cols$ (used in the proof of \cref{obs:trees_cw_le3}) with the set $\cols_{1}$, then we may assume that prior to taking the disjoint union of all typed polytrees in %$\struc^{\inst}$ 
 $\se \setminus \database$ (during the construction process detailed in \cref{obs:trees_cw_le3}) that we have recolored each connection element to a unique color in $\cols_{1}$. We refer to this colored structure as %$(\struc^{\inst},\coloring_{1})$
 $(\se \setminus \database, \coloring_{1})$, and use this fact below to bound the cliquewidth of $\se$. Note that if we color connection elements in the above way, then $\cw{\se \setminus \db} \le 2 \cdot |\sig| + n + 2 \leq 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, with the last inequality following from the fact that the Skolem chase will only connect connection roots to at most $2 \cdot |\sig|$ typed polytrees. Since $\db$ is a finite graph, we know that $\cw{\db} \leq k$, for $k = |\adom{\db}|$; hence, we may assume that the set of colors used to color the graph of $\db$ is $\cols_{2} = \{t \ | \ t \in \adom{\db}\}$, which we assume to be disjoint from all colors in $\coloring_{1}$. We refer to this colored structure as $(\db,\coloring_{2})$, and define $(\struc, \coloring) = (\se \setminus \db,\coloring_{1}) \disun (\db,\coloring_{2})$. Now, for each typed polytree in $(\se \setminus \db,\coloring_{1})$ that has a connection element with color $l$, we apply either $\add{R,(l,t)}{\struc, \coloring}$ or $\add{R,(t,l)}{\struc, \coloring}$ (depending on if the connection element is connected with an edge typed with the predicate $R$ to the connection root, or away from the connection root, respectively), where $t$ is the color of the connection root in $(\db,\coloring_{2})$. We can therefore see that $\cw{\se} \leq |\adom{\database}| + 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, thus proving the observation.
\end{proof}
\end{comment}
%\piotr{This needs some attention, as the proof is more involved now.}
%In the sequel, we will use $\se$ and the $\pred{add}_{R,\vl}$ operation to reconstruct $\sa$ and prove that $\cw{\sa}$ is bounded. However, a specific coloring is required to prove this claim, which is distinct from the coloring used to prove that $\cw{\se}$ is bounded. Thus, we define a new coloring below %that permits us to conclude \cref{thm:binary} 
% by making use of the fact that $\ruleset$ is $\fus$.\footnote{We note that this is not simply a matter of finding the desired coloring, but rather, is a matter of ``recoloring'' in the proper way (see \cref{obs:cross-coloring}).}
%


\msubsection{Rewriting datalog rules}
We transform the datalog subset of $\ruleset$ into a new rule set $\rulesetnorm$\!, which we then use to fix a set of colors and establish the finiteness of $\cw{\sa}$.
%
Letting $\rulesetdl$ denote the set of all datalog rules from $\ruleset$, we note the following useful equation:
$\sa = \sat{\db \cup \se,\rulesetdl}$ ($\dag$).
%
For any $\rpred \in \sig$, we let $\rew{\rpred}$ denote the datalog rule set %\footnote{Recall that in this section, $\sig$ is a fixed binary signature.}
$\set{\varphi(\vx, \vy) \to \rpred(\vy) \mid \exists{\vx} \varphi(\vx, \vy) \in \rewrs{\ruleset}{\rpred(\vy)}}$
%\begin{align*}
%\set{\varphi(\vx, y) \to \rpred(y) & \mid \exists{\vx} \varphi(\vx, y) \in \rewrs{\ruleset}{\rpred(y)}}  \hspace{4.5ex} \text{ if }\arity{\rpred}=1,\\[-1ex]
%\set{\varphi(\vx, y,z) \to \rpred(y,z) & \mid \exists{\vx} \varphi(\vx, y,z) \in \rewrs{\ruleset}{\rpred(y,z)}} \ \text{ if }\arity{\rpred}=2,
%\end{align*}
giving rise to the overall datalog rule set
$
\rulesetnorm = {\bigcup}_{\rpred \in \sig} \rew{\rpred}.
$
We now show that the rule set $\rulesetnorm$ admits an important property:

\begin{lemma}\label{lem:trigger-for-each-rewritten-rule}
For any $\rpred(\vt) \in \sa \setminus (\db \cup \se)$, there exists a trigger $(\rho, h)$ in $\db \cup\se$ with $\rho \in \rulesetnorm$ such that applying $(\rho, h)$ adds $\rpred(\vt)$ to $\db \cup\se$.
\end{lemma}
\prm{\begin{proof}
Given that $\ruleset$ is $\fus$, it follows that for any $\arity{\rpred}$-tuple $\vt$ of terms from $\db \cup \se$, there exists a CQ $\exists \vx \thephi(\vx,\vy) \in \rewrs{\ruleset}{\rpred(\vy)}$ such that the following holds:
%
$$\sat{\db \cup \se,\ruleset} \models \rpred(\vt) \ \ \ \ifandonlyif \ \ \ \db \cup \se \models \exists \vx \thephi(\vx,\vt).
$$
%
Thus, said trigger exists for some $\rho \in \rew{\rpred}$ in $\db \cup \se$.
\end{proof}}
\pin{\begin{proof}
Given that $\ruleset$ is $\fus$, it follows that for any $\arity{\rpred}$-tuple $\vt$ of terms from $\db \cup \se$, there exists a CQ $\exists \vx \thephi(\vx,\vy) \in \rewrs{\ruleset}{\rpred(\vy)}$ such that the following holds:
$\sat{\db \cup \se,\ruleset} \models \rpred(\vt) \ \ifandonlyif \ \db \cup \se \models \exists \vx \thephi(\vx,\vt).
$
Thus, said trigger exists for some $\rho \in \rew{\rpred}$ in $\db \cup \se$.
\end{proof}}
%
From \prm{the above lemma }\pin{\cref{lem:trigger-for-each-rewritten-rule} }and ($\dag$), we \prm{can }conclude $\ksat{1}{\db \cup \se,\rulesetnorm} \;=\; \sa$ ($\ddag$).
%
This \prm{equation }tells us that we can apply \prm{all }rules of $\rulesetnorm$  \prm{within a single }\pin{in one }step to obtain \prm{the same result as }$\sa$. %Using this fact, we can determine (and provide a bound for) the size of the neighborhood in $\se$ that is needed to apply any given rule from $\rulesetnorm$. 
Ultimately, we will leverage this \prm{observation }to bound the cliquewidth of $\sa$.
%, which suffices to conclude \cref{thm:binary}.
%
In view of ($\ddag$), we may reformulate \cref{lem:binary-main} as follows:

\begin{lemma}\label{lem:binary-reformulated}
$\ksat{1}{\db \cup \se, \rulesetnorm}$ has finite cliquewidth.
\end{lemma}

%We dedicate the remainder of the section to establishing the above lemma, which implies the desired result (\cref{thm:binary}).

\msubsection{Separating connected from disconnected rules}
\prm{In the next step}\pin{Next}, we distinguish between two types of rules in $\rulesetnorm$\!.
%We define a datalog rule to be {\em connected} \iffi the variables in its head share the same connected component of its body; a datalog rule is defined to be {\em disconnected} otherwise. 
We \prm{define}\pin{say} a datalog rule \prm{to be}\pin{is} {\em disconnected} \iffi \prm{variables in its head}\pin{its head variables} belong to distinct connected components in its body; otherwise it is called {\em connected}. 
We let $\rulesetnormcon$ denote all connected rules of $\rulesetnorm$ and let $\rulesetnormminus$ denote all disconnected rules\prm{, that is, $\rulesetnorm = \rulesetnormcon \;\uplus\; \rulesetnormminus$}.
%
One can observe that upon applying connected rules, frontier variables can only be mapped to -- and hence connect -- ``nearby terms'' of $\db \cup \se$ (using a path-based distance, bounded by the size of rule bodies), which, together with our insights about the structure of $\db \cup \se$, permits the construction of a tree decomposition of finite width, giving rise to the following lemma:

\begin{lemma}\label{cor:skeleton-plus-has-bounded-cw} 
$\ksat{1}{\db \cup \se,\rulesetnormcon}$ has finite treewidth.
\end{lemma}
%\begin{proof}
%See \cref{appendix:binary} for details.
%\end{proof}

Note that this lemma does not generalize to all of $\rulesetnorm$, since disconnected rules from $\rulesetnormminus$ might realize ``concept products'' as in $\pred{A}(x) \wedge \pred{A}(y) \to \pred{E}(x,y)$. Clearly, such rules from $\rulesetnormminus$ are the reason why $\bts$ fails to subsume $\fus$. Let us define 
$\sep = \ksat{1}{\db \cup \se,\rulesetnormcon}.$
As $\ksat{1}{\se,\rulesetnorm} = \ksat{1}{\sep,\rulesetnormminus}$, all that is left to show is:

\begin{lemma}\label{lem:binary-reformulated-plus}
$\ksat{1}{\sep, \rulesetnormminus}$ has finite cliquewidth.
\end{lemma}

\msubsection{Searching for a suitable coloring}
Having established the finite treewidth of $\sep$ by \cref{cor:skeleton-plus-has-bounded-cw}, its finite cliquewidth can be inferred by \cref{thm:tree-width-implies-clique-width}, implying the existence of a well-decorated tree $\mathcal{T}$ with $\inst^{\mathcal{T}} = \sep$. Moreover, we know that $\sep$ already contains all terms of $\sa$. Thus, all that remains is to ``add'' the missing datalog atoms of $\sa \setminus \sep$ to $\inst^\mathcal{T}$. Certainly, the coloring function $\fcn{col}^\mathcal{T}_\varepsilon$ provided by $\mathcal{T}$ cannot be expected to be very helpful in this task. To work around this, the following \pin{technical} lemma ensures that an arbitrary coloring can be installed on top of a given instance of finite cliquewidth. 
%We note that the full proof of the lemma can be found in the \cref{appendix:binary}.

\begin{lemma}[Recoloring Lemma]%[Recoloring]
\label{cor:recoloring}
Let $\inst$ be an 
%countable 
instance 
%over a binary signature $\sig$ 
satisfying $\cw{\inst} = n$ and let $\coloring' : \adom{\inst} \to \cols'$ be an arbitrary coloring of~$\inst$. Then $\cw{\inst,\coloring'} \leq (n+1) \cdot |\cols'|.$
%\piotr{$\cw{\inst, \coloring'}$.}
\end{lemma}
\begin{proof}(Sketch) Let $\cw{\inst} = n$ be witnessed by a well-decora\-ted tree $\mathcal{T}$. Let $\cols$ with $|\cols|=n$ be the set of colors used in $\mathcal{T}$. We construct a well-decorated tree $\mathcal{T}^{\coloring'}$ representing $(\inst,\coloring')$ and using the color set $(\cols \times \cols') \;\uplus\; \cols' $, thus
witnessing $\cw{\inst,\coloring'} \leq (n+1) \cdot |\cols'|$. 
We obtain $\mathcal{T}^{\coloring'}$ from $\mathcal{T}$ by modifying each node $s$ of $\mathcal{T}$ as follows:
\begin{itemize}
%    \item If $s$ is labeled with $\pred{c}_k$, we change it to $\pred{c}_{(k, k')}$, where $k'=\coloring'(\const{c})$ if $\const{c} \in \mathrm{Cnst}$, and $k'=\coloring'(s)$ otherwise. 
    \item If $s$ is labeled with $\pred{*}_k$, we change it to $\pred{*}_{(k, \coloring'(s))}$. 
    \item If $s$ is labeled with $\pred{c}_k$ with $\const{c} \in \mathrm{Cnst}$, we change it to $\pred{c}_{(k, \coloring'(\const{c}))}$. 
    \item If $s$ is labeled with $\pred{Add}_{\rpred,k}$, we replace $s$ with a sequence of nodes, one for  each decorator in $\set{\pred{Add}_{\rpred,(k,\ell)} \mid \ell \in \cols'}$. We proceed in an analogous fashion for decorators $\pred{Add}_{\rpred,k,k'}$ and $\pred{Recolor}_{k \to k'}$.
    \item If $v$ is labeled with other decorators, we keep it as is.
\end{itemize}
Last, on top of the obtained tree, we apply a ``color projection'' to $\cols'$ by adding recoloring statements of the form $\pred{Recolor}_{(k,\ell) \to \ell}$ for all $(k,\ell) \in \cols \times \cols'$.
To complete the construction, we add the missing nodes to $\mathcal{T}^{\coloring'}$, each decorated with $\pred{Void}$.
\end{proof}

%\vspace{-8pt}
%\noindent
%\pin{(Proof can be found in the \cref{appendix:binary}.)}
%\vspace{2pt}
%\subsection*{\large Search for suitable types}

We proceed by defining types for elements in $\sep$, giving rise to the desired coloring.
For the following, note that by definition, any rule from $\rulesetnormminus$ must have two frontier variables.

\begin{definition}%[Types in $\sep$]
Let $\rho \in \rulesetnormminus$ with $\body(\rho) = \thephi(x_1, x_2,\vy)$, with $x_1$, $x_2$ frontier variables. %\footnote{Note that $x_1 \neq x_2$, otherwise $\rho \in \rulesetnormcon$.} 
 Let us define
$
%\begin{align*}
\rho_1(x) =%&\; 
\exists{\vy x_2}\; \thephi(x, x_2, \vy)
\ \text{and}\ 
\rho_2(x) =%&\; 
\exists{\vy x_1}\; \thephi(x_1, x, \vy).
%\end{align*}
$
%
Then, for a term $t \in \adom{\sep}$, we define its {\em type} $\tau(t)$ as $\big\{\rho_i(x) \mid \rho \in \rulesetnormminus ,\ \sep \models \rho_i(t), i \in \set{1,2}\big\}.$\defend
\end{definition}


\noindent
\prm{Enough groundwork has been laid }\pin{Now, we }define our new coloring function $\coloringe$. Given a term $t$ of $\sep$, we let
$
\coloringe(t) = \tau(t).
$

%Now that we have defined the coloring $\coloringe$, we take $\prcoloringe$ as in \cref{def:recoloring}. Recall, that while $\prcoloringe(t) = \coloringe(t)$ for every term of $\sep$ it has expanded co-domain, required for the following to hold:

\begin{corollary}
There exists an $n_\exists \in \mathbb{N}$ with $\cw{\sep, \coloringe} = n_\exists$.
\end{corollary}
\begin{proof}
From \cref{cor:skeleton-plus-has-bounded-cw} and \cref{thm:tree-width-implies-clique-width}, we know that $\cw{\sep}$ is finite. Hence, there exists a natural number $n$ and a coloring $\coloring$ such that $\cw{\sep, \coloring} = n$. Moreover, the codomain of $\coloringe$ is finite, say $n'$. Thus, we get $n_\exists = (n+1)\cdot n'$ by \cref{cor:recoloring}.
\end{proof}

\msubsection{Coping with disconnected rules}
We now conclude the proof of \cref{lem:binary-reformulated-plus}, i.e., we show that $\cw{\so, \coloringe} \leq n_\exists$, thereby proving \cref{thm:binary}. To this end, consider some rule $\rho \in \rulesetnormminus$. As stated earlier, we can assume that $\rho$ is of the~form
%We now finalize the result by establishing $\cw{\so, \coloringe} \leq n_\exists$, thereby showing \cref{lem:binary-reformulated-plus} and thus proving \cref{thm:binary}. To this end, consider some rule $\rho \in \rulesetnormminus$. As stated earlier, we can assume that $\rho$ is of the~form
%
$
\thephi(x_1, x_2, \vy) \to \rpred(x_1, x_2).
$
%
From this, we obtain the following useful correspondence:

\begin{lemma}\label{lem:col_query_correspondency}
For any $t,t' \in \adom{\sep}$ and $\rho \in \rulesetnormminus$,
$$\sep \models \exists{\vy}\thephi(t,t',\vy) \text{ \ \ \ifandonlyif \ \ } \rho_1(x) \in \tau(t) \text{ and } \rho_2(x) \in \tau(t').$$
\end{lemma}
%
\begin{proof}
\prm{The forward direction} \pin{($\Rightarrow$)} follows from the definition of each set. For \prm{the backward direction} \pin{$(\Leftarrow)$}, we exploit disconnectedness and split $\thephi(x_1, x_2, \vy)$ into two distinct parts. Let $\thephi_1(x_1, \vy_1)$ be the connected component of $\thephi(x_1, x_2, \vy)$ that contains $x_1$, and $\thephi_2(x_2, \vy_2)$ denote the remainder (which includes the connected component of $x_2$). By assumption, $\vy_1$ and $\vy_2$ are disjoint, whence $\exists{\vy}\thephi(t,t',\vy)$ is equivalent to $\exists{\vy_1} \thephi_1(t, \vy_1) \wedge \exists{\vy_2} \thephi_2(t', \vy_2)$. Note that $\rho_1(x) \in \tau(t)$ implies $\sep \models \exists{\vy_1} \thephi_1(t, \vy_1)$, while $\rho_2(x) \in \tau(t')$ implies $\sep \models \exists{\vy_2} \thephi_2(t', \vy_2)$. Therefore, $\sep \models \exists{\vy} \thephi(t, t', \vy)$.
\end{proof}






\begin{lemma}\label{lem:adding_per_rule}
Let $\rho \in \rulesetnormminus$ be of the form 
$\thephi(x_1, x_2, \vy) \to \rpred(x_1, x_2)$. Then,
$$\hspace{-12ex}
\bigcup_%
{\hspace{12ex}
\rho_1\!(x)\in\,\ell,\ \rho_2\!(x)\in\,\ell'
}\hspace{-12ex}
\fcn{Add}_{\rpred,\ell,\ell'}(\sep, \coloringe) = \sep \cup \big\{\rpred(t,t') \mid \sep\models\exists{\vy}\thephi(t,t',\vy) \big\}.$$
\end{lemma}
\begin{proof}
All $\sep$ atoms are contained in both sides of the equation.
Considering any $\rpred(t,t') \not\in \sep$ we find it contained in the left-hand side \iffi $\rho_1(x) \in \coloringe(t) = \tau(t)$ and $\rho_2(x) \in \coloringe(t') = \tau(t')$ \iffi  $\sep \models \exists{\vy}\thephi(t,t'\vy)$ (by \cref{lem:col_query_correspondency}) \iffi $\rpred(t,t')$ is contained in the right-hand side of the equation.
\end{proof}

\noindent
Of course, the right hand side of the equation in \cref{lem:adding_per_rule} coincides with $\ksat{1}{\sep,\{\rho\}}$. 
\prm{We observe -- given that the coloring $\coloringe$ remains unaltered -- that the finitely many distinct applications of $\fcn{Add}_{\rpred,\ell,\ell'}$ in \cref{lem:adding_per_rule} are independent and can be sequentialized without changing the result. Moreover, no such application increases the cliquewidth of the colored instance it is applied to. Since these arguments can be lifted to the application of \emph{all} rules from $\rulesetnormminus$, we obtain}
\pin{We observe -- given that the coloring $\coloringe$ remains unaltered -- that the finitely many distinct applications of $\fcn{Add}_{\rpred,\ell,\ell'}$ in \cref{lem:adding_per_rule} are independent and can be chained without changing the result. Further, no such application increases the cliquewidth of the instance it is applied to. Since these arguments can be lifted to the application of \emph{all} rules from $\rulesetnormminus$, we get}
%
$$
\fcn{cw} \Big(
\sep \cup 
\hspace{-15ex}
\bigcup_%
{\hspace{15ex}
\thephi(x_1, x_2, \vy) {\to} \rpred(x_1, x_2) \, \in \, \rulesetnormminus} 
\hspace{-15ex}
\big\{\rpred(t,t') \mathrel{\big|} \sep\models\exists{\vy}\thephi(t,t',\vy) \big\}\Big) \leq n_\exists.
$$ 
%
Observe that the considered instance is equal to $\so$. Hence, we have established %\pin{(in sequence)} 
\cref{lem:binary-reformulated-plus}, 
concluding \cref{lem:binary-reformulated}, 
which finishes the proof of \cref{lem:binary-main}, 
thus entailing the desired \cref{thm:binary}.

==> ICDT 2023 Updated LaTeXFiles/clique-width.tex <==
\section{Cliquewidth and its Properties}\label{sec:cliquewidth}

In this section, we will propose a width measure, for which we use the term \emph{cliquewidth}.
Our definition of this measure works for arbitrary countable instances %over binary signatures% 
and thus properly generalizes Courcelle's earlier eponymous notions for finite directed edge-labelled graphs \cite{CourEngBook} and countable un\-label\-led un\-di\-rec\-ted graphs \cite{Cou04}, as well as
Grohe and Turán's cliquewidth notion for finite instances of arbitrary arity \cite{GroheT04}.
%While a straightforward generalization to arbitrary signatures (along the lines of Grohe and Turán's cliquewidth notion for finite instances \cite{GroheT04}) is easy to define, we will argue that it falls short of our expectations in the infinite setting. 

\subsection{Cliquewidth of Countable Instances}\label{sec:cwdef}

Intuitively, the notion of cliquewidth is based on the idea of assembling the considered structure (e.g., instance or graph) from its singleton elements (e.g., terms or nodes). To better distinguish these elements during assembly, each may be assigned an initial color (from some finite set $\cols$). The ``assembly process'' consists of successively applying the following operations to %one or two 
previously assembled node-colored structures:%\footnote{More formally, a \emph{colored instance} is a pair $(\instance,\coloring)$ such that $\instance$ is an instance and $\coloring$ is a function mapping elements of $\adom{\instance}$ to colors in a set $\cols$.} 
\begin{itemize}
    \item take the disjoint union of two structures ($\oplus$),
    \item uniformly assign the color $k'$ to all hitherto $k$-colored elements ($\fcn{Recolor}_{k\to k'}$),
    \item given a predicate $\rpred$ and a color sequence $\vk$ of length $\arity{\rpred}$, add $\rpred$-atoms for all tuples of appropriately colored elements ($\fcn{Add}_{\rpred,\vk}$).
%    \item for a binary predicate $\rpred$, add $\rpred$-edges linking each $k$-colored element to every $k'$-colored element ($\fcn{Add}_{\rpred,k,k'}$);
%    \item for a unary predicate $\rpred$, assign $\rpred$ to all $k$-colored elements ($\fcn{Add}_{\rpred,k}$). 
\end{itemize}
Then, the cliquewidth of a structure is the minimal number of colors needed to assemble it \prm{(or rather, some \prm{arbitrarily }colored version of it)} through successive applications of the above operations. % to given (colored) singleton elements.
For finite structures (e.g., graphs and instances), this is a straightforward, conceivable notion. 
In order to generalize it to the countably infinite case, one has to find a way to describe infinite assembly processes. 
%Toward this end, note that in the finite case, the description of the assembly process can be encoded as a nested function-expression using the above operators. 
In the finite case, an ``assembly plan'' can be described by an algebraic expression using the above operators, which in turn can be represented by its corresponding ``syntax tree.'' The more elusive idea of an ``infinite assembly plan'' is then implemented by allowing for infinite, ``unfounded'' syntax trees.
%, which might be likened to non-terminating recursion.
 We formalize this idea of ``assembly-plan-encoding syntax trees'' by representing them as countably infinite instances of a very particular shape.

\newcommand{\szero}{\pred{Succ}_0}
\newcommand{\sone}{\pred{Succ}_1}
\newcommand{\ibtree}{\mathcal{T}_\mathrm{bin}}
\newcommand{\decorum}{\mathrm{Dec}(\cols, \mathrm{Cnst},\Sigma)}

\begin{definition}
We define the \emph{infinite binary tree} to be the instance
$$
\ibtree = \big\{\szero(s,s0) \ \big| \ s {\,\in\,} \{0,1\}^*\big\} \cup 
          \big\{ \sone(s,s1) \ \big| \ s {\,\in\,} \{0,1\}^*\big\}
$$
with binary predicates $\szero$ and $\sone$.
That is, the\prm{infinitely many} nulls of $\ibtree$ are denoted by finite sequences of $0$ and $1$. The \emph{root} of $\ibtree$ is the null identified by the empty sequence, denoted $\varepsilon$.

%SOLVED: \piotr{I would prefer, for the sake of proofs, to have here some set of colors $\cols$, instead of $n$ and fixed $\set{0,\ldots, n}$.}
Given a finite set $\cols$ of \emph{colors}, a finite set $\mathrm{Cnst}\subseteq \mathfrak{C}$ of constants, and a finite signature $\Sigma$, the set $\decorum$ of \emph{decorators} consists of the following unary predicate symbols: 
%(for $k,k'{\in\,} \cols$, $\rpred{\,\in\,} \Sigma$, and $\arity{\rpred}$-tuples $\vk$ from $\cols$):
%SOLVED: \thomas{Because of $k\in \{ 0, \ldots, n \}$ we actually use $n+1$ colors.}

%\smallskip
%\noindent\begin{minipage}[t]{0.59\linewidth}
%\begin{itemize}
%\item $\const{c}_k$ for every $\const{c} \in \mathrm{Cnst} \cup\{\const{*}\}$,
%\item $\pred{Add}_{\rpred,\vk}$
%\end{itemize}
%\end{minipage}
%\begin{minipage}[t]{0.4\linewidth}
%\begin{itemize}
%\item $\pred{Recolor}_{k\to k'}$,
%\item $\oplus$, and
%$\pred{Void}$.
%\end{itemize}
%\end{minipage}\\[1ex]
%
\smallskip
\noindent\begin{minipage}[t]{0.57\linewidth}
\begin{itemize}
\item $\const{c}_k$ for any $\const{c} \in\mathrm{Cnst} \cup\{\const{*}\}$ and $k\in\cols$,
\item $\pred{Add}_{\rpred,\vk}$ for any $\rpred\in\Sigma$ and $\vk\in\cols^{\arity{\rpred}}$,
%\item $\pred{Add}_{\rpred,k,k'}$ for every $\rpred\in \Sigma_2$,
\end{itemize}
\end{minipage}
\begin{minipage}[t]{0.42\linewidth}
\begin{itemize}
\item $\pred{Recolor}_{k\to k'}$ for $k,k'\in \cols$,
\item $\oplus$, and
%\item 
$\pred{Void}$.
\end{itemize}
\end{minipage}\\[1ex]

%
A \emph{$(\cols,\mathrm{Cnst},\Sigma)$-decorated infinite binary tree} (or, \emph{decorated tree} for short) is $\ibtree$ extended with facts over $\decorum$ that only use nulls from the original domain of $\ibtree$, i.e., from $\{0,1\}^*$.
A decorated tree $\mathcal{T}$ is called a  \emph{well-decorated tree} \iffi
\begin{itemize}
\item for every null $s \in \{0,1\}^*$, $\mathcal{T}$ contains exactly one fact $\mathrm{Dec}(s)$ with  $\mathrm{Dec} \in \decorum$,
\item for every $\const{c}\in \mathrm{Cnst}$, $\mathcal{T}$ contains at most one fact of the form $\pred{c}_k(s)$,
%%%
%% THE FOLLOWING MODIFICATION WAS PLAIN WRONG AND HAS BEEN REVERTED -- DO NOT REINTRODUCE!!!
%%
%% \item for every null $s \in \{0,1\}^*$ and every $c\in \mathrm{Cnst}$, $\mathcal{T}$ contains at most one fact of the form $c_k(s)$;
%%
%% NOTE THAT CONSTANTS NEED TO BE UNIQUE ACROSS THE WHOLE MODEL!!!
%%%
\item if $\pred{Add}_{\rpred,\vk}(s) \in \mathcal{T}$ or $\pred{Recolor}_{k\to k'}(s) \in \mathcal{T}$,
       then $\pred{Void}(s0)\not\in \mathcal{T}$ and $\pred{Void}(s1) \in \mathcal{T}$,
\item if $\oplus(s) \in \mathcal{T}$, then $\pred{Void}(s0),\pred{Void}(s1) \not\in \mathcal{T}$,
\item if $\pred{Void}(s) \in \mathcal{T}$ or $\pred{c}_k(s) \in \mathcal{T}$, then  $\pred{Void}(s0),\pred{Void}(s1) \in \mathcal{T}$.\defend
%\item if $\pred{Recolor}_{k\to k'}(s) \in \mathcal{T}$\!, $\pred{Add}_{\rpred,k,k'}(s) \in \mathcal{T}$\!, or $\pred{Add}_{\rpred,k}(s) \in \mathcal{T}$\!, then $\pred{Void}(s0)\not\in \mathcal{T}$ and $\pred{Void}(s1) \in \mathcal{T}$.

\end{itemize}
\end{definition}

Recall that, due to Rabin's famous Tree Theorem \cite{Rabin69}, 
%the MSO theory of $\ibtree$ is decidable, that is, 
%there exists a procedure taking an MSO sentence $\Xi$ as input and decides if $\ibtree \models \Xi$. 
the validity of a given MSO sentence $\Xi$ in $\ibtree$ is decidable.
Also, it should be obvious that, given a decorated tree, checking well-decoratedness can be done in first-order logic. More precisely, fixing $\cols$, $\Sigma$, and $\mathrm{Cnst}$,  there is a first-order sentence $\Phi_\mathrm{well}$ such that for any $(\cols,\mathrm{Cnst},\Sigma)$-decorated tree $\mathcal{T}$, $\mathcal{T}$ is well-decorated \ifandonlyif $\mathcal{T} \models \Phi_\mathrm{well}$. 

\begin{definition}\label{def:entities-tree-to-instance}
Let $\mathcal{T}$ be a $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated tree.
We define the function $\fcn{ent}^\mathcal{T}\!:\{0,1\}^* \to 2^{\mathrm{Cnst} \cup \{0,1\}^*}$ mapping each null $s \in \{0,1\}^*$ to its \emph{entities} (a set of nulls and constants) as follows:
%
$$\fcn{ent}^\mathcal{T}\!(s) = \big\{ ss' \mid \pred{*}_k(ss') \in \mathcal{T}, s' \in \{0,1\}^*\big\} \cup \big\{ \const{c} \mid \pred{c}_k(ss') \in \mathcal{T}, \const{c}\in \mathrm{Cnst}, s' \in \{0,1\}^*\big\}.$$
%
Every tree node $s$ also endows each of its entities with a \emph{color} from $\cols$ through the function $\fcn{col}^\mathcal{T}_s: \fcn{ent}^\mathcal{T}\!(s) \to \cols$ in the following way:
%
$$ \fcn{col}^\mathcal{T}_s\!(e) = \begin{cases}
k &\!\! \text{if } e=\const{c}\in \mathrm{Cnst} \text{ and } \pred{c}_k(s)\in \mathcal{T}, \text{or if } e=s\in \{0,1\}^* \text{ and } \pred{*}_k(s)\in \mathcal{T},\\
%k &\!\! \text{if } e=\const{c}\in \mathrm{Cnst} \text{ and } \pred{c}_k(s)\in \mathcal{T}, \\
%k &\!\! \text{if } e=s\in \{0,1\}^* \text{ and } \pred{*}_k(s)\in \mathcal{T}, \\
k' &\!\! \text{if } \pred{Recolor}_{k\to k'}(s)\in \mathcal{T} \text{ and } \fcn{col}^\mathcal{T}_{s0}(e) = k,\\
\fcn{col}^\mathcal{T}_{s0}(e) &\!\! \text{if } \pred{Recolor}_{k\to k'}(s)\in \mathcal{T} \text{ and } \fcn{col}^\mathcal{T}_{s0}(e) \neq k, \text{or if } \pred{Add}_{\rpred,\vk}(s)\in \mathcal{T},\\
%\fcn{col}^\mathcal{T}_{s0}(e) {\neq} k,\\
%\fcn{col}^\mathcal{T}_{s0}(e) &\!\! \text{if } \pred{Add}_{\rpred,\vk}(s)\in \mathcal{T},\\
\fcn{col}^\mathcal{T}_{sb}(e) &\!\! \text{if } {\oplus}(s) \in \mathcal{T}, e \in \fcn{ent}^\mathcal{T}\!(sb), \text{ and } b \in \{0,1\}.\\
\end{cases}$$
%
\prm{Furthermore, e}\pin{E}very node $s$ is assigned a set of $\Sigma$-atoms over its entities as indicated by the sets $\mathrm{Atoms}_s$\pin{:}\prm{ defined by}
$$ \mathrm{Atoms}_s = 
\begin{cases}
\{\top(\const{c})\} & \!\!\text{if } \pred{c}_k(s)\in \mathcal{T}\!, \const{c} \in \mathrm{Cnst}, \\
\{\top(s)\} & \!\!\text{if } {\pred{*}_k(s)}\in \mathcal{T}, \\
%\{\rpred(e) \mid \fcn{col}^\mathcal{T}_{s}\!(e)=k\} & \!\!\text{if } \pred{Add}_{\rpred,k}(s)\in \mathcal{T}; \\
%\{\rpred(e_1,e_2) \mid \fcn{col}^\mathcal{T}_{s}\!(e_i)=k_i\} & \!\!\text{if } \pred{Add}_{\rpred,k_1,k_2}(s)\in \mathcal{T};\\
\{\rpred(\ve) \mid \fcn{col}^\mathcal{T}_{s}\!(\ve)=\vk\} & \!\!\text{if } \pred{Add}_{\rpred,\vk}(s)\in \mathcal{T},\\
\emptyset & \!\!\text{otherwise.}\\
\end{cases}$$
Defining a \emph{colored instance} as a pair $(\instance,\coloring)$ of an instance $\instance$ and a function $\coloring$ mapping elements of $\adom{\instance}$ to colors in a set $\cols$, we now associate each node $s$ in $\mathcal{T}$ with the %n \emph{$\cols$-
colored $\Sigma$-instance $(\instance^\mathcal{T}_s,\coloring^\mathcal{T}_s)$, 
%(with $\coloring^\mathcal{T}_s: \adom{\instance^\mathcal{T}_s} \to \cols$), 
with
$\instance^\mathcal{T}_s = {\bigcup}_{s'\in \{0,1\}^*}\mathrm{Atoms}_{ss'}$
and
$
\coloring^\mathcal{T}_s = \fcn{col}^\mathcal{T}_{s}.
$
Finally, we define the \emph{colored instance $(\instance^\mathcal{T}\!,\coloring^\mathcal{T})$ represented by $\mathcal{T}$} as $(\instance^\mathcal{T}_\varepsilon\!,\coloring^\mathcal{T}_\varepsilon)$ where $\varepsilon$ is the root of $\mathcal{T}$.
 %$(\instance,\coloring)$ such that a $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated tree $\mathcal{T}$ exists with $(\instance,\coloring) = (\instance^\mathcal{T}\!,\coloring^\mathcal{T})$.\defend
\end{definition}

\begin{definition}
Given a colored instance $(\instance,\coloring)$ over a finite set $\mathrm{Cnst}$ of constants and a countable set of nulls as well as a finite signature $\Sigma$,
the \emph{cliquewidth} of $(\instance,\coloring)$, written $\cw{\instance,\coloring}$, is defined to be the smallest natural number $n$ such that $(\instance,\coloring)$ is isomorphic to a colored instance represented by some $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated tree with $|\cols|=n$.
If no such number exists, we let \mbox{$\cw{\instance,\coloring}= \infty$}. The cliquewidth $\cw{\instance}$ of an instance $\instance$ is defined to be the minimum cliquewidth over all of its colored versions.\defend
\end{definition}

\begin{example}\label{ex:cw-transitivity}
The instance \mbox{$\inst_{<} =  \{\rpred(n,m) \mid n,m \in \mathbf{N}, n < m\}$} has a cliquewidth of $2$, witnessed by the well-decorated tree corresponding to the (non-well-founded) expression $E$ impli\-cit\-ly defined by $E = \fcn{Add}_{\rpred,1,2}({\const{*}_1} \oplus \fcn{Recolor}_{1\to 2}(E))$. 
\end{example}
%
%SR: has been integrated in previous definition
%
%\piotr{Moved those two definitions here}
%\begin{definition}
%Given an instance $\inst$ over some signature $\sig$ and a mapping $\coloring : \termset(\inst) \to \cols$ %where $\cols$ is some set of colors. We say that $\cw{\inst, \coloring} = |\cols|$ \ifandonlyif there %exists a $(\cols,\conset(\inst),\sig)$-well-decorated tree $\mathcal{T}$ such that $\inst^{\mathcal{T}}$ %is isomorphic to $\inst$ and that $\mathrm{col}^\mathcal{T}_\varepsilon = \coloring$.
%\end{definition}
%
We will later use the following operation on decorated trees.
%
\begin{definition}
Let $(\inst,\coloring)$ be a colored instance and $\mathcal{T}$ be a well-decorated tree witnessing that $\cw{\inst, \coloring} \leq n$. Then for any $\rpred \in \Sigma$
we let $\fcn{Add}_{\rpred,\vk}(\inst, \coloring)$ denote the instance $\inst^{\mathcal{T'}}$ represented by the well-decorated tree $\mathcal{T'}$ defined as follows:
\vspace{-0.3ex}
\begin{itemize}
    \item The root $\varepsilon$ of $\mathcal{T'}$ is decorated by $\addd{\rpred,\vk}$,
    \item the left sub-tree of $\varepsilon$ is isomorphic to $\mathcal{T}$,
    \item the right sub-tree of $\varepsilon$ is wholly decorated with $\pred{Void}$.\defend
    \end{itemize}
\end{definition}

%\begin{definition}
%Let $\inst$ be an instance, $\coloring$ be a coloring of terms of $\inst$, and $\mathcal{T}$ be a well-decorated tree witnessing that $\cw{\inst, \coloring} \leq n$. Then, $\fcn{Add}_{\rpred,\ell,\ell'}(\inst, %\coloring)$ (or, $\fcn{Add}_{\rpred, \ell}(\inst, \coloring)$) is taken to be the instance $\inst^{\mathcal{T'}}$ represented by the well-decorated tree $\mathcal{T'}$ defined as follows:
%\begin{itemize}
%    \item The root $\varepsilon$ of $\mathcal{T'}$ is decorated by $\addd{\rpred,\ell,\ell'}$ ($\addd{\rpred, \ell}$, respectively);
%    \item the left sub-tree of $\varepsilon$ will be isomorphic to $\mathcal{T}$;
%    \item the right sub-tree of $\varepsilon$ will be wholly decorated with $\pred{Void}$.
%    \end{itemize}
%\end{definition}

\subsection{Finite-Cliquewidth Sets and Decidability}\label{sec:fcw-decidability}

We now identify a new class of rule sets for which DaMSOQ query entailment is decidable, that is, the class of \emph{finite-cliquewidth sets}. 

\begin{theorem}\label{thm:cliquewidth-k-MSO-decidable}
For a fixed $n\in \mathbb{N}$, determining if a given MSO formula~$\Xi$ 
%over a signature $\Sigma$ 
has a model $\inst$ with $\cw{\inst} \leq n$ is decidable. Thus, cliquewidth is MSO-friendly.
\end{theorem}
%
\begin{proof}\!(Sketch)
We use the classical idea of MSO interpretations.
Picking $\cols=\{1,\ldots,n\}$, one shows that for every given MSO sentence $\Xi$, one can compute an MSO sentence $\Xi'$, %that, next to $\szero$ and $\sone$, uses only unary predicatesthe
such that for every $(\cols,\mathrm{Cnst},\Sigma)$-well-deco\-rated tree $\mathcal{T}$, $\instance^\mathcal{T} \models \Xi$ \iffi $\mathcal{T} \models \Xi'$. 
Thus, checking if $\Xi$ holds in some $\mathrm{Cnst},\Sigma$-instance of cliquewidth ${\leq}{n}$ can be done by checking if $\Xi'$ holds in some $(\cols,\mathrm{Cnst},\Sigma)$-well-decorated tree, which in turn is equivalent to the existence of a $(\cols,\mathrm{Cnst},\Sigma)$-decorated tree that is a model of $\Xi'\wedge \Phi_\mathrm{well}$. 
Obtain~$\Xi''$ from $\Xi'\wedge \Phi_\mathrm{well}$ by re\-in\-ter\-pre\-ting all unary predicates as MSO set variables that are quantified over existentially. $\Xi''$ is an MSO formula over the signature $\{\szero,\sone\}$ which is valid in $\ibtree$ \iffi some decoration exists that makes $\Xi'\wedge \Phi_\mathrm{well}$ true. Thus, we have reduced our problem to checking the validity of a MSO sentence in $\ibtree$, which is decidable by Rabin's Tree Theorem \cite{Rabin69}. 
\end{proof}

With this insight in place and the appropriate rule set notion defined, we can leverage \Cref{thm:decidablequerying} for our decidability result. 

\begin{definition}%[finite-cliquewidth sets]
A rule set $\ruleset$ %over a binary signature 
is called a \emph{finite-cliquewidth set} ($\fcs$) \ifandonlyif for any database $\database$, there exists a universal model for $(\database,\ruleset)$ of finite cliquewidth.
\defend
\end{definition}

\begin{corollary}\label{cor:fcsdecidable}
For every $\fcs$ rule set $\ruleset$, 
the query entailment problem $(\database,\ruleset) \models (\mathfrak{q},\Xi)$ for databases $\database$, and DaMSOQs $(\mathfrak{q},\Xi)$ is decidable.
%the problem of checking $(\db, \ruleset) \models (\mathfrak{q},\Xi)$ for any given database $\database$ and DaMSOQ $(\mathfrak{q},\Xi)$ is decidable.
\end{corollary}

In view of \cref{ex:cw-transitivity}, it is not hard to verify that the rule set $\ruleset^\infty_\mathrm{tran}$ from the introduction is $\fcs$.
Yet, it is neither $\bts$ (as argued before), nor $\fus$, which can be observed from the fact that it does not admit a finite rewriting of the BCQ $\epred(\const{a},\const{b})$.
Notably, it also does not exhibit \emph{finite controllability} ($\mathbf{fc}$), another generic property that guarantees decidability of query entailment~\cite{Ros06}. 
A rule set $\ruleset$ is $\mathbf{fc}$ \iffi for every $\db$ and CQ $q$ with $(\db,\ruleset) \not\models q$ there exists a \emph{finite} \mbox{(possibly non-}\mbox{universal) model} $\inst \models (\db,\ruleset)$ with $\inst \not\models q$.  
Picking $\db=\{\epred(\const{a},\const{b})\}$ and $q=\exists x \epred(x,x)$ reveals that $\ruleset^\infty_\mathrm{tran}$ is not $\fc$. Therefore, $\fcs$ encompasses rule sets not captured by any of the popular general decidability classes (namely, $\bts$, $\fus$, and $\fc$). On another note, is no surprise that, akin to $\bts$, $\fus$, and $\fc$, the membership of a rule set in $\fcs$ is undecidable, which can be argued exactly in the same way as for $\bts$ and $\fus$ \cite{BagLecMugSal11}.


\subsection{Cliquewidth and~Treewidth}\label{sec:cw-vs-tw}

We now show that for binary signatures, the class of instances with finite cliquewidth subsumes the class of instances with finite tree\-width,\prm{implying that $\fcs$ generalizes $\bts$}
\pin{implying $\bts \subseteq \fcs$.} %in the binary case. 

\begin{theorem}\label{thm:tree-width-implies-clique-width}
Let $\inst$ be a countable instance over a binary signature. If $\inst$ has finite treewidth, then $\inst$ has finite cliquewidth.
\end{theorem}
%
\begin{proof}\!(Sketch) We convert a tree decomposition $T$ of $\inst$ with a width $n$ into a well-decorated tree: (1) By copying nodes, transform $T$ into an infinite binary tree $T'$.  (2) For each term $t$ from $\inst$, let the \emph{pivotal} node of $t$ in $T'$ be the node closest to the root containing $t$. For any two terms $t$ and $t'$ from $\inst$ co-occurring in an atom, their pivotal nodes are in an ancestor relationship. (3) Assign one of $n+1$ ``slots'' to every term \prm{such}\pin{so} that \prm{inside}\pin{in} each node of $T'$, every element has a distinct slot. (4) Extract a well-decorated tree from $T'$ by transforming every node into the following bottom-up sequence of operations: (i) $\oplus$-assemble the input from below, (ii) introduce every element for which the current node is pivotal with a color that encodes ``open link requests'' to elements (identified by their slots) further up, (iii) satisfy the color-link requests \prm{transmitted }from below via $\pred{Add}$, (iv) remove the satisfied requests by $\pred{Recolor}$.
\end{proof}
%
We note that the converse of \Cref{thm:tree-width-implies-clique-width} does not hold: Despite its finite cliquewidth, the treewidth of instance $\instance_<$ from \Cref{ex:cw-transitivity}
is infinite, as its $\rpred$-edges form an infinite clique.


To the informed reader, \Cref{thm:tree-width-implies-clique-width} might not come as a surprise, given that this relationship is known to hold for 
%finite labelled graphs \cite{CourEngBook} and 
countable unlabelled undirected graphs\footnote{This follows as a direct consequence of a compactness property relating the cliquewidth of countable undirected graphs to that of their finite induced subgraphs.}~\cite{Cou04}.
%, and also for finite instances of arbitrary arity \cite{GroheT04}.
It does, however, cease to hold for infinite structures with predicates of higher arity. 
%(with our cliquewidth notion naturally extended to higher-arity $\fcn{Add}$ operations, similar to Grohe and Turán \cite{GroheT04}). 

\begin{example}\label{ex:badnewsternary}
Let $\rpred$ be a ternary predicate. %Observe that the 
 The instance $\inst_\mathrm{tern} = \{ \rpred(-1,n,n{+}1) \mid n\in \mathbb{N} \}$ has a treewidth of $2$, however, it does not have finite cliquewidth (see \cref{app:example-15-justification}). Concomitantly, the rule set $\ruleset_\mathrm{tern} = \{ \rpred(v,x,y) \to \exists z \rpred(v,y,z) \}$ is $\bts$, but not $\fcs$.  
% Explanation put in Appendix
\end{example}

\noindent
While this result may be somewhat discouraging, one can show that its effects can be greatly mitigated by the technique of reification.

\begin{definition}
Given a finite signature $\Sigma = \Sigma_{\leq2} \uplus \Sigma_{\geq3}$ divided into at-most-binary and higher-arity predicates, we define the \emph{reified version} of $\Sigma$ as the binary signature $\Sigma^{\smash{\mathrm{rf}}} = \Sigma_{\leq2} \uplus \Sigma^{\smash{\mathrm{rf}}}_{\smash{2}}$ with
$\Sigma^{\smash{\mathrm{rf}}}_2= \{\rpred_i \mid \rpred\in \Sigma_{\geq3}, 1\leq i \leq \arity{\rpred}\}$ a fresh set of binary predicates.
The~function $\fcn{reify}$ maps atoms over $\Sigma_{\leq2}$ to themselves, while any higher-arity atom $\alpha=\rpred(t_1,...\,,t_k)$ with $k\geq 3$ is mapped~to the
%%NEW
set $\{\rpred_i(u_\alpha,t_i) \mid 1\leq i \leq k\}$,
%%OLD
%conjunction $\bigwedge_{1\leq i \leq \arity{\rpred}} \rpred_i(u_\alpha,t_i)$,
where $u_\alpha$ is a fresh null or variable. We lift $\fcn{reify}$ to instances, rules, and queries in the natural way. 
\defend
\end{definition}

It is best to think of the ``reification term'' $u_\alpha$ as a locally existentially quantified variable. In particular, in rule heads, $u_\alpha$ will be existentially quantified. Moreover, in datalog queries, $\fcn{reify}$ is only applied to $\Sigma_\mathrm{EDB}$-atoms, while $\Sigma_\mathrm{IDB}$-atoms are left unaltered; this ensures that the result is again a datalog query.

\begin{example}
Consider the instance $\inst_\mathrm{tern}$ from \Cref{ex:badnewsternary}. We observe that
$\fcn{reify}(\inst_\mathrm{tern}) =\\ \{ \rpred_1(u_n,-1), \rpred_2(u_n,n), \rpred_3(u_n,n{+}1) \mid n\in \mathbb{N} \}$ has a treewidth of $3$ and a cliquewidth of $6$, witnessed by 
the (non-well-founded) expression $\fcn{Add}_{\rpred_1,5,1}(\const{*}_1 \oplus E)$, where %the subexpression 
$E$ is implicitly defined via
$ E = \fcn{Recolor}_{2\to 3} (\fcn{Recolor}_{4\to 5} (\fcn{Recolor}_{3\to 6}(\fcn{Add}_{\rpred_3,4,3}(\fcn{Add}_{\rpred_2,4,2}(\const{*}_2 \oplus (\const{*}_4 \oplus E))))))$.
%\begin{align*}
% E & = \fcn{Recolor}_{2\to 3} (\fcn{Recolor}_{4\to 5} (\fcn{Recolor}_{3\to 6}(E'))) \\
% E'& = \fcn{Add}_{\rpred_3,4,3}(\fcn{Add}_{\rpred_2,4,2}(\const{*}_2 \oplus (\const{*}_4 \oplus E))).
%\end{align*}
\end{example}
Let us list in all brevity some pleasant and fairly straightforward properties of reification:
\begin{itemize}[leftmargin=5ex]
\item[(i)] 
If $\tw{\instance}$ is finite, then so are  
 $\tw{\fcn{reify}(\instance)}$ and $\cw{\fcn{reify}(\instance)}$.
\item[(ii)] 
$\sat{\fcn{reify}(\instance),\fcn{reify}(\ruleset)} \equiv \fcn{reify}(\sat{\instance,\ruleset})$.
\item[(iii)] 
If $\ruleset$ is $\bts$, then $\fcn{reify}(\ruleset)$ is $\bts$ and $\fcs$.
\item[(iv)] 
$(\database,\ruleset) \models (\mathfrak{q},\Xi)$ \iffi $(\fcn{reify}(\database), \fcn{reify}(\ruleset)) \!\models \!(\fcn{reify}(\mathfrak{q}),\fcn{reify}(\Xi))$.
\end{itemize}
%Let us list some pleasant properties of reification:
%%\begin{itemize}
%%    \item 
%(i) If $\instance$ has finite treewidth, then both %treewidth and clique\-width of 
% $\tw{\fcn{reify}(\instance)}$ and $\cw{\fcn{reify}(\instance)}$ are finite;
%%    \item 
%(ii) if $\ruleset$ is $\bts$, then $\fcn{reify}(\ruleset)$ is $\bts$ and $\fcs$;
%%    \item 
%(iii) $(\database,\ruleset) \models (\mathfrak{q},\Xi)$ \iffi $(\fcn{reify}(\database), \fcn{reify}(\ruleset)) \models \fcn{reify}((\mathfrak{q},\Xi))$;
%(iv) $\sat{\hspace{-0.3mm}\fcn{reify}(\instance),\!\fcn{reify}(\ruleset)\hspace{-0.3mm}}$ is isomorphic to $\fcn{reify}(\sat{\instance\!,\hspace{-0.3mm}\ruleset})$.
%%\end{itemize}

\begin{example}
Revisiting \Cref{ex:badnewsternary}, we can confirm that $\fcn{reify}(\ruleset_\mathrm{tern})$ comprising the rule
$\rpred_1(u,v) \wedge \rpred_2(u,x) \wedge \rpred_3(u,y) \to \exists u'z \big( \rpred_1(u',v) \wedge \rpred_2(u',y) \wedge \rpred_3(u',z)\big)$ is $\bts$ and $\fcs$.
\end{example}

The above insights regarding reification allow us to effortlessly reduce any query entailment problem over an arbitrary $\bts$ rule set to a reasoning problem
over a binary $\fcs$ one. Also, reification is a highly local transformation; it can be performed independently and atom-by-atom on $\database$, $\ruleset$, and $(\mathfrak{q},\Xi)$. Therefore, restricting ourselves to $\fcs$ rule sets %(and hence to binary signatures) 
does not deprive us of the expressiveness, versatility, and reasoning capabilities offered by arbitrary $\bts$ rule sets over arbitrary signatures, which includes the numerous classes based on guardedness: guarded and frontier-guarded rules as well as their respective variants weakly, jointly, and glut-(frontier-)guarded rules \cite{BagLecMugSal11,CaliGK13,KrotzschR11}. 
%
It is noteworthy that our line of argument also gives rise to an independent proof of decidability of query entailment for $\bts$:\footnote{Note that this result establishes entailment for arbitrary DaMSOQs, while previously reported results \cite{BagLecMugSal11,CaliGK13} only covered CQs. But even when restricting the attention to CQ entailment, the proofs given in these (mutually inspired) prior works do not appear entirely conclusive to us: both invoke a result by Courcelle \cite{Cou90}, which, as stated in the title of the article and confirmed by closer inspection, only deals with classes of \emph{finite} structures/graphs with a uniform treewidth bound. Hence, the case of infinite structures is not covered, despite being the prevalent one for universal models. Personal communication with Courcelle confirmed that the case of arbitrary countable structures -- although generally believed to hold true -- is not an immediate consequence of his result.}

\begin{theorem}
For every $\bts$ rule set $\ruleset$, the query entailment problem $(\database,\ruleset) \models (\mathfrak{q},\Xi)$ for databases $\database$, and DaMSOQs $(\mathfrak{q},\Xi)$ is decidable.
\end{theorem}

% SOMEBODY HAD CHANGED THE ABOVE INTO THE FOLLOWING:
%
%\begin{theorem}
%For any $\bts$ rule set $\ruleset$, database $\database$, and DaMSOQ $(\mathfrak{q},\Xi)$, the query entailment problem $\database,\ruleset \models (\mathfrak{q},\Xi)$ is decidable.
%\end{theorem}
%
% THIS IS NOT THE SAME. 
% IF YOU FIX ALL THREE THINGS UPFRONT (AS DONE HERE), 
% THE PROBLEM IS TRIVIALLY DECIDABLE (SINCE THE ANSWER IS 
% CONSTANTLY "YES" OR CONSTANTLY "NO", AND FOR EITHER
% EXISTS AN ALGORITHM OUTPUTTING IT)

\begin{proof}
As argued\prm{ above}, \prm{the problem }$(\database,\ruleset) \models (\mathfrak{q},\Xi)$ \prm{can be reduced }\pin{reduces }to $(\fcn{reify}(\database),\fcn{reify}(\ruleset)) \models (\fcn{reify}(\mathfrak{q}),\fcn{reify}(\Xi))$. As $\ruleset$ is $\bts$, so is 
$\fcn{reify}(\ruleset)$. The latter being binary, we conclude that it is \prm{also }$\fcs$. Then, the claim follows from decidability of DaMSOQ entailment for $\fcs$ rule sets (\Cref{cor:fcsdecidable}). 
\end{proof}


%\subsection{Motivating examples}

%\piotr{TODO Explain motivation}


%\begin{example}\label{ex:chain-transitivity}
%Let $\ruleset_{chain}$ be the following set of ERs:
%\begin{align*}
%    E(x,y) &\to \exists{z} \; E(y,z)\\
%    E(x,y),E(y,z) &\to E(x,z)
%\end{align*}
%It should be clear that $\ruleset_{chain}$ is $\bcs$ but not $\bts$ nor $\fus$.
%\end{example}



==> ICDT 2023 Updated LaTeXFiles/conclusions.tex <==
\section{Conclusions and Future Work}

In this paper, we have introduced a generic framework, by means of which model-theoretic properties of a class of existential rule sets can be harnessed to establish that the entailment of \emph{datalog/MSO queries} -- a very expressive query formalism subsuming numerous popular query languages -- is decidable for that class.
%
We have put this framework to use by introducing \emph{finite-cliquewidth sets} and clarified this 
%%%%
% I verified that the following genitive form is accepted (though the alternative <<class'>> is, too). I prefer that one as it indicates what happens phonologically (speak: "classeez") 
%%%%
class's 
%%%%
relationship with notable others, resulting in the insight that a plethora of known as well as hitherto unknown decidability results can be uniformly obtained via the decidability of DaMSOQ entailment over finite-cliquewidth sets of rules.
Our results entail various appealing directions for follow-up investigations: 
\begin{itemize}
\item 
Certainly, the class of single-headed binary $\fus$ rule sets is not the most general fragment of $\fus$ subsumed by $\fcs$. We strongly conjecture that many of the known, syntactically defined, ``concrete subclasses'' of $\fus$ are actually contained in $\fcs$, and we are confident that corresponding results can be established.
\item
Conversely, we are striving to put the notion of $\fcs$ to good use by identifying comprehensive, syntactically defined subclasses of $\fcs$, enabling decidable, highly expressive querying beyond the realms of $\bts$, $\fus$, or $\mathbf{fc}$.
As a case in point, the popular modeling feature of \emph{transitivity} of a relation has been difficult to accommodate in existing frameworks \cite{BagetBMR15,GanzingerMV99,KieronskiR21,SzwastT04}, whereas the observations presented in this paper seem to indicate that $\fcs$ can tolerate transitivity rules well and natively. 
\item
Finally, we are searching for even more general MSO-friendly width notions that give rise to classes of rule sets subsuming $\fcs$, and which also encompass $\bts$ natively, without arity restrictions or ``reification detours.'' 
\end{itemize}
%
Aside from these major avenues for future research, there are also interesting side roads worth exploring:
\begin{itemize}
\item 
Are there other, more general model-theoretic criteria of ``structural well-behavedness'' that, when ensured for universal models, guarantee decidability of query entailment ``just'' for (U)CQs?
Clearly, if we wanted $\fus$ to be subsumed by such a criterion, it would have to accept structures like $\ginf$ (i.e., infinite grids) and we would have to relinquish decidability of DaMSOQ entailment. 
\item
More generally: Are there other ``decidability sweet spots'' between expressibility of query classes and structural restrictions on universal models?
\end{itemize}

==> ICDT 2023 Updated LaTeXFiles/cw-binary.tex <==

\section{Comparing FCS and FUS}\label{sect:cw-binary}

We have seen that the well-known $\bts$ class is subsumed by the $\fcs$ class (directly for arities ${\leq}2$, and via reification otherwise). As discussed in the introduction, another prominent class of rule sets (incomparable to $\bts$) with decidable CQ entailment is the $\fus$ class. We dedicate the remainder of the paper to mapping out the relationship between $\fcs$ and $\fus$, obtaining the following two results (established in \cref{sec:binary} and \cref{sec:higher-arity}, respectively):

\begin{theorem}\label{thm:binary}
Any \prm{finite-unification set }\pin{$\fus$ rule set }of single-headed rules over a binary signature is \prm{a finite-cliquewidth set}\pin{$\fcs$}.
\end{theorem}

%Surprisingly this is not the case generally. This constitutes our second main contribution:

\begin{theorem}\label{thm:higher-arity}
There exists a \prm{finite-unification set }\pin{$\fus$ rule set }of multi-headed rules over a binary signature that is not \prm{a finite-cliquewidth set}\pin{$\fcs$}.
\end{theorem}
%
%Note that,\prm{ sadly,} the \prm{necessary }restriction to single-headed rules prevents us from \prm{wielding the powers of }\pin{using any kind of }reification\prm{ in this setting}.
%
As a consequence of these findings, the necessary restriction to single-headed rules prevents us from wielding the powers of reification in this setting.


%In this section we will go over a few technicalities used in later proofs. 
%
%
%
%Let us quickly define the following shorthand:
%\begin{definition}
%Let $\inst$ be an instance, $\coloring$ be a coloring of terms of $\inst$, and $\mathcal{T}$ be a well-decorated tree witnessing that $\cw{\inst, \coloring} = k$. Then by $\add{R,l,l'}{\inst, \coloring}$ (or $\add{R, l}{\inst, \coloring}$) we will denote $\inst^{\mathcal{T'}}$ where $\mathcal{T'}$ is the following well-decorated tree:
%\begin{itemize}
%    \item The root note $\varepsilon$ of $\mathcal{T'}$ will be decorated with $\addd{R,l,l'}$ (or $\addd{R, l}$),
%    \item The left sub-tree of $\varepsilon$ will be isomorphic to $T$,
%    \item The right sub-tree of $\varepsilon$ will be wholly decorated with $\mathrm{Void}$
%    \end{itemize}
%\end{definition}





%%%%%%%%%%%%%%%%%%%%%%%%% COMMENT
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{proof} 
\piotr{TODO, prove it for new definition}
\piotr{TODO, find add and replace with macro}
Let $\inst$, $\coloring$, $\coloring'$, and $\coloring \times \coloring'$ be as above. We prove the result by induction on the structure of $(\inst, \coloring)$. 

\textit{Base case.} %Let $(\struc^{\inst}, \coloring) \in \mathfrak{L}_k$ be a basic $k$-colored finite structure, i.e. $\sdom^{\inst} = \{t\}$. Then, letting $(\coloring \times \coloring')(t)$ be the color of $t$, it is immediate that $(\struc^{\inst}, \coloring \times \coloring') \in \mathfrak{L}_{k\cdot k'}$.
 Let $(\inst, \coloring) \in \mathfrak{L}_k$ be a basic $k$-colored finite structure, i.e., $\adom{\inst} = \{t\}$. Then, letting $(\coloring \times \coloring')(t)$ be the color of $t$, it is immediate that $(\inst, \coloring \times \coloring') \in \mathfrak{L}_{k\cdot k'}$.

\textit{Inductive step.} %We split the inductive step into three cases depending on if the last operation used to obtain $(\struc^{\inst}, \coloring)$ is $\disun$, $\mathrm{add}_{R,\vl}$, or $\mathrm{recolor}_{i\to j}$. In each case, we assume that $(\struc^{\inst}, \coloring) \in \mathfrak{L}_k$.

 We split the inductive step into three cases depending on if the last operation used to obtain $(\inst, \coloring)$ is $\disun$, $\pred{Add}_{R,\vl}$, or $\pred{Recolor}_{i\to j}$. In each case, we assume that $(\inst, \coloring) \in \mathfrak{L}_k$.

%$\disun$. Suppose that $(\struc^{\inst}, \coloring)$ is the product of a disjoint union, i.e. there exist two finite colored structures $(\struc_{1},\coloring_{1})$ and $(\struc_{2},\coloring_{2})$ such that $(\struc^{\inst}, \coloring) = (\struc_{1},\coloring_{1}) \disun (\struc_{2},\coloring_{2})$ and where $\codom{\coloring_{1}} = \codom{\coloring_{2}} = \codom{\coloring}$. By our assumption that $(\struc^{\inst}, \coloring) \in \mathfrak{L}_k$, we know that $(\struc_{1},\coloring_{1}), (\struc_{2},\coloring_{2}) \in \mathfrak{L}_k$. By IH, it follows that $(\struc_1, \coloring_1 \times \coloring'), (\struc_2, \coloring_2 \times \coloring') \in \mathfrak{L}_{k\cdot k'}$, from which it follows that $(\struc^{\inst}, \coloring \times \coloring') \in \mathfrak{L}_{k\cdot k'}$.

$\disun$. Suppose that $(\inst, \coloring)$ is the product of a disjoint union, i.e., there exist two finite colored structures $(\struc_{1},\coloring_{1})$ and $(\struc_{2},\coloring_{2})$ such that $(\inst, \coloring) = (\struc_{1},\coloring_{1}) \disun (\struc_{2},\coloring_{2})$ and where $\codom{\coloring_{1}} = \codom{\coloring_{2}} = \codom{\coloring}$. By our assumption that $(\inst, \coloring) \in \mathfrak{L}_k$, we know that $(\struc_{1},\coloring_{1}), (\struc_{2},\coloring_{2}) \in \mathfrak{L}_k$. By IH, it follows that $(\struc_1, \coloring_1 \times \coloring'), (\struc_2, \coloring_2 \times \coloring') \in \mathfrak{L}_{k\cdot k'}$, from which it follows that $(\inst, \coloring \times \coloring') \in \mathfrak{L}_{k\cdot k'}$.

%$\mathrm{add}_{R,\vl}$. Suppose that there exists a finite colored structure $(\struc_{1}, \coloring)$ such that $(\struc^{\inst}, \coloring) = \add{R,\vl}{\struc_{1}, \coloring}$ for $R \in \sig$ and $\vl = (l_{1}, \ldots, l_{\arity{R}}) \in  \{1,\ldots, k\}^{\arity{R}}$. By our assumption that $(\struc^{\inst}, \coloring) \in \mathfrak{L}_k$, we know that $(\struc_{1}, \coloring) \in \mathfrak{L}_k$, from which it follows that $(\struc_{1}, \coloring \times \coloring') \in \mathfrak{L}_{k \cdot k'}$ by IH. Let us define the following set of colors:
%\begin{center}
%$(l_{i},l') \in \cols_{R}$ \ifandonlyif there exists an $i \in \{1, \ldots, \arity{R}\}$ and there exists a $t \in \aadom{\struc_{1}}$ such that $(\coloring \times \coloring')(t) = (l_{i},l')$.
%\end{center}
%We note that each $l_{i}$, for $i \in \{1, \ldots, \arity{R}\}$, is an element of $\vec{l}$, specified above. Let us now form certain tuples of length $\arity{R}$ from the set $\cols_{R}$, which will be used to lift the $\mathrm{add}_{R,\vl}$ operation to the product setting. We define $\vec{\cols}_{R}$ to be the set of all tuples of the form $((l_{1}, l_{1}'), \ldots, (l_{\arity{R}}, l_{\arity{R}}'))$ such that $(l_{i},l_{j}') \in \cols_{R}$, $l_{i}$ is the $i^{th}$ element of $\vec{l}$, and $l_{j}' \in \codom{\coloring'}$, for $i,j \in \{1, \ldots, \arity{R}\}$. Let $\mathbf{l}_{1}, \ldots, \mathbf{l}_{m}$ be an enumeration of elements from $\vec{\cols}_{R}$. We obtain $(\struc, \coloring \times \coloring')$ in the following manner:
%$$
%(\struc^{\inst}, \coloring \times \coloring') = \mathrm{add}_{R,\mathbf{l}_{1}}(\ldots \mathrm{add}_{R,\mathbf{l}_{m}}(\struc_{1}, \coloring \times \coloring') \ldots )
%$$
%Observe that $\cols_{R} \subseteq \{1, \ldots, k\} \times \{1, \ldots, k'\}$, thus showing that $(\struc^{\inst}, \coloring \times \coloring') \in \mathfrak{L}_{k \cdot k'}$, as desired.

$\pred{Add}_{R,\vl}$. Suppose that there exists a finite colored structure $(\struc_{1}, \coloring)$ such that $(\inst, \coloring) = \add{R,\vl}{\struc_{1}, \coloring}$ for $R \in \sig$ and $\vl = (l_{1}, \ldots, l_{\arity{R}}) \in  \{1,\ldots, k\}^{\arity{R}}$. By our assumption that $(\inst, \coloring) \in \mathfrak{L}_k$, we know that $(\struc_{1}, \coloring) \in \mathfrak{L}_k$, from which it follows that $(\struc_{1}, \coloring \times \coloring') \in \mathfrak{L}_{k \cdot k'}$ by IH. Let us define the following set of colors:
\begin{center}
$(l_{i},l') \in \cols_{R}$ \ifandonlyif there exists an $i \in \{1, \ldots, \arity{R}\}$ and there exists a $t \in \aadom{\struc_{1}}$ such that $(\coloring \times \coloring')(t) = (l_{i},l')$.
\end{center}
We note that each $l_{i}$, for $i \in \{1, \ldots, \arity{R}\}$, is an element of $\vec{l}$, specified above. Let us now form certain tuples of length $\arity{R}$ from the set $\cols_{R}$, which will be used to lift the $\pred{Add}_{R,\vl}$ operation to the product setting. We define $\vec{\cols}_{R}$ to be the set of all tuples of the form $((l_{1}, l_{1}'), \ldots, (l_{\arity{R}}, l_{\arity{R}}'))$ such that $(l_{i},l_{j}') \in \cols_{R}$, $l_{i}$ is the $i^{th}$ element of $\vec{l}$, and $l_{j}' \in \codom{\coloring'}$, for $i,j \in \{1, \ldots, \arity{R}\}$. Let $\mathbf{l}_{1}, \ldots, \mathbf{l}_{m}$ be an enumeration of elements from $\vec{\cols}_{R}$. We obtain $(\inst, \coloring \times \coloring')$ in the following manner:
$$
(\inst, \coloring \times \coloring') = \pred{Add}_{R,\mathbf{l}_{1}}(\ldots \pred{Add}_{R,\mathbf{l}_{m}}(\struc_{1}, \coloring \times \coloring') \ldots )
$$
Observe that $\cols_{R} \subseteq \{1, \ldots, k\} \times \{1, \ldots, k'\}$, thus showing that $(\inst, \coloring \times \coloring') \in \mathfrak{L}_{k \cdot k'}$, as desired.

$\pred{Recolor}_{l_{1} \to l_{2}}$. Suppose there exists a finite colored structure $(\struc_{1}, \coloring_{1})$ such that $(\inst, \coloring) = \recol{i\to j}{\struc_{1}, \coloring_{1}}$. By our assumption that $(\inst, \coloring) \in \mathfrak{L}_k$, we have that $(\struc_{1}, \coloring_{1}) \in \mathfrak{L}_k$. By IH, we may conclude that $(\struc_{1}, \coloring_{1} \times \coloring') \in \mathfrak{L}_{k \cdot k'}$. Let us define the following set of colors:
\begin{center}
$(l_{1},l') \in \cols$ \ifandonlyif there exists a $t \in \aadom{\struc_{1}}$ such that $(\coloring \times \coloring')(t) = (l_{1},l')$.
\end{center}
We let $\mathbf{l}_{1}^{1} = (l_{1},l_{1}'), \ldots, \mathbf{l}_{m}^{1} = (l_{1},l_{m}')$ be an enumeration of elements from $\cols$, and $\mathbf{l}_{1}^{2} = (l_{2},l_{1}'), \ldots, \mathbf{l}_{m}^{2} = (l_{2},l_{m}')$ an enumeration of the same length, obtained by replacing the first element $l_{1}$ of each pair in the former enumeration with $l_{2}$. Let us now lift the $\pred{Recolor}_{l_{1} \to l_{2}}$ operation to the product setting. The finite colored structure $(\inst, \coloring \times \coloring')$ is obtainable as follows:
$$
(\inst, \coloring \times \coloring') = \pred{Recolor}_{\mathbf{l}_{m}^{1} \to \mathbf{l}_{m}^{2}}(\ldots \pred{Recolor}_{\mathbf{l}_{1}^{1} \to \mathbf{l}_{1}^{2}}(\struc_{1}, \coloring_{1} \times \coloring') \ldots )
$$
Observe that $\cols \subseteq \{1, \ldots, k\} \times \{1, \ldots, k'\}$, thus showing that $(\inst, \coloring \times \coloring') \in \mathfrak{L}_{k \cdot k'}$, as desired.
\end{proof}
\end{comment}



==> ICDT 2023 Updated LaTeXFiles/decidability.tex <==
\section{A Generic Decidability Argument}

In this section, we provide an abstract framework for establishing de\-ci\-da\-bi\-li\-ty of entailment for a wide range of queries, 
%applicable to all rule sets that satisfy certain model-theoretic conditions.
based on 
cer\-tain model-theoretic criteria being met 
%sa\-tis\-faction of cer\-tain model-theoretic conditions 
by the considered rule set. 
We first recall the classical notion of a (Boolean) datalog query, and after, we specify the class of queries considered in our frame\-work.

\begin{definition}
Given a signature $\sig$, a \emph{(Boolean) datalog query} $\mathfrak{q}$ over $\sig$ is represented by a  
finite set $\ruleset_\mathfrak{q}$ of datalog rules with predicates from $\sig_{\mathrm{EDB}}\uplus\sig_{\mathrm{IDB}}$ where  $\sig_{\mathrm{EDB}}{\,\subseteq\,} \sig$ and $\sig_{\mathrm{IDB}}{\,\cap\,} \sig=\emptyset$ %, where (i) $\sig_{\mathrm{EDB}} \cap \sig_{\mathrm{IDB}} = \emptyset$, 
such that (i) $\sig_{\mathrm{EDB}}$-atoms do not occur in rule heads of $\ruleset_\mathfrak{q}$% 
%SOLVED: \tim{Does (i) mean: ``if $R \in \sig_{\mathrm{EDB}}$, then there exists a $\rho \in \ruleset_\mathfrak{q}$ such that $R$ occurs in $body(\rho)$, but $R$ does not occur in $head(\rho')$ for all $\rho' \in \ruleset_\mathfrak{q}$'' ?}
%SEBASTIAN: No, it doesn't. I rephrased it to make it more clear
, and (ii) $\sig_{\mathrm{IDB}}$ contains a distinguished nullary predicate $\mathtt{Goal}$. 
%
Given an instance $\instance$ and a datalog query $\mathfrak{q}$\prm{ over $\Sigma$}, we say that $\mathfrak{q}$ \emph{holds in} $\instance$ (\prm{or, }$\instance$ \emph{satisfies} $\mathfrak{q}$), written $\instance\models\mathfrak{q}$, \iffi $\mathtt{Goal}\in\sat{\instance,\ruleset_\mathfrak{q}}$. Query entailment is\prm{ then} defined via satisfaction as usual.
%We note that \emph{entailment} of a datalog query $\mathfrak{q}$ from a rule set $\ruleset$ and database $\db$, written $\ruleset,\database \models \mathfrak{q}$ is defined as with 
\defend
\end{definition}

Datalog queries can be equivalently expressed as sentences in second-order logic (with the $\sig_{\mathrm{IDB}}$ predicates quantified over) or in least fixed-point logic (LFP). For our purposes, the given formulation is the most convenient; e.g., it makes clear that the second-order entailment problem $(\db, \ruleset) \models \mathfrak{q}$ reduces to the first-order entailment problem $(\db,\ruleset\cup\ruleset_\mathfrak{q}) \models \mathtt{Goal}$. 
%
\begin{definition}
A \emph{datalog/MSO query (DaMSOQ)} over a signature $\sig$
is a pair $(\mathfrak{q},\Xi)$, where~$\mathfrak{q}$ is a datalog query over $\sig$ and $\Xi$ is a monadic second-order (MSO)\footnote{For an introduction to monadic second-order logic, see~\cite[Section 1.3]{CourEngBook}.} sentence equivalent to~$\mathfrak{q}$. 
Satisfaction and entailment of DaMSOQs is defined via any of their constituents. 
\defend
\end{definition}
Consequently, DaMSOQs are the (semantic) intersection of datalog and MSO queries. While representing DaMSOQs as a pair $(\mathfrak{q},\Xi)$ is logically redundant, it is purposeful and necessary: the below decision procedure requires both constituents as input and it is not generally possible to compute one from the other. Arguably, the most comprehensive, known DaMSOQ fragment that is well-investigated and has a syntactic definition is that of \emph{nested monadically defined queries}, a very expressive yet computationally manageable formalism \cite{RudKro13}, subsuming (unions of) Boolean CQs,
%\footnote{E.g., any BCQ $\exists \vx \phi(\vx)$ corresonds to the DaMSOQ $\big(\{\phi(\vx) \to \mathtt{Goal}\},\exists \vx \phi(\vx)\big)$.}
 \emph{monadic datalog queries}~\cite{Cosmadakis88}, \emph{conjunctive 2-way regular path queries}~\cite{FlorescuLS98}, and nested versions thereof (e.g. \emph{regular queries}~\cite{ReutterRV17} and others~\cite{BourhisKR14}).

%%
%DaMSOQs encompass various classes of queries:
%%Many types of queries are expressible as DaMSOQs: 
%(unions of) Boolean CQs,\footnote{E.g., any BCQ $\exists \vx \phi(\vx)$ corresonds to the DaMSOQ $\big(\{\phi(\vx) \to %\mathtt{Goal}\},\exists \vx \phi(\vx)\big)$.} \emph{conjunctive 2-way regular path queries}~\cite{FlorescuLS98}, %\emph{monadic datalog queries}~\cite{Cosmadakis88}, and \emph{(nested) monadically defined queries} \cite{RudKro13}.
%Our generic decidability result covers all of those.

\begin{definition}\label{def:MSOfriendly}
Let $\Sigma$ be a finite signature.
A \emph{width measure} (for $\Sigma$) is a function $\fcn{w}$ mapping every countable instance over $\Sigma$ to a value from $\mathbb{N} \cup \{\infty\}$.
We call $\fcn{w}$ \emph{MSO-friendly} \iffi there exists an algorithm that, taking a number $n \in \mathbb{N}$ and an MSO sentence $\Xi$ as input,
\vspace{-0.5ex}
\begin{itemize}
\item never terminates if $\Xi$ is unsatisfiable, and
\item always terminates if $\Xi$ has a model $\instance$ with
$\fcn{w}(\instance)\leq n$.\defend
\end{itemize} 
\end{definition}

As an unsophisticated example, note that the \emph{expansion} function $\fcn{expansion}: \inst \mapsto |\adom{\inst}|$, mapping every countable instance to the size of its domain, is an MSO-friendly width measure: there are up to isomorphism only finitely many instances with $n$ elements, which can be computed and checked. As a less trivial example, the notion of treewidth has also been reported to fall into this category~\cite{BagLecMugSal11}.

\begin{definition}
Let $\fcn{w}$ be a width measure.
A rule set $\ruleset$ is called a \emph{finite-$\fcn{w}$ set} \iffi for every database $\database$, there exists a universal model $\instance^*$ of $(\db,\ruleset)$  satisfying $\fcn{w}(\instance^*) \in \mathbb{N}$.\defend
\end{definition}

Note that the finite width required by this definition does not need to be uniformly bounded: it may depend on the database and thus grow beyond any finite bound. This is already the case when using the $\fcn{expansion}$ measure from above, giving rise to the class of \emph{finite-expansion sets} ($\fes$), coinciding with the notion of \emph{core-chase terminating} rule sets~\cite{DeuNasRem08}.    

\begin{theorem}\label{thm:decidablequerying}
Let $\fcn{w}$ be an MSO-friendly width measure and let $\ruleset$ be a \emph{finite-$\fcn{w}$ set}.
Then, the entailment problem $(\db, \ruleset) \models (\mathfrak{q},\Xi)$ for any \prm{given }database $\database$ and DaMSOQ $(\mathfrak{q},\Xi)$ is decidable.
\end{theorem}

\begin{proof}
We prove decidability by providing two semi-deci\-sion procedures: one terminating whenever  
$(\db,\ruleset)\models (\mathfrak{q},\Xi)$, the other terminating whenever $(\db,\ruleset) \not\models (\mathfrak{q},\Xi)$. Then, these two procedures, run in parallel, constitute a decision procedure.
\begin{itemize}
    \item Detecting $(\db,\ruleset) \models (\mathfrak{q},\Xi)$. We note that $(\db,\ruleset) \models (\mathfrak{q},\Xi)$ \iffi $(\db,\ruleset) \models \mathfrak{q}$ \iffi $(\db,\ruleset\cup\ruleset_\mathfrak{q})\models \mathtt{Goal}$. The latter is a first-order entailment problem. Thanks to the completeness of first-order logic \cite{God29FOLcomp}, we can recursively enumerate all the consequences of $(\db,\ruleset\cup\ruleset_\mathfrak{q})$ and terminate as soon as we find $\mathtt{Goal}$ among those, witnessing entailment of the query.
    \item Detecting $(\db,\ruleset) \not\models (\mathfrak{q},\Xi)$. 
    %
    %Then, some model $\instance$ of $(\db,\ruleset)$ exists with $\instance\not\models (\mathfrak{q},\Xi)$. 
    %
    In that case, there must exist some model $\instance$ of $(\db,\ruleset)$ with $\instance\not\models (\mathfrak{q},\Xi)$. Note that such ``countermodels'' can be characterized by the MSO formula $\bigwedge\!\db \wedge \bigwedge\! \ruleset \wedge \neg\Xi$.
    %
    Moreover, any universal model $\instance^*$ of $(\db,\ruleset)$ must satisfy $\instance^*\not\models (\mathfrak{q},\Xi)$, which can be shown (by contradiction) as follows: Let $\instance^*$ be a universal model of $(\db,\ruleset)$ and suppose $\instance^*\models (\mathfrak{q},\Xi)$, i.e., $\instance^*\models \mathfrak{q}$. Since satisfaction of datalog queries is preserved under homomorphisms and $\instance^*$ is universal, we know there exists a homomorphism from $\instance^*$ to $\instance$, implying $\instance\models \mathfrak{q}$, and thus $\instance\models (\mathfrak{q},\Xi)$, contradicting our assumption. As $\rs$ is a finite-$\fcn{w}$ set, there exists a universal model $\instance^*$ of $(\db,\ruleset)$ for which $\fcn{w}(\instance^*)$ is finite. Hence, the following procedure will terminate, witnessing non-entailment: enumerate all natural numbers in their natural order and for each number $n$ initiate a parallel thread with the algorithm from \Cref{def:MSOfriendly} with input $n$ and $\bigwedge\!\db \wedge \bigwedge\! \ruleset \wedge \neg\Xi$ (the algorithm is guaranteed to exist due to MSO-friendliness of $\fcn{w}$). Terminate as soon as one thread does.\qedhere
%    \item Detecting $(\db,\ruleset) \not\models (\mathfrak{q},\Xi)$. In that case, there must exist some model $\instance$ of $(\db,\ruleset)$ with $\instance\not\models (\mathfrak{q},\Xi)$. Note that such ``countermodels'' can be characterized by the MSO formula $\bigwedge\!\db \wedge \bigwedge\! \ruleset \wedge \neg\Xi$. But then we can show that $\instance^*\not\models (\mathfrak{q},\Xi)$ must also hold for any universal model $\instance^*$ of $(\db,\ruleset)$: toward a contradiction, suppose $\instance^*\models (\mathfrak{q},\Xi)$, i.e., $\instance^*\models \mathfrak{q}$. Since satisfaction of datalog queries is preserved under homomorphisms, and by universality, we know there exists a homomorphism from $\instance^*$ to $\instance$, we have $\instance\models \mathfrak{q}$, and thus $\instance\models (\mathfrak{q},\Xi)$, contradicting our assumption. Now, by assumption, there exists at least one universal model $\instance^*$ for which $\fcn{w}(\instance^*)$ is finite. Then the following procedure will terminate, witnessing non-entailment: Enumerate all natural numbers\prm{ in their natural order} and for each \prm{number }$n$ run a parallel thread with the algorithm from \Cref{def:MSOfriendly} with input $n$ and $\bigwedge\!\db \wedge \bigwedge\! \ruleset \wedge \neg\Xi$ (the algorithm \prm{is guaranteed to }exist\pin{s} due to MSO-friendliness of $\fcn{w}$). Terminate as soon as one thread does.\qedhere
\end{itemize}
\end{proof}


==> ICDT 2023 Updated LaTeXFiles/higher-arities-previous.tex <==
\section{Results for Multi-Headed Rules}\label{sec:higher-arity}

We will now prove \cref{thm:higher-arity} implying that for multi-headed rules, $\fus$ is no longer subsumed by $\fcs$. To this end, we exhibit a $\fus$ rule set which may unavoidably lead to universal models of infinite cliquewidth. 

We let $\sigi = \set{\hpred, \vpred, \origin}$ be a signature where $\hpred$ and $\vpred$ are binary predicates and $\origin$ is a unary predicate. Let us define $\rsgrid$ to be the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} & \top & \rightarrow \exists x \; (\hpred(x,x) \land \vpred (x,x)) \\[0.5ex]
\text{(grow)} & \top & \rightarrow \exists y \exists y'\; (\hpred(x,y) \land \vpred (x,y')) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists y' \; (\hpred(x',y') \land \vpred(y,y'))
\end{array}
$$

We make use of $\rsgrid$ to establish \cref{thm:higher-arity} (see \cref{sect:main-results}), whose proof is split into two parts. First, we provide a database $\dbg$ to form a knowledge base $(\dbg, \rsg)$ for which no universal model of finite cliquewidth exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\subsection{$\rsgrid$ is not a finite-cliquewidth set}


We devote this section to establishing the subsequent lemma, which serves as one of the two main lemmata sufficient to conclude \cref{thm:higher-arity}.


\begin{lemma}\label{lem:no-universal-model-cw}
Let $a$ be a constant and let $\dbg = \set{\origin(a)}$ be a database. Then, no universal model of finite cliquewidth exists for $\kbaseg$.
\end{lemma}


With the aim of establishing the lemma above, we define the instance $\ginf$ below, where $a$ is a constant and $x_{i,j}$ and $y$ are nulls for $i,j \in \mathbb{N}$. To provide the reader with further intuition, a graphical depiction of $\ginf$ is given in \cref{fig:ginf}.
\begin{eqnarray*}
\ginf & = & \{\origin(a),\hpred(a,x_{1,0}),\vpred(a,x_{0,1}),\hpred(y,y),\vpred(y,y)\} \\
 & & \cup \big\{\hpred(x_{i,j},x_{i+1,j}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} \\
 & & \cup \big\{\vpred(x_{i,j},x_{i,j+1}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} 
\end{eqnarray*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/ginf.pdf}
    \caption{ The instance $\ginf$.}
    \label{fig:ginf}
\end{figure}

It is straightforward to show that $\ginf$ serves as a model of $\kbaseg$, and a routine exercise to prove that $\ginf$ is universal. Hence, we have the following:

\begin{observation}\label{obs:ginf-is-universal-model}
$\ginf$ is a universal model of $\kbaseg$.
\end{observation}

%\begin{proof} Let $\model = (\dom,\inter)$ be any model of $\kbaseg$. Then, it follows that (i) $\inter(a) \in \inter(\origin)$, (ii) there exists some $d_{0} \in \dom$ such that $d \in \inter[d/x](\hpred) \cap \inter[d/x](\vpred)$, (iii) for any $d_{1} \in \dom$, there exist $d_{2}, d_{3} \in \dom$ such that $(\inter(d_{1})\inter(d_{2}) \in \inter(\hpred)$ and $(\inter(d_{1})\inter(d_{3}) \in \inter(\vpred)$, and (iv) for any $d_{4}, d_{5}, d_{6} \in \dom$, if $(d_{4},d_{5}) \in \inter(\hpred)$ and $(d_{4},d_{6}) \in \inter(\vpred)$, then there exists a $d_{7} \in \dom$ such that 
%\end{proof}


%It is well known~\cite{} that all grid like structures have infinite cliquewidth. 
%\thomas{The original proof for (undirected!) grids w.r.t. cliquewidth was done in \cite[\thm~4]{GolumbicRot99}, where grids are considered as (undirected) graphs. We probably(?) should be ``careful'' here since we have two types of edges and are in the directed setting. It's not that it wouldn't work or anything... But we probably should make a short argument why it does hold here.}

%It is well known that infinite grids over a signature consisting of single binary relation have infinite cliquewidth (see \cite[\thm~4]{GolumbicRot99} for the reference). Consider the following:

%It is known that \thomas{Change to finite!} infinite grids constructed over a signature with a single binary relation have infinite cliquewidth~\cite[\thm~4]{GolumbicRot99}. By making use of this fact, and the subsequent two claims, we can prove \cref{fact:grid-has-unbounded-cw} below.

It is known that the cliquewidth of an $n \times n$ grid tends to infinity as $n$ tends to infinity~\cite[\thm~4]{GolumbicRot99}, entailing that any infinite grid will have an infinite cliquewidth since the cliquewidth of any instance bounds the cliquewidth of any induced sub-instance from above. By making use of this fact, along with the subsequent two, we can prove \cref{fact:grid-has-unbounded-cw} below.

\begin{fact}
        Let $\sig$ be a binary signature, $\epred$ be a binary relational symbol, 
        $\inst$ be an instance over $\sig$, and $\inst' = \set{\epred(t,t') \ | \ \rpred(t,t') \in \inst, \rpred \in \sig}$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}

    
\begin{fact}
        Let $\sig$ be a signature consisting of a single binary relational symbol $E$, let $\inst$ be an instance over $\sig$, and let $\inst' = \set{\epred(t',t) \ | \ \epred(t,t') \in \inst} \cup \inst$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}



\begin{observation}\label{fact:grid-has-unbounded-cw}
$\ginf$ has an infinite cliquewidth.
\end{observation}
\begin{proof} The observation follows from the previous two facts, the fact that infinite grids have infinite cliquewidth, and the fact that adding a set of the form $\{\origin(a), \hpred(y, y), \vpred(y, y) \}$ with $a$ a constant and $y$ a null to any instance does not lower its cliquewidth.
\end{proof}

We now leverage the above result to demonstrate that {\em every} universal model of $\kbaseg$ has an infinite cliquewidth. Observe that if we consider any homomorphism from $\ginf$ to itself, then (i) the null $y$ must be mapped to itself as no other terms are associated with loops, and (ii) the constant $a$ must be mapped to itself, thus anchoring the image of $\ginf$ under the homomorphism at the origin of the grid (indicated by $A(a)$) shown in \cref{fig:ginf}, thus ensuring that each term of the grid will map to itself accordingly. It follows that any homomorphism from $\ginf$ to itself will be the identity function, giving rise to the following observation.

\begin{observation}\label{obs:identity}
If $h: \ginf \to \ginf$ is a homomorphism then $h$ is the identity.
\end{observation}

We now make use of the above observation to show that every universal model of $\kbaseg$ contains a sub-instance that is isomorphic to $\ginf$, thus ensuring that every universal model of $\kbaseg$ is of infinite cliquewidth (by \cref{fact:grid-has-unbounded-cw} and the fact that the cliquewidth of an instance is greater than or equal to the cliquewidth of any induced sub-instance). From this lemma, we may conclude \cref{lem:no-universal-model-cw}.

\begin{lemma}
Every universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$.
\end{lemma}

\begin{proof}
Let $\unimod$ be a universal model of $\kbaseg$. As $\ginf$ is a universal model (by \cref{obs:ginf-is-universal-model} above), we know that two homomorphisms $h\colon \ginf \to \unimod$ and $h'\colon \unimod \to \ginf$ exist between $\unimod$ and $\ginf$. Let us consider the homomorphism $h' \circ h$. By \cref{obs:identity}, the homomorphism $h'\circ h$ is the identity on $\ginf$, implying that $h$ is injective. Furthermore, $h$ is reflective, and hence, constitutes an embedding. To show this, suppose that $p\in\sigi$ and let $\vt$ be a tuple of length $\arity{p}$ from $\ginf$. If $p(h(\vt))$ holds in $\unimod$ , then $p((h' \circ h)(\vt))$ holds in $\ginf$, but since $h'\circ h$ is the identity on $\ginf$, we immediately obtain that $p(\vt)$  holds in $\ginf$. Finally, note that the image of $\ginf$ under $h$ serves as the induced sub-instance of $\unimod$ that is isomorphic to $\ginf$, completing the proof.
\end{proof}



\subsection{$\rsgrid$ is a finite unification set}

As we have now shown that $\rsgrid$ is not a finite-cliquewidth set, we focus our attention on demonstrating \cref{lem:rsg-is-fus}, which is stated below, and from which we may conclude the final main result (\cref{thm:higher-arity}).

\begin{lemma}\label{lem:rsg-is-fus}
$\rsg$ is $\fus$.
\end{lemma}

As the rule $(loop)$ is a member of $\rsg$, every BCQ that is free of constants can be trivially re-written, implying the following:

\begin{observation}\label{obs:bcq-no-const-trivial}
Every BCQ that is free of constants is FO-rewritable with respect to $\rsg$.
\end{observation}

%\piotr{Here is a link for Xrewrite \url{https://arxiv.org/pdf/1405.2848.pdf}}

Showing that a provided rule set is $\fus$ is a notoriously difficult task.\footnote{This should not be too surprising however, as being $\fus$ is an undecidable property~\cite{BagLecMugSal11}.} To this end, we hand-tailor a rewriting algorithm to be used for the proof of~\cref{lem:rsg-is-fus}. However, one can refer to existing rewriting algorithms, e.g. XRewrite~\cite{GotOrsPie14}, for additional intuition. Finally, it is important to note that the proof closely follows the ideas provided in \cite{OstMarCarRud22}.


\subsection{Necessary definitions}

%As we are considering a binary signature, we will treat queries as graphs with the company of standard graph theoretic notions. \thomas{Does this suffice or would Reviewer 2 state: ``The term \emph{graph} has not been defined. Suggest strong reject.''?}

%Since each CQ can be viewed as an instance, and each instance can be viewed as a structure (see \tim{Sect ?}), we will hereafter interpret queries as their corresponding structures. Moreover, we note that since the signature $\sigi$ contains only binary predicates, we can view queries as directed, binary graphs.

We first introduce special queries, referred to as \emph{marked queries}, which are queries supplemented with a set of markings, the significance of which, is to keep track of what terms of the CQs are mapped to constants in a given database throughout the course of rewriting. A marked CQ is defined to be a pair $(q, M)$ where $q$ is a CQ and the set of markings $M$ is a subset of terms (i.e. variables and constants) of $q$. Given an instance $\inst$ we say that $\inst \models (q,M)$ $\iffi$ there exists a homomorphism $h$ mapping $q$ to $\inst$ such that for every term $t$ of $q$ we have $t \in M$ $\iffi$ $h(t)$ is a constant in $\inst$.

We now make a useful observation, which follows by considering the structures that arise when applying the rules from $\rsgrid$ to any given database. Afterward, we show that marked queries take on a special form when interpreted on the instance $\sg$, where $\db$ is an arbitrary database.

\begin{observation}\label{obs:buildup-for-properly-marked-chase}
Let $\db$ be a database. Then,
\begin{itemize}
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom of $\sg$ and $t'\in \adom{\db}$, then $t\in \adom{\db}$;
    \item if there is a cycle $C \subseteq \sg$ that contains at least one constant, then $C \subseteq \db$;
    \item if $\rpred(t_1,t'), \rpred(t_2,t') \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1\in  \adom{\db}$, then $t_2\in  \adom{\db}$;
    \item if $\rpred(a,t), \rpred(b,t) \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $a\neq b$ are constants, then $t$ is a constant.
\end{itemize}
\end{observation}

Keeping the above observation in mind, we define the notion of a {\em properly marked CQ}.

\begin{definition}\label{def:properly-marked}
A marked CQ $(q, M)$ is {\em properly marked} when:
\begin{itemize}
    \item if $a$ is a constant in $q$, then $a \in M$;
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom in $q$ and $t' \in M$, then $t \in M$;
    \item if there is a cycle $C$ in $q$ that contains at least one constant, then all terms of $C$ are contained in $M$;
    \item if $\rpred(t_1,t')$ and $\rpred(t_2,t')$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1 \in M$, then $t_2 \in M$;
    \item if $\rpred(a,t)$ and $\rpred(b,t)$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $a\neq b$ are constants, then $t \in M$.
\end{itemize}
\end{definition}

\begin{observation}\label{obs:query-extendable-properly-marked}
If $\sg \models q$, then there exists a set of markings $M$ such that $(q,M)$ is properly marked and $\sg \models (q,M)$.
\end{observation}

\begin{proof} Suppose that $\sg \models q$. Then, we know that a homomorphism $h$ exists mapping terms from $q$ into $\sg$. Let $M$ be the set of terms from $q$ such that $h(t)$ is mapped to a constant in $\sg$. One can readily check if $(q,M)$ is properly marked, and if not, add the terms from $q$ to $M$ accordingly until a properly marked CQ $(q,M')$ is constructed such that $\sg \models (q,M)$.
\end{proof}

From \cref{obs:buildup-for-properly-marked-chase} and \cref{def:properly-marked} we immediately conclude the following:

\begin{corollary}
Let $(q, M)$ be a marked query, and $\db$ be any database. If $\sg \models \mq$, then $\mq$ is properly marked.
\end{corollary}

Let us refer to a marked CQ $(q, M)$ as {\em alive} given that it is properly marked and $M$ does not contain all terms of $q$. In the case where every term of a properly marked CQ is marked, we refer to the CQ as {\em dead}.

To prove~\cref{lem:rsg-is-fus} it suffices to prove the following lemma, which we direct our attention to in the subsequent section. 

\begin{lemma}\label{lem:rsg-is-fus-reformulated}
For any properly marked CQ $(q, \prmark)$ there exists a set of dead queries $rew(q,\prmark)$ such that for any database $\db$ the following holds: 
\begin{center}
$\sg \models (q,\prmark)$ \ $\iffi$ \ $\exists{Q' \in rew(q, \prmark)}, \db \models Q'.$
\end{center}
\end{lemma}

\subsection{Rewriting Alive Queries}

We begin this section by proving the following lemma, which will later prove useful in rewriting queries relative to $\rsgrid$.

\begin{lemma}\label{lem:exists-maximal}
%For every alive CQ there exists at least one variable with no out-going edges.
If a marked CQ $(q,\prmark)$ is alive, then there exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{lemma}
\begin{proof} Let the marked CQ $(q,\prmark)$ be alive. Then, by the definition above, we know that there exists a set of terms in $q$ that are not a members of $M$. Since $(q,\prmark)$ is properly marked, by \cref{def:properly-marked}, we know that all such terms are not constants, and hence, all such terms must be variables. Let us refer to all such terms as \emph{unmarked variables}. If we consider the sub-instance of the CQ induced by all unmarked variables, we can see that (i) it forms a directed acyclic graph as all cycles of the CQ must be in $M$ by \cref{def:properly-marked}, which (ii) is non-empty as $(q,\prmark)$ is alive. Hence, there must exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$, which corresponds to a sink in the directed acyclic graph described above.
\end{proof}

We will refer to unmarked variables -- such as those described in the above proof -- which possess no out-going edges, as {\em maximal}. These maximal variables will be used to initiate our rewriting process. 

\begin{lemma}\label{lem:maximal-cases}
Let $x$ be a maximal variable of an alive CQ $(q, \prmark)$. Then, one of the following holds:
\begin{enumerate}
    \item \label{lem:maximal-cases-one} $x$ occurs in exactly one atom  $\rpred(t,x)$, with $\rpred\in \{\hpred,\vpred\}$ for some term $t$ of $q$;
    \item \label{lem:maximal-cases-two} $x$ occurs in exactly two atoms $\hpred(t_{\hpred},x)$ and $\vpred(t_{\vpred},x)$ for some terms $t_{\hpred},t_{\vpred}$ of $q$;
    \item \label{lem:maximal-cases-three} there exist at least two distinct terms $t\neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are atoms of $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{enumerate}
\end{lemma}

%Now, in the light~\cref{lem:maximal-cases} we will present four operations that when combined will compute rewritings required by \cref{lem:rsg-is-fus-reformulated}.

\medskip
\noindent
{\bf Rewriting Operations.}
We now make use of~\cref{lem:maximal-cases} to define three operations that compute rewritings. When exhaustively applied to a query, we obtain the rewritings required by \cref{lem:rsg-is-fus-reformulated}. Given an alive CQ $(q, \prmark)$ we define the following three operations:

\begin{definition}[$\cutop$]\label{def:cut}
Let $x$ be a maximal variable of $(q, \prmark)$ satisfying case \ref{lem:maximal-cases-one} of \cref{lem:maximal-cases}, i.e. $x$ occurs in exactly one atom $\rpred(t,x)$ of $q$ with $\rpred\in \{\hpred, \vpred\}$. Then, letting $\query = \query' \cup \{\rpred(t,x)\}$, we define
\[
  \cutop((q,\prmark), \set{x}) =
  \begin{cases}
     (q' \cup \{\top(c)\}, \prmark)  & \text{if $t$ is a constant $c$} \\
      & \text{not occurring in $\query'$;}\\
     (q', \prmark) & \text{otherwise.}
  \end{cases}
\]
%Then, $\cutop((q,\prmark), \set{x}) = (q', \prmark)$, where $q'$ is the sub-query of $q$ with the atom containing $x$ removed.
\end{definition}


\begin{definition}[$\reduceop$]\label{def:reduce}
Let $x, t_{\hpred}$, and $t_{\vpred}$ be as in case \ref{lem:maximal-cases-two} of \cref{lem:maximal-cases}, meaning that there exist two atoms of the form $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ in $q$. We define $q'$ to be the same as $q$, but where $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ are replaced by $\hpred(x', t_{\vpred})$ and $\vpred(x', t_{\hpred})$, and where $x'$ is fresh. We now %by replacing $\hpred(t_{\hpred}, x),\vpred(t_{\vpred}, x)$ with $\hpred(x', t_{\vpred}), \vpred(x', t_{\hpred})$, where $x'$ is a fresh variable. 
 define $\reduceop((q,\prmark), \set{x}) = \set{ (q', \prmark), (q', \prmark \cup \set{x'})}$. 
\end{definition}

\begin{definition}[$\mergeop$]\label{def:merge}
Let $x, t$, and $t'$ be as in case \ref{lem:maximal-cases-three} of \cref{lem:maximal-cases}. We let $q'$ be obtained from $q$ by replacing all occurrences of $t$ in $q$ with $t'$ and define $\mergeop((q, \prmark), \set{x, t, t'}) = (q' \cup \{\top(t)\}, \prmark)$.
\end{definition}

Let us briefly describe how rewritings are computed by means of the above operations. %First, when given a CQ $q$ that is satisfied on $\sg$, we extend the CQ to a properly marked CQ $(q,M)$, which can always be accomplished by \cref{obs:query-extendable-properly-marke}.  
 Given an alive CQ $(q,M)$, we know that one of the three rewriting operations will be applicable (by \cref{lem:maximal-cases}), which we note, may return a \emph{set} of rewritings if the $\reduceop$ operation is applied. We ultimately obtain the set $rew(q, \prmark)$ of rewritings of $(q,\prmark)$ by sequentially applying the three rewriting operations to all alive queries within the set of rewritings, until all marked queries in the set are dead, at which point, the rewriting process terminates. As shown below, we can always apply a rewriting operation to a CQ if it is alive (i.e. rewriting is complete), and also, applying such an operation preserves satisfaction on $\sg$ (i.e. rewriting is sound). We note that the soundness proofs can be found in \cref{appendix:higher-arity}.

\begin{observation}[Completeness]\label{obs:high-completeness}
If a CQ is alive then at least one of above operations can be applied to it.
\end{observation}
\begin{proof}
Follows from~\cref{def:cut,def:reduce,def:merge}, and~\cref{lem:maximal-cases}.
\end{proof}

Let us now prove the soundness of the above operations:

\begin{lemma}[Soundness --- $\cutop$]\label{lem:high-soundness-cut}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x$ is as in \cref{def:cut}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \cutop(\mquery, \set{x}).$$
\end{lemma}


\begin{lemma}[Soundness --- $\reduceop$]\label{lem:high-soundness-reduce}
Let $\db$ be a database and let $Q$ be an alive CQ. If $x$ is as in \cref{def:reduce} and $\reduceop(\mquery, \set{x}) = \set{\mquery_{1}, \mquery_{2}}$, then
$$\sg \models \mquery \ \text{\iffi} \ \exists i \in \{1,2\}, \sg \models \mquery_{i}.$$
\end{lemma}


\begin{lemma}[Soundness --- $\mergeop$]\label{lem:high-soundness-merge}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x, t$, and $t'$ are as in \cref{def:merge}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \mergeop(\mquery, \set{x, t, t'}).$$
\end{lemma}


\medskip
\noindent
{\bf Termination.}
Given two queries $\mquery$ and $\mquery'$, we write $\mquery \stepop \mquery'$ \iffi $\mquery'$ can be obtained from $\mquery$ by applying $\reduceop$, $\cutop$, or $\mergeop$. We let $\stepop^*$ denote the transitive closure of $\stepop$.


%\begin{observation}\label{obs:limit-on-variables}
%Let $\mquery$ and $\mquery'$ be two marked queries. If $\mquery \stepop \mquery'$ then $|\varset(\mquery)| \geq |\varset(\mquery')|$.
%\end{observation}

\begin{lemma}[Termination]\label{lem:termination}
For any properly marked CQ $\mquery$ the set of properly marked queries $\set{Q' \;|\; \mquery \stepop^* \mquery'}$ is finite.
\end{lemma}

\begin{proof} Observe that $\cutop$ deletes the only atom containing the considered maximal variable and $\mergeop$ reduces the number of atoms containing the considered maximal variable. Moreover, neither $\cutop$ nor $\mergeop$ introduce converging atoms of the form $\hpred(t_{1},t)$ and $\vpred(t_{2},t)$ when applied. Since the operation $\reduceop$ reduces the number of such converging atoms in a properly marked CQ as well, and since all such operations either preserve or decrease the number of terms occurring the query, it follows that the rewriting process will eventually terminate. 
\end{proof}

By \cref{obs:high-completeness} (Completeness), \cref{lem:high-soundness-cut,lem:high-soundness-reduce,lem:high-soundness-merge} (Soundness), and \cref{lem:termination} (Termination), we may conclude~\cref{lem:rsg-is-fus-reformulated}, thus completing the proof of \cref{lem:rsg-is-fus}.

==> ICDT 2023 Updated LaTeXFiles/higher-arities.tex <==
\subsection{The Case of Multi-Headed Rules}\label{sec:higher-arity}

We will now prove \cref{thm:higher-arity}, which implies that for multi-headed rules $\fus \not\subseteq \fcs$. To this end, we exhibit a $\fus$ rule set that yields universal models of infinite clique\-width. 
Let $\sigi = \set{\hpred, \vpred%\mpr{, \origin}{}
}$ %\pr{with binary predicates $\hpred$, $\vpred$ and  a unary predicate $\origin$}{
with $\hpred, \vpred$ binary predicates%}
. Let $\rsgrid$ denote the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} &  & \rightarrow \exists \, x \ \; \big(\,\hpred(x\,,x\,) \land \vpred (x,x\,)\big) \\[0.5ex]
\text{(grow)} &  & \rightarrow \exists yy' \big(\,\hpred(x\,,y\,) \land \vpred (x,y')\big) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists \, y' \; \big(\,\hpred(x'\!,y') \land \vpred(y,y')\big)
\end{array}
$$
We make use of $\rsgrid$ to establish \cref{thm:higher-arity}% (see \cref{sect:main-results})
, the proof of which consists of two parts. First, we provide a database $\dbg$ to form a knowledge base $(\dbg, \rsg)$ for which no universal model of finite cliquewidth exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\msubsection{$\rsgrid$ is not a finite-cliquewidth set}
Toward establishing this result, let $\dbg = \set{%\mpr{\origin(a)}{
\top(\const{a})}%}
$ and define the instance $\ginf$, where $\const{a}$ is a constant and $y$ as well as $x_{i,j}$ with $i,j \in \mathbb{N}$ are nulls: 
\begin{eqnarray*}
\ginf & = & \big\{%\mpr{\origin(a),}{}
\hpred(\const{a},x_{1,0}),\vpred(\const{a},x_{0,1}),\hpred(y,y),\vpred(y,y)\big\} \\
 & & \cup\,\big\{\hpred(x_{i,j},x_{i+1,j}), \vpred(x_{i,j},x_{i,j+1}) \mid  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\}.
% & & \cup\,\big\{\vpred(x_{i,j},x_{i,j+1}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} 
\end{eqnarray*}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{ginf.pdf}
    \vspace{-1ex}
    \caption{ The instance $\ginf$.}
    \label{fig:ginf}
\end{figure}

\cref{fig:ginf} depicts $\ginf$ graphically.
The following lemma summarizes consecutively established properties of $\ginf$ and its relationship with $\kbaseg$.

\begin{lemma}
With $\ginf$ and $\kbaseg$ as given above, we obtain:
\begin{itemize}
\item $\ginf$ has infinite cliquewidth,
\item $\ginf$ is a universal model of $\kbaseg$,
\item the only homomorphism $h: \ginf \to \ginf$ is the identity,
\item any universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$,
\item $\kbaseg$ has no universal model of finite cliquewidth.
\end{itemize}
\end{lemma}

From the last point (established via the insight that taking induced subinstances never increases clique\-width), the announced result immediately follows.

\begin{lemma}\label{lem:no-universal-model-cw}
$\rsg$ is not $\fcs$.
\end{lemma}



\msubsection{$\rsgrid$ is a finite-unification set}
Unfortunately, $\rsg$ does not fall into any of the known syntactic $\fus$ subclasses and showing that a provided rule set is $\fus$ is a notoriously difficult task in general.\footnote{This should not be too surprising however, as being $\fus$ is an undecidable property~\cite{BagLecMugSal11}.}
At least, thanks to the rule $(\mathrm{loop})$, every BCQ that is free of constants is always entailed and can thus be trivially re-written. %\sebastian{What about queries that have A?}
%
For queries involving constants, we provide a hand-tailored query rewriting algorithm, along the lines of prior work exploring the multifariousness of $\fus$ \cite{OstMarCarRud22}. The required argument is quite elaborate and we just sketch the main ideas here due to space restrictions.

We make use of special queries, referred to as \emph{marked queries}: queries with some of their terms ``marked''  with the purpose of indicating terms that need to be mapped to database constants in the course of rewriting. The notion of query satisfaction is lifted to such marked CQs, which enables us to identify the subclass of \emph{properly marked queries} as those who actually have a match into some instance $\sg$, where $\db$ is an arbitrary database.

With these notions at hand, we can now define a principled rewriting procedure consisting of the exhaustive application of three different types of transformation rules. We show that this given set of transformations is in fact sound and complete, i.e., it produces correct first-order rewritings upon termination. Last, we provide a  termination argument by showing that the operations reduce certain features of the rewritten query. Thus, we arrive at the second announced result, completing the overall proof.

\begin{lemma}\label{lem:rsg-is-fus}
$\rsg$ is $\fus$.
\end{lemma}

\subsection{Fus and Expressive Queries}

\newcommand{\TM}{{\scaleobj{0.8}{\mathit{TM}}}}

Let us put the negative result of \cref{sec:higher-arity} into perspective.
Thanks to \cref{cor:fcsdecidable}, we know that $\fcs$ ensures decidability of arbitrary DaMSOQ entailment, a quite powerful class of queries. By contrast, $\fus$ is a notion tailored to CQs and unions thereof. As it so happens, searching for a method to establish decidability of DaMSOQ entailment for arbitrary $\fus$ rule sets turns out to be futile. This even holds for a fixed database and a fixed rule set. 
\begin{lemma}
DaMSOQ entailment is undecidable for $(\dbg,\rsg)$.
\end{lemma}
The corresponding proof is rather standard:
One can, given a deterministic Turing machine $\mathit{TM}$, create a DaMSOQ $(\mathfrak{q}_\TM,\Xi_\TM)$ that is even expressible in monadic datalog and, when evaluated over $\ginf$, uses the infinite grid to simulate a run of that Turing machine, resulting in a query match \ifandonlyif $\mathit{TM}$ halts on the empty tape.
As $\ginf$ is a universal model of $(\dbg,\rsg)$, and DaMSOQ satisfaction is preserved under homomorphisms, the entailment $(\dbg,\rsg) \models (\mathfrak{q}_\TM,\Xi_\TM)$ coincides with the termination of $\mathit{TM}$, concluding the argument.

==> ICDT 2023 Updated LaTeXFiles/introduction.tex <==
\section{Introduction}

Querying under \emph{existential rules}\footnote{Existential rules are also referred to as \emph{tuple-generating dependencies} (TGDs)~\cite{AbiteboulHV95}, \emph{conceptual graph rules}~\cite{SalMug96}, Datalog$^\pm$~\cite{Gottlob09}, and \emph{$\forall \exists$-rules}~\cite{BagLecMugSal11} in the literature.} (henceforth often shortened to \emph{rules}) is a popular topic in database theory and knowledge representation. For arbitrary rule sets, query entailment is undecidable~\cite{ChandraLM81}, motivating research into fragments for which decidability can be regained.

To this end, a very useful conceptual tool
%which has not only proven useful for describing querying methods, but also for identifying %classes of rule sets with decidable query entailment, 
is the \emph{chase}~\cite{Chase84}: For a database $\database$ and rule set $\ruleset$, the (possibly non-terminating) chase procedure yields a \emph{universal model}~\cite{DeuNasRem08}, satisfying all queries entailed by $\database$ and $\ruleset$. This allows for reducing query entailment to query evaluation.

Rule sets admitting finite universal models (a property equivalent to being a \emph{finite-expansion set}~\cite{BagLecMugSal11} or \emph{core-chase terminating}~\cite{DeuNasRem08}) are particularly well-behaved. 
%
%This is witnessed by the fact that classes thereof subsume a wide variety of so-called \emph{concrete classes}~\tim{\cite{}}, syntactically defined classes of rule sets based on diverse notions of \emph{acyclicity}~\tim{\cite{}}.
%
%syntactically defined so-called \emph{concrete classes} of rules based on diverse notions of \emph{acyclicity}.
%
But even in cases where universal models are necessarily infinite, they may still be sufficiently ``tame'' to allow for decidable query entailment, as is the case with the class of \emph{bounded-treewidth sets} ($\bts$)~\cite{BagLecMugSal11}. A rule set $\ruleset$ qualifies as $\bts$ \iffi for every database~$\database$, there exists a universal model of $\database$ and $\ruleset$ whose \emph{treewidth} (a structural measure originating from graph theory) is finite.
%bounded by some $n\in \mathbb{N}$. 
The $\bts$ class subsumes the $\fes$ class, and gives rise to decidable query entailment for a sizable family of concrete, syntactically defined classes of rule sets 
%deploying more or less refined versions of guardedness~
\cite{BagLecMugSal11,CaliGK13,KrotzschR11}.     

While $\bts$ is a fairly general class, it still fails to contain rather simple rule sets; e.g., the rule set $\ruleset^\infty_\mathrm{tran}$, consisting of the two rules
%%%%
% CAUTION: THE SECOND OF THE FOLLOWING RULES WAS WRONG: 
% IT HAD AN \exists z IN FRONT OF THE SECOND RULE HEAD.
% I REMOVED IT. PROBABLY IT WAS JUST A COPY-PASTE ERROR
% BY ME, BUT JUST TO BE SAFE, I LEFT THIS COMMENT
%%%%
$
\epred(x,y) \to \exists z \epred(y,z)$ and $\epred(x,y) \wedge \epred(y,z) \to \epred(x,z),
$
falls outside the $\bts$ class. To give an idea as to why this holds, consider any database $\db$ containing an $\epred$-fact (e.g., $\epred(\const{a},\const{b})$): the chase will yield a universal model resembling the transitive closure of an infinite $\epred$-path, a clique-like structure of infinite treewidth. What is more, not only does $\ruleset^\infty_\mathrm{tran}$ fail to be $\bts$, it also fails to fall under the other generic decidability criteria: it is neither \emph{finitely controllable} (which would guarantee the existence of a finite ``countermodel'' for each non-entailed query) nor $\fus$ (see below). Yet, results for  description logics confirm the decidability of (conjunctive) query entailment over $\ruleset^\infty_\mathrm{tran}$ (see~\cite{GlimmLHS08,OrtizRS11}), in\-cen\-ti\-vi\-zing a generalization of the decidability criteria mentioned above.

%\tim{Note: Depending on if we adopt fus, FO-rewritable, etc. we will potentially have to do a bit of re-writing above and/or below.}

The class of \emph{finite-unification sets} ($\fus$)~\cite{BagLecMugSal11}, incomparable with $\bts$, gives rise to decidable query entailment thanks to \emph{first-order rewritability}. Such rule sets may feature non-guarded rules \cite{CaliGP12}; for instance, they may include \emph{concept products} \cite{RudolphKH08,BourhisMP17}, which create a biclique linking instances of two unary predicates, as in 
$
\pred{Elephant}(x) \wedge \pred{Mouse}(y) \to \pred{BiggerThan}(x,y).
$

The above examples demonstrate a crucial weakness of the $\bts$ class: its inability to tolerate universal models exhibiting ``harmless'' unbounded clique-like structures. Opportunely, the graph-theoretic notion of \emph{cliquewidth}~\cite{CourEngBook} overcomes this problem, while retaining most of treewidth's desirable properties. Inspired by this less mainstream, but more powerful concept, we introduce \emph{finite-cliquewidth sets}~($\bcws$) of rules. Our contributions are as follows:
%As the original cliquewidth notion is tailored to finite undirected graphs, some (not entirely straightforward) generalizations are necessary to adapt it to countable instances, while at the same time, preserving its advantageous properties. Our contributions can be summarized as follows:
\vspace{-0.3ex}
\begin{itemize}
    \item We introduce a generic framework for utilizing certain model-theoretic measures to establish decidability of entailment for a comprehensive class of queries (dubbed \emph{datalog/MSO queries}, or \emph{DaMSOQs} for short) that significantly extends conjunctive queries. 
    
    \item Generalizing the eponymous notion from finite graph theory, we introduce the model-the\-o\-re\-tic measure of \emph{cliquewidth} for countable instances over arbitrary signatures. Based on our framework, we show that the derived notion of \emph{finite-cliquewidth sets} %$\fcs$ 
    guarantees decidability of DaMSOQ entailment. In particular, we demonstrate that $\ruleset^\infty_\mathrm{tran}$ is indeed $\fcs$, thus showing that $\fcs$ incorporates rule sets outside $\bts$ and $\fus$.
    
    \item We compare the $\fcs$ and $\bts$ classes, obtaining: (good news) for binary signatures, $\fcs$ subsumes $\bts$, which (bad news) does not hold for higher-arity signatures, but (relieving news) $\fcs$ still ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\begin{itemize}
        %\item[] 
 %       \underline{Good News}: For unary and binary signatures, $\fcs$ subsumes $\bts$;\\
        %\item[] 
 %       \underline{Bad News}: For higher-arity signatures, $\fcs$ does not subsume $\bts$;
        %This inclusion does not generalize to higher arities.\\ 
        %\item[] 
 %       \underline{Relievin}g\underline{ News}: Yet, $\fcs$ ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\end{itemize}
    \item We compare the $\fcs$ and $\fus$ classes, obtaining: (good news) for sets of single-headed rules over signatures of arity ${\leq}2$, $\fcs$ subsumes $\fus$, which (bad news) does not hold for multi-headed rules, but (relieving news) this could not be any different as there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.
    %\begin{itemize}
        %\item 
  %      \underline{Good News}: For sets of single-headed rules over unary and binary signatures, $\fcs$ subsumes $\fus$;\\
        %\item 
 %       \underline{Bad News}: This inclusion does not hold for multi-headed rules.\\ 
        %\item 
 %       \underline{Relievin}g\underline{ News}: It couldn't be any different, since there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.\\  
    %\end{itemize}
    
%    \item On the negative side, we expose a rule set $\rsgrid$ that is FO-rewritable (and thus admits decidable CQ entailment) but is not $\bcws$---thereby showing that $\bcws$ does not subsume $\fus$, although, this is to be expected as decidability is lost when considering the entailment of more expressive queries from the DaMSOQ family.
%    \item On the positive side, we show that $\bcws$ \emph{does} subsume $\fus$ for all single-head rule sets over binary signatures. The proof of this fact is highly nontrivial, and serves as this paper's deepest result.  
\end{itemize}

%\noindent\textbf{For space reasons, we defer technical details to the appendix.} 


%So called \emph{abstract classes} of existential rule sets have an undecidable membership problem, but they comprise a wide range of rule sets and provide a uniform argument for the decidability of query answering.   



%Existential rules are important <- query entailment is easy <- chase provides universal models. However even the chase fails when existential rules are not constrained. Thus many subclasses that provide decidable query entailment were introduced {\em bounded cliquewidth sets} and FUS/BDD/FO-rewritable covering most of those. With the reasons for the decidablility of query entailment for those classes are well understood it is believed that admitting grid-like universal models lead to undecidability of query entailment. In this paper we show that this is the case for binary signatures --- bcs class subsumes fus --- and surprisingly that it is not true for higher arities.

%Say things about BDD, FUS, FO-rewritability only there.

==> ICDT 2023 Updated LaTeXFiles/long-introduction.tex <==
\section{Introduction}

The problem of querying under \emph{existential rules}\footnote{Existential rules are also referred to as \emph{tuple-generating dependencies} (TGDs)~\cite{AbiteboulHV95}, \emph{conceptual graph rules}~\cite{SalMug96}, Datalog$^\pm$~\cite{Gottlob09}, and \emph{$\forall \exists$-rules}~\cite{BagLecMugSal11} in the literature.} (henceforth often shortened to \emph{rules}) is a popular topic in the research fields of database theory and knowledge representation. For arbitrary rule sets, query entailment is undecidable~\cite{ChandraLM81}, motivating research into expressive fragments for which decidability can be regained.

A theoretical tool which has not only proven useful for describing querying methods, but also for identifying classes of rule sets with decidable query entailment, is the \emph{chase}~\cite{Chase84}. Given a database $\database$ and a rule set $\ruleset$, the (potentially non-terminating) chase procedure yields a so-called \emph{universal model}~\cite{DeuNasRem08}. Universal models satisfy exactly those queries entailed by $\database$ and $\ruleset$ and thus allow for the reduction of query entailment to query evaluation.

Rule sets admitting finite universal models (a property equivalent to being a \emph{finite-expansion set}~\cite{BagLecMugSal11} or \emph{core-chase terminating}~\cite{DeuNasRem08}) are particularly well-behaved. 
%
%This is witnessed by the fact that classes thereof subsume a wide variety of so-called \emph{concrete classes}~\tim{\cite{}}, syntactically defined classes of rule sets based on diverse notions of \emph{acyclicity}~\tim{\cite{}}.
%
%syntactically defined so-called \emph{concrete classes} of rules based on diverse notions of \emph{acyclicity}.
%
But even in cases where universal models are necessarily infinite, they may still be sufficiently ``tame'' to allow for decidable query entailment, as is the case with the class of \emph{bounded-treewidth sets} ($\bts$)~\cite{BagLecMugSal11}. A rule set $\ruleset$ qualifies as $\bts$ \iffi for every database~$\database$, there exists a universal model of $\database$ and $\ruleset$ whose \emph{treewidth} (a structural measure originating from graph theory) is bounded by some $n\in \mathbb{N}$. The $\bts$ class subsumes class of finite expansion sets ($\fes$), and gives rise to decidable query entailment for a sizable family of concrete, syntactically defined classes of rule sets deploying more or less refined versions of guardedness~\cite{BagLecMugSal11,CaliGK13,KrotzschR11}.     

While $\bts$ is a fairly general class, it still fails to contain rather simple rule sets; e.g., the rule set $\ruleset^\infty_\mathrm{tran}$, consisting of the two rules
%%%%
% CAUTION: THE SECOND OF THE FOLLOWING RULES WAS WRONG: 
% IT HAD AN \exists z IN FRONT OF THE SECOND RULE HEAD.
% I REMOVED IT. PROBABLY IT WAS JUST A COPY-PASTE ERROR
% BY ME, BUT JUST TO BE SAFE, I LEFT THIS COMMENT
%%%%
$$
\epred(x,y) \to \exists z \epred(y,z) \quad\text{and}\quad \epred(x,y) \wedge \epred(y,z) \to \epred(x,z),
$$
falls outside the $\bts$ class. To give an idea as to why this holds, consider any database $\db$ containing an $\epred$-fact (e.g., $\epred(\const{a},\const{b})$): the chase will yield a universal model resembling the transitive closure of an infinite $\epred$-path, a clique-like structure of infinite treewidth. What is more, not only does $\ruleset^\infty_\mathrm{tran}$ fail to be $\bts$, it also fails to fall under the other generic decidability criteria: it is neither $\fus$ (described below) nor \emph{finitely controllable} (which would guarantee the existence of a finite ``countermodel'' for each non-entailed query). In spite of this, results for description logics confirm the decidability of (conjunctive) query entailment over $\ruleset^\infty_\mathrm{tran}$ (see~\cite{GlimmLHS08,OrtizRS11}), in\-cen\-ti\-vi\-zing a generalization of the decidability criteria mentioned above.

%\tim{Note: Depending on if we adopt fus, FO-rewritable, etc. we will potentially have to do a bit of re-writing above and/or below.}

On a separate, but related note: the $\bts$ class is incomparable with the class of \emph{finite-unification sets} ($\fus$)~\cite{BagLecMugSal11}, another class giving rise to decidable query entailment thanks to \emph{first-order rewritability}. Such rule sets may feature non-guarded rules \cite{CaliGP12}; for instance, they may include \emph{concept products} \cite{BourhisMP17,RudolphKH08}, which create a biclique linking instances of two unary predicates, as in 
$$
\pred{Elephant}(x) \wedge \pred{Mouse}(y) \to \pred{BiggerThan}(x,y).
$$

The above examples demonstrate a crucial weakness of the $\bts$ class, namely, its inability to tolerate universal models exhibiting ``harmless'' unbounded clique-like structures. Opportunely, the graph-theoretic notion of \emph{cliquewidth}~\cite{CourEngBook} overcomes this problem, while retaining most of the desirable properties associated with the notion of treewidth. Inspired by this less mainstream, but more powerful concept, we set out to introduce \emph{finite-cliquewidth sets}~($\bcws$) of rules. As the original cliquewidth notion is tailored to finite undirected graphs, some (not entirely straightforward) generalizations are necessary to adapt it to countable instances, while at the same time, preserving its advantageous properties.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We introduce an abstract framework showing how to utilize specific types of model-theoretic measures to establish the decidability of query entailment for a comprehensive class of queries (dubbed \emph{datalog / monadic second-order queries}, or \emph{DaMSOQs} for short) that significantly extends the class of conjunctive queries. 
    
    \item Generalizing the eponymous notion from finite graph theory, we introduce the model-theoretic measure of \emph{cliquewidth} for countable instances over arbitrary signatures. Based on our framework, we show that the derived notion of \emph{finite-cliquewidth sets} %$\fcs$ 
    guarantees decidability of DaMSOQ entailment. In particular, we demonstrate that $\ruleset^\infty_\mathrm{tran}$ is indeed $\fcs$, thus showing that $\fcs$ incorporates rule sets outside $\bts$ and $\fus$.
    
    \item We compare the $\fcs$ and $\bts$ classes, obtaining: (good news) for binary signatures, $\fcs$ subsumes $\bts$, which (bad news) does not hold for higher-arity signatures, but (relieving news) $\fcs$ still ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\begin{itemize}
        %\item[] 
 %       \underline{Good News}: For unary and binary signatures, $\fcs$ subsumes $\bts$;\\
        %\item[] 
 %       \underline{Bad News}: For higher-arity signatures, $\fcs$ does not subsume $\bts$;
        %This inclusion does not generalize to higher arities.\\ 
        %\item[] 
 %       \underline{Relievin}g\underline{ News}: Yet, $\fcs$ ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\end{itemize}
    \item We compare the $\fcs$ and $\fus$ classes, obtaining: (good news) for sets of single-headed rules over signatures of arity ${\leq}2$, $\fcs$ subsumes $\fus$, which (bad news) does not hold for multi-headed rules, but (relieving news) this could not be any different as there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.
    %\begin{itemize}
        %\item 
  %      \underline{Good News}: For sets of single-headed rules over unary and binary signatures, $\fcs$ subsumes $\fus$;\\
        %\item 
 %       \underline{Bad News}: This inclusion does not hold for multi-headed rules.\\ 
        %\item 
 %       \underline{Relievin}g\underline{ News}: It couldn't be any different, since there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.\\  
    %\end{itemize}
    
%    \item On the negative side, we expose a rule set $\rsgrid$ that is FO-rewritable (and thus admits decidable CQ entailment) but is not $\bcws$---thereby showing that $\bcws$ does not subsume $\fus$, although, this is to be expected as decidability is lost when considering the entailment of more expressive queries from the DaMSOQ family.
%    \item On the positive side, we show that $\bcws$ \emph{does} subsume $\fus$ for all single-head rule sets over binary signatures. The proof of this fact is highly nontrivial, and serves as this paper's deepest result.  
\end{itemize}

%\noindent\textbf{For space reasons, we had to defer technical details, discussions and most proofs to the appendix.}

\noindent\textbf{For space reasons, we defer technical details and most proofs to the appendix.}


%So called \emph{abstract classes} of existential rule sets have an undecidable membership problem, but they comprise a wide range of rule sets and provide a uniform argument for the decidability of query answering.   



%Existential rules are important <- query entailment is easy <- chase provides universal models. However even the chase fails when existential rules are not constrained. Thus many subclasses that provide decidable query entailment were introduced {\em bounded cliquewidth sets} and FUS/BDD/FO-rewritable covering most of those. With the reasons for the decidablility of query entailment for those classes are well understood it is believed that admitting grid-like universal models lead to undecidability of query entailment. In this paper we show that this is the case for binary signatures --- bcs class subsumes fus --- and surprisingly that it is not true for higher arities.

%Say things about BDD, FUS, FO-rewritability only there.

==> ICDT 2023 Updated LaTeXFiles/notation.tex <==
%%%Commands used to reference lemmas, observations, etc. in text

\newcommand{\msubsection}[1]{\medskip{\noindent\bf{}#1{}.}}

\newtheorem{innercustomlem}{Lemma}
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}
  
  \newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
\newtheorem{innercustomobs}{Observation}
\newenvironment{customobs}[1]
  {\renewcommand\theinnercustomobs{#1}\innercustomobs}
  {\endinnercustomobs}
  
\newtheorem{innercustomcor}{Corollary}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomcor}

%%% Structures
\newcommand{\signature}{\Sigma}
\newcommand{\ball}[2]{\mathrm{Ball}_{#1}(#2)}
\newcommand{\bball}[2]{\overline{\mathrm{Ball}}_{#1}(#2)}
\newcommand{\dist}[1]{\fcn{dist}(#1)}
\newcommand{\instance}{\mathcal{I}}
\newcommand{\inst}{\instance}
\newcommand{\database}{\mathcal{D}}
\newcommand{\db}{\database}
\newcommand{\adom}[1]{\fcn{dom}(#1)}
\newcommand{\aadom}[1]{\fcn{dom}(#1)}
\newcommand{\unimod}{\mathcal{U}}
\newcommand{\cnst}{\mathrm{Cnst}}


%%% Chase stuff
\newcommand{\trigs}{tr}
\newcommand{\trigsr}{tr_{\ruleset}}


%%%clique-width related notation
\newcommand{\relstr}{\mathcal{A}}
\newcommand{\coloring}{\lambda}
\newcommand{\coloringe}{\lambda_\exists}
\newcommand{\prcoloringe}{\overline{\coloring}_{\exists}}
\newcommand{\coloringee}{\lambda_{k_{\exists}}}
\newcommand{\ke}{k_{\exists}}
\newcommand{\cols}{\mathbb{L}}
\newcommand{\colstructs}{\mathfrak{M}_{\sig, \cols}}
\newcommand{\crelstr}{\mathcal{C}}
\newcommand{\numcolors}[1]{L(#1)}
\newcommand{\val}[1]{val(#1)}
\newcommand{\term}{T}
\newcommand{\unitn}{\mathbbm{1}_{n}}
\newcommand{\unit}{\mathbbm{1}}
\newcommand{\arity}[1]{\fcn{ar}(#1)}
\newcommand{\cw}[1]{\fcn{cw}(#1)}
\newcommand{\length}[1]{\fcn{len}(#1)}
\newcommand{\disun}{\oplus}
\newcommand{\add}[2]{\pred{Add}_{#1}(#2)}
\newcommand{\addd}[1]{\pred{Add}_{#1}}
\newcommand{\recol}[2]{\pred{Recolor}_{#1}(#2)}
\newcommand{\subterm}{\sqsubseteq}
\newcommand{\sdom}{\mathcal{V}}
\newcommand{\srel}{\mathcal{E}}


%%%FUNCTION STUFF
\newcommand{\hism}{h}
\newcommand{\sub}{\sigma}
\newcommand{\safesub}{\sigma^{\safe}}
\newcommand{\treewidth}[1]{\fcn{tw}(#1)}
\newcommand{\tw}[1]{\fcn{tw}(#1)}
\newcommand{\safe}{\mathit{safe}}
\newcommand{\head}{\fcn{head}}
\newcommand{\body}{\fcn{body}}
\newcommand{\fcomp}{\circ}
\newcommand{\codom}[1]{\fcn{codom}(#1)}
\newcommand{\fcn}[1]{\mathsf{#1}}
\newcommand{\orig}{\fcn{orig}}
\newcommand{\ent}{\fcn{ent}}
\newcommand{\col}{\fcn{col}}

%%%NAMES OF EXISTENTIAL RULE SETS
\newcommand{\ruleset}{\calr}
\newcommand{\rs}{\ruleset}
\newcommand{\rr}{RR}
\newcommand{\disc}{DISC}
\newcommand{\fri}{FR1}
\newcommand{\g}{G}
\newcommand{\gbts}{\mathbf{gbts}}
\newcommand{\bfgbts}{\mathbf{bfgbts}}
\newcommand{\bts}{\mathbf{bts}}
\newcommand{\bcs}{\mathbf{fcs}}
\newcommand{\adbts}{\mathbf{adbts}}
\newcommand{\bfbts}{\mathbf{bfbts}}
\newcommand{\fes}{\mathbf{fes}}
\newcommand{\agrd}{\mathbf{aGRD}}
\newcommand{\fus}{\mathbf{fus}}
\newcommand{\adgs}{\mathbf{adgs}}
\newcommand{\wadgs}{\mathbf{wadgs}}
\newcommand{\wgbts}{\mathbf{wgbts}}
\newcommand{\bcws}{\bcs}
\newcommand{\fcs}{\mathbf{fcs}}
\newcommand{\fc}{\mathbf{fc}}

%%%Forward and Backward Chaining Notation
\newcommand{\chase}{\mathbf{Ch}}
\newcommand{\sa}{\mathbf{Ch}_{\infty}}
\newcommand{\se}{\mathbf{Ch}_{\exists}}
\newcommand{\sep}{\mathbf{Ch}_{\exists+}}
\renewcommand{\so}{\ksat{1}{\sep,\rulesetnormminus}}
\newcommand{\fchain}[1]{\chase(#1)}
\newcommand{\ksat}[2]{\chase_{#1}(#2)}
\newcommand{\sat}[1]{\ksat{\infty}{#1}}
\newcommand{\sate}[1]{\ksat{\exists}{#1}}
\newcommand{\satee}{\sate{\ruleset, \database}}
\newcommand{\bchain}[1]{\beta(#1)}
\newcommand{\cutp}{cutp}
\newcommand{\derseq}{\mathcal{D}}
\newcommand{\der}{\mathcal{D}}
\newcommand{\kbaseg}{(\dbg,\rsg)}


%%%Logic Names
\newcommand{\gf}{\mathcal{GF}}

%%% FO-rewritability
\newcommand{\rew}[1]{\fcn{rew}(#1)}
\newcommand{\rewrs}[2]{\fcn{rew}_{#1}(#2)}

%%%Logical Notation
\newcommand{\calm}{\mathcal{M}}
\newcommand{\calr}{\mathcal{R}}
\newcommand{\calro}{\widetilde{\mathcal{R}}}
\newcommand{\calrl}{\mathcal{R}^{l}}
\newcommand{\calrr}{\mathcal{R}^{r}}
\newcommand{\struc}{\mathcal{A}}
\newcommand{\grid}{\mathcal{G_{\infty}}}
\newcommand{\dom}{D}
\newcommand{\inter}{I}
\newcommand{\env}{\xi}
\newcommand{\model}{\mathcal{M}}
\newcommand{\lang}{\mathcal{L}}
\newcommand{\langsig}{\mathcal{L}_{\sig}}
\newcommand{\conset}{\mathrm{con}}
\newcommand{\nullset}{\mathrm{nul}}
\newcommand{\termset}{\fcn{terms}}
\newcommand{\varset}{\mathrm{var}}
\newcommand{\predset}{\mathrm{pred}}
\newcommand{\assign}[1]{[\![#1]\!]}
\newcommand{\formset}{\Gamma}
\newcommand{\formsetii}{\Delta}
\newcommand{\kb}{\mathcal{K}}
\newcommand{\sig}{\Sigma}
\newcommand{\pred}[1]{\mathtt{#1}}
\newcommand{\const}[1]{\mathtt{#1}}
\newcommand{\thephi}{\varphi}

%%%MISC
\newcommand{\fr}{\mathit{fr}}
\newcommand{\tree}{T}
\newcommand{\set}[1]{\{#1\}}

\newcommand{\VX}{\vec{X}}
\newcommand{\VY}{\vec{Y}}

\newcommand{\vk}{\smash{\vec{k}}}
\newcommand{\vs}{\vec{s}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vX}{\vec{X}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vvv}{\vec{v}}
\newcommand{\vY}{\vec{Y}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vT}{\vec{T}}
\newcommand{\va}{\vec{a}}
\newcommand{\vb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\vl}{\vec{l}}
\newcommand{\vu}{\vec{u}}
\newcommand{\sigi}{\sig_\mathrm{grid}}
\newcommand{\rsg}{\ruleset_\mathrm{grid}}
\newcommand{\dbg}{\database_\mathrm{grid}}
\newcommand{\ginf}{\mathcal{G}_{\infty}}
\newcommand{\sg}{\sat{\db,\rsg}}
\newcommand{\mq}{(q, M)}
\newcommand{\hpred}{\pred{H}}
\newcommand{\vpred}{\pred{V}}
\newcommand{\rpred}{\pred{R}}
\newcommand{\ppred}{\pred{P}}
\newcommand{\epred}{\pred{E}}
\newcommand{\origin}{\pred{A}}
\newcommand{\goal}{\mathtt{Goal}}
\newcommand{\rsgrid}{\ruleset_\mathrm{grid}}
\newcommand{\prmark}{M}
\newcommand{\mquery}{Q}
\newcommand{\query}{q}

%%%WRITING ABBREVIATIONS
\newcommand{\etc}{$\ldots$ } %Etcetera
\newcommand{\sect}{Sect.} %Section
\newcommand{\dfn}{Def.} %Definition
\newcommand{\lem}{Lem.} %Lemma
\newcommand{\thm}{Thm.} %Theorem
\newcommand{\cor}{Cor.} %Corollary
\newcommand{\prp}{Prop.} %Property
\newcommand{\fig}{Fig.} %Figure
\newcommand{\app}{Appx.} %Appendix
\newcommand{\ifandonlyif}{\textit{iff} } %if and only if
\newcommand{\iffi}{\textit{iff} } %if and only if
\newcommand{\suchthat}{ such that } %Such that
\newcommand{\ih}{IH } %Induction Hypothesis
\newcommand{\rem}{Rmk.} %Remark
\newcommand{\resp}{resp.}
\newcommand{\cptr}{Ch.}
\newcommand{\exmpl}{Ex.}
\newcommand{\alg}{Alg.}
\newcommand{\FUS}{FUS }

%%% Commenting
\definecolor{piotr}{RGB}{250, 100, 100}
\definecolor{thomas}{RGB}{50, 190, 50}
\definecolor{tim}{RGB}{0, 0, 250}
\definecolor{sebastian}{RGB}{153, 50, 204}
\newcommand{\piotr}[1]{\textbf{\textcolor{black}{piotr}}: {\color{piotr}#1}} \newcommand{\thomas}[1]{\textbf{\textcolor{black}{thomas}}: {\color{thomas}#1}} \newcommand{\tim}[1]{\textbf{\textcolor{black}{tim}}: {\color{tim}#1}} \newcommand{\sebastian}[1]{\textbf{\textcolor{black}{sebastian}}: {\color{sebastian}#1}}
\newcommand{\todoiftime}{\piotr{TODO if we have enough time left before PODS.}}

% for normal mode suggestions
\newcommand{\pr}[2]{\textcolor{red}{\sout{#1}}\textcolor{teal}{#2}}

% for math mode suggestions
\newcommand{\mpr}[2]{\textcolor{red}{\text{\sout{$#1$}}}\textcolor{teal}{#2}}
%\newcommand{\piotr}[1]{} \newcommand{\thomas}[1]{} \newcommand{\tim}[1]{}

%%% Proof specific
\newcommand{\DL}{\scaleobj{0.8}{\mathrm{DL}}}

\newcommand{\rulesetdl}{\ruleset_{\smash{\DL}}}
\newcommand{\rulesetnorm}{\ruleset_{\smash{\DL}}^{\mathrm{rew}}}
\newcommand{\rulesetnormcon}{\ruleset_{\smash{\DL}}^{\mathrm{conn}}}
\newcommand{\rulesetnormminus}{\ruleset_{\smash{\DL}}^{\mathrm{disc}}}
%\newcommand{\rulesetnormminus}{\rulesetnorm \!\setminus\! \rulesetnormcon}
\newcommand{\diam}{d_{\mathrm{DL}}}

\newcommand{\hypenoperator}[2]{\operatorname{#1-#2}}
\newcommand{\op}[0]{\operatorname{op}}
\newcommand{\rednet}{\hypenoperator{red}{nett}}
\newcommand{\cutop}{\operatorname{cut}}
\newcommand{\mergeop}{\operatorname{merge}}
\newcommand{\reduceop}{\operatorname{reduce}}
\newcommand{\stepop}{\rightrightarrows}
\newcommand{\rank}[1]{\operatorname{rank}(#1)}
\newcommand{\cost}[1]{\operatorname{cost}(#1)}
\newcommand{\multiset}[1]{\set{#1}_{m}}
\newcommand{\minusone}{\text{\tiny -1}}
\newcommand{\Hm}{H^{\minusone}}
\newcommand{\Vm}{V^{\minusone}}
\newcommand{\Em}{V^{\minusone}}
\newcommand{\neigh}[2]{\mathit{#2^#1}}
\newcommand{\ldist}[2]{\fcn{dist}_{#1}(#2)}

%\newcommand{\smallldots}{...\,}
\newcommand{\smallldots}{\ldots}
\DeclareMathOperator*{\smallbigwedge}{{\textstyle\bigwedge}}

\newcommand{\defend}{\hfill\ensuremath{\Diamond}}


%\ICDT macros
\newcounter{SHOWNEW}
\setcounter{SHOWNEW}{1}

\newcommand{\ifcmd}[2]{
    \ifthenelse{\value{SHOWNEW}>0}
        {#2}
        {#1}
}

\ifcmd
    {\newcommand{\prm}[1]{\textcolor{red}{#1}}}
    {\newcommand{\prm}[1]{}}
    
\ifcmd
    {\newcommand{\pct}[2]{\textcolor{red}{#1} \textcolor{teal}{#2}}}
    {\newcommand{\pct}[2]{#2}}
    
\ifcmd
    {\newcommand{\pin}[1]{\textcolor{teal}{#1}}}
    {\newcommand{\pin}[1]{#1}}


==> ICDT 2023 Updated LaTeXFiles/other/binary-ball.tex <==
\section{Results for Binary Signatures}



In this section, we will prove the first of our two main results, \textit{viz.} \cref{thm:binary}. We fix a binary signature $\sig$, a finite unification set $\ruleset$ of single-headed rules over $\sig$, and a database $\database$ over $\sig$ for the remainder of the section. To prove \cref{thm:binary}, it suffices to show that the clique-width of $\sat{\ruleset, \database}$ is bounded, hence, we dedicate this section to establishing the following lemma.

\begin{lemma}\label{lem:binary-main}
%There exists an $n \in \mathbb{N}$ s.t. $\cw{\sat{\ruleset, \database}} \leq n$. 
$\sat{\ruleset, \database}$ has bounded clique-width.
\end{lemma}

Having fixed the rule set $\ruleset$ and the database $\database$, we abbreviate $\sat{\ruleset, \database}$ as $\sa$.

\subsection{Looking Past Datalog}

Let $\se \subseteq \sa$ be the instance containing the existential atoms of $\sa$, that is, the atoms derived via the non-datalog rules of $\ruleset$. We %let the structure of $\se$  be $\struc^{\se} = (\sdom^{\se}, \srel^{\se})$, and 
 note that $\se$ is a crucial building block in the proof of \cref{lem:binary-main} as it satisfies the following observation:


%%%COMMENT%%%
\begin{comment}
\tim{Concerning the sentence: ``If $\sa$ can be derived in multiple ways, we fix a single derivation sequence to determine which atoms are existential.'' which was the second sentence above. Isn't it enough to observe that the atom contains at least one null without consulting a derivation? Since databases only contain constants, we should immediately be able to conclude that any atom with a null was derived via a non-datalog rule. Perhaps we should delete this sentence then, if you agree.}
\piotr{No :) Consider the following rule set $R=$ \begin{itemize}
    \item $A(x) \to \exists{y} E(x,y)$
    \item $A(x) \to \exists{y} F(x,y)$
    \item $E(x,y) \to F(x,y)$
    \item $F(x,y) \to E(x,y)$
\end{itemize}
And the following instance $\set{A(a), E(a,t), F(a, t)} = 
\sat{R, \set{A(a)}}$ there is no way to determine which atom is datalog and which is existential. As a matter of fact, the result of the restricted chase very much depends on the order of rule application. Consider $\set{A(a), E(a, t) F(a, t), E(a, t'), F(a, t')}$. We should discuss that somewhere in the paper as well.
}
\end{comment}
%%%COMMENT%%%



\begin{observation}\label{obs:sate-is-forest}
%Let $\inst = \se \setminus \database$. Then, $\struc^{\inst} = (\sdom^{\inst}, \srel^{\inst})$ is a typed polyforest of bounded degree.
$\se \setminus \database$ is a typed polyforest of bounded degree.
\end{observation}

\begin{proof}
See \cref{appendix} for details.
\end{proof}

From this we can derive the following:

\begin{corollary}\label{cor:skeleton-has-bounded-cw}
%The clique-width of $\struc^{\se}$ is bounded.
 The clique-width of $\se$ is bounded.
\end{corollary}

\begin{proof} %Let $\inst = \se \setminus \db$ and define $\struc^{\inst} = (\sdom^{\inst}, \srel^{\inst})$. 
 By \cref{obs:sate-is-forest}, we know that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest of bounded degree, and by \cref{obs:trees_cw_le3}, we know %$\cw{\struc^{\inst}} \le 2 \cdot |\sig| + 2$
 $\cw{\se \setminus \database} \le 2 \cdot |\sig| + 2$. For some set of typed polytrees in the typed polyforest %$\struc^{\inst}$
 $\se \setminus \database$ (of which there are only finitely many), each has a unique term (which we call a \emph{connection element}) that is connected to a term of $\db$ in %$\struc^{\se}$ 
 $\se$ (which we call a \emph{connection root}). Let $n$ be the number of connection elements in %$\struc^{\inst}$ 
 $\se \setminus \database$ and define the set $\cols_{1} = \{m \in \mathbb{N} \ | \ m \leq n\}$ of colors, which we assume w.l.o.g. to be fresh. Observe that if we additionally extend the set of colors $\cols$ (used in the proof of \cref{obs:trees_cw_le3}) with the set $\cols_{1}$, then we may assume that prior to taking the disjoint union of all typed polytrees in %$\struc^{\inst}$ 
 $\se \setminus \database$ (during the construction process detailed in \cref{obs:trees_cw_le3}) that we have recolored each connection element to a unique color in $\cols_{1}$. We refer to this colored structure as %$(\struc^{\inst},\coloring_{1})$
 $(\se \setminus \database, \coloring_{1})$, and use this fact below to bound the clique-width of $\se$. Note that if we color connection elements in the above way, then $\cw{\se \setminus \db} \le 2 \cdot |\sig| + n + 2 \leq 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, with the last inequality following from the fact that the Skolem chase will only connect connection roots to at most $2 \cdot |\sig|$ typed polytrees. Since $\db$ is a finite graph, we know that $\cw{\db} \leq k$, for $k = |\adom{\db}|$; hence, we may assume that the set of colors used to color the graph of $\db$ is $\cols_{2} = \{t \ | \ t \in \adom{\db}\}$, which we assume to be disjoint from all colors in $\coloring_{1}$. We refer to this colored structure as $(\db,\coloring_{2})$, and define $(\struc, \coloring) = (\se \setminus \db,\coloring_{1}) \disun (\db,\coloring_{2})$. Now, for each typed polytree in $(\se \setminus \db,\coloring_{1})$ that has a connection element with color $l$, we apply either $\add{R,(l,t)}{\struc, \coloring}$ or $\add{R,(t,l)}{\struc, \coloring}$ (depending on if the connection element is connected with an edge typed with the predicate $R$ to the connection root, or away from the connection root, respectively), where $t$ is the color of the connection root in $(\db,\coloring_{2})$. We can therefore see that $\cw{\se} \leq |\adom{\database}| + 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, thus proving the observation.
\end{proof}



In the sequel, we will use $\se$ and the $\mathrm{add}_{R,\vl}$ operation to reconstruct $\sa$ and prove that $\cw{\sa}$ is bounded. However, a specific coloring is required to prove this claim, which is distinct from the coloring used to prove that $\cw{\se}$ is bounded. Thus, we define a new coloring below %that permits us to conclude \cref{thm:binary} 
 by making use of the fact that $\ruleset$ is $\fus$.\footnote{We note that this is not simply a matter of finding the desired coloring, but rather, is a matter of ``recoloring'' in the proper way (see \cref{obs:cross-coloring}).}
 
\subsection{Rewriting Datalog Rules}

Given our rule set $\ruleset$, we re-write the subset of $\ruleset$ containing all datalog rules into a new rule set, which we denote $\rulesetnorm$. Since $\rulesetnorm$ is a finite set and since the body of each rule in $\rulesetnorm$ is a finite conjunction of atomic formulae, we know that a natural number exists that uniformly bounds the diameter of the body of each rule in $\rulesetnorm$.\footnote{See \cref{sec:preliminaries} for the definition of \emph{diameter}.} Moreover, since our signature $\sig$ is assumed to be finite, it follows that only a finite number of finite instances with finite branching can be constructed with a diameter that fits within the natural number bound. Therefore, we can leverage our re-writing to define a finite set of colors---consisting of the aformentioned finite instances---which will play a central role in demonstrating that $\cw{\sa}$ is bounded.

Let us define $\ruleset_{DL}$ to be the subset of $\ruleset$ containing all datalog rules, and note the following useful equation:
\begin{equation}\label{eq:sa-satse}
\sa = \sat{\ruleset_{DL}, \se}.
\end{equation}

For any relational symbol $R \in \sig$, we define the rule set $\rew{R}$ to be the following:\footnote{Recall that in this section $\sig$ is a fixed binary signature.}
$$
\set{\varphi(\vx, y,z) \to R(y,z) \;|\; \exists{\vx} \varphi(\vx, y,z) \in \rewrs{\ruleset}{R(y,z)}}
$$
and
$$
\rulesetnorm = \bigcup_{R \in \sig} \rew{R}.
$$
We now show that the rule set $\rulesetnorm$ admits an important property:

\begin{lemma}\label{lem:trigger-for-each-rewritten-rule}
For any atom $R(t_{1},t_{2}) \in \sa \setminus \se$ there exists a trigger $(\rho, h)$ in $\se$ with $\rho \in \rulesetnorm$ such that applying $(\rho, h)$ adds $R(t_{1},t_{2})$ to $\se$.
\end{lemma}
\begin{proof}
From the fact that $\ruleset$ is $\fus$, we can conclude that for any ordered pair $(t_{1},t_{2})$ of terms from $\se$, there exists a CQ $\exists \vx \phi(\vx,y,z) \in \rewrs{\ruleset}{R(y,z)}$ such that the following holds:
%
$$\sat{\ruleset, \se} \models R(t_{1},t_{2}) \ \ifandonlyif \ \se \models \exists \vx \phi(\vx,t_{1},t_{2}).
$$
%
Thus, we know that the desired trigger exists for some rule of $\rew{R}$ in $\se$.
\end{proof}

From the above lemma and \cref{eq:sa-satse} we can conclude the following:
\begin{equation}\label{eq:skeleton}
\ksat{1}{\rulesetnorm, \se} \;=\; \sa
\end{equation}

The above equation tells us that we can apply all rules of $\rulesetnorm$ within a single step to obtain the same result as $\sa$. Using this fact, we can determine (and provide a bound for) the size of the neighborhood in $\se$ that is needed to apply any given rule from $\rulesetnorm$. Ultimately, this observation will be used to bound the clique-width of $\sa$, which suffices to conclude \cref{thm:binary}.

\begin{definition}\label{def:diameter}
Let us denote twice the maximal diameter of any connected component in any rule body of $\rulesetnorm$ as $\diam$.
\end{definition}

One the basis of \cref{eq:skeleton} above, we may restate \cref{lem:binary-main} in an equivalent manner as:

\begin{lemma}\label{lem:binary-reformulated}
$\ksat{1}{\rulesetnorm, \se}$ has bounded clique-width.
\end{lemma}

We dedicate the remainder of the section to establishing the above lemma, which implies the desired result (\cref{thm:binary}).



\subsection{Searching for a Suitable Coloring}

Now we are almost ready to define the new coloring for $\se$. Consider the following definition:

\medskip \noindent {\bf Neighbourhoods in $\se$.} % Let $\struc^{\se} = (\sdom^{\se},\srel^{\se})$ be the structure obtained from the instance $\se$ as defined in \cref{sec:cliquewidth}. Given a term $t \in \sdom^{\se}$ and a natural number $n$, we define $\ball{n}{t}$ to be the induced subset of $\se$ over the set $\set{t' \in dom(\sdom^{\se}) \;|\; \dist{t,t'} \leq n}$.\footnote{We note that $\dist{t,t'}$ denotes the \emph{distance} between $t$ and $t'$, i.e. the length of the path (not necessarily directed) connecting $t$ and $t'$.} We refer to $t$ as the {\em central term} of $\ball{n}{t}$. We define $\bball{n}{t}$ to be the equivalence class modulo the isomorphism relation of the instance $\ball{n}{t} \cup R(t)$, where $R$ is a fresh unary predicate such that $R \not\in \sig$. We note that the inclusion of $R(t)$ is helpful as it permits us to reconstruct the central term of a neighbourhood from its given equivalence class.
 Given a term $t \in \adom{\se}$ and a natural number $n$, we define $\ball{n}{t}$ to be the induced subset of $\se$ over the set $\set{t' \in \adom{\se} \;|\; \dist{t,t'} \leq n}$.\footnote{We note that $\dist{t,t'}$ denotes the \emph{distance} between $t$ and $t'$, i.e. the length of the path (not necessarily directed) connecting $t$ and $t'$.} We refer to $t$ as the {\em central term} of $\ball{n}{t}$, and define $\bball{n}{t}$ to be the equivalence class modulo the isomorphism relation of the instance $\ball{n}{t} \cup \{ R(t) \}$, where $R$ is a fresh unary predicate such that $R \not\in \sig$. We note that the inclusion of $R(t)$ is helpful as it permits us to reconstruct the central term of a neighbourhood from its given equivalence class.

Enough groundwork has been laid to define the new coloring function $\coloringe$ for $\se$. Given a term $t$ of $\se$, we define:
$$
\coloringe(t) = \bball{\diam}{t}
$$
and argue that the image of $\coloringe$ is finite.

\begin{observation}\label{obs:finite-balls}
For every $n \in \mathbb{N}$ the set $\set{\bball{n}{t} \;|\; t \in \adom{\se}}$ is finite.
\end{observation}


\begin{proof} Since $\se \setminus \database$ is a typed polytree of bounded degree, $\database$ is finite, and $\sig$ is finite, for any given $n \in \mathbb{N}$, only a finite number of $\bball{n}{t}$ exist.
\end{proof}

%Now that we have defined the coloring $\coloringe$, we make use of it to show that another coloring $\prcoloringe$ can be defined such that for some natural number $\ke$, $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$. Toward this end, it suffices to prove the following lemma:

Now that we have defined the coloring $\coloringe$, we make use of it to define another---almost identical---coloring $\prcoloringe$ such that for some natural number $\ke$, $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$. The only feature distinguishing $\prcoloringe$ from $\coloringe$ is that $\codom{\prcoloringe}$ is defined to be a superset of $\codom{\coloringe}$. As argued in the corollary below, expanding the co-domain of $\coloringe$ with a specific number of colors %, while still retaining the its finiteness, 
 ensures that a sufficient, albeit still finite, number of colors are used in bounding $\cw{\se}$. Let us now prove the following corollary:

%From the above lemma, we may conclude the following:


\begin{corollary}
There exists a number $k_\exists \in \mathbb{N}$ such that $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$.
\end{corollary}
\begin{proof}
From \cref{cor:skeleton-has-bounded-cw}, we know that $\cw{\se}$ is bounded. Hence, there exists a $\coloring$ and $k$ such that $(\se, \coloring) \in \mathfrak{L}_{k}$. We define $(\coloring\times\coloringe)(t) = (\coloring(t), \coloringe(t))$ and let $k' = |\codom{\coloringe}| \in \mathbb{N}$, which we know exists by \cref{obs:finite-balls} and the definition of $\coloringe$ above. For every finite induced subinstance $\inst$ of $\se$, we know that $(\inst,\coloring|_{\adom{\inst}}) \in \mathfrak{L}_{k}$ by our assumption that $(\se, \coloring) \in \mathfrak{L}_{k}$. Hence, by \cref{obs:cross-coloring}, we may conclude that $(\inst, (\coloring\times\coloringe)|_{\adom{\inst}}) \in \mathfrak{L}_{k \cdot k'}$. Since this holds for every finite induced subinstance, we may conclude that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$ holds by \cref{def:cw}.

To complete the proof, let us define the set of colors $\cols = \codom{\coloring \times \coloringe} \cup \codom{\coloringe}$ as well as the following coloring:
\begin{center}
$\prcoloringe(t) = \coloringe(t)$
\end{center}
where we assume that $\codom{\prcoloringe} = \cols$. If we let $k_{\exists} = k \cdot k' + k'$, then by the above fact that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$, we may conclude that $(\se, \prcoloringe) \in \mathfrak{L}_{k_{\exists}}$.
%From \cref{cor:skeleton-has-bounded-cw}, we know that $\cw{\se}$ is bounded. Hence, there exists a $\coloring$ and $k$ such that $(\se, \coloring) \in \mathfrak{L}_{k}$. We define $(\coloring\times\coloringe)(t) = (\coloring(t), \coloringe(t))$ and let $k' = |\codom{\coloringe}| \in \mathbb{N}$, which we know exists by \cref{obs:finite-balls} and the definition of $\coloringe$ above. For every finite induced subinstance $\inst$ of $\se$, which is colored by $(\coloring\times\coloringe)|_{\adom{\inst}}$, we know that $(\inst, (\coloring\times\coloringe)|_{\adom{\inst{}}}) \in \mathfrak{L}_{k \cdot k'}$ by \cref{obs:cross-coloring}. Since this holds for every induced subinstance we conclude that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$ also holds.
%To finish the proof it is enough to project every color of $\coloring\times\coloringe$ onto a second coordinate using $\mathrm{recolor}$ operations. \thomas{To facilitate the projection, we also need to add the $k'$ colors from the image of $\coloringe{}$ to the overall number of used ones. For the numbers of colors this means that we can use up to $k\cdot k' + k'$ many. To be symmetric about it, we might also add the ``original'' ones, amounting to an additional $k'$ colors. Hence $k\cdot k' + k' + k$ does the job as $k_{\exists}$. For better presentability one upper bound would also be $(k+1)\cdot (k'+1)$. Another conservative estimate leaves us at $k_{\exists} = 3\cdot k\cdot k'$.}
\end{proof}

\subsection{From $\se$ to $\so$}

In this section, we show that $(\so, \prcoloringe) \in \mathfrak{L}_{\ke}$, from which we may conclude \cref{lem:binary-reformulated}, and thus, \cref{thm:binary}. More specifically, we show that $(\so, \prcoloringe)$ can be constructed by making use of $(\se, \prcoloringe) \in \mathfrak{L}_{\ke}$ and the $\mathrm{add}_{R, \vl}$ operations. This goal is achieved by introducing the datalog atoms obtained by applying the rules from $\rulesetnorm$ to $\se$. We focus on the case where we consider binary atoms, as the unary case is analogous.

%All we need to do is to introduce to $(\se, \coloringe)$ the datalog atoms derivable by $\rulesetnorm$ in $\se$. We will show this for binary atoms, as the unary case is analogous.

Let $\rho \in \rulesetnorm$ and suppose that $\head(\rho) = R(x,y)$, i.e. the head of $\rho$ is a binary atom. We may assume w.l.o.g. that $\rho$ is of the following form:
%
$$
\rho = \phi_{1}(\vx, x) \land \phi_{2}(\vy, y) \land \phi_{3}(\vz) \to R(x, y)
$$
%
where $\phi_{1}(\vx, x)$ and $\phi_{2}(\vy, y)$ denote the maximal connected components in $\body(\rho)$ containing all occurrences of $x$ and $y$ respectively, and with $\psi(\vz)$ denoting the remaining conjunction of atoms in $\body(\rho)$. We now define the following two sets of colors, which are both assumed to be subsets of $\adom{\se} \times \adom{\se}$:
\begin{flushleft}
$(t,t') \in \cols_{\coloring}$ \ifandonlyif $\ball{\diam}{t} \models \phi_{1}(\vx, t)$, $\ball{\diam}{t'} \models \phi_{2}(\vy, t')$, and $\se \models \phi_{3}(\vz)$;
\end{flushleft}
\begin{flushleft}
$(t,t') \in \cols_{\rho}$ \ifandonlyif $\se \models \phi_{1}(\vx, t) \land \phi_{2}(\vy, t') \land \phi_{3}(\vz)$.
\end{flushleft}
%$$
%\begin{array}{rcl}
%   \cols_\coloring & = & \set{\;(t,t') \in dom(\se)^2 \;|\; \ball{\diam}{t} \models \phi(\vx, t) \;\wedge\\
%    & &  \hspace{3.43cm} \ball{\diam}{t'} \models \phi'(\vx', t') \;\wedge\\
%    & &  \hspace{3.43cm}\se \models \psi(\vz)\;}.\\
%   \cols_\rho & = &  \set{(t,t') \in dom(\se)^2 |\se \models \phi(\vx, t), \phi'(\vx', t'), \psi(\vz)}.
%\end{array}
%$$
%
Both sets $\cols_\coloring$ and $\cols_\rho$ contain pairs of terms $(t,t')$ such that $R(t,t')$ results from applying $\rho$ to $\se$. %The set $\cols_\coloring$ is a subset of $A_\rho$ that contains the pair $(t, t')$ if it can be derived using only a small neighbourhood around $t$ and $t'$ and some general information on $\se$. As it turns out:
 By making use of \cref{def:diameter}, it is straightforward to establish that both sets coincide:

\begin{observation}\label{obs:binary-unary-case-ball}
$\cols_\coloring = \cols_\rho$.
\end{observation}
\begin{proof}
As the inclusion $\cols_\rho \subseteq \cols_\coloring$ follows directly from the definition of each set, we focus on showing the converse, i.e. that $\cols_{\coloring} \subseteq \cols_\rho$. If we assume that $(t,t') \in \cols_{\coloring}$, then we have that $\se \models \phi_{1}(\vx, t) \land \phi_{2}(\vy, t') \land \phi_{3}(\vz)$. By \cref{def:diameter}, we know that $\diam$ is {\em twice the maximal diameter of any connected component in any rule body of $\rulesetnorm$}, which ensures that $\ball{\diam}{t}$ and $\ball{\diam}{t'}$ are sufficiently large enough so that $\ball{\diam}{t} \models \phi_{1}(\vx, t)$ and $\ball{\diam}{t'} \models \phi_{2}(\vy, t')$ (since by our assumption we know that $\se \models \phi_{1}(\vx, t)$ and $\se \models \phi_{2}(\vy, t')$). Since $\se \models \phi_{3}(\vz)$ directly follows from our assumption, we have that $(t,t') \in \cols_{\rho}$, which proves the claim.
\end{proof}

Let us now define the following set, which will be used in the subsequent observation: 
$$
B_\coloring = \set{(\bball{\diam}{t}, \bball{\diam}{t'}) \;|\; (t,t') \in \cols_\coloring}.
$$

\begin{observation}
For each $(l,l') \in B_\coloring$, $\mathrm{add}_{R,(l,l')}(\se, \prcoloringe) = (\se \cup \set{R(t,t') \;|\; (t,t') \in \cols_{\rho}},\; \prcoloringe) \in \mathfrak{L}_{\ke}$.
\end{observation}

\begin{proof} Suppose that $(l,l') \in B_\coloring$. Then, we know that $R(t,t')$ is a fresh atom in $\mathrm{add}_{R,(l,l')}(\se, \prcoloringe)$ \ifandonlyif $\prcoloringe(t) = \bball{\diam}{t} = l$ and $\prcoloringe(t') = \bball{\diam}{t'} = l'$ \ifandonlyif $(t,t') \in \cols_{\coloring}$ (by the definition of $B_\coloring$ above) \ifandonlyif $(t,t') \in \cols_{\rho}$ (by \cref{obs:binary-unary-case-ball} above), thus proving the claim.
\end{proof}

%\begin{proof}
%Follows from \cref{obs:binary-unary-case-ball} and the fact that $\prcoloringe(t) = \bball{\diam}{t}$.
%\end{proof}

Proceeding similarly for the other rules of $\rulesetnorm$, we obtain the following: 
%
$$
(\se \cup \bigcup_{\rho \in \rulesetnorm} \set{R(t,t') \;|\; (t,t') \in \cols_\rho},\;\; \prcoloringe) \in \mathfrak{L}_{\ke}
$$ 
%
Observe that the first component is equal to $\so$. Hence, we may conclude \cref{lem:binary-reformulated}, which entails \cref{thm:binary}.

==> ICDT 2023 Updated LaTeXFiles/other/boring-comments.tex <==
\piotr{\begin{itemize}
    \item capital Latin letters for predicates
    \item $a,b,c$ for constants
    \item $x,y,z$ for variables
    \item $t,u,v,w$ for terms/nodes/nulls/vertices be careful with instances having constants
    \item $h$ for homomorphisms
    \item $f$ for general functions
    \item mathcal capital Latin $\mathcal{I}$ for instances
    \item mathcal D for databases (only constants allowed) $\mathcal{D}$
    \item $\phi, \psi$ - body and head of ex-rule
    \item $\rho$ for ex-rule
    \item $\alpha, \beta, \gamma$ for atoms of instances and databases
\end{itemize}}

\piotr{\begin{itemize}
    \item We should consider only Boolean queries with constants, as this will make everything easier to process and should not make our results weaker.
\end{itemize}}

\piotr{\begin{itemize}
    \item Instance is a set of Atoms build from terms from constants + nulls over a signature
    \item Database uses only constants
\end{itemize}}

\tim{
\begin{itemize}
    \item Let's us "cliquewidth" as opposed to "clique-width", since it seems (looking through a few papers here) that "treewidth" is usually used rather than "tree-width" (thus, things are kept analogically consistent).
    \item Also, for all classes of existential rules, we should use macros that write the name of the class (an abbreviation) in lower case bold letters; e.g. $\fus$, $\bcws$, etc.
\end{itemize}}

\thomas{\begin{itemize}
    \item Naming convention for our bcs: ``semantic bcs''?
    \item FES vs. $\fes$ resolved in favor of the latter (as is actually the FUS vs. $\fus$ one); use the command
    \item Maybe every equation in a proper equation-environment?
    \item subinstance vs. sub-instance \piotr{I vote for the latter.}
    \item for induced sub<smth>: Should we denote such a relation via $\le$ (to also contrast with $\subseteq$)?
\end{itemize}}

\tim{\begin{itemize}
    \item $A, B, C$ for sets of atoms (make a note that the context will determine when predicates are being used or sets, i.e. allow for ambiguity because easy to differentiate)
    \item We used both $l$ and $i, j$ to denote colors, though in the binary section I have started using $l$ with annotations (e.g. primes, subscripts, etc.). Perhaps we should stick to using this for colors?
    \item Use "rule set" to describe a set of ERs as opposed to "set of existential rules" or "set of ERs" to (i) maintain consistency, and (ii) because it is short and saves space.
    \item We use the abbreviation "ER" now instead of "existential rule" as it saves space.
\end{itemize}}

==> ICDT 2023 Updated LaTeXFiles/other/cor_skeleton-plus-has-bounded-cw.tex <==
%\subsection{Proof of \cref{cor:skeleton-plus-has-bounded-cw}}\label{sec:cor:skeleton-plus-has-bounded-cw}
\piotr{Proofread this, low priority.}

 %Let $\inst$ be a finite instance, then with its {\em diameter} we will define a following natural number $\max_{t,t' \in \inst}(\ldist{\inst}{t,t'})$.

\begin{customlem}{\ref{cor:skeleton-plus-has-bounded-cw}}
$\ksat{1}{\rulesetnormcon, \se}$ has bounded treewidth.
\end{customlem}
\begin{proof}
Given an instance $\inst$ and two its terms $t, t'$ define the {\em distance} $\ldist{\inst}{t,t'}$ from $t$ to $t'$ in $\inst$ as the minimal length of any path from $t$ to $t'$ treating binary atoms of $\inst$ as undirected edges. Also, let $\db$ denote database fixed in \cref{sec:binary}.

For a null $t$ of $\se$ and a natural number $n$ let {\em neighbourhood} $\neigh{n}{t}$ of $t$ of distance $n$ be a following set of terms $\set{t \in \termset(\se) \;|\; \ldist{\se}{t, t'} \leq n}$. Also let $\neigh{n}{\db} = \set{t \;|\; \exists{c\in\adom{\db}}\;\ldist{\se}{t,c} < n}$

Let $T_n = {V_n, E_n}$ be a following tree decomposition:
\begin{itemize}
    \item $V_n = \set{\neigh{n}{t} \;|\; t \in \nullset(\se) } \cup \set{r}$, where $r = \termset(\db)$.
    \item $E_n = \set{(\neigh{n}{t}, \neigh{n}{t'}) \;|\;  \wedge\exists{R\in\sig}\; \se \models R(t,t') \vee R(t', t)} \;\cup\;\\ \set{(r, \neigh{n}{t}) \;|\;  \exists{c \in \conset(\db)}\; \exists{R\in\sig} \se \models R(t,t') \vee R(t', t)}$.
\end{itemize}

Now we will argue that for every $n > 1$ tree $T_n$ is a tree decomposition of $\se$ as:
\begin{itemize}
    \item $\bigcup_{v\in V_n}v$ is equal to $\termset(\se)$.
    \item Each atom $R(t,t')$ of $\se$ is indeed contained in one of bags of $V_n$, namely $\neigh{n}{t}$, as $n > 1$.
    \item From the definition of neighbourhood, one can note that for each term $t$ in $\se$, the sub-graph of $T_n$ induced by the nodes $v$ of $V$ such that $t \in v$ is connected. 
\end{itemize}

Recall from \cref{obs:sate-is-forest} that $\se$ has a bounded degree. Thus observe that for every $n\in\mathbb{N}$ there exists $k \in \mathbb{N}$ such that for every term $t$ of $\se$ we have $|\neigh{n}{t}| < k$. Thus width of $T_n$ is bounded.

Let $d \in \mathbb{N}$ be such that for every rule $\rho \in \rulesetnormcon$, and its frontier variables $x,y$, the following holds $d \geq \ldist{\body(\rho)}{x,y}$. Note that such a $d$ exists because $x$ and $y$ share the same connected component of $\body(\rho)$. Finally, observe that for every atom $R(t,t')$ of $\ksat{1}{\rulesetnormcon, \se} \setminus \se$ we have that $t,t' \in \neigh{d}{t}$ or $t,t' \in \neigh{d}{\db}$. From this we conclude that $T_d$ is a tree decomposition of $\ksat{1}{\rulesetnormcon, \se}$ of bounded width.

\end{proof}

==> ICDT 2023 Updated LaTeXFiles/other/fes-and-tbs.tex <==
\section{Finite Unification Sets and Bounded Treewidth Sets}

\begin{definition}[Finite Expansion Set ($\fes$)] A set of existential rules $\calr$ is called a \emph{finite expansion set ($\fes$)} \ifandonlyif for every fact $F$, there exists an integer $k$ such that $F_{k} = \ksat{k}{F,\calr} \equiv \ksat{k+1}{F,\calr} = F_{k+1}$. We refer to $F_{k}$ as a \emph{full derivation} of $F$.
\end{definition}

\piotr{Word theorem should be reserved only to our results.}
\begin{theorem}
If $\calr$ is a $\fes$, then it is BCQ entailment is decidable. 
\end{theorem}

\begin{proof}
See~\cite[\prp~5]{BagLecMugSal11}.
\end{proof}


\thomas{In the preliminaries we define ``fact'' to mean a atomic sentence (i.e. a grounded atom). In the following definition(s!) we use the notion of ``fact'' that is a collection of atomic formulae. There is a clash here that needs to be discussed.}
\piotr{sure, we still need to rewrite this section to fit the rest of the paper.}


==> ICDT 2023 Updated LaTeXFiles/other/fo-rewritability.tex <==
\medskip \noindent {\bf Rewritings and finite unification sets.}
Given a rule set $\ruleset$ and a CQ $\phi(\vx)$ we say that a UCQ $\psi(\vx)$ is a {\em rewriting} of $\phi(\vx)$ under the rule set $\ruleset$ \ifandonlyif for any database $\database$ and any tuple of its elements $\va$ the following holds:
%
$$\sat{\database,\ruleset} \models \phi(\va) \ \ifandonlyif \ \database \models \psi(\va).$$
%
a rule set $\ruleset$ is a {\em finite unification set} ($\fus$) \iffi for every query there exists a UCQ rewriting \cite{BagLecMugSal11}. This property is also referred to as \emph{first-order rewritability}.
%
If a rule set $\ruleset$ is $\fus$, then for any given CQ $\phi(\vx)$ we denote its rewriting under $\ruleset$ with $\rewrs{\ruleset}{\phi(\vx)}$.




==> ICDT 2023 Updated LaTeXFiles/other/main-results.tex <==
\section{Main contributions}\label{sect:main-results}
\piotr{Should we merge this section with the introduction?}

Given a rule set $\ruleset$ and a CQ $\phi(\vy)$ we say that a UCQ $\psi(\vy)$ is a {\em rewriting} of $\phi(\vy)$ under the rule set $\ruleset$ \ifandonlyif for any database $\database$ and any tuple of its elements $\va$ the following holds:
%
$$\sat{\ruleset, \database} \models \phi(\va) \ \ifandonlyif \ \database \models \psi(\va).$$
 
Following~\cite{BagLecMugSal11}, we say that a rule set $\ruleset$ has the {\em finite unification set property} (is $\fus$) if for every query there exists a UCQ rewriting. If a rule set $\ruleset$ is $\fus$, then for any given CQ $\phi(\vx)$ we denote its rewriting under $\ruleset$ with $\rewrs{\ruleset}{\phi(\vx)}$.

And so in the case of binary signatures the bounded cliquewidth sets contain FO-rewritable sets:

\begin{theorem}\label{thm:binary}
\tim{
Any FO-rewritable set of single-headed existential rules over a binary signature is a bounded-cliquewidth set.
}
\end{theorem}


Surprisingly this is not the case generally. This constitutes our second main contribution:

\begin{theorem}\label{thm:higher-arity}
There exists a FO-rewritable set of existential rules that is not bounded-cliquewidth set.
\end{theorem}

==> ICDT 2023 Updated LaTeXFiles/other/obs_cross-coloring.tex <==

\begin{customobs}{\ref{obs:cross-coloring}}
Let $\inst$ be a finite instance. Moreover, let $\coloring : \adom{\inst} \to \{1, \ldots, k\}$ and $\coloring' : \adom{\inst} \to \{1, \ldots, k'\}$ be two colorings with $(\coloring \times \coloring')(t) = (\coloring(t), \coloring'(t))$, for each $t \in \adom{\inst}$. If $\cw{\inst, \coloring} = k$, then $\cw{\inst, \coloring \times \coloring'} = k \cdot k'$.
\end{customobs}

\begin{proof}
Since $\ruleset$ is a set of single-headed rules over a binary signature, and since we only consider non-datalog rules (as $\se \setminus \database$ only contains atoms derived by the non-datalog rules from $\ruleset$), we know that each rule $\rho$ applied during the Skolem chase is of the form $\phi(\vec{x},y) \rightarrow head(\rho)$ with $head(\rho) \in \{\exists z R(y,z), \exists z R(z,y), \exists z \exists z' R(z,z')\}$. That is to say, for each rule $\rho$, $\fr(\rho) = 1$ or $\fr(\rho) = 0$. Observe that if a rule of frontier $1$ is applied during the Skolem chase, then it gives rise to a single edge (typed with the predicate $R$ occurring in the head of the rule) in %$\struc^{\inst}$
 $\se \setminus \database$ that can either be directed toward (if $\head(\rho) = \exists z R(y,z)$) or away from (if $\head(\rho) = \exists \vec{z} R(z,y)$) the frontier term it is attached to. If a rule of frontier $0$ is applied during the Skolem chase, then it creates a disconnected typed edge that corresponds to, and gives rise to, a new typed polytree in %$\struc^{\inst}$. 
 $\se \setminus \database$. Hence, we can see that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest. Moreover, as we are using the Skolem chase and due to the fact that $\ruleset$ is finite, there can only be a finite number of typed edges added to each vertex in the typed polyforest, ensuring that it is of bounded degree.
\end{proof}

\thomas{Proof with new definition}
\begin{proof}
  Let $(\inst, \coloring)$ be a colored instance and $\coloring'\colon\adom{\inst}\to \{ 1, \ldots, k' \}$ another coloring for $\inst$. Furthermore, let $\cw{\inst, \lambda} = k$. Then there exists for a finite set of colors $\cols = \{ 1, \ldots, k \}$ a well $(\cols, Cnst, \Sigma)$-decorated tree $\mathcal{T}$ such that $\inst^{\mathcal{T}}=\inst$ and $\mathit{col}^\mathcal{T} = \coloring$.
  For $\cols' = \{1, \ldots, k \} \times \{ 1, \ldots, k'\}$ we obtain a $(\cols', Cnst, \Sigma)$-decorated tree $\mathcal{T}'$ inductively over the nodes of $\mathcal{T}$ and $\mathcal{T}'$ in the following way:
  
  \textit{Transformations.} Let $s, s'\in \{ 0,1 \}^{\ast}$ and $N_{p} \subseteq (\{ 0,1 \}^{\ast})^{2}$.% We define $\mathcal{T}_{s}$ to be the subtree of $\mathcal{T}$ issued from $s$.
    \begin{enumerate}
        \item\label{item: Transformation1} If $\oplus(s)\in \mathcal{T}_{s}$, then $\oplus(s') \in \mathcal{T}^{s}$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation2} If for $c\in Cnst \cup \{ \ast \}$ and $l\in\cols$ $c_{l}(s)\in \mathcal{T}$, then $c_{(l, \lambda'(s))}(s')\in \mathcal{T}^{s}$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation3} If $\mathrm{Void}(s)\in \mathcal{T}_{s}$, then add $\mathrm{Void}(s')$ to $\mathcal{T}'$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation4} If for $R\in\Sigma_1$ and $l\in\cols$ $\mathrm{Add}_{R, l}(s)\in\mathcal{T}_{s}$, then add %\[ \{ \mathrm{Add}_{R, (l, i)}(0^{i-1}), \mathrm{Void}_(0^{j-1}1) \, | \, 1\le i, j \le k'\} \]
        \[ \{ \mathrm{Add}_{R, (l, i)}(0^{i-1}) \, | \, 1\le i, j \le k'\} \]to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i\le k'$ the pairs $(s0, s'0^{i})$ and $(s1, s'0^{i-1}1)$.% and set $s_0 = s0$ and $s'_0 = s'0^{k'}$.
        \item\label{item: Transformation5} If for $R\in\Sigma_2$ and $l_1, l_2\in\cols$ $\mathrm{Add}_{R, l_1, l_2}(s)\in\mathcal{T}_s$, then add %\[ \{ \mathrm{Add}_{R, (l_1, i), (l_2, j)}(0^{i-1 + (j-1)\cdot k'}), \mathrm{Void}(0^{i-1 + (j-1)\cdot k'}1) \, | \, 1\le i, j \le k' \} \]
        \[ \{ \mathrm{Add}_{R, (l_1, i), (l_2, j)}(0^{i-1 + (j-1)\cdot k'}) \, | \, 1\le i, j \le k' \} \] to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i, j\le k'$ the pairs $(s0, s'0^{i + (j-1)\cdot k'})$ and $(s1, s'0^{i-1 + (j-1)\cdot k'}1)$.% set $s_0 = s0$ and $s'_0 = s'0^{k'\cdot k'}$.
        \item\label{item: Transformation6} If for $l_1, l_2\in\cols$ $\mathrm{Recolor}_{l_1 \to l_2}(s)\in\mathcal{T}_{s}$, then add %\[ \{ \mathrm{Recolor}_{(l_1, i) \to (l_2, j)}(0^{i-1 + (j-1)\cdot k'}), \mathrm{Void}(0^{i-1 + (j-1)\cdot k'}1) \, | \, 1\le i,j \le k' \} \]
        \[ \{ \mathrm{Recolor}_{(l_1, i) \to (l_2, j)}(0^{i-1 + (j-1)\cdot k'}) \, | \, 1\le i, j \le k' \} \] to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i, j\le k'$ the pairs $(s0, s'0^{i + (j-1)\cdot k'})$ and $(s1, s'0^{i-1 + (j-1)\cdot k'}1)$.% set $s_0 = s0$ and $s'_0 = s'0^{k'\cdot k'}$.
    \end{enumerate}
  
  \textit{Base case.} Initialize $N_{p} = \{ (\varepsilon, \varepsilon) \}$. Then apply the appropriate transformation for the tuple $(\varepsilon, \varepsilon)$.% $\mathcal{T}_{\epsilon} = \mathcal{T}$ and add the pair(s) $(s_0, s'_0)$ (and $(s_1, s'_1)$) if obtained from the transformation) to the set $N_p$.
    
  \textit{Induction Step.} Suppose $N_p$ already contains more than $(\varepsilon, \varepsilon)$. With $\prec$ we denote the usual prefix order on $\{ 0,1 \}^{\ast}$. We define a partial order on $N_p$ in the following way: \[ (s_1, s_1') < (s_2, s_2') \quad \text{\ifandonlyif} \quad s_1 \prec s_2 \text{ or } s_1 = s_2 \land s_1' \prec s_2' \, . \] Take the tuple $(s,s')\in N_p$ such that $(s,s')$ is a $|s'|$-minimal $<$-maximal element in $N_p$. Then apply the appropriate transformation to $(s,s')$.
  
  Finally, obtain $\mathcal{T}' = \mathcal{T}_{bin}\cup \bigcup_{s\in\mathcal{T}_{bin}}\mathcal{T}^{s}$.
  
  \thomas{\textit{TODO: Properties of $N_p$.}}
    \begin{enumerate}
        \item\label{item: N_property1} If $(s, s')\in N_p$ with $c\in Cnst \cup \{ \ast \}$ and $c_l(s)\in\mathcal{T}$ for some $l\in \cols$, then $c_{(l, \lambda'(s))}(s')\in \mathcal{T}'$ and $s'$ is the unique $s''\in \{ 0, 1\}^{\ast}$ such that $(s,s'')\in N_p$.
            \begin{subproof}
                Let $s\in \{ 0,1 \}^{\ast}$ and for some $l\in \cols$ and $c\in Cnst$ it holds that $c_l(s)\in \mathcal{T}$. Furthermore, suppose that $s', s''\in \{ 0,1 \}^{\ast}$ such that $(s, s'), (s,s'')\in N_p$ with $c_{(l, \lambda'(s))}(s'), c_{(l, \lambda'(s))}(s'')\in \mathcal{T}^{s}$. This can only happen, if there was previously a transformation applied for $r, s''' \in \{ 0,1 \}^{\ast}$ to $(r, s''')\in N_p$ with $\mathrm{Succ}_0(r, s)\in \mathcal{T}$ and $s''' \prec s', s''$ such that either
                \begin{enumerate}
                    \item\label{item: N_property1_a} for $R\in\Sigma_1$ and $m\in\cols$ $\mathrm{Add}_{R, m}(r)\in\mathcal{T}$, or
                    \item\label{item: N_property1_b} for $R\in\Sigma_2$ and $m_1, m_2\in\cols$ $\mathrm{Add}_{R, m_1, m_2}(r)\in\mathcal{T}$, or
                    \item\label{item: N_property1_c} for $m_1, m_2\in\cols$ $\mathrm{Recolor}_{m_1 \to m_2}(r)\in\mathcal{T}$.
                \end{enumerate}
                But then w.l.o.g. (in case \ref{item: N_property1_a}) $s' = s'''0^{i}$ and $s'' = s'''0^{j}$ with $1\le i < j, \le k'$ or (in cases \ref{item: N_property1_b} and \ref{item: N_property1_c}) $s' = s'''0^{i}$ and $s'' = s'''0^{j}$ with $1\le i < j, \le k'\cdot k'$. But then, by the Inductions Step, Transformation \ref{item: Transformation2} is only applied to the tuple $(s, s'''0^{k'})$ (in case \ref{item: N_property1_a}) or $(s, s'''0^{k'\cdot k'})$ (in cases \ref{item: N_property1_b} and \ref{item: N_property1_c}) as this is $<$-maximal for the introduced $N_p$-pairs. Hence $s'''0^{k'\cdot k'} = s' = s''$, showing uniqueness. Furthermore, by Transformation \ref{item: Transformation2} we obtain $c_{(l, \lambda'(s))}(s'), c_{(l, \lambda'(s))}(s'')\in \mathcal{T}^{s}$.
            \end{subproof}
        \item\label{item: N_property2} If $(s, s')\in N_p$ with $\mathrm{Void}(s)\in\mathcal{T}$, then $\mathrm{Void}(s')\in \mathcal{T}'$ and for all $s''\in\{ 0,1 \}^{\ast}$ with $s' \prec s''$ we have $\mathrm{Void}(s'')$.
            \begin{subproof}
                If $(s, s')\in N_p$, application of Transformation \ref{item: Transformation3} yields $\mathrm{Void}(s')\in \mathcal{T}'$. As then $(s0, s'0), (s1, s'1)$ are added to $N_p$, applications of Transformation \ref{item: Transformation3} to both will yield $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\in \mathcal{T}'$. Inductively we obtain for all $s''\in\{ 0,1 \}^{\ast}$ with $s' \prec s''$ we have $\mathrm{Void}(s'')$.
            \end{subproof}
    \end{enumerate}
  
  \thomas{\textit{TODO: Proof}} $\mathcal{T}'$ is a well $(\cols', Cnst, \Sigma)$-decorated tree.
    \begin{itemize}
        \item For every $s\in \{ 0,1 \}^{\ast}$, $Dec(s)\in\mathcal{T}'(s)$ for exactly one $Dec \in Dec(\cols', Cnst, \Sigma)$ by constructions.
        \item Since, by construction, if for $c\in Cnst$, $(l_1, l_2)\in \cols'$ and $s'\in\{ 0,1 \}^{\ast}$ it holds that $c_{(l_1, l_2)}(s')\in\mathcal{T}'$, then there is a $s\in\{ 0,1 \}^{\ast}$ such that $c_{l_1}(s')\in\mathcal{T}$ and $(s, s')\in N_p$. By Property \ref{item: N_property1} $s'$ is unique for $s$. On the other hand, Transformation \ref{item: Transformation2} is only executed, if there is a pair $(s, s')\in N_p$ with $c_{l_1}(s')\in\mathcal{T}$. In conclusion, for every $s'\in \{ 0,1 \}^{\ast}$, $c\in Cnst$, and $l\in\cols'$ there is at most one fact of the form $c_{l}(s')\in\mathcal{T}'$.
        \item If $\mathrm{Void}(s')\in\mathcal{T}'$ or $c_{(l_1, l_2)}(s')\in \mathcal{T}'$, then $\mathrm{Void}(s'0), \mathrm{Void}(s'1)$. In the case of $\mathrm{Void}(s')\in \mathcal{T}'$ this follow immediately from Property \ref{item: N_property2}. If on the other hand $c_{(l_1, l_2)}(s')\in \mathcal{T}'$ we observe that there exists by construction exactly one $s\in\{0,1 \}^{\ast}$ such that $c_{l_1}(s)\in\mathcal{T}$ and $(s, s')\in N_p$. Note that $c_{(l_1, l_2)}(s')$ was then produced by application of Transformation \ref{item: Transformation2} and $(s0, s'0), (s1, s1')$ will have been added to $N_p$. Application of Transformation \ref{item: Transformation3} then has yielded $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\in \mathcal{T}'$ as $\mathrm{Void}(s0), \mathrm{Void}(s1)\in\mathcal{T}$.
        \item If $\oplus(s')\in\mathcal{T}$ then $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\not\in \mathcal{T}'$ follows by construction.
        \item If for $l, l'\in\cols'$ we have $\mathrm{Recolor}_{l\to l'}(s') \in \mathcal{T}'$ or $\mathrm{Add}_{R,l,l'}(s') \in \mathcal{T}'$ or $\mathrm{Add}_{R,l}(s') \in \mathcal{T}'$ then by definition of Transformations \ref{item: Transformation4} - \ref{item: Transformation6} $\mathrm{Void}(s'0)\not\in \mathcal{T}'$ and $\mathrm{Void}(s'1) \in \mathcal{T}'$ hold by construction.
    \end{itemize}
  
  \thomas{\textit{TODO: Proof}} $\mathcal{I}^{\mathcal{T}'} \cong \mathcal{I}^{\mathcal{T}}$ and $\mathrm{col}_{\epsilon}^{\mathcal{T}'} = \coloring \times \coloring'$.
  Obtaining the isomorphism works as follows: By Property \ref{item: N_property1} for every $(s,s')\in N_p$ such that for some $c\in Cnst\cup\{ \ast \}$ and $l\in \cols$ it holds that $c_{l}(s)\in\mathcal{T}$, $s'$ is unique.
  
  --- WORK IN PROGRESS ---
\end{proof}

==> ICDT 2023 Updated LaTeXFiles/other/obs_sate-is-forest.tex <==
%\subsection{Proof of \cref{obs:sate-is-forest}}\label{sec:obs:sate-is-forest}
\begin{customobs}{\ref{obs:sate-is-forest}}
$\se \setminus \database$ is a typed polyforest of bounded degree.
\end{customobs}

\begin{proof}
Since $\ruleset$ is a set of single-headed rules over a binary signature, and since we only consider non-datalog rules (as $\se \setminus \database$ only contains atoms derived by the non-datalog rules from $\ruleset$), we know that each rule $\rho$ applied during the Skolem chase is of the form $\phi(\vec{x},y) \rightarrow head(\rho)$ with $head(\rho) \in \{\exists z R(y,z), \exists z R(z,y), \exists z \exists z' R(z,z')\}$. That is to say, for each rule $\rho$, $\fr(\rho) = 1$ or $\fr(\rho) = 0$. Observe that if a rule of frontier $1$ is applied during the Skolem chase, then it gives rise to a single edge (typed with the predicate $R$ occurring in the head of the rule) in %$\struc^{\inst}$
 $\se \setminus \database$ that can either be directed toward (if $\head(\rho) = \exists z R(y,z)$) or away from (if $\head(\rho) = \exists \vec{z} R(z,y)$) the frontier term it is attached to. If a rule of frontier $0$ is applied during the Skolem chase, then it creates a disconnected typed edge that corresponds to, and gives rise to, a new typed polytree in %$\struc^{\inst}$. 
 $\se \setminus \database$. Hence, we can see that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest. Moreover, as we are using the Skolem chase and due to the fact that $\ruleset$ is finite, there can only be a finite number of typed edges added to each vertex in the typed polyforest, ensuring that it is of bounded degree.
\end{proof}

==> ICDT 2023 Updated LaTeXFiles/other/old-clique-width.tex <==

\section{Clique-width and Related Notions}\label{sec:cliquewidth}

\piotr{\begin{itemize}
    \item Discuss clique-width with examples
    \item Introduce bounded clique-width sets
    \item Discuss its importance
    \item Push observations and lemmata which do not contribute to the story to the separate subsection
\end{itemize}}


\medskip \noindent {\bf Cliquewidth.}
We define the notion of clique-width following the formalization provided in \cite[\dfn~15]{GroheT04}.
For a standard definition of a clique-width for graphs one can refer (for example) to \cite[\dfn~2.89]{CourEngBook}.

A {\em structure} is a generalization of an instance that may contain isolated terms (terms that do not appear in any atom). To denote the set of terms of a structure $\struc$ we write $\aadom{\struc}$. Given a finite set of colors $\cols$ a {\em colored structure} is a pair $(\struc, \coloring)$ where $\struc$ is a structure and and $\coloring$ is a function from $\aadom{\struc} \to \cols$.

\tim{
I re-wrote the above paragraph (shown below) to make the definition of structure more explicit. If you find it to be to verbose, feel free to simplify it, or even remove it altogether if you find it unnecessary. I find having the explicit definition is helpful for the reader however as it ensures they have a clear understanding of the meaning of the object being discussed. Also, I've used this notation and terminology in re-writings of the binary section, though it can be amended/easily changed depedning on how we decide to move forward.
}

\tim{
A {\em $\sig$-structure} $\struc$ (which we refer to as a \emph{structure} more simply when the signature $\sig$ is clear from the context) is a pair $(\sdom,\srel)$, where $\sdom$ is a non-empty set of points, referred to as \emph{terms}, and $\srel$ is a family $\{R \ | \ R \in \sig\}$ of relations such that $R \subseteq \sdom^{\arity{R}}$. Observe that structures generalize the notion of an instance as they may contain isolated terms (terms that do not appear in any atom). Hence, every instance $\inst$ can be transformed into a corresponding structure $\struc^{\inst} = (\sdom^{\inst},\srel^{\inst})$, where $\sdom^{\inst} = \aadom{\inst}$, $\srel^{\inst}$ is the set of predicates occurring in $\inst$, and where for any $R \in \srel^{\inst}$, $\vt \in R$ \ifandonlyif $R(\vt) \in \inst$. For a given structure $\struc = (\sdom, \srel)$, we let $\aadom{\struc}$ denote the set of terms in a structure, that is, $\aadom{\struc} = \sdom$. Given a finite set of colors $\cols$ a {\em colored structure} is defined to be a pair $(\struc, \coloring)$ where $\struc$ is a structure and and $\coloring$ is a function from $\aadom{\struc} \to \cols$.
}

\tim{It might be good to note somewhere for the reader that the codomain of colorings is held constant throughout the following construction process.} 

Given a set $\cols$ of $k$ colors a {\em basic $k$-colored finite structure} is a single term or constant $t$ colored with any of colors in $\cols$. We define the set $\mathfrak{L}_k$ of colored finite structures as a minimal set containing basic $k$-colored and closed under following operations:

\begin{itemize}
    \item $\add{A,\vl}{\struc, \coloring}$ adds the following atoms to the colored finite structure $\set{A(\vt) \;|\; \vt \in \aadom{\struc}^{\arity{A}} \wedge \coloring(\vt) = \vl}$, where $A \in \sig$ and \tim{$\vl \in \cols^{\arity{A}}$}.
    \item $\recol{i\to j}{\struc, \coloring}$ recolors $i$-colored terms of $(\struc, \coloring)$ to color~$j$.
    \item $\disun$ takes a disjoint union of the colored finite structures. \thomas{$i, j\in \cols$}
\end{itemize}

\begin{definition}[Clique-width]\label{def:cw}
Given a finite instance $\inst$ we define the {\em clique-width} $\cw{\inst}$ as the smallest $k$ such that there exists a coloring $\coloring$ such that $(\inst, \coloring)$ is in $\mathfrak{L}_k$. \\
\thomas{Given an infinite instance $\inst$ we define its {\em clique-width} $\cw{\inst}$ as the supremum over the clique-widths of all finite induced substructures of $\inst$.}
\end{definition}

\thomas{In the case of finite structures our notion of clique-width coincides with the one from \cite{GroheT04}. The infinite case though diverges from the literature in general as clique-width definitions are usually intricately linked with the terms representing the structures. Those terms lend itself to be extended to infinite ones. Unfortunately this usually does not allow for ``nice'' compactness behavior akin to ``for an infinite structure $\struc{}$ it holds that if every finite induced substructure has clique-width of at most $n$, then so does the structures $\struc{}$ itself''. For more details we refer the reader to e.g. \cite{Cou04}. Luckily, as the cited work shows, boundedness of clique-width does admit a compactness property, i.e. it is true that ``for an infinite structure $\struc{}$ it holds that if there is a {\em uniform} bound $n$ on the clique-width of all finite induced substructures of $\struc{}$ then the clique-width of $\struc{}$ itself is bounded by a number $f(n)$'' where $f$ is a function $\mathbb{N}\to\mathbb{N}$ that is not the identity. TODO, maybe in an observation?}
Now we need to extend our definition to the instances in general not only finite instances.
\piotr{TODO}

\tim{Note: As per our discussion we need to generalize the following to typed polytrees (https://en.wikipedia.org/wiki/Polytree) and also I think we should discuss forests of typed polytrees to make the observation correspond directly to Corollary 8.
}

\begin{observation}\label{obs:trees_cw_le3}
Let $\struc$ be a oriented forest over a finite binary signature\footnote{\thomas{Or should we call this ``edgecolors''? Call it ``edge-colored oriented...'' or something like that?}} $\Sigma$. Then $\cw{\struc} \le 2 \cdot |\Sigma| + 2$.
\end{observation}
\begin{proof}
\thomas{proof sketch for poly forest.} First note that in the case of an infinite oriented forest, every induced finite substructure is an oriented forest as well. Thanks to our definition of clique-width it is thus enough to analyze only the construction of those finite oriented forests. Furthermore, since finite oriented forests are finite, they are the disjoint union of finitely many finite oriented trees. Hence we can concentrate only on finite oriented trees at first. In the construction process, each of those oriented trees will be constructed seperately and in a final step we successively and disjointly unify them. \\
Given a finite oriented tree of a finite binary signature. Then we will define the following set of colors: $\cols{} = \{ E^{+}, E^{-} \, | \, E \in \Sigma \}\cup \{ \texttt{D}, \texttt{R} \}$. Then we construct the oriented tree in the following way:
\begin{enumerate}
    \item leafs will be introduced as the basic structures colored by in the following way: If there is an $E\in\Sigma$-edge ending/starting in the leaf, we will color it by the color $E^{+}$ or $E^{-}$ respectively. Else we will color it with $\texttt{D}$.
    \item If two subtrees of are joined at a node and both subtrees are already constructed, we do the following: We disjointly unify the subtrees. The resulting forest will be disjointly unified with a new basic structure colored with $\texttt{R}$. Then we apply succesively, until we cannot do it any further, the following:
    For each $E \in \Sigma$ such that there is a node of color $E^{+}$ or $E^{-}$:
    \begin{enumerate}
        \item apply the operation $\add{E, (E^{-}, \texttt{R})}{}$ or $\add{E, (\texttt{R}, E^{+})}{}$ depending whether there is a node colored $E^{+}$ or $E^{-}$. If both are the case, apply those operations succesively;
        \item then recolor all nodes of color $E^{+}$ and of color $E^{-}$ to $\texttt{D}$;
        \item and finally recolor all nodes of color $\texttt{R}$ corresponding to whether there is an $F\in\Sigma$-edge incoming (color with $F^{+}$) or outgoing (color with $F^{-}$).
    \end{enumerate}
\end{enumerate}
This process will terminate after finitely many steps, which is easy to see: If a node is not of color $\texttt{D}$, then it is either a leaf node freshly introduced (that has in the oriented tree we want to construct some incoming or outgoing edge), or a root node of an already constructed oriented subtree , or it is a node acting as a ``new root'', merging already constructed oriented subtrees to a bigger oriented subtree. Since we only discuss finite oriented trees, we can only add finitely many leaf nodes or merge finitely many oriented subtrees until we obtain the whole oriented tree we wish to construct.

\end{proof}



==> ICDT 2023 Updated LaTeXFiles/other/old-higher.tex <==
\section{Results for Higher Arity Signatures}
%Tim: I moved the commands that were here to the MISC section of the "notation" file.

We dedicate this section to the proof of \cref{thm:higher-arity}, i.e. we show that even if we utilize a binary signature, then permitting the use of non-single-headed rules in a given finite unification set can unbound the clique-width of an associated universal model. We let $\sigi = \set{\hpred, \vpred, \origin}$ be a signature where $\hpred$ and $\vpred$ are binary predicates and $\origin$ is a unary predicate. Let us define $\rsgrid$ to be the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} & \top & \rightarrow \exists x \; (\hpred(x,x) \land \vpred (x,x)) \\[0.5ex]
\text{(grow)} & \top & \rightarrow \exists y \exists y'\; (\hpred(x,y) \land \vpred (x,y')) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists y' \; (\hpred(x',y') \land \vpred(y,y'))
\end{array}
$$

\piotr{Discuss the multi-head higher arity here if necessary, it could be done earlier as well.}

We make use of $\rsgrid$ to establish \cref{thm:higher-arity}, whose proof is split into two parts. First, we provide a database $\dbg$ to form a knowledge base $(\rsg, \dbg)$ for which no universal model of bounded clique-width exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\subsection{$\rsgrid$ is not a bounded clique-width set}


We will devote the rest of this section to the proof of the following lemma:



\begin{lemma}\label{lem:no-universal-model-cw}
Let $a$ be a constant and let $\dbg = \set{A(a)}$ be a database then, there is no universal model of $\kbaseg$ with a bounded clique-width.
\end{lemma}


Let $\ginf$ be an instance that is the infinite quarter-grid as depicted on the \cref{fig:ginf}, where all terms other that the constant $a$ are nulls.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/ginf.pdf}
    \caption{ The instance $\ginf$.}
    \label{fig:ginf}
\end{figure}

\begin{observation}\label{obs:ginf-is-universal-model}
The instance $\ginf$ is a universal model of $\kbaseg$.
\end{observation}



%It is well known~\cite{} that all grid like structures have unbounded clique-width. 
%\thomas{The original proof for (undirected!) grids w.r.t. clique-width was done in \cite[\thm~4]{GolumbicRot99}, where grids are considered as (undirected) graphs. We probably(?) should be ``careful'' here since we have two types of edges and are in the directed setting. It's not that it wouldn't work or anything... But we probably should make a short argument why it does hold here.}

It is well known that infinite grids over a signature consisting of single binary relation have unbounded clique-width (see \cite[\thm~4]{GolumbicRot99} for the reference). Consider the following:

\begin{observation}\label{fact:grid-has-unbounded-cw}
The instance $\ginf$ has unbounded clique-width.
\end{observation}
\begin{proof}
    Consider the two following claims:
    \begin{claim}
        Let $\sig$ be a binary signature, $E$ be a binary relational symbol and $\inst$ be any instance over $\sig$. Then the instance $\inst' = \set{E(t,t') | A(t,t') \in \inst, A \in \sig}$ satisfies $\cw{\inst} \geq \cw{\inst'}$.
    \end{claim}
    \begin{subproof}[Proof]
    \todoiftime
    \end{subproof}
    
    \begin{claim}
        Let $\sig$ be a signature consisting of a single binary relational symbol $E$ and $\inst$ be any instance over $\sig$.  Then the instance $\inst' = \set{E(t',t) | E(t,t') \in \inst} \cup \inst$ satisfies $\cw{\inst} \geq \cw{\inst'}$.
    \end{claim}
    \begin{subproof}[Proof]
    \todoiftime
    \end{subproof}
    
    Finally note that adding $\set{A(a^{\arity{A}}) | A \in \sigi}$ to any instance does not lower its clique-width. \thomas{How about $\set{P(a^{\arity{P}}) | P \in \sigi}$ or $R$ instead of $P$? $A$ does not feel well-chosen here, considering that we only have three relations symbols in our signature of which one is called $A$. We could even write it out as $\{ A(a), H(a, a), V(a, a) \}$, because $a^{\arity{A}}$ is also a bit weird.}
\end{proof}

\begin{observation}\label{obs:identity}
If $h: \ginf \to \ginf$ is a homomorphism then $h$ is \thomas{the} identity.
\end{observation}

\piotr{define what is induced sub-instance if we do not do that already.}
\begin{lemma}
Every universal model of $\kbaseg$ contains $\ginf$ as an induced sub-instance.
\end{lemma}
\thomas{Restatement of the lemma:
\begin{lemma}
Every universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$.
\end{lemma}
Reason for restatement: Induced sub-instance means we see exactly that structure. But it is easy to see that we could kind of ``rename'' the elements in $\unimod$, such that $\ginf$ is not formally an induced sub-instance.}
\begin{proof}
Take any universal model $\unimod$ of $\kbaseg$. From the fact that $\ginf$ is a universal model as well we conclude the existence of two homomorphisms $h\colon \ginf \to \unimod$ and $h'\colon \unimod \to \ginf$. Consider the homomorphism $h' \circ h$ and note that, from~\cref{obs:identity}, it needs to be an identity. 
\thomas{(Rewriting from last sentence.) Observe that from \cref{obs:identity} the homomorphism $h'\circ h$ has to be the identity on $\ginf$. Hence $h$ has to be injective. Furthermore $h$ is even reflective, hence constitutes an embedding. Let $P\in\sigi$ and $\vt$ be a tuple of length $\arity{P}$ from $\ginf$. If $P(h(\vt))$ holds in $\unimod$ , then $P(h'(h(\vt)))$ holds in $\ginf$. But since $h'\circ h$ is the identity on $\ginf$ we immediately obtain $P(\vt)$. Finally note that the image of $\ginf$ under $h$ is isomorphic to $\ginf$ and hence we obtain the claim.}
\end{proof}

\subsection{$\ruleset_{grid}$ is a finite unification set}


As promised in this section we will prove the following lemma:
\begin{lemma}\label{lem:rsg-is-fus}
$\rsg$ is $\fus$.
\end{lemma}

Clearly, given rule $(loop)$ of $\rsg$, we can see that every BCQ that does not contain constants has a trivial rewriting. Thus, consider the following:

\begin{observation}\label{obs:bcq-no-const-trivial}
Every BCQ that contains no constants is FO-rewritable with respect to $\rsg$.
\end{observation}

\piotr{Here is a link for Xrewrite \url{https://arxiv.org/pdf/1405.2848.pdf}}
Proving that a provided rule set is FO-rewritable is a notoriously difficult task\footnote{This should not be much surprising as FO-rewritability is an undecidable property~\cite{fus-is-undecidable-property}.}. To this end, we hand-tailor a rewriting algorithm to be used only for the proof of~\cref{lem:rsg-is-fus}. However, one can refer to existing rewriting algorithms (XRewrite~\cite{xrewrite} being a notable example) for additional intuitions. Finally, it is important to note that the proof itself is closely following the ideas provided in \cite{hopefully-pods-paper}.

\subsection{Necessary definitions}
As we are considering a binary signature, we will treat queries as graphs with the company of standard graph theoretic notions. \thomas{Does this suffice or would Reviewer 2 state: ``The term \emph{graph} has not been defined. Suggest strong reject.''?}

A {\em marked query} is a pair $(q, M)$ where $q$ is a BCQ and $M$ is a subset of terms (variables and constants) of $q$. Given an instance $\inst$ we say that $\inst \models (q,M)$ if and only if there exists a homomorphism $h: q \to \inst$ such that for every term $t$ of $q$ we have $t \in M$ if and only if $h(t)$ is a constant in $\inst$.

Consider the following:
\begin{observation}\label{obs:buildup-for-properly-marked-chase}
Let $\db$ be any database. Then:
\begin{itemize}
    \item if $H(t,t')$ or $V(t,t')$ is an atom of $\sg$ and $t'\in \adom{\db}$  then $t\in \adom{\db}$,
    \item if there is a cycle $C$ in $\sg$ then $C$ is a subset of $\db$, 
    \item if $E(t_1,t')$ and $E(t_2,t')$ are two atoms in  $\sg$ (where $E\in\{H, V\}$) and $t_1\in  \adom{\db}$ then  also $t_2\in  \adom{\db}$.
    \item if $E(a,t)$ and $E(b,t)$ are two atoms in $\sg$ (where $E\in\{H, V\}$) and $a\neq b$ are constants then $t$ is a constant as well.
\end{itemize}
\end{observation}

Having this observation in mind we define the notion of a {\em properly marked query}.

\begin{definition}\label{def:properly-marked}
A marked query $(q, M)$ is {\em properly marked} when:
\begin{itemize}
    \item if $a$ is a constant of $q$ then $a \in M$,
    \item if $H(t,t')$ or $V(t,t')$ is an atom of $q$ and $t' \in M$ then $t \in M$,
    \item if there is a cycle $C$ in $q$ then terms of $C$ are contained in $M$,
    \item if $E(t_1,t')$ and $E(t_2,t')$ are two atoms in  $q$ (where $E\in\{H, V\}$) and $t_1 \in M$ then $t_2 \in M$.
    \item if $E(a,t)$ and $E(b,t)$ are two atoms in $q$ (where $E\in\{H, V\}$) and $a\neq b$ are constants then $t \in M$.
\end{itemize}
\end{definition}

From \cref{obs:buildup-for-properly-marked-chase} and \cref{def:properly-marked} we immediately conclude the following:

\begin{corollary}
Let $(q, V)$ be a marked query, and $\db$ be any database. If $\sg \models \mq$ then $\mq$ is properly marked.
\end{corollary}

From now on any properly marked query $(q, V)$ such that $V$ is not containing all terms of $q$ will be called {\em alive}. In the case when every term of a properly marked query is marked we will call such a query {\em totally marked}.

To prove~\cref{lem:rsg-is-fus} it is enough to prove the following:

\begin{lemma}\label{lem:rsg-is-fus-reformulated}
For any properly marked query $(q, V)$ there exists a set of totally marked queries $rew(q,V)$ such that for any database $\db$ the following holds: 
$$\sg \models (q,v) \iff \exists{Q' \in rew(q, V)} \db \models Q'.$$
\end{lemma}

\subsection{Rewriting Alive Queries}

Consider the following:

\begin{lemma}\label{lem:exists-maximal}
For every alive query there exists at least one variable with no out-going edges.
\end{lemma}
\begin{proof}
A query is alive if it is properly marked and there exists at least one unmarked variable. From the first we notice that the sub-query induced on the unmarked variables is a directed and acyclic graph. From the second we know that this graph is non-empty.
\end{proof}

Such unmarked variables with no out-going edges will be called {\em maximal}. Those maximal variables will be used as a starting points for the rewriting process. 

\begin{lemma}\label{lem:maximal-cases}
Let $x$ be a maximal variable of a live query $(q, V)$. Then one of the following conditions holds:
\begin{enumerate}
    \item \label{lem:maximal-cases-one} $x$ occurs in exactly one atom  $E(t,x)$, with $E\in \{H,V\}$ for some term $t$ of $q$,
    \item \label{lem:maximal-cases-two} $x$ occurs in exactly two atoms $H(t_H,x)$ and $V(t_V,x)$ for some terms $t_H,t_V$ of $q$,
    \item \label{lem:maximal-cases-three} there exist at least two distinct terms $t\neq t'$ and $E \in \{H,V\}$ such that $E(t,x)$ and $E(t',x)$ are atoms of $q$.
\end{enumerate}
\end{lemma}

Now, in the light~\cref{lem:maximal-cases} we will present four operations that when combined will compute rewritings required by \cref{lem:rsg-is-fus-reformulated}.

\medskip
\noindent
{\bf Five operations}
Given an alive query $(q, V)$ we define:

\begin{definition}[$\cutop$]\label{def:cut}
Let $x$ be a maximal variable of $(q, V)$ such as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-one} then $\cutop((q,V), x) = (q', V)$ where $q'$ is a sub-query of $q$ with the atom containing $x$ removed.
\end{definition}

\begin{definition}[$\reduceop$]\label{def:reduce}
Let $x, t_H, t_V$ be as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-two} then let $q'$ be obtained from $q$ by replacing $H(t_H, x),V(t_V, x)$ with $H(x', t_V), V(x', t_H)$ 
where $x'$ is a fresh variable. Then let $\cutop((q,V), x) = \set{ (q', V), (q', V \cup {x'})}$. \thomas{Shouldn't that be $\reduceop((q,V), x) = \set{ (q', V), (q', V \cup {x'})}$?}
\end{definition}

\begin{definition}[$\mergeop$]\label{def:merge}
Let $x, t, t'$ be as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-three} then let $q'$ be obtained from $q$ by replacing all occurrences of $t$ in $q$ with $t'$. Then let $\mergeop((q, V), x, t, t') = (q', V)$.
\end{definition}

\begin{observation}[Completeness]\label{obs:high-completeness}
If a query is alive then at least one of above operations can be applied to it.
\end{observation}
\begin{proof}
Follows from~\cref{def:cut,def:reduce,def:merge}, and~\cref{lem:maximal-cases}.
\end{proof}

Now we will prove the soundness for those operations:

\begin{lemma}[Soundness --- $\cutop$]\label{lem:high-soundness-cut}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models \cutop(Q, x)$$
if $x$ is as in \cref{def:cut}.
\end{lemma}
\begin{proof}
TODO
\end{proof}

\begin{lemma}[Soundness --- $\reduceop$]\label{lem:high-soundness-reduce}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models Q' \vee Q''$$
if $x$ is as in \cref{def:reduce} and $\reduceop(Q, x) = \set{Q', Q''}$.

\end{lemma}
\begin{proof}
TODO
\end{proof}

\begin{lemma}[Soundness --- $\mergeop$]\label{lem:high-soundness-merge}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models \mergeop(Q, x, t, t')$$
if $x, t, t'$ are as in \cref{def:merge}.
\end{lemma}
\begin{proof}
TODO
\end{proof}

\medskip
\noindent
{\bf Rank of an alive query}

Given a BCQ $Q$ a {\em path} is a finite sequence $P$ such that:

\piotr{cleanup variables $x,y,z,t,u,\ldots$ for consistency with the rest of the paper.} 
 \begin{itemize}
    \item Each of the elements of $P$ is either $E(t,z)$ or $\Em(z,t)$ for some $E(t,z)$ from $q(Q)$, where $E\in\{H,V\}$ 
    \item if $E(s,t)$ and $E'(u,z)$ are two consecutive elements of $P$ then $t=u$ (where $E,E'\in\{H,V,\Hm, \Vm \}$);
    \item No term of $Q$ can be visited in $P$ twice.
 \end{itemize}
 
 We will write $P = P' \cdot E(x,y)$ to denote a path $P$ extends $P'$ with $E(x,y)$. In some cases we write $P = P' \cdot E$ to avoid clutter. Also, by writing $P(x,y)$ we state that $P$ starts in $x$ and ends in $y$.

Given a marked query $Q$ and any path $P$ in $Q$ we define its {\em cost} in the following way:
\begin{itemize}
    \item $\cost{\varepsilon} = |\adom{Q}|$
    \item $\cost{P \cdot E} = \cost{P}$, \hfill for $E \in \set{H, \Hm}$
    \item $\cost{P \cdot V} = \cost{P} + 1$
    \item $\cost{P \cdot \Vm} = \cost{P} - 1$
\end{itemize}

and its {\em rank} as:

\begin{itemize}
    \item $\rank{\varepsilon} = 0$
    \item $\rank{P \cdot E} = \rank{P} + \cost{P \cdot E}$ for $E \in \set{H, \Hm, V, \Vm}$
\end{itemize}

Given a properly marked query\footnote{Recall, that we consider BCQs that contain at least one constant, thus the set of marked variables of any properly marked query cannot be empty.} $\mq$ and any of its unmarked variables $x \in M$ we define the \emph{rank of $x$ in $\mq$}, $\rank{x, \mq}$, as:
$$\rank{x, \mq} = \min(\set{\rank{P(t,x)} | t \in M})$$

And finally, given a properly marked query $\mq$ we define its rank $\rank{\mq}$ as:
$$(|\adom{q}|, \multiset{ \rank{t, \mq} | t \in terms(q) \wedge t \not\in M})$$
with $\multiset{}$ simply denoting a multi-set. For two properly marked queries $Q$ and $Q'$ such that $\rank{Q} = (n, \mathcal{P})$ and $\rank{Q'} = (n', \mathcal{P}')$ we write $\rank{Q} < \rank{Q'}$ if: $n < n'$ or $\mathcal{P}$ is lexicographically smaller than $\mathcal{P}'$ when $\mathcal{P}$ and $\mathcal{P}'$ are treated as ordered lists. It should be clear that the order $<$ on ranks of properly marked queries is well ordered.

\medskip
\noindent
{\bf Termination}
Now we will show that our rewriting process terminates. 

\begin{lemma}[Termination --- $\cutop$]\label{lem:high-termination-cut}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\rank{\cutop(Q, x)} < \rank{Q}$$
if $x$ is as in \cref{def:cut}.
\end{lemma}
\begin{proof}
Note that operation $\cutop$ removes one unmarked variable from $Q$. Thus the active domain of $Q$ is strictly greater than that of $\cutop(Q, x)$.
\end{proof}

\piotr{Be extremely cautious when proofreading this proof}
\begin{lemma}[Termination --- $\reduceop$]\label{lem:high-termination-reduce}
Let $\db$ be any database and let $Q$ be an alive query then:
$$ \rank{Q'} < \rank{Q} \wedge \rank{Q''} < \rank{Q}$$
if $x$ is as in \cref{def:reduce} and $\reduceop(Q, x) = \set{Q_1, Q_2}$.
\end{lemma}
\thomas{The $Q'$ and $Q''$ put me a bit off here. Are those actually $Q_1$ and $Q_2$ respectively, or ..?}
\begin{proof}
Let $Q = \mq$ and let $Q' = (q', M')$ be any of the queries in $\set{Q_1, Q_2}$. Also, let $x$ be the removed variable and let $x'$ be the newly introduced variable.
First we will show the following:
\begin{claim}
Let $y$ be any unmarked variable of $Q$ other than $x$. Then $\rank{x, Q} \geq \rank{x, Q'}$.
\end{claim}
\thomas{Why do you need to introduce the $y$ if you only compare the ranks with respect to $x$ and different queries?}
\begin{subproof}[Proof]
Let $P(t,y)$ be a path of minimal rank from some marked term $t$ of $Q$ to $y$. If $P$ does not visit $x$ then $P$ is a path in $Q'$ as well and so $\rank{y, Q} \geq \rank{y, Q'}$. If $P$ visits $x$ then it is of one of the two following forms: $$P = P_1 \cdot H(t_H, x)\cdot\Vm(x, t_V)\cdot P_2$$ or $$P = P_1' \cdot V(t_V, x)\cdot\Hm(x, t_H) \cdot P_2'.$$ Assume the first case, then $P'(t,y) = P_1 \cdot \Vm(t_H, x)\cdot H(x, t_V) P_2$ is a path from $t$ to $y$ in $Q'$. \thomas{$P'$ does utilize $x$ though. So it is probably not $x$ here?} Observe that the rank of $P'$ is strictly smaller than the rank of $P$. The second case is analogous.
\end{subproof}

Consider:
\begin{observation}
$\rank{x, Q} > \rank{x', Q'}$.
\end{observation}
\thomas{What is $x'$? It's probably the $x'$ from the definition of the $\reduceop$ operation, but I think that should be clarified here. Is it also the same term that will appear in relation to my last comment?}
\begin{subproof}[Proof]
Note that if If $x' \in M'$ then $\rank{x', Q'} = 0$ and thus $\rank{x, Q} > \rank{x', Q'}$ as $x \not\in M$.

Let $P(t,x)$ be a path of minimal rank from some marked term $t$ of $Q$ to $x$. Notice that $P$ is of one of the two following forms: $P = P_1 \cdot H(t_H, x)$ or $P = P_1' \cdot V(t_V, x)$.
Assume that $P = P_1 \cdot H(t_H, x)$. Notice that $P_V = P_1 \cdot \Vm(t_H, x)$ \thomas{Again, is that $x$ or shouldn't it be $x'$ as we now go ``the different'' $V$, though counter the direction of that edge, down.} is a path in $Q'$ and that $\rank{P_V} = \rank{P} - 1$. The second case is analogous.
\end{subproof}

Finally, note that $|\adom{q}| = |\adom{q'}|$. 
\end{proof}

\begin{lemma}[Termination --- $\mergeop$]\label{lem:high-termination-merge}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\rank{\mergeop(Q, x)} < \rank{Q}$$
if $x, t, t'$ are as in \cref{def:merge}.
\end{lemma}
\begin{proof}
Note that operation $\mergeop$ removes one variable from $Q$. Thus the active domain of $Q$ is strictly greater than that of $\mergeop(Q, x)$.
\end{proof}

Finally, from completeness (\cref{obs:high-completeness}), soundness (\cref{lem:high-soundness-cut,lem:high-soundness-reduce,lem:high-soundness-merge}), and termination (\cref{lem:high-termination-cut,lem:high-termination-reduce,lem:high-termination-merge}) we conclude~\cref{lem:rsg-is-fus-reformulated} thus finishing the proof of \cref{lem:rsg-is-fus}.

==> ICDT 2023 Updated LaTeXFiles/other/old-partition-width.tex <==
\section{Clique-width and Partition-width}

\subsection{New Definition}

\begin{comment}
Let $\cols$ be an infinite set of \emph{colors}. For $C\subseteq \cols$ we define a set $F_{C}$ consisting of the following operation symbols:
\begin{itemize}
	\item For every $n\in C$ let $\unitn$ be a (fresh) constant symbol (i.e. a symbol of rank $0$).
	\item For every predicate $\mathtt{R}\in\sigma$ and tuple $\vc\subseteq C$ of length $\arity{\mathtt{R}}$ let $\add{\mathtt{R}, \vc}{}$ be a unary symbol (rank $1$).
	\item For every two colors $l_1, l_2\in C$ let $\recol{l_1\to l_2}{}$ be a unary symbol (rank $1$).
	\item Let $\oplus$ be a binary symbol (rank $2$).
\end{itemize}
Lastly, we introduce an extended signature $F_{C}^{\mathbf{0}}$, in which we add
\begin{itemize}
	\item a fresh constant-symbol $\mathbf{0}$.
\end{itemize}
\end{comment}
Let $\cols$ be an infinite set of \emph{colors} and $\Sigma = \Sigma_1 \oplus \Sigma_2$ a finite relational signature with unary ($\Sigma_1$) and binary ($\Sigma_2$) relational symbols. As a small technicality, we introduce a fresh unary predicate $\top$ that holds on all terms from $\adom{\inst}$ for a given instance $\inst$.
\begin{definition}
	Let $\Sigma$ be a finite binary relational signature, $\inst$ be an instance. For $C\subseteq\cols$ and $\lambda\colon\adom{\inst} \to C$ we call the tuple $(\inst, \lambda)$ a \emph{$C$-colored instance}, or \emph{colored instance} for short.\\
	Two $C$-colored instances $(\inst_1, \lambda_1)$ and $(\inst_2, \lambda_2)$ are called \emph{isomorphic}, $(\inst_1, \lambda_1) \cong_{\Sigma, C} (\inst_2, \lambda_2)$ iff $\inst_1 \cong_{\Sigma} \inst_2$ with an isomorphism $h\colon \inst_1\to\inst_2$ and there exists a bijection $\kappa\colon \cols \to \cols$ such that $\kappa \circ \lambda_1 = \lambda_2 \circ h$. \\
	For fixed $\Sigma$ and $C$ we call the isomorphy-class of a colored instance $(\inst, \lambda)$ under $\cong_{\Sigma, C}$ an \emph{abstract $C$-colored instance}.
\end{definition}
\begin{definition}
	For $C\subseteq \cols$ we define a set $F_{C}$ consisting of the following operation symbols:
	\begin{itemize}
		\item Let $\bold{0}$ be a instance-construction-constant (\emph{ic-constant} for short) symbol.
		\item For every $n\in C$ and $\mathcal{P}\subseteq \Sigma_{1}$ let $\unit_{n, \mathcal{P}}$ be a ic-constant symbol .
		\item For every $n\in C$, $\mathcal{P}\subseteq \Sigma_{1}$, and $c \in K$ let $c_{n, \mathcal{P}}$ be a ic-constant symbol.
		\item For every binary predicate $\mathtt{R}\in\Sigma$ and pair $(l_1, l_2)\in C^2$ of length $\arity{\mathtt{R}}$ let $\add{\mathtt{R}, (l_1,l_2)}{}$ be a unary ic-symbol.
		\item For every two colors $l_1, l_2\in C$ let $\recol{l_1\to l_2}{}$ be a unary ic-symbol.
		\item Let $\oplus$ be a binary ic-symbol.
	\end{itemize}
	For a given $C\subseteq \cols$ let $T(F_{C})$ denote the set of all terms over $F_{C}$.
\end{definition}
Let $\Sigma$ be some relational signature. To each $t\in F_{C}$ we associate a finite abstract $C$-colored instance\footnote{For simplicity we drop the isomorphism class in the exposition and work with a representant.} $(\inst, \lambda)$ with $\lambda\colon \adom{\inst} \to C$ by defining a \emph{valuation map} $\val{t}$ inductively. First we introduce the interpretations of the ic-symbols on the class of abstract $C$-colored instances over $\Sigma$
\begin{itemize}
	\item $\val{\mathbf{0}}$ is the empty instance colored by $\lambda\colon \emptyset \to C$.
	\item For every $n\in C$ and $\mathcal{P}\subseteq \Sigma_{1}$ let $\val{\unit_{n, \mathcal{P}}}$ be the instance $\{ \top(t) \}\cup \{ R(t) \, | \, R\in \mathcal{P} \}$ colored by $\lambda\colon t \mapsto n$.
	\item For every $n\in C$, $\mathcal{P}\subseteq \Sigma_{1}$, and constant $c\in \mathfrak{C}$ let $\val{c_{n, \mathcal{P}}}$ be the instance $\{ \top(c) \}\cup \{ R(c) \, | \, R\in \mathcal{P} \}$ colored with $\lambda\colon c \mapsto n$.
	\item For every binary predicate $\mathtt{R}\in\sigma$, pair $(l_1,l_2)\in C^2$, and abstract colored instance $(\inst, \lambda)$ let $\add{\mathtt{R}, (l_1,l_2)}{(\inst, \lambda)}$ be the instance $(\inst', \lambda)$, where $\adom{\inst'} = \adom{\inst}$, and \[ \inst' = \inst \cup \{ R(t_1, t_2) \, | \, \lambda((t_1, t_2)) = (l_1,l_2) \} \, .\]
	\item For every two colors $l_1, l_2\in C$ and colored instance $(\inst, \lambda)$ let $\recol{l_1\to l_2}{(\inst, \lambda)} = (\inst, \lambda')$ where $\lambda' = h\circ \lambda$ with $h_{l_1\to l_2} \colon C \to C$ with \[ h(x) := \begin{cases} l_2, \quad \text{if } x = l_1 \\ x, \quad \text{else} \end{cases} \, . \]
	\item For two $C$-colored instances $(\inst_1, \lambda_1), (\inst_2, \lambda_2)$ we let $(\inst_1, \lambda_1) \oplus (\inst_2, \lambda_2) = (\inst', \lambda')$ where with $\adom{\inst_2'}\cap\adom{\inst_1} \subset \mathfrak{C}$, $(\inst_2', \lambda_2') \cong_{\Sigma, C} (\inst_2, \lambda_2)$, $\inst = \inst_1 \cup \inst_2'$, and $\lambda = \lambda_1 \cup\lambda_2'$ the abstract $C$-colored instance $(\inst, \lambda)$ is the disjoint union of both instances.
\end{itemize}
Hence, for every finite \emph{instance-construction-term} (or \emph{ic-term}) $T$ over $F_{C}$, $\val{T}$ is defined inductively as follows:
\begin{itemize}
	\item For every ic-symbol $\mathtt{k}\in F_{C}$ let $\val{\mathtt{k}}$ be as defined above.
	\item For every unary ic-symbol $f\in F_{C}$ and finite ic-term $t\in F_{C}$ let \[ \val{f(t)} = f(\val{t}) \, . \]
	\item For every binary ic-symbol $f\in F_{C}$ and finite ic-terms $t_1, t_2\in F_{C}$ let \[ \val{f(t_1, t_2)} = f(\val{t_{1}}, \val{t_{2}}) \, . \]
\end{itemize}
To describe also countably infinite instances via ic-terms, we need to lift both the ic-terms and there valuation to the infinite case.

%Our first step will be to identify each term with there \emph{syntax-tree}. As our operations are at most of arity $2$, we utilize subtrees of the complete binary tree $2^{< \omega}$ (consisting of all finite sequences over $\{ 0, 1 \}$ with the usual prefix ordering). 
\begin{definition}
	A \emph{syntax-tree over $F_{C}$} of an ic-term is a partial map \[ T \colon 2^{<\omega} \to F_{C} \] with domain $\dom(T)\subseteq 2^{<\omega}$ satisfying the following properties:
	\begin{itemize}
		\item $\dom(T)$ non-empty,
		\item $\dom(T)$ is prefix-closed (i.e. if $\alpha\beta \in 2^{<\omega}$ with $\alpha\beta\in \dom(T)$ then $\alpha\in\dom(t)$)
		\item if $\alpha 1\in\dom(T)$ then $\alpha 0\in\dom(t)$.
		\item Furthermore, for $\alpha\in\dom(T)$ if $t(\alpha) = f$ then for all $i \in\{ 0, 1 \}$ we have $\alpha i\in\dom(T)$ iff $i< \arity{f}$.
	\end{itemize}
	For $T$ a syntax-tree we define as $L_{T}$ the set of all leafs of $T$ (i.e. the set of all $\alpha \in L_{T}$ such that $\alpha 0 \not\in L_{T}$ and $\alpha 1 \not\in L_{T}$) \\
	$T$ is called \emph{well-formed} if there are only finitely many $a\in \mathfrak{C}$ such that there exists exactly one $n\in C$ and exactly one $\alpha\in L_{T}$ such that  $f(\alpha) = a_{n}$. \\
	We define $T^{\infty}(F_{C})$ to consist of all syntax-trees over $F_{C}$.
\end{definition}
We will use ``ic-term'' and ``syntax-tree over $F_{C}$'' interchangably.
\begin{observation}
	Finite syntax-trees over $F_{C}$ correspond one-to-one to terms $t\in F_{C}$.
\end{observation}
In order to lift the valuation-map to infinite ic-terms we will utilize the notion of the \emph{$n$-depth truncation} of a tree.
\begin{definition}
	Let $T\in T^{\infty}(F_{C})$ and $k\in \mathbb{N}$, the \emph{$k$-depth truncation of $T$}, $T^{(k)}$ is defined inductively as follows:
	\begin{itemize}
		\item $T^{(0)} = \mathbf{0}$
	\end{itemize}
	and for $k> 0$
	\begin{itemize}
		\item if $T = T_{1}\oplus T_{2}$ then $T^{(k)} = (T_{1}\oplus T_{2})^{(k)} = T_{1}^{(k-1)}\oplus T_{2}^{(k-1)}$,
		\item for $f\in F_{C}$ unary, $f(T)^{(k)} = f(T^{(k-1)})$,
		\item for $n\in C$, $\unitn^{(k)} = \unitn$,
		\item for $n\in C$ and $a\in\mathfrak{C}$, $a_{n}^{(k)} = a_{n}$,
		\item $\mathbf{0}^{(k)} = \mathbf{0}$.
	\end{itemize}
\end{definition}
Furthermore we define a partial order on the set of syntax-trees):
\begin{definition}
	\begin{itemize}
		\item Let $T, T' \in T(F_{C})$ for some $C\subseteq \cols$. Then $T \prec T'$ iff we have $c\in T(F_{C} \cup \{ u_1, \ldots, u_k \})$ and $T'_{1}, \ldots, T'_{k}\in T(F_{C})$ such that $T = c[\bold{0}, \ldots, \bold{0}]$ and $T' = c[T'_{1}, \ldots, T'_{k}]$.
		\item For $T'\in T^{\infty}(F_{C})$ and $T \in T(F_{C})$, we define $T\prec T'$ to hold iff in the previous setup we have $T', T'_{1}, \ldots, T'_{k}\in T^{\infty}(F_{C})$.
	\end{itemize}
\end{definition}
\begin{observation}
	Note that every ascending chain of finite trees, i.e. $(T_{i})_{i < \omega} \subseteq T(F_{C})$ such that \[ T_{0} \prec T_{1} \prec T_{2} \prec \cdots \] has a least upper bound in $T^{\infty}(F_{C})$. See \cite[Section 2]{Cou78} for approximation of infinite terms by finite ones.
\end{observation}
\begin{comment}
With this partial order defined, we need to introduce one more tool: The \emph{$n$-depth truncation} of a term $t\in T^{\infty}(F_{C})$ which we define inductively:
\begin{itemize}
	\item $t^{(0)} = \bold{0}$
	\item For $n>0$ we set
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(n)} = t_{1}^{(n-1)} \oplus t_{2}^{(n-1)}$
		\item $f(t_{1})^{(n)} = f(t_{1}^{(n)})$ for every unary $f$
		\item $\unit_{1}^{(n)} = \unit_{1}$ and $\bold{0}^{(n)} = \bold{0}$.
	\end{itemize}
\end{itemize}
Note that $t^{(n)}$ for every term $t\in T^{\infty}(F_{C})$ is in fact a finite term over $F_{C}$, i.e. $t^{(n)}\in T(F_{C})$.
\end{comment}

\begin{observation}
	If $T,T'\in T(F_{C})$ with $T\prec T'$ then $\val{T}$ is an induced sub-instances of $\val{T'}$.
\end{observation}
\begin{observation}
	If $T\in T^{\infty}(F_{C})$ then
	\begin{equation*}
		T^{(0)} \prec T^{(1)} \prec \cdots
	\end{equation*}
	which induces an ascending chain of induced sub-instances
	\begin{equation*}
		\val{T^{(0)}} \le \val{T^{(1)}} \le \cdots
	\end{equation*}
\end{observation}
\begin{definition}
	If $T\in T^{\infty}(F_{C})$ is an infinite syntax-tree, then $\val{T} = \bigcup_{i < \omega} \val{T^{(i)}}$.
\end{definition}

\begin{comment}
We extend this idea to all functional signatures $F$ with at most binary function symbols, i.e. $F^{\mathbf{0}}$ will always contain the additional fresh constant-symbol $\mathbf{0}$ if we want to make it obvious that we are now using $\mathbf{0}$.
For a given $C\subseteq \cols$ let $T(F_{C}^{\mathbf{0}})$ denote the set of all terms over $F_{C}^{\mathbf{0}}$.
Let $\Sigma$ be some relational signature. To each $t\in F_{C}^{\mathbf{0}}$ we can associate a(n ismorphism class of a) finite (possibly empty) colored structure\footnote{For simplicity we drop the isomorphism class in the exposition.} $(\mathfrak{A}, \lambda)$ with $\lambda\colon A \to C$ by defining a \emph{valuation map} $\val{t}$ inductively. First we introduce the interpretations of the operation symbols on the class of $C$-colored relational structures over $\Sigma$ and also give already the valuation of the constant symbols
\begin{itemize}
	\item $\val{\mathbf{0}}$ is the empty structure (hence the coloring $\lambda\colon \emptyset \to C$ is the unique map $\emptyset$).
	\item For every $n\in C$ let $\val{\unitn}$ be the structure with one element, no relations holding and the coloring $\lambda$ mapping the unique domain element to $n$.
	\item For every predicate $\mathtt{R}\in\sigma$, tuple $\vc\subseteq C$ of length $\arity{\mathtt{R}}$, and colored relational structure $(\mathfrak{A}, \lambda)$ let $\add{\mathtt{R}, \vc}{(\mathfrak{A}, \lambda)}$ be the structure $(\mathfrak{B}, \lambda)$, where $B = A$, for all constant symbols $\mathtt{c} \in \Sigma$ we have $c^{\mathfrak{B}}= c^{\mathfrak{A}}$, for all $\mathtt{P}\in \Sigma\setminus \{ \mathtt{R} \}$ we have $\mathtt{P}^{\mathfrak{B}} = \mathtt{P}^\mathfrak{A}$ and \[ \mathtt{R}^{\mathfrak{B}} = \mathtt{R}^{\mathfrak{A}} \cup \{ \overline{b} \in B^{\arity{\mathtt{R}}} \, | \, \lambda(\overline{b}) = \vl \} \, .\].
	\item For every two colors $a, b\in C$ and colored relational structure $(\mathfrak{A}, \lambda)$ let \[ \recol{a\to b}{(\mathfrak{A}, \lambda)} = (\mathfrak{A}, \lambda')\] where for $h_{a\to b} \colon C \to C$ with \[ h_{a\to b}(x) := \begin{cases} b, \quad \text{if } x = a \\ x, \quad \text{else} \end{cases} \] we have $\lambda' = h_{a\to b}\circ \lambda$.
	\item For two $C$-colored structures $(\mathfrak{A}, \lambda_1), (\mathfrak{B}, \lambda_2)$ we let $(\mathfrak{A}, \lambda_1) \oplus (\mathfrak{B}, \lambda_2)$ be the disjoint union of both structures.
\end{itemize}
We now lift the valuation map from the constant symbols to finite terms in the natural way:
\begin{itemize}
	\item For every constant-symbol $\mathtt{k}\in F_{C}^{\mathbf{0}}$ let $\val{\mathtt{k}}$ be as defined above.
	\item For every unary operation-symbol $f\in F_{C}$ and finite term $t\in F_{C}$ let \[ \val{f(t)} = f(\val{t}) \, . \]
	\item For every binary operation-symbol $f\in F_{C}$ and finite terms $t_1, t_2\in F_{C}$ let \[ \val{f(t_1, t_2)} = f(\val{t_{1}}, \val{t_{2}}) \, . \]
\end{itemize}
\begin{observation}
    Obviously, restricting $F_{C}^{\mathbf{0}}$ to $F_{C}$ yields a valid valuation map, too.
\end{observation}
Until now we only deal with finite terms and hence can describe only finite colored structures with those. As we are interested to also describe countably infinite colored structures, our next goal will be to introduce infinite terms and then extend the valuation map to those.

Our first step will be to identify each term with its \emph{syntax-tree}. We define this in the general setting with $F$ being an algebraic signature containing function symbols up to arity $2$. As our operations are at most of arity $2$, we utilize subtrees of the complete binary tree $2^{< \omega}$ (consisting of all finite sequences over $\{ 0, 1 \}$ with the usual prefix ordering). 
\begin{definition}
	A \emph{syntax-tree over $F$} is a partial map \[ t \colon 2^{<\omega} \to F \] with domain $\dom(t)\subseteq 2^{<\omega}$ satisfying the following properties:
	\begin{itemize}
		\item $\dom(t)$ non-empty,
		\item $\dom(t)$ is prefix-closed (i.e. if $\alpha\beta \in 2^{<\omega}$ with $\alpha\beta\in \dom(t)$ then $\alpha\in\dom(t)$)
		\item if $\alpha 1\in\dom(t)$ then $\alpha 0\in\dom(t)$.
		\item Furthermore, for $\alpha\in\dom(t)$ if $t(\alpha) = f$ then for all $i \in\{ 0, 1 \}$ we have $\alpha i\in\dom(t)$ iff $i< \arity{f}$.
	\end{itemize}
	For $t$ a syntax-tree we define as $L_{t}$ the set of all leafs of $t$ (i.e. the set of all $\alpha \in \dom(t)$ such that $\alpha 0 \not\in \dom(t)$ and $\alpha 1 \not\in \dom(t)$)
\end{definition}
\begin{observation}
	Finite syntax-trees over $F_{C}$ correspond one-to-one to terms $t\in F_{C}$.
\end{observation}
We define $T^{\infty}(F)$ to consist of all syntax-trees over $F$.

We will now lift the valuation-map to infinite terms (which are infinite syntax-trees). For this we will utilize the notion of the \emph{$n$-depth truncation} of a tree.
\begin{definition}
	 For an arbitrary algebraic signature $F$ with arity at most $2$, let $t\in T^{\infty}(F)$ and $k\in \mathbb{N}$. The \emph{$k$-depth truncation of $t$} is the finite term $t^{(k)}\in T(F^{\bold{0}})$ defined inductively as follows:
	\begin{itemize}
		\item $t^{(0)} = \bold{0}$
	\end{itemize}
	and for $k> 0$
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(k)} = t_{1}^{(k-1)}\oplus t_{2}^{(k-1)}$,
		\item for $f\in F$ unary, $f(t)^{(k)} = f(t^{(k-1)})$,
		\item for $n\in C$, $\unitn^{(k)} = \unitn$,
%		\item $\bold{0}^{(k)} = \bold{0}$.
	\end{itemize}
\end{definition}
We can define a partial order on the set of syntax-trees in the following way (note that adding variable symbols to the signature corresponds to having the ability to substitute terms for those variable symbols):
\begin{itemize}
	\item Let $t, t' \in T(F_{C})$ for some $C\subseteq \cols$. Then $t \prec t'$ iff we have $c\in T(F_{C} \cup \{ u_1, \ldots, u_k \})$ and $t'_{1}, \ldots, t'_{k}\in T(F_{C})$ such that $t = c[\bold{0}, \ldots, \bold{0}]$ and $t' = c[t'_{1}, \ldots, t'_{k}]$.
	\item Furthermore, for $t'\in T^{\infty}(F_{C})$ and $t \in T(F_{C})$, we define $t \prec t'$ to hold iff in the previous setup we have $t', t'_{1}, \ldots, t'_{k}\in T^{\infty}(F_{C})$.
\end{itemize}
\begin{observation}
	Note that every ascending chain of finite trees, i.e. $(t_{i})_{i < \omega} \subseteq T(F_{C})$ such that \[ t_{0} \prec t_{1} \prec t_{2} \prec \cdots \] has a least upper bound in $T^{\infty}(F_{C})$. (Quote 3, Section 2 of Courcelle Paper).
\end{observation}
With this partial order defined, we need to introduce one last tool: The \emph{$n$-depth truncation} of a term $t\in T^{\infty}(F_{C})$ which we define inductively:
\begin{itemize}
	\item $t^{(0)} = \bold{0}$
	\item For $n>0$ we set
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(n)} = t_{1}^{(n-1)} \oplus t_{2}^{(n-1)}$
		\item $f(t_{1})^{(n)} = f(t_{1}^{(n)})$ for every unary $f$
		\item $\unit_{1}^{(n)} = \unit_{1}$ and $\bold{0}^{(n)} = \bold{0}$.
	\end{itemize}
\end{itemize}
Note that $t^{(n)}$ for every term $t\in T^{\infty}(F_{C})$ is in fact a finite term over $F_{C}$, i.e. $t^{(n)}\in T(F_{C})$.
\begin{observation}
	If $t,t'\in T(F_{C})$ then $\val{t}$ is an induced substructure of $\val{t'}$.
\end{observation}
\begin{observation}
	If $t\in T^{\infty}(F_{C})$ then
	\begin{equation*}
		t^{(0)} \prec t^{(1)} \prec \cdots
	\end{equation*}
	which induces an ascending chain of induced substructures
	\begin{equation*}
		\val{t^{(0)}} \le \val{t^{(1)}} \le \cdots
	\end{equation*}
\end{observation}
With this we can finally define a valuation-function that maps each syntax-tree $t\in T^{\infty}(F_{C})$ to a colored structure in the following way:
\begin{itemize}
	\item If $t\in T(F_{C})$, then $\val{t}$ is as previously defined.
	\item If $t\in T^{\infty}(F_{C})$ is an infinite syntax-tree, then $\val{t} = \bigcup_{i < \omega} \val{t^{(i)}}$.
\end{itemize}
With this we can finally define cliquewidth.
\end{comment}
\begin{definition}
	Let $\inst$ be a countable instance over $\Sigma$. We define its \emph{cliquewidth} as the minimal $k\in \mathbb{N}$ ($\cw{\inst}=k$ for short) such that there exist a $C\subseteq \cols$ with $|C|=k$, a map $\lambda \colon A \to C$ and a term $t\in T^{\infty}(F_{C})$ such that $\val{t} = (\inst, \lambda)$. If there is no such $n\in \mathbb{N}$, we set $\cw{\inst}= \infty$. \piotr{Moreover, for a map $\coloring$ we will write $\cw{\inst, \coloring}$ = k if the co-domain of $\coloring$ is of size $k$ and there exists a term $t$ such that $\val{t} = (\inst, \coloring)$.}
\end{definition}
\piotr{We will use $\mathrm{add}_{R,(l,l')}(\instance, \coloring)$ as a shorthand for\\ $\val{\mathrm{add}_{R,(l,l')}(t)}$ where $t$ is such that $\val{t} = (\instance, \coloring)$.}

\begin{comment}
As another tool we introduce several formula talking about finite syntax-trees over $F_{C}$. The main idea behind those is that they track first, whether a tuple of elements will be put into a relation while evaluating the term and second, which color individual elements will have. Let $t\in T(F_{C})$ (note: a finite term!) and $\mathtt{R}\in\Sigma$ a relational symbol.
\begin{itemize}
	\item Let $\psi_{C}(t, x, i)$ with $x\in L_{t}$ and $i\in C$ denote the sentence saying that $x$ will have the color $i$ at the root of $t$.
	\item We denote by $\phi_{\mathtt{R}}(t, \overline{x})$ the sentence saying the following: For a tuple $\overline{x}\in L_{t}^{\arity{\mathtt{R}}}$ if there is a node $u$ in $t$ such that all $\overline{x}_{i}$ have $u$ as an ancestor, $t(u) = \add{R, \vl}{}$ and for all $0\le i\le \arity{\mathtt{R}}$ it holds that $\psi_{C}(t/u, \overline{x}_i, \vl_{i})$.
\end{itemize}
\begin{observation}
	As long as $x, y$ are both of depth $\le n-1$ we have $\psi_{C}(t, x, i)$ iff $\psi_{C}(t^{(n)}, x, i)$ and $\phi_{\mathtt{R}}(t, \overline{x})$ iff $\phi_{\mathtt{R}}(t^{(n)}, \overline{x})$.
\end{observation}
We use this observation in order to extend the valuation map in the following way:
\begin{definition}
	Let $t\in T^{\infty}(F_{C})$ be a term over $F_{C}$. Then $\val{t} = (\mathfrak{A}, \lambda)$ with
	\begin{itemize}
		\item $A = L_{t}$,
		\item \thomas{\textbf{TODO: Constants!}}
		\item for every $\mathtt{R}\in\Sigma$ and $\overline{a}\in A^{\arity{\mathtt{R}}}$ it holds that $\overline{a}\in \mathtt{R}^{\mathfrak{A}}$ iff there exists a $k\in\mathbb{N}$ such that $\phi_{\mathtt{R}}(t^{(n)}, \overline{a})$ holds.
		\item for all $a\in A$ we define $\lambda(a) = i$ iff there exists $n\in \mathbb{N}$ such that $\psi_{C}(t^{(n)}, a, i)$.
	\end{itemize}
\end{definition}
\begin{lemma}
	On finite terms, this valuation is equivalent to our former definition.
\end{lemma}
\end{comment}

\subsection{Clique-width terms are partition-width terms}

Hence, given the MSO-decidability, we only have to discuss the translation of a term for clique-width to a corresponding/equivalent ``partition-width'' term. For this, let us introduce those terms:

Firstly, a \emph{graded set of colors} is a set $C$ that is partitioned into finite and nonempty sets $C_{n}$ for $n<\omega$. We call colors $c\in C_{n}$ \emph{colors of arity $n$}. Naturally we define a \emph{$C$-coloring} $\chi$ on a structure $\mathfrak{M}$ as a map associating to each tuple $\bold{a}\in M^{n}$ a $n$-ary color, i.e. $\chi(\bold{a})\in C_{n}$.

We will now define update-instructions and associated operations in a signature $\mathcal{Y}_{C, \Sigma}$ where $\Sigma$ is our signature. Note that we will only define a reduced form to make it fit nice and snuggly.

An \emph{update instruction} is a tuple $(n, 2, \overline{I}, \overline{c}, d, S)$ where:
\begin{itemize}
	\item $n < \omega$,
	\item $\overline{I}$ is a partition $\oplus_{i<2}I_{i} = [n]$ of $[n]$ into $2$ classes,
	\item $\overline{c}\in C^{2}$ is a sequence of $2$ colors such that the arity of $c_i$ is $|I_{i}|$,
	\item $d\in C_{n}$ is a color of arity $n$; and
	\item $S\subseteq \Sigma$ is a set of $n$-ary relational symbols.
\end{itemize}
The number $n$ is the arity of the instruction.

Which leads us the definition of an \emph{ordered $2$-update}, which is a set $\Theta$ of update instructions such that it contains for every $n, \overline{I}, \overline{c}$ exactly one update instruction $(n, 2, \overline{I}, \overline{c}, d, S)$. Because of demanding the uniqueness of the update instructions for every $n, \overline{I}, \overline{c}$ we can introduce the notation for the ordered $2$-update as a familiy of functions \[ \Theta_{n}(\overline{I}; \overline{c}) = (d, S)  \text{ iff } (n, 2, \overline{I}, \overline{c}, d, S) \in \Theta \, . \]

With all that said, we will now define the \emph{ordered sum} associated with an ordered $2$-update as follows: For two $C$-colored structures $(\mathfrak{M}_{0}, \chi_{0})$ and $(\mathfrak{M}_{1}, \chi_{1})$ and an ordered $2$-update $\theta$ the ordered sum $(\mathfrak{M}_{0}, \chi_{0}) \oplus_{\Theta}(\mathfrak{M}_{1}, \chi_{1})$ is defined as the $C$-colored structure $(\mathfrak{N}, \eta)$ such that
\begin{itemize}
	\item $\mathfrak{N}$ is the disjoint union of $\mathfrak{M}_{0}$ and $\mathfrak{M}_{1}$,
	\item and the additional application of the following operation afterwards: For every tuple $\bold{a} \in N^{n}$ with $n<\omega$, if $\Theta_{n}(\overline{I}; \overline{c}) = (d, S)$ where \[ I_{i} := \{ k < n \, | \, a_k \in M_{i} \} \quad \text{and} \quad c_{i} := \chi_{i}(\bold{a}|_{I_{i}}) \quad \text{for } i\in \{ 0, 1 \} \] we add $\bold{a}$ to all relations $R\in S$ and set the new color to $\eta(\bold{a})$.
\end{itemize}
Lastly, we introduce our basic $C$-colored structures, acting as our ground terms from the term point-of-view: Let $c_{n}\in C_{n}$ be a sequence of $C$-colors, then we denote by $\overline{c}$ the $C$-colored structure $(\mathfrak{D}, \zeta)$ whith the universe $D := \{ 0 \}$, empty relations $R^{\mathfrak{D}} = \emptyset$ and the unique $n$-tuple in $\mathfrak{D}$ being colored by $c_{n}$ for every $n<\omega$.

We introduce the signature $\mathcal{Y}^{<, 2}_{C, \tau}$ for a graded set of colors $C$ and a signature $\tau$ consisting of all operations of the form $\oplus_{\Theta}$ and $\overline{c}$.
We now can build terms over this signature that evaluate in the obvious way to $C$-colored structures.

As a last but very important preparation, we want to show, that our ``clique-width operations'' can be expressed by the operations of the signature $\mathcal{Y}^{2, <}_{C, \tau}$. For this we note several things: First our clique-width notion (and every clique-width notion in general) just utilizes unary colors, whereas terms from $\mathcal{Y}^{2, <}_{C, \tau}$ uses a range of multi-arity colors. This will not make much difference; intuitively we introduce just one ``dummy color'' for tuples of length bigger then $1$ and only properly utilize the unary ones.

First note, that clique-width terms consist of basic colored structures, disjoint unions, and, at least in the finite case, ``between'' two disjoint unions a finite sequence of the  unary ``add'' and ``recolor'' operations, i.e., given two graphs or colored structures $\mathfrak{M}_{0}, \mathfrak{M}_{1}$ we have something along the lines of \[ f_n ( f_{n-1} (\cdots f_1(\mathfrak{M}_{0}\oplus \mathfrak{M}_{1}))) \, , \] where $f_{1}, \ldots, f_{n}$ are among the unary operations $\recol{a\to b}{}$ and $\add{R, \vl}{}$ with $a, b$ colors, $\vl$ a tuple of colors of length $\arity{R}$ sucht that the given term is now a subterm issued from another disjoint union. Intuitively, we want to roll all those operations (the disjoint union $\mathfrak{M}_{0}\oplus \mathfrak{M}_{1}$ together with $f_n ( f_{n-1} (\cdots f_1()))$ into one operation via the updates). Lastly, note that even an infinite chain of unary operations here should be fine \thomas{(but this is subject to discussion, as it is not strictly needed!)}.

For a relational signature $\tau$ with maximal arity $m$ (if it is infinite we set $m=\omega$) and a finite(!) set of colors $K\subseteq \cols$ (for clique-width!), we define $C$ as a set of graded colors to be the (disjoint) union of the following sets:
\begin{itemize}
	\item $C_{0} = \{ \mathtt{d}_{0} \}$,
	\item $C_{1} = K$,
	\item $C_{i} = K^{i}$ for every $1 < i \le m$ (if $m$ is finite, else $i< m$)
	\item $C_{i} = \{ \mathtt{d}_{i} \}$ for every $m < i < \omega$ if $m$ is finite.
\end{itemize}
The only thing the $C_{i}$ for $i > 1$ do is to keep track of the individual color in the tuples. Nothing more.

\thomas{\textbf{Maybe this should be moved?} In the next step we ``translate'' our constant-symbols/basic-structures: $\unitn$: The associated coloring sequence $\overline{c}$ will consist of the following colors: $c_{0} = \mathtt{d}_{0}$, for $1< i \le m$ we have $c_{i} = (n, \ldots, n)$ and for $m < i$ we have $c_{i} = \mathtt{d}_{i}$. The associated basic-structure (hence the valuation on atomic terms) is obvious to define with the previous definitions.}

\textbf{The subsequent translation will not be that straight forward.}
We collect for the sequence $(f_i)_i$ in the set \[ ADD := \{ i < \omega \, | \, f_i = \add{R, \vl}{} \text{ for some } R\in\tau \text{ and } \vl\in C_{1}^{\arity{R}} \} \] all indices where an add-operation appears. Analogous, for the recoloring operations, let \[ REC := \{ i < \omega \, | \, f_i = \recol{a\to b}{} \text{ for some } a, b \in C_{1}^{\arity{R}} \} \, . \] 

For every $k\in ADD$ we define a binary relation $RT_{k}\subseteq C_{1}\times C_{1}$ called the \emph{recolor-trace} of the $k$-th operation and a set $CS_{k} \subseteq C_{1}\times C_{1}$ called the \emph{color-subsumption relation} of the $k$-th operation (which is an add-operation!) in the following way: Let $REC_{< k}$ be the set of all indices from $REC$ that are smaller then $k$. Let \[ a \to_{REC, <k} b \text{ iff } \exists i\in REC_{< k}. f_{i} = \recol{a\to b}{} \, .  \] 
Let $RT_{k}$ be defined as follows: $(a, b)\in RT_{k}$ iff there exists a maximal $\to_{REC, <k}$ path from $a$ to $b$ \textbf{or} $a = b$.
Hence $RT_{k}$ traces the complete color-changes that happen via recoloring operations until up to the $k$-th operation.
\begin{observation}
	$RT_{k}$ is  a functional binary relation, i.e. for every $a\in C_{1}$ there exists exactly one $b\in C_{1}$ such that $(a,b)\in RT_{k}$.
\end{observation}
\begin{proof}
	trivial.
\end{proof}
Note that we thus can also view $RT_{k}$ as a map $RT_{k}\colon C_{1} \to C_{1}$. This abuse of notation will be used in the future, so we say here that
\[ (a,b)\in RT_{k} \quad \text{iff} \quad RT_{k}(a) = b \] and the previous observation justifies this.
\begin{comment}
Then $RT_{k}$ is the transitive closure of $<_{rec}$. $RT_{k}$ thus collects all the pairs $(a,b)$ up until (and excluding) the $k$-th operation in the sequence, such that every $a$-colored element will be $b$-colored eventually during all the recoloring-operations appearing in the operations-sequence before the $k$-th operation.
\end{comment}
Suppose $f_{k} = \add{R, \vl}{}$, then \[ CS_{k} := \{ (c, l) \in RT_{k} \, | \, \exists i. l = \vl_i \} \, .\]
Now we have every tool together, to define some preliminary updates $\Theta^{(k)}$. The update-instructions come in several flavors.

\textbf{The case $n=0$ is trivial:} We only have $\overline{I} = (\emptyset, \emptyset)$, $\overline{c} = (\mathtt{d}_{0}, \mathtt{d}_{0})$ as arguments available. Hence:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{0}(\overline{I}; \overline{c}) &= (\mathtt{d}_{0}, \emptyset)
	\end{split}
\end{equation*}

\textbf{We now start properly with $n = 1$.} The arguments of $\Theta^{(k)}_{1}(\overline{I}; \overline{c})$ can only have the following forms:
\begin{itemize}
	\item Then $\overline{I} = ({0}, \emptyset)$ or $\overline{I} = (\emptyset, {0})$ and
	\item $\overline{c} = (c, \mathtt{d}_{0})$ or $\overline{c} = (\mathtt{d}_{0}, c)$ respectively with $c\in C_{1}$.
\end{itemize}
So we have to define the $(d,S)$ for $\Theta^{(k)}_{1}(\overline{I}; \overline{c}) = (d,S)$. This we do in the following fashion for which we have two cases:

\textbf{Case 1:} Suppose $R$ is unary. Then $\vl$ is actually a one-tuple $\vl = l\in C_{1}$. Then:
\begin{equation*}
	\begin{split}
	\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \{ R \}) \text{ iff } (c,d)\in RT_{k} \text{ and } d = l \\
	\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \text{ and } d \neq l \\
	\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \{ R \}) \text{ iff } (c,d)\in RT_{k} \text{ and } d = l \\
	\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \text{ and } d \neq l
	\end{split}
\end{equation*}
Those update-instructions do two things simultaneously: First we recolor all elements in one step to the color after every recoloring in our clique-width operation setup until step $k$ is done and secondly, we add at every node that was colored $l$ (either originally or after the previous recolorings) the unary relation $R$.

\textbf{Case 2:} Suppose $R$ is not unary. Then:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \\
		\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k}
	\end{split}
\end{equation*}
Here we just recolor.

\textbf{Suppose now that $m \ge n> 1$.} %Since we do not color tuples or length bigger then $1$, we simulate this by using a ``dead'' color $\mathtt{d}_{n}$. For every update-instruction we will now have $\Theta^{(k)}_{n}(\overline{I}, \overline{c}) = (\mathtt{d}_{n}, S)$, where we only need to concern ourselves with the definition of $S$ for each $n, \overline{I}, \overline{c}$.
Then for every $\overline{I}, \overline{c}$ we do the following: As we only have $2$-partitions of $[n]$, we only need to worry about $\overline{I} = (I_{0}, I_{1})$ and $\overline{c} = (c_{0}, c_{1})$ with $c_{i} \in C_{|I_{i}|}$. We will now define a color $c\in C_{n}$ that aims at ``shuffling" $c_{0}$ and $c_{1}$ together, so that the restriction on the indices in $|I_{0}|$ and $|I_{1}|$ respectively yield the colors $c_{0}$ and $c_{1}$ again, again respectively.For this, we will at first order naturally the numbers in $I_{0}$ and $I_{1}$ respectively by the relation $\prec_{0}$ and $\prec_{1}$. Then we bijectively map $(I_{i}, \prec_{i})$ to the unique initial segment of $(\omega, <)$ via $f_{i}$. $f_{i}$ will also be an order isomorphism. Lastly, interpreting the $c_{i}$ as maps themselves, we note, that their domain is the exact unique initial segment of $(\omega, <)$ that is isomorphic to $(I_{i}, \prec_{i})$. Hence we obtain in the first step two maps $h_{i} := c_{i} \circ f_{i}$ for $i\in \{ 0, 1 \}$ that associate to each number $i\in [n]$ seen as a position the corresponding unary color, which we implicitly keep track of in the case of colors of arity bigger then $1$. By taking the union of those maps (as there domains are disjoint, this is a unique extension of $h_{0}$ by $h_{1}$) we obtain a map $h_{\overline{I}; \overline{c}}$ that maps each ``position'' $i\in [n]$ to its corresponding color. Furthermore, this map gives as the ``shuffling'' we were so intent on looking for. Lastly, we can interpret $h_{\overline{I}; \overline{c}}$ itself as a $n$-tuple and hence by construction $h_{\overline{I}; \overline{c}}\in C_{n}$.

For the following note that after the previous discussion, we can obtain another $n$-tuple of colors from $h_{c}$ by ``applying'' the functional relation $RT_{k}$: $d = RT_{k}(h_{c}) = RT_{k} \circ h_{c}$. This will be our shorthand of describing the state of the individual $1$-colors being tracked by the $n$-color $h_{c}$ after all recoloring operations until the $k$-th operation in our sequence have been applied.
With this we now have only two cases to consider.

\textbf{Case 1:} $R$ is of arity $n$. Then $\vl$ is also a $n$-tuple, more precisely $\vl\in C_{n}$ by definition. Then for every $\overline{I}, \overline{c}$:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (RT_{k}(h_{\overline{I}; \overline{c}}), \{ R \}) \text{ iff }  RT_{k}(h_{\overline{I}; \overline{c}}) = \vl \\
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (d, \emptyset) \text{ iff }  RT_{k}(h_{\overline{I}; \overline{c}}) \neq l
	\end{split}
\end{equation*}

\textbf{Case 2:} $R$ is not of arity $n$. Then for every $\overline{I}, \overline{c}$:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (d, \emptyset)
	\end{split}
\end{equation*}


\textbf{Lastly, for $n> m$}, the update instructions are even simpler. As we do not have any relational symbols of arity $n$ in this case, every update-instruction will give $\emptyset$ for the second component and $\mathtt{d}_{n}$ for the colorings. Formally, for every $\overline{I}, \overline{c}$ we have
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (\mathtt{d}_{n}, \emptyset)
	\end{split}
\end{equation*}

All in all this defines an ordered update $\Theta^{(k)} = \bigcup_{i<\omega}\Theta^{(k)}_{i}$. Unfortunately we are not done yet, since we define for every $k\in ADD$ such an ordered update, but our goal is to define it for the whole sequence. So here our definition will be:
\[ \Theta_{n}(\overline{I}, \overline{c}) := (d, S) \] where
\begin{itemize}
	\item $d = d^{(j)}$ for the smallest $j< \omega$ such that $\Theta^{(j)}_{n}(\overline{I}, \overline{c}) = (d^{(j)}, S_{j})$ and for every $i> k$ we have $\Theta^{(i)}_{n}(\overline{I}, \overline{c}) = (d^{(i)}, S_{i})$ with $d^{(j)} = d^{(i)}$ (in the finite case this is trivial, but in the infinite it is not much more difficult!\footnote{Every $n$-ary color depends on the finitely many colors in $C_{1}$. And the recolor-operations, when only sued for this finite set, can only make finitely many changes to the tuples until they have to stabilize!})
	\item $S = \bigcup_{i< \omega}S_{i}$ where $\Theta^{(i)}_{n}(\overline{I}, \overline{c}) = (d^{(i)}, S_{i})$.
\end{itemize}


Hence:
\begin{proposition}
	Clique-width terms (finite or infinite), can be expressed via the $\mathcal{Y}^{<, 2}_{C, \tau}$-terms.
\end{proposition}
\begin{proof}
	The definition of the valuation for partition-width terms is coincides with ours for the clique-width terms.
\end{proof}


\begin{lemma}
	Every countable structure $\mathfrak{M}$ with a bounded clique-width of $k$ has a bounded partition width.
\end{lemma}
\begin{proof}
	First we translate a clique-width term into a ``partition-width term''. Then we use the number of colors in our translation to obtain bounds on the partition-width via established results.
\end{proof}

\begin{theorem}
	\thomas{$\cw$ is an MSO-friendly width measure.}%Then the MSO-Theory of the class of all countable structures $\mathfrak{A}$ with $\cw{\mathfrak{A}}\le k$ is decidable.
\end{theorem}
\begin{proof}
	Use the result for partition-width with the previous lemma.
	\sebastian{Needs to be made more precise.}
\end{proof}

\begin{comment}
\subsection{Compactness: The countable case}

\thomas{\textbf{TODO:} We want to show the compactness for our clique-width definition in order to lift the more colloquial formulation as used by Grohe-Turan. For this we do in fact need the partition-width. Then we addapt the Courcelle-Compactness prove for partition-width over $2^{< \omega}$}

\thomas{\textbf{Proper TODO:}
\begin{itemize}
	\item Lift notion of syntax-tree to partition-width terms (i.e. $T(\mathcal{Y}^{<, 2}_{C, \tau})$ and $T^{\infty}(\mathcal{Y}^{<, 2}_{C, \tau})$)
	\item introduce order on syntax-trees
	\item show the ascending-chain-interpretation property for partition-width-terms
	\item need layouts
	\item flipping of number of types. Maybe we can use here results from Achim.
\end{itemize}}
\end{comment}

==> ICDT 2023 Updated LaTeXFiles/other/old-prelims.tex <==

\subsection{Logical Preliminaries}

\thomas{Question: Considering, that we have our ``meta-algebra'' over which we not only have the terms but also a algebra of structures, shouldn't we also kind of make a note on that somewhere? Technically we \textbf{do} work with functional signatures there.}
We make use of a first-order language that employs constant symbols, but no other function symbols. We let  $\conset := \{a,b,c,\ldots\}$ be a set of \emph{constants}, $\varset := \{x, y, z, \ldots\}$ be a set of \emph{variables}, and define a \emph{term} to be either a constant or variable. We use $t$, $s$, \etc (possibly annotated) to denote terms and define the set of terms $\termset := \conset \cup \varset$. Moreover, we let $\predset := \{p, q, r, \ldots\}$ be a set of \emph{predicates} containing infinitely many predicates for each arity $k \in \mathbb{N}$, using $\arity{p}$ to denote the arity of a predicate $p$, and refer to a formula of the form $p(t_{1}, \ldots, t_{k})$ (for $p$ a predicate of arity $k$ and $t_{1}, \ldots, t_{k}$ terms) as an \emph{atom}. Our first-order language is defined accordingly.


\begin{definition}[The Language $\lang$] We define the first-order \emph{language} $\lang$ to be the set of formulae generated via the BNF grammar shown below:
$$
A ::= p(t_{1}, \ldots, t_{n}) \ | \ \bot \ | \ A \land A \ | \ A \rightarrow A \ | \ \exists x A \ | \ \forall x A
$$
where $t_{i} \in \conset \cup \varset$ for each $i \in \{1, \ldots, n\}$, $x \in \varset$, and $p \in \predset$ is a predicate symbol such that $\arity{p} = k$.
\end{definition}
\thomas{Do we want to use capital-latin for formulae/sentences? Some prefer to use big-greek (more precisely $\Phi$ and $\Psi$) for sentences and small-greek (i.e. $\varphi$ and $\psi$) for non-sentence formulae (though I personally prefer the small-greek ones across the board for formulae!). This decision might have also an impact on naming rules, where $\varrho$ would be a naturally choice in the ``small-greek'' setting.}
\piotr{I think capital for sentences and small for other is quite clear. It is also nice to use capital letters for queries without explicitly naming free variables. For example $Q$ and $q(\vx)$}
We use $A$, $B$, $C$, $\ldots$ (possibly annotated) to denote formulae from our language and use $A(t/x)$ to denote the formula obtained by substituting the term $t$ for the each free occurrence of $x$ in $A$. Note, we assume that the reader is familiar with the concept of a free variable, bound variable, and occurrences thereof. Given a set of formulae $\formset \subseteq \lang$, we define $\conset(\formset)$, $\varset(\formset)$, $\termset(\formset)$, and $\predset(\formset)$ to be the set of constants, variables, terms, and predicates occurring in the formulae of $\formset$, respectively. When $\formset$ is a singleton $\{A\}$, we simply write $\conset(A)$, $\varset(A)$, $\termset(A)$, and $\predset(A)$, omitting the set brackets.





\begin{definition}[Structure, Environment, Model] We define a \emph{structure} to be an ordered pair $\struc := (\dom,\inter)$, where $\dom$ is a non-empty set called the \emph{domain} and $\inter$ is an \emph{assignment} such that 


\begin{itemize}

\item[(i)] for each constant symbol $c$, $\inter(c) \in \dom$;

\item[(ii)] for each predicate symbol $p$ with $\arity{p} = k$, $\inter(p) \subseteq \dom^{k}$.

\end{itemize}

An \emph{environment} $\env$ is a function such that for each variable $x$, $\env(x) \in \dom$ and we write $\env[d/x]$ to mean the environment $\env$ but where the variable $x$ is mapped to the element $d \in \dom$. Last, we define a \emph{model} to be an ordered pair $\model := (\struc, \env)$, where $\struc$ is a structure and $\env$ is an environment.

\end{definition}


\begin{definition}[Term Assignment] Let  $\model := (\struc, \env)$ be a model with $\struc := (\dom,\inter)$. We define the \emph{assignment} of a term $t$, written $\assign{t}^{\struc}_{\env}$, to be a function $\assign{\cdot}^{\struc}_{\env} : \conset \cup \varset \mapsto \dom$ defined as follows: 

\begin{itemize}

\item[(i)] if $t \in \conset$, then $\assign{t}^{\struc}_{\env} := \inter(t)$;

\item[(ii)] if $t \in \varset$, then $\assign{t}^{\struc}_{\env} := \env(t)$.

\end{itemize}
\end{definition}




\begin{definition}[Semantics] Let $\model := (\struc, \env)$ be a model with $\struc := (\dom, \inter)$.

\begin{itemize}

\item $\model \models p(t_{1}, \ldots, t_{n})$ \ifandonlyif $(\assign{t_{1}}^{\struc}_{\env}, \ldots, \assign{t_{n}}^{\struc}_{\env}) \in \inter(p)$;

\item $\model \not\models\bot$;

\item $\model \models A \land B$ \ifandonlyif $\model \models A$ and $\model \models B$;

\item $\model \models A \rightarrow B$ \ifandonlyif if $\model \models A$, then $\model \models B$;

\item $\model \models \exists x A$ \ifandonlyif there exists an element $d \in \dom$ such that $(\struc,\env[d/x]) \models A$.

\item $\model \models \forall x A$ \ifandonlyif for each element $d \in \dom$, $(\struc,\env[d/x]) \models A$.

\end{itemize}

We say that a formula $A$ is \emph{valid} \ifandonlyif for all models $\model$, $\model \models A$. We say that a multiset $\formset$ of formulae \emph{entails} a multiset $\formsetii$, written $\formset \models \formsetii$, \ifandonlyif for all models $\model$, if $\model \models A$ for all $A \in \formset$, there exists a formula $B \in \formsetii$ such that $\model \models B$.
\end{definition}



\subsection{Existential Rule Preliminaries}

We define a \emph{conjunct} $C(\vec{x})$ to be a conjunction of atoms, where $\vec{x}$ represents the set of all variables $x_{1}, \ldots, x_{n}$ occurring in $C$. Also, we define a \emph{fact} and a \emph{Boolean conjunctive query (BCQ)} to be an existentially closed conjunct, and so, although facts are used to model data and BCQs are used to model queries, both have the same logical form. In the following, we will often view conjuncts, facts, and BCQs as sets of atoms, and will use $C$, $F$, and $Q$ (possibly annotated) to denote each type of entity, respectively.

\begin{definition}[Existential Rule] We define an \emph{existential rule (ER)} to be a formula of the form $R := \forall \vec{x} \forall \vec{y} (B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}))$ where $B := \body(R)$ and $H := \head(R)$ are conjuncts, referred to as the \emph{head} and the \emph{body} of $R$, respectively. The \emph{frontier} of $R$, written $\fr(R)$, is the set of variables $\varset(H) \cap \varset(B) = \vec{y}$.
\end{definition}

In practice, we will omit the universal quantifiers when writing existential rules, i.e. instead of writing $\forall \vec{x} \forall \vec{y} (B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}))$ we will write $B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})$.

\begin{definition}[Substitution, Homomorphism] Given a set of variables $V$ and a set of terms $T$, a \emph{substitution} $\hism$ is a mapping $\hism : V \mapsto T$, and given a formula $A$, $\hism(A)$ is the formula obtained by replacing each occurrence of a free variable $x \in V$ in $A$ with $\hism(x)$.

A \emph{safe substitution} is a bijection from a set of variables $V$ to a set of fresh variables, that is, to a set of variables that do not occur within the formulae one is considering.

Given two facts $F$ and $Q$, a \emph{homomorphism} from $Q$ to $F$ is a substitution $\hism : \varset(Q) \mapsto \termset(F)$ such that $\hism(Q) \subseteq F$. We say that $Q$ \emph{maps to} $F$ \ifandonlyif there exists a homomorphism from $Q$ to $F$.
\end{definition}



\begin{definition}[Forward Chaining Terminology]
\piotr{We need a way to refer to elements of $\sat{R, A}$, I propose to call them {\em atoms}}

\piotr{We need to define what a Datalog rule is.}

\piotr{Make sure that restricted chase vs oblivious chase is explained somewhere.}

\piotr{Make sure that we use restricted chase.}

We say that an existential rule $R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})$ is \emph{applicable} to a fact $F$ \ifandonlyif there is a homomorphism $\hism$ mapping $B(\vec{x},\vec{y})$ to $F$. The \emph{application of $R$ to $F$ according to $\hism$} yields the fact $\fchain{F,R,\hism} = F \cup \hism(\hism'(H(\vec{y},\vec{z})))$, where $\hism'$ is a safe substitution on the variables $\vec{z}$. (NB. We often use $\hism^{\safe}$ to denote the composition $\hism \circ \hism'$.) An application of $R$ to $F$ according to $\hism$ is \emph{redundant} \ifandonlyif $\fchain{F,R,\hism} \equiv F$. 

An \emph{$\calr$-derivation} is a sequence $(F = F_{0}), (R_{0},\hism_{0},F_{1}), \ldots, (R_{n-1},\hism_{n-1},F_{n})$ such that for all $i \in \{0, \ldots, n-1\}$, $R_{i} \in \calr$ and $\pi_{i}$ is a homomorphism from $\body(R_{i})$ to $F_{i}$ such that $F_{i+1} = \fchain{F_{i}, R_{i}, \hism_{i}}$. We say that a fact $F'$ is \emph{$\calr$-derivable} from a fact $F$ \ifandonlyif there exists a derivation sequence starting with $F$ and ending with $F'$.
\end{definition}


\begin{definition}[$k$-Saturation~\cite{BagLecMugSal11}] Let $F$ be a fact with $\calr$ a set of ERs. We define:
$$
\Pi(\calr,F) := \{(R,\hism) \ | \ R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}) \text{ and }
$$
$$
\hism \text{ is a homomorphism from $B$ to $F$.} \}
$$
We define the \emph{direct saturation} of $F$ with $\calr$ to be:
$$
\fchain{F,\calr} := F \cup \bigcup_{(R,\hism) \in \Pi(\calr,F)} \hism^{\safe}(H(\vec{y},\vec{z})) \text{ with } R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})
$$
We define the \emph{$k$-saturation} of $F$ with $\calr$ to be $\ksat{k}{F,\calr}$, which is inductively defined as follows:
$$
\ksat{0}{F,\calr} = F \text{ and, for $i > 0$, } \ksat{i}{F,\calr} = \fchain{\ksat{i-1}{F,\calr},\calr}
$$
Last, we define $\ksat{\infty}{F,\calr} := \bigcup_{k \in \mathbb{N}} \ksat{k}{F,\calr}$.
\end{definition}

A \emph{knowledge base (KB)} $\kb := (F,\calr)$ is an ordered pair composed of a fact $F$ and a finite set of existential rules $\calr$. We use the notation $\kb \models Q$ as shorthand for $F,\calr \models Q$. The \emph{BCQ entailment} problem is the following: given a KB $\kb$ and a BCQ $Q$, is it the case that $\kb \models Q$?









==> ICDT 2023 Updated LaTeXFiles/other/tree-width.tex <==
\medskip \noindent {\bf Treewidth and bounded treewidth sets.}
Let $\inst$ be an instance. A \emph{tree decomposition} of $\inst$ is a (potentially infinite) tree $\tree = (V,E)$ with $V \subseteq 2^{\adom{\inst}}$, where:
\begin{itemize}

\item each $X \in V$ is a set of terms of $\inst$ with $\bigcup_{X \in V} X = \adom{\inst}$;

\item for each atom $p(t_{1}, \ldots,t_{n})$ in $\inst$, there is an $X \in V$ such that $\{t_{1}, \ldots,t_{n}\} \subseteq X$;

\item for each term $t$ in $\inst$, the subgraph of $T$ induced by the nodes $X$ with $t \in X$ is connected.
\end{itemize}

We define the \emph{width} of a tree decomposition to be equal to the largest node minus 1. Last, we define the \emph{treewidth} of an instance $\inst$ to be the minimal width among all of its tree decompositions, and denote the treewidth of $\inst$ as $\treewidth{\inst}$.


%\thomas{``semantic $\bts$?''}
%\begin{definition}[Bounded-treewidth set]

We define a set of existential rules $\ruleset$ to be a \emph{bounded-treewidth set ($\bts$)} \ifandonlyif for any database $\database$, there is a universal model for $\database$ and $\ruleset$ of finite treewidth.\footnote{We note that the term ``\emph{finite} treewidth set'' might be more appropriate and coherent with our terminology, but we stick to the established name. Also, the $\bts$ notion is not used entirely consistently in the literature; it sometimes also refers to structural properties of a specific type of chase. The ``semantic $\bts$'' notion adopted here subsumes all the others.}
%\end{definition}

==> ICDT 2023 Updated LaTeXFiles/other/very-old-clique-width.tex <==
\section{Clique-width and Related Notions}\label{sec:cliquewidth}


\thomas{One thing to think about: I would lobby for following Courcelle and look at \emph{isomorphy-classes} of colored structures! This should also help us make our algebra of colored structures work the way we actually want to.}
We define a \emph{signature} $\sig$ to be a pair $(P,ar)$ such that $P \subseteq \predset$ and $ar$ is the arity function restricted to $P$. When $\sig = (P,ar)$, we write $p \in \sig$ to mean $p \in P$. Moreover, we let $\langsig$ denote the restriction of our language $\lang$ to the use of predicates from the signature $\sig$.

\begin{definition}[Colored Relational Structure] Let $\sig$ be a signature. We define a \emph{relational structure} $\relstr$ to be a pair $(V,\{E_{p} \ | \ p \in \sig\})$ where $V$ is a non-empty set of points called \emph{vertices} and for each $p \in \sig$, $E_{p} \subseteq V^{\arity{p}}$. We define a \emph{colored relational structure} $\crelstr$ to be a pair $(\relstr, \coloring)$ such that $\relstr = (V,\{E_{p} \ | \ p \in \sig\})$ is a relational structure and $\coloring : V \to \mathbb{L}$ is a \emph{coloring} mapping each vertex $V$ to an element of some countably infinite set of colors $\cols$. The set of all finite relational structures over signature $\sig$ and the set of colors $\cols$ will be denoted with $\colstructs$.
\end{definition}

\thomas{A note on ``expressivity'' of ``our'' clique-width notion in relation to partition width: Take an infinite linear order (for example $(\mathbb{Q}, <)$ with the usual ordering). Then add the following inbetweenness relation $R$ to the structure with \[ R = \{ (x,y,z) \, | \, x < y < z \} \]. Then the structure $(\mathbb{Q}, <, R)$ has infinite ``unitarily colored'' width (i.e., our clique-width for example) and finite partition-width. This proofs that partition width is strictly more expressive (or more precisely that \emph{bounded} partition-width captures more structures). I admit, that at the top of my head I do not see a partition-refinement, that might help with getting a finite partition-width here (I am probably just dense and thus see the fact that $\mathbb{Q}$ is dense too as a problem...).}

\begin{definition}[Number of Colors] Let $\crelstr = (\relstr, \coloring)$ be a colored relational structure. The \emph{number of colors} of $\crelstr$ is defined to be $\numcolors{\crelstr} := |image(\coloring)|$.
\end{definition}

Let us now describe how colored relational structures are built from atomic graphs (referred to as \emph{units}) by making use of special operations. We define the \emph{n-unit} colored relational structure as follows:
\thomas{Is ``n-unit colored...'' good? Because we actually color that unit-structure with the color $n$.}
\piotr{I do not understand this comment :/}
\thomas{It sounds like the $n$ is part of the ``unit'' and not associated with the ``colored'' part. I am not sure about a change like saying ``unit $n$-colored'' structure, but that would at least communicate way I felt to make the comment in the first place. The problem with this ``new'' option is however, that now the $n$ seems more rigid then in the proposed version (where having it in front of the unit makes it ``feel'' more dynamic). Still... ``$n$-unit colored'' kind of throws me off a bit.}
\piotr{ok, I would not worry about that, n-unit colored is fine}
\thomas{probably yes. Kind of funny to observe other authors write their texts in real time.}
\piotr{:D}
\piotr{I am going to use your idea from the very long green comment, and this part is going into prelims}\piotr{I am taking it back, I will use what Tim wrote, adjust it and put into preliminaries. The thing is, that we need an "easy to understand" definition rather than "beautiful"}
$$
\unitn := (V,\{E_{p} \ | \ p \in \sig\},\coloring)
$$
where $V = \{\unit\}$, $E_{p} = \emptyset$ for each $p \in \sig$, and $\coloring(\unit) = n$. Furthermore, while constructing colored relational structures, we will use the \emph{disjoint union} $\disun$ of two colored relational structures $\crelstr = (V,\{E_{p} \ | \ p \in \sig\}, \coloring)$ and $\crelstr' = (V',\{E_{p}' \ | \ p \in \sig\}, \coloring')$, defined as follows:
$$
\crelstr \disun \crelstr' = (V \cup V', \{E_{p} \cup E_{p}' \ | \ p \in \sig\}, \coloring \cup \coloring')
$$
where we assume that $V \cap V' = \emptyset$.

The \emph{add} operation, which adds hyper-edges to a colored relational structure given that such hyper-edges satisfy a certain coloring of vertices, requires the use of sequences of natural numbers from $\mathbb{N}^{k}$. We will often use $\vec{n}$ as shorthand for a sequence $(n_{1}, \ldots, n_{k})$ and let $\length{\vec{n}}$ denote the length of the sequence, i.e. for $\vec{n} = (n_{1}, \ldots, n_{k})$, $\length{\vec{n}} = k$. Similarly, we use $\vec{v}$ to represent a sequence of vertices $(v_{1}, \ldots, v_{k})$ from a given (colored) relational structure, and for a coloring $\coloring$, we define $\coloring(\vec{v}) = (\coloring(v_{1}), \ldots, \coloring(v_{k}))$ to be the coloring applied componentwise. We now define the add operation
$$
\add{p}{(V,\{E_{p} \ | \ p \in \sig\},\coloring),\vec{n}} = (V,\{E_{p}' \ | \ p \in \sig\},\coloring)
$$
where $\length{\vec{n}} = \arity{p}$ and
\[
  E_{\relstr}' =
  \begin{cases}
       E_{\relstr} & \text{if $r \in \sig \setminus \{p\}$} \\
       E_{p} \cup \{\vec{v} \in V^{\arity{p}} \ |\ \coloring(\vec{v}) = \vec{n} \} & \text{otherwise.}
  \end{cases}
\]

Last, we define the \emph{recolor} operation which takes a function $h : \mathbb{N} \to \mathbb{N}$ such that $|\{n \in \mathbb{N} \ | \ h(n) \neq n\}|$ is finite and applies it to the coloring of a given colored relational structure:
$$
\recol{h}{(\relstr,\coloring)} = (\relstr,h \fcomp \coloring)
$$

\thomas{In the following block I might have a completely different idea. First of all, if we are talking about terms and the term-algebra it would be a better idea to not bring up any interpretation of the symbols, as terms in the term-algebra are purely syntactic objects devoid of meaning (looking at ``$\unitn$ is among the set...''). We thus have to do the following:
\begin{enumerate}
    \item disambiguate between the \emph{syntactic object} $\unitn$ which is ``just a symbol'' and
    \item its interpretation in the algebra of structures by means of the \emph{structure} $\unitn$.
\end{enumerate}
Then there is the nice property, that the term-algebra (over the generating set described by the constant symbols, which are the ``syntactic'' $\unitn$) is actually \emph{the} free algebra over that generating set (up to isomorphism). This entails that every map from the generating set into every algebra with the same signature (that map has to be the one sending syntactic-$\unitn$ to the structure (or ``semantic'') $\unitn$ to ensure what I will now say about homomorphisms) can be \emph{uniquely} extended to a homomorphism from the term-algebra into and onto our algebra of structures (we assume every structure to be constructible by our operations which they are, especially the finite ones). In fact that very homomorphism \emph{is} our valuation map. The recursive definition is baked into the fact that we work with the term-algebra which is the free-algebra in our setting. Note:
\begin{enumerate}
    \item The term-algebra used here does \emph{not} make use of variable symbols! We are only working on grounded terms.
    \item This might be a hurdle for infinite structures!
    \item Maybe use superscripts to signify interpretations of symbols in a specific structure.
\end{enumerate}
\textbf{Bonus remark:} Refers actually to the Definition of Environment, Model and to some extend Term Assignments. Do we really want to have the environments in the definition of models? They seem to assign to each variable symbol a domain element. This feels like a ``very dynamic'' way to define a model to be a bit euphemistic. On the other hand, $\xi[d/x]$ seems weird, because one could possibly think about $x$ being substituted by $d$ (and some authors use that even the other way round!). And that would not make much sense as $\xi$ is a map with domain the variables!}
Let us now introduce \emph{colored relational structure terms (CRS-terms)}, which will be evaluated over the class of colored relational structures. Such terms are crucial for defining the clique-width of relational structures. Such terms are defined via the following grammar in BNF:
$$
\term ::= \unitn \ | \ \term \disun \term \ | \ \add{p,\vec{n}}{T} \ | \ \recol{h}{T}
$$
where $\unitn$ is among the set $\{\unitn \ | \ n \in \mathbb{N}\}$, $p \in \sig$, $\vec{n}$ is among the finite sequences of natural numbers \thomas{$\vec{n}$ is a sequence of natrual numbers of length arity of $p$!}, and $h$ is a name from a countable set of names (disjoint from all previously mentioned symbols). The value of a term is defined as follows:

\begin{definition}[Value] We define the \emph{value} $\val{\term}$ of a CRS-term $\term$ recursively on the structure of the term such that $\val{\unitn} = \unitn$, $\val{\term \disun \term'} = \val{\term} \disun \val{\term'}$, $\val{\add{p,\vec{n}}{\term}} = \add{p,\vec{n}}{\val{\term}}$, and $\val{\recol{h}{\term}} = \recol{h}{\val{\term}}$.
\end{definition}

We use $\term \sqsubseteq \term'$ to indicate that $\term$ is a sub-term of $\term'$.

\begin{definition}[Clique-width] We define the \emph{clique-width of a CRS-term} as
$$
\cw{\term} = \sup\{\numcolors{\val{\term}} \ | \ \term' \subterm \term \}.
$$
The \emph{clique-width of a relational structure} is defined as
$$
\cw{\relstr} = \inf\{n \in \mathbb{N} \ | \ \exists \term, \exists \coloring (\val{\term} = (\relstr,\coloring) \text{ and } \cw{T} = n)\}.
$$
\end{definition}

\thomas{Though I think that, considered the ``boundedness behavior'' our clique-width definition is equivalent to the one by Courcelle, we probably should still at least note or, even better, proof that they relate ``close enough''. My initial guess is probably again a upper bound of twice ``our'' clique-width and a lower bound of ``our'' clique-width for the ``Courcelle clique-width''. Still we introduce a ``new'' notion of clique-width and it would be good to have that covered.}

\begin{observation}\label{obs:cross-coloring}
Let $\struc$ be a relational structure, let $\coloring : dom(\struc) \to \cols$ and $\coloring' : dom(\struc) \to \cols'$ be two coloring functions, where $\cols$ and $\cols'$ are some sets of colors. If $\cw{\struc, \coloring} = k$ and $\cw{\struc, \coloring'} = k'$ then $\cw{\struc, \coloring^{\times}} \leq k \cdot k'$ where $\coloring^{\times}(a) = (\coloring(a), \coloring'(a))$.
\end{observation}
\begin{proof}
\piotr{easy, TODO}
\end{proof}

\begin{observation}\label{obs:trees_cw_le3}
Let $\struc$ be a (rooted and directed) tree. Then $\cw{\struc} \le 3$.
\end{observation}
\begin{proof}
\thomas{easy, sketched in the following:} Construct the tree in a bottom up fashion. Introduce the leafs as a specific color (let's say \textcolor{blue}{blue}). Then add those nodes in \textcolor{red}{red} that are ``complete parent nodes'' of already ``existing'' nodes (i.e. we want to have subtrees of the whole tree with height $1$ (or $2$ depending on the readers fancy of defining tree-height)). Connect \textcolor{red}{red} to \textcolor{blue}{blue}.
Now do recursively/inductively the following: Add the nest layer of ``complete parents'' in \textcolor{thomas}{green}, connect \textcolor{thomas}{green} to \textcolor{red}{red} and recolor \textcolor{red}{red} to \textcolor{blue}{blue} and \textcolor{thomas}{green} to \textcolor{red}{red}. We are done, when the root of the (directed) tree is added.
All in all we only use $3$ colors and hence have clique-width $\le 3$.
\textbf{Very important note:} The tree structure of the given tree has to be essentially completely copied for the syntax-tree of the clique-width term! This means, we do those iterations on specific disjoint parts of the tree kind of ``in parallel''. The clique-width term will be, written as its syntax tree, only the same tree as the original one if one ``ignores'' the recoloring operations (they just add very short paths between nodes of the tree). That's why it also is just a sketch (because one could get the idea, that all leaves will be connected to one parent note in the first step and the rest would be superfluous drivel).
\end{proof}
\thomas{As a side-note: In the undirected case one could use a result from Courcelle (findable in ``The Book'') which states in that case that the clique-width is bounded on the upper side by $3\cdot 2^{\treewidth{\struc} - 1}$. Then use that the tree-width of a tree is $1$. In general this does not hold for the directed case, but as seen in the sketch, it should work with directed/rooted trees just fine.}

==> ICDT 2023 Updated LaTeXFiles/prelims.tex <==
\section{Preliminaries}\label{sec:preliminaries}

\medskip \noindent {\bf Syntax and formulae.}
We let $\mathfrak{T}$ denote a set of {\em terms}, defined as the union of three countably infinite, 
mutually disjoint sets of \emph{constants}~$\mathfrak{C}$, \emph{nulls}~$\mathfrak{N}$, and \emph{variables}~$\mathfrak{V}$. We use $\const{a}$, $\const{b}$, $\const{c}$, $\ldots$ (occasionally annotated) to denote constants, and use $x$, $y$, $z$, $\ldots$ (occasionally annotated) to denote both nulls and variables.
% in an ambiguous manner, specifying when a symbol is used to represent one as opposed to the other. 
A \emph{signature}~$\sig$ is a finite set of \emph{predicate symbols} (called \emph{predicates}), which are capitalized ($\epred$, $\rpred$, $\ldots$).
Throughout the paper, we assume a fixed signature $\sig$, unless stated otherwise. For each predicate~\mbox{$\rpred \in \sig$}, we denote its 
\emph{arity} with~$\arity{\rpred}$. \prm{We speak of \emph{binary signatures} whenever $\sig$}\pin{We say $\sig$ is \emph{binary} if it} contains only predicates of arity ${\leq}2$. We assume $\sig$ to contain a special, ``universal'' unary predicate $\top$, assumed to hold of every term.\footnote{Assuming the presence of such a built-in \emph{domain predicate} $\top$ does not affect our results, but it allows for a simpler and more concise presentation.} 
An \emph{atom} over~$\sig$ is an expression  of the form~$\rpred(\vt)$, where~$\vt$ is an~$\arity{\rpred}$-tuple of terms. \prm{A \emph{ground atom} is an atom~$\rpred(\vt)$, where~$\vt$ consists only of constants}\pin{If $\vt$ consists only of constants, then $\rpred(\vt)$ is a \emph{ground atom}}.
An \emph{instance}~$\instance$ over~$\sig$ is a (possibly countably infinite)
set of atoms over constants and nulls, whereas a~$\emph{database}$~$\database$ is
a finite set of ground atoms. The \emph{active domain}~$\adom{\mathcal{X}}$ 
of a %n instance~$\instance$ 
 set of atoms $\mathcal{X}$ is the set of terms \prm{(i.e., constants and nulls) }appearing in the atoms of $\mathcal{X}$.\prm{Clearly, databases and instances can be seen as model-theoretic structures, so we use $\models$ to indicate satisfaction as usual.} Moreover, as instances over binary signatures can be viewed as directed edge-labelled graphs\prm{ whose edges are typed with predicates}, we often use graph-theoretic terminology when discussing such objects. 

\renewcommand{\smallldots}{...\,}

\medskip \noindent {\bf Homomorphisms\prm{ and substitutions}.}\prm{A \emph{substitution} is a partial function over~$\mathfrak{T}$.}
Given sets $\mathcal{X}$, $\mathcal{Y}$ of atoms, a~\emph{homomorphism} from $\mathcal{X}$ to $\mathcal{Y}$ is a \prm{substitution}\pin{mapping} \prm{$h$ from the terms of~$\mathcal{X}$ to the terms of~$\mathcal{Y}$}\pin{\mbox{$h:\adom{\mathcal{X}}\to\adom{\mathcal{Y}}$}} that satisfies:
(i)~\prm{$\rpred(h(t_1), \smallldots, h(t_n)) \in \mathcal{Y}$, for all~$\rpred(t_1, \smallldots, t_n) \in \mathcal{X}$}\pin{$\rpred(h(\vt)) \in \mathcal{Y}$, for all~$\rpred(\vt) \in \mathcal{X}$}%
, 
and 
(ii)~$h(\const{a}) = \const{a}$, for each~$\const{a} \in \mathfrak{C}$%
. 
$\mathcal{X}$ and $\mathcal{Y}$ are \emph{homomorphically equivalent} (written $\mathcal{X} \equiv \mathcal{Y}$) \iffi homomorphisms exist from $\mathcal{X}$ to $\mathcal{Y}$ and from $\mathcal{Y}$ to $\mathcal{X}$.
A~homomorphism $h$ is an \emph{isomorphism} \iffi it is bijective and $h^{-1}$ is also a homomorphism. 
An instance~$\instance'$ is an \emph{induced sub-instance} of an instance $\instance$ \iffi (i) $\instance' \subseteq \instance$ and (ii) \prm{if $\rpred(t_1,\smallldots,t_n) \in \instance$ and $t_1,\smallldots,t_n \in \adom{\instance'}$, then $\rpred(t_1,\smallldots,t_n) \in \instance'$}\pin{if $\rpred(\vt) \in \instance$ and $\vt \subseteq \adom{\instance'}$, then $\rpred(\vt) \in \instance'$}.
\renewcommand{\smallldots}{\ldots}

\medskip \noindent {\bf Existential rules.}
An \emph{(existential) rule} $\rho$ is a first-order sentence $\forall{\vx\vy} \; \phi(\vx, \vy)
\rightarrow \exists{\vz} \; \psi(\vy, \vz)$,
where~$\vx$, $\vy$, and $\vz$ are mutually disjoint tuples of variables, and both 
the \emph{body}~$\phi(\vx, \vy)$ and the \emph{head}~$\psi(\vy, \vz)$ of~$\rho$  (denoted with~$\body(\rho)$ and~$\head(\rho)$, respectively) are conjunctions (possibly empty, sometimes \prm{denoted }\pin{seen }as sets) of atoms \prm{containing}\pin{over} %constants and 
 the indicated variables. The \emph{frontier} $\fr(\rho)$ of $\rho$ is the set of variables $\vy$ shared between the body and the head. \prm{For better readability, we}\pin{We o}ften omit the universal quantifiers prefixing existential rules. 
%
\prm{We say that a}\pin{A} rule~$\rho$ is \mbox{(i)~\emph{$n$-ary}} \iffi all predicates appearing in~$\rho$ are of arity at most~$n$, \mbox{(ii) \emph{single-headed}} \iffi $\head(\rho)$ contains \prm{at most one atom}\pin{a single atom}, (iii) \emph{datalog} \iffi $\rho$ does not contain an existential quantifier\prm{, and (iv) \emph{non-datalog} \iffi $\rho$ contains an existential quantifier}\pin{ (otherwise \emph{non-datalog})}. We call a finite set of existential rules $\ruleset$ a {\em rule set}. Satisfaction of a rule $\rho$  (a rule set $\ruleset$) by an instance $\instance$ is defined as usual and is written $\instance \models \rho$ ($\instance \models \ruleset$, respectively). Given a database $\database$ and a rule set $\ruleset$, we define the pair $(\db,\ruleset)$ to be a \emph{knowledge base}, and define an instance $\instance$ to be a \emph{model} of \prm{the knowledge base (i.e., of $\database$ and $\ruleset$)}\pin{$(\database, \ruleset)$}, written $\instance\models (\database,\ruleset)$, \iffi $\database \subseteq \instance$ and $\instance \models \ruleset$. A model $\instance$ of $(\database,\ruleset)$ is called \emph{universal} \iffi there is a homomorphism from $\instance$ into every model of $(\database,\ruleset)$. 

\medskip \noindent {\bf Rule application and Skolem chase.} A rule $\rho\,\, = \,\, \phi(\vx,\vy) \rightarrow \exists \vz \psi(\vy,\vz)$ is \emph{appli\-ca\-ble} to an instance $\instance$ \ifandonlyif there is a homomorphism $\hism$ \prm{mapping}\pin{from} $\phi(\vec{x},\vec{y})$ to $\instance$. We then call $(\rho, \hism)$ a \emph{trigger} of $\instance$.
The \emph{application} of a trigger $(\rho, \hism)$ in $\instance$ yields the instance $\fchain{\inst,\rho,\hism} = \instance \cup {\bar\hism}(\psi(\vec{y},\vec{z}))$, where $\bar\hism$ extends $\hism$, mapping each variable $z$ from $\vz$ to a null denoted \smash{$z_{\rho,\hism(\vy)}$.} 
%As $\bar\hism(\psi(\vec{y},\vec{z}))$ is unique for a given rule and mapping of its frontier variables,%
Note that this entails
$\fchain{\fchain{\inst,\rho,\hism},\rho,\hism'} = \fchain{\inst,\rho,\hism}$ whenever $\hism(\vy) = \hism'(\vy)$. 
%Consequently $\bar\hism(\psi(\vec{y},\vec{z}))$ is unique for a given rule and mapping of its frontier variables\prm{, %with the effect that applying $\rho$ twice with homomorphisms that agree on the frontier variables does not produce more %atoms, that is,}\pin{,}
%and therefore $\hism(\vy) = \hism'(\vy)$ implies $\fchain{\fchain{\inst,\rho,\hism},\rho,\hism'} = %\fchain{\inst,\rho,\hism}$. 
%
Moreover, applications of different rules or the same rule with different frontier-mappings are independent, so their order is irrelevant. Hence we can define the parallel one-step application of all applicable rules as
$$\ksat{1}{\inst,\ruleset} = 
\hspace{-9ex}\bigcup_{\hspace{9ex}\rho\in \ruleset,\,(\rho, \hism) \text{\,trigger of\,} \instance}\hspace{-9ex} 
\fchain{\inst,\rho,\hism}.$$     
%
Then, we define the \emph{(breadth-first) Skolem chase sequence} by letting 
$\ksat{0}{\inst,\ruleset} = \inst$ and $\ksat{i+1}{\inst,\ruleset} = \ksat{1}{\ksat{i}{\inst,\ruleset}, \ruleset}$, ultimately obtaining the \emph{Skolem chase} $\sat{\inst,\ruleset} = \bigcup_{i\in \mathbb{N}} \ksat{i}{\inst,\ruleset}$. We note that the Skolem chase of a countable instance is countable, as  is the number of overall rule applications performed to obtain $\sat{\inst,\ruleset}$. 

\begin{comment}
\piotr{Fair sequence!}
\medskip \noindent {\bf Restricted chase} 
Given an instance $\inst$ and a set of existential rules $\ruleset$ we define $\ksat{0}{\inst,\ruleset}$ as $\inst$. Given $\ksat{i}{\ruleset, \inst}$ we enumerate the set of triggers in $\ksat{i}{\ruleset, \inst}$ and apply them one by one, denoting the resulting structure as $\ksat{i + 1}{\inst,\ruleset}$. Note that during this process some triggers may become satisfied prior to being reached in the enumeration; when this happens, we do not apply the satisfied trigger. Moreover, each trigger will become satisfied at some point in time, as we only consider countably infinite instances. We define the {\em restricted chase} $\sat{\ruleset, \inst}$ of $\ruleset$ and $\inst$ as:
$$\bigcup_{i\in \mathbb{N}} \ksat{i}{\ruleset, \inst}$$

The sequence of triggers applied to build $\sat{\ruleset, \inst}$ is called a {\em derivation}. It should be clear that there might be multiple derivations resulting in the same final structure.
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ROLLED BACK, INTEGRATED AND ADJUSTED; PLEASE DON'T TOUCH WITHOUT TALKING BACK %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip \noindent {\bf (Unions of) conjunctive queries and their entailment.}
A {\em conjunctive query} (CQ) is a  formula $\query(\vy) = \exists \vx \, \phi(\vx, \vy)$ with $\phi(\vx, \vy)$ a conjunction (sometimes written as a set) of atoms over the variables from $\vx,\vy$ and constants.
 The variables from $\vy$ are called {\em free}. A \emph{Boolean} CQ (or BCQ) is a CQ with no free variables.
 A \emph{union of conjunctive queries} (UCQ) $\psi(\vy)$ is a disjunction of CQs with free variables $\vy$. 
 We will treat UCQs as sets of CQs. %{\bf In our paper we will consider mostly Boolean queries (with constants)} with the reason being notational convenience. 
\prm{Satisfaction of a BCQ $\query = \exists \vx \, \phi(\vx)$ in an instance $\instance$ is defined as usual and coincides with the existence of a homomorphism from $\phi(\vx)$ to $\instance$.}\pin{A BCQ $\query = \exists \vx \, \phi(\vx)$ is satisfied in an instance $\instance$ if there exists a homomorphism from $\phi(\vx)$ to~$\instance$.} $\instance$ satisfies a union of BCQs if it satisfies at least one of its disjuncts.
An instance $\inst$ and rule set $\ruleset$ \emph{entail} a BCQ $\query = \exists \vx \, \phi(\vx)$, written $(\inst, \ruleset) \models \query$  \iffi $\phi(\vx)$ maps homomorphically into every model of $\inst$ and $\ruleset$. This coincides with  the existence of a homomorphism from $\phi(\vx)$ into any universal model of $\inst$ and $\ruleset$ (e.g., the Skolem chase $\sat{\inst, \ruleset}$).

\medskip \noindent {\bf Rewritings and finite-unification sets.}
Given a rule set $\ruleset$ and a CQ $\query(\vy)$, we say that a UCQ $\psi(\vy)$ is a {\em rewriting} of $\query(\vy)$ under the rule set $\ruleset$ \ifandonlyif for any database $\database$ and any tuple of its elements $\vec{\const{a}}$ the following holds: 
$\sat{\database,\ruleset} \models \query(\vec{\const{a}}) \ \ifandonlyif \ \database \models \psi(\vec{\const{a}}).$
%
A rule set $\ruleset$ is a {\em finite-unification set} ($\fus$) \iffi for every CQ, there exists a UCQ rewriting \cite{BagLecMugSal11}. This property is also referred to as \emph{first-order rewritability}.
%
If a rule set $\ruleset$ is $\fus$, then for any given CQ~$\query(\vy)$, we fix one of its rewritings under $\ruleset$ and denote it with $\rewrs{\ruleset}{\query(\vy)}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ROLLED BACK, INTEGRATED AND ADJUSTED; PLEASE DON'T TOUCH WITHOUT TALKING BACK %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\medskip \noindent {\bf Treewidth and bounded-treewidth sets.}
Let $\inst$ be an instance. A \emph{tree decomposition} of $\inst$ is a (potentially infinite) tree $\tree = (V,E)$, where:
\begin{itemize}

\item  $V \subseteq 2^{\adom{\inst}}$, that is, each node $X \in V$ is a set of terms of $\inst$, and $\bigcup_{X \in V} X = \adom{\inst}$,

\item for each $\rpred(t_{1}, ...\,,t_{n}) \in \inst$, there is an $X \in V$ with $\{t_{1}, ...\,,t_{n}\} \subseteq X$,

\item for each term $t$ in $\inst$, the subgraph of $T$ induced by the nodes $X$ with $t \in X$ is connected.
\end{itemize}

The \emph{width} of a tree decomposition is set to be the maximum over the sizes of all its nodes minus $1$, if such a \prm{finite} maximum exists; otherwise, it is set to $\infty$. Last, we define the \emph{treewidth} of an instance $\inst$ to be the minimal width among all of its tree decompositions, and denote the treewidth of $\inst$ as $\treewidth{\inst}$.
%
A set of rules $\ruleset$ is a \emph{bounded-treewidth set} ($\bts$) \ifandonlyif for any database $\database$, there is a universal model for $(\database,\ruleset)$ of finite treewidth.\footnote{The term ``\emph{finite}-treewidth set'' would be more fitting and in line with our terminology, but we stick to the established name. Also, the $\bts$ notion is not used entirely consistently in the literature; it sometimes refers to structural properties of a specific type of chase. The ``semantic $\bts$'' notion adopted here subsumes all the others.}



\begin{comment}
Let $\cols$ be any countable infinite set of colors (the set of natural numbers or the set of all finite instances could be used here). We define the {\em colored instance} as a pair $(\inst, \coloring)$ where $\inst$ is an instance and $\coloring$ is a coloring function from its terms to $\cols$.

Given a set of colors $\cols$ and a signature $\sig$ let us describe a process that later will help us to define the notion of cliquewidth.

Let $\unitn$ be a single node\footnote{while we generally disallow isolated nodes in instances but here we make a small convenient exception.} colored with $n \in cols$. We are allowed to take the \emph{disjoint union} $(\inst, \coloring) \disun (\inst', \coloring')$ of two colored instances -- we assume that the sets of terms of $(\inst, \coloring)$ $(\inst', \coloring')$ have an empty intersection.  

Given a relational symbol $A \in \sig$ and a tuple of colors $\vl \in \cols^{\arity{A}}$ we define $\add{A,\vl}{\inst, \coloring}$ as $(\inst \cup \mathcal{A}, \coloring)$ where $$\mathcal{A} = \set{A(\vt) \;|\; \vt \in \aadom{\inst}^{\arity{A}} \wedge \coloring(\vt) = \vl}.$$

Last, we define the \emph{recolor} operation which takes a function $h : \mathbb{N} \to \mathbb{N}$ such that $|\{n \in \mathbb{N} \ | \ h(n) \neq n\}|$ is finite and applies it to the coloring of a given colored instance:
$$
\recol{h}{(\relstr,\coloring)} = (\relstr,h \fcomp \coloring)
$$

It should be clear that this procedure can be denoted with terms from the following grammar $\mathfrak{L}$:
$$
\term ::= \unitn \ | \ \term \disun \term \ | \ \add{p,\vec{n}}{T} \ | \ \recol{h}{T}
$$
with the associated value $\value{T}$ of the term $T$ being the resulting colored instance.


\begin{observation}\label{obs:cross-coloring}
Let $\struc$ be a relational structure, let $\coloring : \mathrm{dom}(\struc) \to \cols$ and $\coloring' : \mathrm{dom}(\struc) \to \cols'$ be two coloring functions, where $\cols$ and $\cols'$ are some sets of colors. If $\cw{\struc, \coloring} = k$ and $\cw{\struc, \coloring'} = k'$ then $\cw{\struc, \coloring^{\times}} \leq k \cdot k'$ where $\coloring^{\times}(a) = (\coloring(a), \coloring'(a))$.
\end{observation}
\begin{proof}
\piotr{easy, TODO}
\end{proof}

\begin{observation}\label{obs:trees_cw_le3}
Let $\struc$ be a (rooted and directed) tree. Then $\cw{\struc} \le 3$.
\end{observation}
\begin{proof}
\thomas{easy, sketched in the following:} Construct the tree in a bottom up fashion. Introduce the leafs as a specific color (let's say \textcolor{blue}{blue}). Then add those nodes in \textcolor{red}{red} that are ``complete parent nodes'' of already ``existing'' nodes (i.e., we want to have subtrees of the whole tree with height $1$ (or $2$ depending on the readers fancy of defining tree-height)). Connect \textcolor{red}{red} to \textcolor{blue}{blue}.
Now do recursively/inductively the following: Add the nest layer of ``complete parents'' in \textcolor{thomas}{green}, connect \textcolor{thomas}{green} to \textcolor{red}{red} and recolor \textcolor{red}{red} to \textcolor{blue}{blue} and \textcolor{thomas}{green} to \textcolor{red}{red}. We are done, when the root of the (directed) tree is added.
All in all we only use $3$ colors and hence have clique-width $\le 3$.
\textbf{Very important note:} The tree structure of the given tree has to be essentially completely copied for the syntax-tree of the clique-width term! This means, we do those iterations on specific disjoint parts of the tree kind of ``in parallel''. The clique-width term will be, written as its syntax tree, only the same tree as the original one if one ``ignores'' the recoloring operations (they just add very short paths between nodes of the tree). That's why it also is just a sketch (because one could get the idea, that all leaves will be connected to one parent note in the first step and the rest would be superfluous drivel).
\end{proof}
\thomas{As a side-note: In the undirected case one could use a result from Courcelle (findable in ``The Book'') which states in that case that the clique-width is bounded on the upper side by $3\cdot 2^{\treewidth{\struc} - 1}$. Then use that the tree-width of a tree is $1$. In general this does not hold for the directed case, but as seen in the sketch, it should work with directed/rooted trees just fine.}
\end{comment}

==> higher-arities-previous.tex <==
\section{Results for Multi-Headed Rules}\label{sec:higher-arity}

We will now prove \cref{thm:higher-arity} implying that for multi-headed rules, $\fus$ is no longer subsumed by $\fcs$. To this end, we exhibit a $\fus$ rule set which may unavoidably lead to universal models of infinite cliquewidth. 

We let $\sigi = \set{\hpred, \vpred, \origin}$ be a signature where $\hpred$ and $\vpred$ are binary predicates and $\origin$ is a unary predicate. Let us define $\rsgrid$ to be the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} & \top & \rightarrow \exists x \; (\hpred(x,x) \land \vpred (x,x)) \\[0.5ex]
\text{(grow)} & \top & \rightarrow \exists y \exists y'\; (\hpred(x,y) \land \vpred (x,y')) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists y' \; (\hpred(x',y') \land \vpred(y,y'))
\end{array}
$$

We make use of $\rsgrid$ to establish \cref{thm:higher-arity} (see \cref{sect:main-results}), whose proof is split into two parts. First, we provide a database $\dbg$ to form a knowledge base $(\dbg, \rsg)$ for which no universal model of finite cliquewidth exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\subsection{$\rsgrid$ is not a finite-cliquewidth set}


We devote this section to establishing the subsequent lemma, which serves as one of the two main lemmata sufficient to conclude \cref{thm:higher-arity}.


\begin{lemma}\label{lem:no-universal-model-cw}
Let $a$ be a constant and let $\dbg = \set{\origin(a)}$ be a database. Then, no universal model of finite cliquewidth exists for $\kbaseg$.
\end{lemma}


With the aim of establishing the lemma above, we define the instance $\ginf$ below, where $a$ is a constant and $x_{i,j}$ and $y$ are nulls for $i,j \in \mathbb{N}$. To provide the reader with further intuition, a graphical depiction of $\ginf$ is given in \cref{fig:ginf}.
\begin{eqnarray*}
\ginf & = & \{\origin(a),\hpred(a,x_{1,0}),\vpred(a,x_{0,1}),\hpred(y,y),\vpred(y,y)\} \\
 & & \cup \big\{\hpred(x_{i,j},x_{i+1,j}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} \\
 & & \cup \big\{\vpred(x_{i,j},x_{i,j+1}) \ | \  (i,j) \in (\mathbb{N} \times \mathbb{N}) \setminus \{(0,0)\} \big\} 
\end{eqnarray*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/ginf.pdf}
    \caption{ The instance $\ginf$.}
    \label{fig:ginf}
\end{figure}

It is straightforward to show that $\ginf$ serves as a model of $\kbaseg$, and a routine exercise to prove that $\ginf$ is universal. Hence, we have the following:

\begin{observation}\label{obs:ginf-is-universal-model}
$\ginf$ is a universal model of $\kbaseg$.
\end{observation}

%\begin{proof} Let $\model = (\dom,\inter)$ be any model of $\kbaseg$. Then, it follows that (i) $\inter(a) \in \inter(\origin)$, (ii) there exists some $d_{0} \in \dom$ such that $d \in \inter[d/x](\hpred) \cap \inter[d/x](\vpred)$, (iii) for any $d_{1} \in \dom$, there exist $d_{2}, d_{3} \in \dom$ such that $(\inter(d_{1})\inter(d_{2}) \in \inter(\hpred)$ and $(\inter(d_{1})\inter(d_{3}) \in \inter(\vpred)$, and (iv) for any $d_{4}, d_{5}, d_{6} \in \dom$, if $(d_{4},d_{5}) \in \inter(\hpred)$ and $(d_{4},d_{6}) \in \inter(\vpred)$, then there exists a $d_{7} \in \dom$ such that 
%\end{proof}


%It is well known~\cite{} that all grid like structures have infinite cliquewidth. 
%\thomas{The original proof for (undirected!) grids w.r.t. cliquewidth was done in \cite[\thm~4]{GolumbicRot99}, where grids are considered as (undirected) graphs. We probably(?) should be ``careful'' here since we have two types of edges and are in the directed setting. It's not that it wouldn't work or anything... But we probably should make a short argument why it does hold here.}

%It is well known that infinite grids over a signature consisting of single binary relation have infinite cliquewidth (see \cite[\thm~4]{GolumbicRot99} for the reference). Consider the following:

%It is known that \thomas{Change to finite!} infinite grids constructed over a signature with a single binary relation have infinite cliquewidth~\cite[\thm~4]{GolumbicRot99}. By making use of this fact, and the subsequent two claims, we can prove \cref{fact:grid-has-unbounded-cw} below.

It is known that the cliquewidth of an $n \times n$ grid tends to infinity as $n$ tends to infinity~\cite[\thm~4]{GolumbicRot99}, entailing that any infinite grid will have an infinite cliquewidth since the cliquewidth of any instance bounds the cliquewidth of any induced sub-instance from above. By making use of this fact, along with the subsequent two, we can prove \cref{fact:grid-has-unbounded-cw} below.

\begin{fact}
        Let $\sig$ be a binary signature, $\epred$ be a binary relational symbol, 
        $\inst$ be an instance over $\sig$, and $\inst' = \set{\epred(t,t') \ | \ \rpred(t,t') \in \inst, \rpred \in \sig}$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}

    
\begin{fact}
        Let $\sig$ be a signature consisting of a single binary relational symbol $E$, let $\inst$ be an instance over $\sig$, and let $\inst' = \set{\epred(t',t) \ | \ \epred(t,t') \in \inst} \cup \inst$. Then, $\cw{\inst} \geq \cw{\inst'}$.
\end{fact}



\begin{observation}\label{fact:grid-has-unbounded-cw}
$\ginf$ has an infinite cliquewidth.
\end{observation}
\begin{proof} The observation follows from the previous two facts, the fact that infinite grids have infinite cliquewidth, and the fact that adding a set of the form $\{\origin(a), \hpred(y, y), \vpred(y, y) \}$ with $a$ a constant and $y$ a null to any instance does not lower its cliquewidth.
\end{proof}

We now leverage the above result to demonstrate that {\em every} universal model of $\kbaseg$ has an infinite cliquewidth. Observe that if we consider any homomorphism from $\ginf$ to itself, then (i) the null $y$ must be mapped to itself as no other terms are associated with loops, and (ii) the constant $a$ must be mapped to itself, thus anchoring the image of $\ginf$ under the homomorphism at the origin of the grid (indicated by $A(a)$) shown in \cref{fig:ginf}, thus ensuring that each term of the grid will map to itself accordingly. It follows that any homomorphism from $\ginf$ to itself will be the identity function, giving rise to the following observation.

\begin{observation}\label{obs:identity}
If $h: \ginf \to \ginf$ is a homomorphism then $h$ is the identity.
\end{observation}

We now make use of the above observation to show that every universal model of $\kbaseg$ contains a sub-instance that is isomorphic to $\ginf$, thus ensuring that every universal model of $\kbaseg$ is of infinite cliquewidth (by \cref{fact:grid-has-unbounded-cw} and the fact that the cliquewidth of an instance is greater than or equal to the cliquewidth of any induced sub-instance). From this lemma, we may conclude \cref{lem:no-universal-model-cw}.

\begin{lemma}
Every universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$.
\end{lemma}

\begin{proof}
Let $\unimod$ be a universal model of $\kbaseg$. As $\ginf$ is a universal model (by \cref{obs:ginf-is-universal-model} above), we know that two homomorphisms $h\colon \ginf \to \unimod$ and $h'\colon \unimod \to \ginf$ exist between $\unimod$ and $\ginf$. Let us consider the homomorphism $h' \circ h$. By \cref{obs:identity}, the homomorphism $h'\circ h$ is the identity on $\ginf$, implying that $h$ is injective. Furthermore, $h$ is reflective, and hence, constitutes an embedding. To show this, suppose that $p\in\sigi$ and let $\vt$ be a tuple of length $\arity{p}$ from $\ginf$. If $p(h(\vt))$ holds in $\unimod$ , then $p((h' \circ h)(\vt))$ holds in $\ginf$, but since $h'\circ h$ is the identity on $\ginf$, we immediately obtain that $p(\vt)$  holds in $\ginf$. Finally, note that the image of $\ginf$ under $h$ serves as the induced sub-instance of $\unimod$ that is isomorphic to $\ginf$, completing the proof.
\end{proof}



\subsection{$\rsgrid$ is a finite unification set}

As we have now shown that $\rsgrid$ is not a finite-cliquewidth set, we focus our attention on demonstrating \cref{lem:rsg-is-fus}, which is stated below, and from which we may conclude the final main result (\cref{thm:higher-arity}).

\begin{lemma}\label{lem:rsg-is-fus}
$\rsg$ is $\fus$.
\end{lemma}

As the rule $(loop)$ is a member of $\rsg$, every BCQ that is free of constants can be trivially re-written, implying the following:

\begin{observation}\label{obs:bcq-no-const-trivial}
Every BCQ that is free of constants is FO-rewritable with respect to $\rsg$.
\end{observation}

%\piotr{Here is a link for Xrewrite \url{https://arxiv.org/pdf/1405.2848.pdf}}

Showing that a provided rule set is $\fus$ is a notoriously difficult task.\footnote{This should not be too surprising however, as being $\fus$ is an undecidable property~\cite{BagLecMugSal11}.} To this end, we hand-tailor a rewriting algorithm to be used for the proof of~\cref{lem:rsg-is-fus}. However, one can refer to existing rewriting algorithms, e.g. XRewrite~\cite{GotOrsPie14}, for additional intuition. Finally, it is important to note that the proof closely follows the ideas provided in \cite{OstMarCarRud22}.


\subsection{Necessary definitions}

%As we are considering a binary signature, we will treat queries as graphs with the company of standard graph theoretic notions. \thomas{Does this suffice or would Reviewer 2 state: ``The term \emph{graph} has not been defined. Suggest strong reject.''?}

%Since each CQ can be viewed as an instance, and each instance can be viewed as a structure (see \tim{Sect ?}), we will hereafter interpret queries as their corresponding structures. Moreover, we note that since the signature $\sigi$ contains only binary predicates, we can view queries as directed, binary graphs.

We first introduce special queries, referred to as \emph{marked queries}, which are queries supplemented with a set of markings, the significance of which, is to keep track of what terms of the CQs are mapped to constants in a given database throughout the course of rewriting. A marked CQ is defined to be a pair $(q, M)$ where $q$ is a CQ and the set of markings $M$ is a subset of terms (i.e. variables and constants) of $q$. Given an instance $\inst$ we say that $\inst \models (q,M)$ $\iffi$ there exists a homomorphism $h$ mapping $q$ to $\inst$ such that for every term $t$ of $q$ we have $t \in M$ $\iffi$ $h(t)$ is a constant in $\inst$.

We now make a useful observation, which follows by considering the structures that arise when applying the rules from $\rsgrid$ to any given database. Afterward, we show that marked queries take on a special form when interpreted on the instance $\sg$, where $\db$ is an arbitrary database.

\begin{observation}\label{obs:buildup-for-properly-marked-chase}
Let $\db$ be a database. Then,
\begin{itemize}
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom of $\sg$ and $t'\in \adom{\db}$, then $t\in \adom{\db}$;
    \item if there is a cycle $C \subseteq \sg$ that contains at least one constant, then $C \subseteq \db$;
    \item if $\rpred(t_1,t'), \rpred(t_2,t') \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1\in  \adom{\db}$, then $t_2\in  \adom{\db}$;
    \item if $\rpred(a,t), \rpred(b,t) \in \sg$ with $\rpred\in\{\hpred, \vpred\}$ and $a\neq b$ are constants, then $t$ is a constant.
\end{itemize}
\end{observation}

Keeping the above observation in mind, we define the notion of a {\em properly marked CQ}.

\begin{definition}\label{def:properly-marked}
A marked CQ $(q, M)$ is {\em properly marked} when:
\begin{itemize}
    \item if $a$ is a constant in $q$, then $a \in M$;
    \item if $\hpred(t,t')$ or $\vpred(t,t')$ is an atom in $q$ and $t' \in M$, then $t \in M$;
    \item if there is a cycle $C$ in $q$ that contains at least one constant, then all terms of $C$ are contained in $M$;
    \item if $\rpred(t_1,t')$ and $\rpred(t_2,t')$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $t_1 \in M$, then $t_2 \in M$;
    \item if $\rpred(a,t)$ and $\rpred(b,t)$ are two atoms in $q$ with $\rpred\in\{\hpred, \vpred\}$ and $a\neq b$ are constants, then $t \in M$.
\end{itemize}
\end{definition}

\begin{observation}\label{obs:query-extendable-properly-marked}
If $\sg \models q$, then there exists a set of markings $M$ such that $(q,M)$ is properly marked and $\sg \models (q,M)$.
\end{observation}

\begin{proof} Suppose that $\sg \models q$. Then, we know that a homomorphism $h$ exists mapping terms from $q$ into $\sg$. Let $M$ be the set of terms from $q$ such that $h(t)$ is mapped to a constant in $\sg$. One can readily check if $(q,M)$ is properly marked, and if not, add the terms from $q$ to $M$ accordingly until a properly marked CQ $(q,M')$ is constructed such that $\sg \models (q,M)$.
\end{proof}

From \cref{obs:buildup-for-properly-marked-chase} and \cref{def:properly-marked} we immediately conclude the following:

\begin{corollary}
Let $(q, M)$ be a marked query, and $\db$ be any database. If $\sg \models \mq$, then $\mq$ is properly marked.
\end{corollary}

Let us refer to a marked CQ $(q, M)$ as {\em alive} given that it is properly marked and $M$ does not contain all terms of $q$. In the case where every term of a properly marked CQ is marked, we refer to the CQ as {\em dead}.

To prove~\cref{lem:rsg-is-fus} it suffices to prove the following lemma, which we direct our attention to in the subsequent section. 

\begin{lemma}\label{lem:rsg-is-fus-reformulated}
For any properly marked CQ $(q, \prmark)$ there exists a set of dead queries $rew(q,\prmark)$ such that for any database $\db$ the following holds: 
\begin{center}
$\sg \models (q,\prmark)$ \ $\iffi$ \ $\exists{Q' \in rew(q, \prmark)}, \db \models Q'.$
\end{center}
\end{lemma}

\subsection{Rewriting Alive Queries}

We begin this section by proving the following lemma, which will later prove useful in rewriting queries relative to $\rsgrid$.

\begin{lemma}\label{lem:exists-maximal}
%For every alive CQ there exists at least one variable with no out-going edges.
If a marked CQ $(q,\prmark)$ is alive, then there exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{lemma}
\begin{proof} Let the marked CQ $(q,\prmark)$ be alive. Then, by the definition above, we know that there exists a set of terms in $q$ that are not a members of $M$. Since $(q,\prmark)$ is properly marked, by \cref{def:properly-marked}, we know that all such terms are not constants, and hence, all such terms must be variables. Let us refer to all such terms as \emph{unmarked variables}. If we consider the sub-instance of the CQ induced by all unmarked variables, we can see that (i) it forms a directed acyclic graph as all cycles of the CQ must be in $M$ by \cref{def:properly-marked}, which (ii) is non-empty as $(q,\prmark)$ is alive. Hence, there must exists a variable $x$ in $q$ such that no atom of the form $\rpred(x,t)$ occurs in $q$ with $\rpred\in \{\hpred,\vpred\}$, which corresponds to a sink in the directed acyclic graph described above.
\end{proof}

We will refer to unmarked variables -- such as those described in the above proof -- which possess no out-going edges, as {\em maximal}. These maximal variables will be used to initiate our rewriting process. 

\begin{lemma}\label{lem:maximal-cases}
Let $x$ be a maximal variable of an alive CQ $(q, \prmark)$. Then, one of the following holds:
\begin{enumerate}
    \item \label{lem:maximal-cases-one} $x$ occurs in exactly one atom  $\rpred(t,x)$, with $\rpred\in \{\hpred,\vpred\}$ for some term $t$ of $q$;
    \item \label{lem:maximal-cases-two} $x$ occurs in exactly two atoms $\hpred(t_{\hpred},x)$ and $\vpred(t_{\vpred},x)$ for some terms $t_{\hpred},t_{\vpred}$ of $q$;
    \item \label{lem:maximal-cases-three} there exist at least two distinct terms $t\neq t'$ such that $\rpred(t,x)$ and $\rpred(t',x)$ are atoms of $q$ with $\rpred\in \{\hpred,\vpred\}$.
\end{enumerate}
\end{lemma}

%Now, in the light~\cref{lem:maximal-cases} we will present four operations that when combined will compute rewritings required by \cref{lem:rsg-is-fus-reformulated}.

\medskip
\noindent
{\bf Rewriting Operations.}
We now make use of~\cref{lem:maximal-cases} to define three operations that compute rewritings. When exhaustively applied to a query, we obtain the rewritings required by \cref{lem:rsg-is-fus-reformulated}. Given an alive CQ $(q, \prmark)$ we define the following three operations:

\begin{definition}[$\cutop$]\label{def:cut}
Let $x$ be a maximal variable of $(q, \prmark)$ satisfying case \ref{lem:maximal-cases-one} of \cref{lem:maximal-cases}, i.e. $x$ occurs in exactly one atom $\rpred(t,x)$ of $q$ with $\rpred\in \{\hpred, \vpred\}$. Then, letting $\query = \query' \cup \{\rpred(t,x)\}$, we define
\[
  \cutop((q,\prmark), \set{x}) =
  \begin{cases}
     (q' \cup \{\top(c)\}, \prmark)  & \text{if $t$ is a constant $c$} \\
      & \text{not occurring in $\query'$;}\\
     (q', \prmark) & \text{otherwise.}
  \end{cases}
\]
%Then, $\cutop((q,\prmark), \set{x}) = (q', \prmark)$, where $q'$ is the sub-query of $q$ with the atom containing $x$ removed.
\end{definition}


\begin{definition}[$\reduceop$]\label{def:reduce}
Let $x, t_{\hpred}$, and $t_{\vpred}$ be as in case \ref{lem:maximal-cases-two} of \cref{lem:maximal-cases}, meaning that there exist two atoms of the form $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ in $q$. We define $q'$ to be the same as $q$, but where $\hpred(t_{\hpred}, x)$ and $\vpred(t_{\vpred}, x)$ are replaced by $\hpred(x', t_{\vpred})$ and $\vpred(x', t_{\hpred})$, and where $x'$ is fresh. We now %by replacing $\hpred(t_{\hpred}, x),\vpred(t_{\vpred}, x)$ with $\hpred(x', t_{\vpred}), \vpred(x', t_{\hpred})$, where $x'$ is a fresh variable. 
 define $\reduceop((q,\prmark), \set{x}) = \set{ (q', \prmark), (q', \prmark \cup \set{x'})}$. 
\end{definition}

\begin{definition}[$\mergeop$]\label{def:merge}
Let $x, t$, and $t'$ be as in case \ref{lem:maximal-cases-three} of \cref{lem:maximal-cases}. We let $q'$ be obtained from $q$ by replacing all occurrences of $t$ in $q$ with $t'$ and define $\mergeop((q, \prmark), \set{x, t, t'}) = (q' \cup \{\top(t)\}, \prmark)$.
\end{definition}

Let us briefly describe how rewritings are computed by means of the above operations. %First, when given a CQ $q$ that is satisfied on $\sg$, we extend the CQ to a properly marked CQ $(q,M)$, which can always be accomplished by \cref{obs:query-extendable-properly-marke}.  
 Given an alive CQ $(q,M)$, we know that one of the three rewriting operations will be applicable (by \cref{lem:maximal-cases}), which we note, may return a \emph{set} of rewritings if the $\reduceop$ operation is applied. We ultimately obtain the set $rew(q, \prmark)$ of rewritings of $(q,\prmark)$ by sequentially applying the three rewriting operations to all alive queries within the set of rewritings, until all marked queries in the set are dead, at which point, the rewriting process terminates. As shown below, we can always apply a rewriting operation to a CQ if it is alive (i.e. rewriting is complete), and also, applying such an operation preserves satisfaction on $\sg$ (i.e. rewriting is sound). We note that the soundness proofs can be found in \cref{appendix:higher-arity}.

\begin{observation}[Completeness]\label{obs:high-completeness}
If a CQ is alive then at least one of above operations can be applied to it.
\end{observation}
\begin{proof}
Follows from~\cref{def:cut,def:reduce,def:merge}, and~\cref{lem:maximal-cases}.
\end{proof}

Let us now prove the soundness of the above operations:

\begin{lemma}[Soundness --- $\cutop$]\label{lem:high-soundness-cut}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x$ is as in \cref{def:cut}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \cutop(\mquery, \set{x}).$$
\end{lemma}


\begin{lemma}[Soundness --- $\reduceop$]\label{lem:high-soundness-reduce}
Let $\db$ be a database and let $Q$ be an alive CQ. If $x$ is as in \cref{def:reduce} and $\reduceop(\mquery, \set{x}) = \set{\mquery_{1}, \mquery_{2}}$, then
$$\sg \models \mquery \ \text{\iffi} \ \exists i \in \{1,2\}, \sg \models \mquery_{i}.$$
\end{lemma}


\begin{lemma}[Soundness --- $\mergeop$]\label{lem:high-soundness-merge}
Let $\db$ be a database and let $\mquery$ be an alive CQ. If $x, t$, and $t'$ are as in \cref{def:merge}, then
$$\sg \models \mquery \ \text{\iffi} \ \sg \models \mergeop(\mquery, \set{x, t, t'}).$$
\end{lemma}


\medskip
\noindent
{\bf Termination.}
Given two queries $\mquery$ and $\mquery'$, we write $\mquery \stepop \mquery'$ \iffi $\mquery'$ can be obtained from $\mquery$ by applying $\reduceop$, $\cutop$, or $\mergeop$. We let $\stepop^*$ denote the transitive closure of $\stepop$.


%\begin{observation}\label{obs:limit-on-variables}
%Let $\mquery$ and $\mquery'$ be two marked queries. If $\mquery \stepop \mquery'$ then $|\varset(\mquery)| \geq |\varset(\mquery')|$.
%\end{observation}

\begin{lemma}[Termination]\label{lem:termination}
For any properly marked CQ $\mquery$ the set of properly marked queries $\set{Q' \;|\; \mquery \stepop^* \mquery'}$ is finite.
\end{lemma}

\begin{proof} Observe that $\cutop$ deletes the only atom containing the considered maximal variable and $\mergeop$ reduces the number of atoms containing the considered maximal variable. Moreover, neither $\cutop$ nor $\mergeop$ introduce converging atoms of the form $\hpred(t_{1},t)$ and $\vpred(t_{2},t)$ when applied. Since the operation $\reduceop$ reduces the number of such converging atoms in a properly marked CQ as well, and since all such operations either preserve or decrease the number of terms occurring the query, it follows that the rewriting process will eventually terminate. 
\end{proof}

By \cref{obs:high-completeness} (Completeness), \cref{lem:high-soundness-cut,lem:high-soundness-reduce,lem:high-soundness-merge} (Soundness), and \cref{lem:termination} (Termination), we may conclude~\cref{lem:rsg-is-fus-reformulated}, thus completing the proof of \cref{lem:rsg-is-fus}.

==> introduction.tex <==
\section{Introduction}

Querying under \emph{existential rules}\footnote{Existential rules are also referred to as \emph{tuple-generating dependencies} (TGDs)~\cite{AbiteboulHV95}, \emph{conceptual graph rules}~\cite{SalMug96}, Datalog$^\pm$~\cite{Gottlob09}, and \emph{$\forall \exists$-rules}~\cite{BagLecMugSal11} in the literature.} (henceforth often shortened to \emph{rules}) is a popular topic in database theory and knowledge representation. For arbitrary rule sets, query entailment is undecidable~\cite{ChandraLM81}, motivating research into fragments for which decidability can be regained.

To this end, a very useful conceptual tool
%which has not only proven useful for describing querying methods, but also for identifying %classes of rule sets with decidable query entailment, 
is the \emph{chase}~\cite{Chase84}: For a database $\database$ and rule set $\ruleset$, the (possibly non-terminating) chase procedure yields a \emph{universal model}~\cite{DeuNasRem08}, satisfying all queries entailed by $\database$ and $\ruleset$. This allows for reducing query entailment to query evaluation.

Rule sets admitting finite universal models (a property equivalent to being a \emph{finite-expansion set}~\cite{BagLecMugSal11} or \emph{core-chase terminating}~\cite{DeuNasRem08}) are particularly well-behaved. 
%
%This is witnessed by the fact that classes thereof subsume a wide variety of so-called \emph{concrete classes}~\tim{\cite{}}, syntactically defined classes of rule sets based on diverse notions of \emph{acyclicity}~\tim{\cite{}}.
%
%syntactically defined so-called \emph{concrete classes} of rules based on diverse notions of \emph{acyclicity}.
%
But even in cases where universal models are necessarily infinite, they may still be sufficiently ``tame'' to allow for decidable query entailment, as is the case with the class of \emph{bounded-treewidth sets} ($\bts$)~\cite{BagLecMugSal11}. A rule set $\ruleset$ qualifies as $\bts$ \iffi for every database~$\database$, there exists a universal model of $\database$ and $\ruleset$ whose \emph{treewidth} (a structural measure originating from graph theory) is finite.
%bounded by some $n\in \mathbb{N}$. 
The $\bts$ class subsumes the $\fes$ class, and gives rise to decidable query entailment for a sizable family of concrete, syntactically defined classes of rule sets 
%deploying more or less refined versions of guardedness~
\cite{BagLecMugSal11,CaliGK13,KrotzschR11}.     

While $\bts$ is a fairly general class, it still fails to contain rather simple rule sets; e.g., the rule set $\ruleset^\infty_\mathrm{tran}$, consisting of the two rules
%%%%
% CAUTION: THE SECOND OF THE FOLLOWING RULES WAS WRONG: 
% IT HAD AN \exists z IN FRONT OF THE SECOND RULE HEAD.
% I REMOVED IT. PROBABLY IT WAS JUST A COPY-PASTE ERROR
% BY ME, BUT JUST TO BE SAFE, I LEFT THIS COMMENT
%%%%
$
\epred(x,y) \to \exists z \epred(y,z)$ and $\epred(x,y) \wedge \epred(y,z) \to \epred(x,z),
$
falls outside the $\bts$ class. To give an idea as to why this holds, consider any database $\db$ containing an $\epred$-fact (e.g., $\epred(\const{a},\const{b})$): the chase will yield a universal model resembling the transitive closure of an infinite $\epred$-path, a clique-like structure of infinite treewidth. What is more, not only does $\ruleset^\infty_\mathrm{tran}$ fail to be $\bts$, it also fails to fall under the other generic decidability criteria: it is neither \emph{finitely controllable} (which would guarantee the existence of a finite ``countermodel'' for each non-entailed query) nor $\fus$ (see below). Yet, results for  description logics confirm the decidability of (conjunctive) query entailment over $\ruleset^\infty_\mathrm{tran}$ (see~\cite{GlimmLHS08,OrtizRS11}), in\-cen\-ti\-vi\-zing a generalization of the decidability criteria mentioned above.

%\tim{Note: Depending on if we adopt fus, FO-rewritable, etc. we will potentially have to do a bit of re-writing above and/or below.}

The class of \emph{finite-unification sets} ($\fus$)~\cite{BagLecMugSal11}, incomparable with $\bts$, gives rise to decidable query entailment thanks to \emph{first-order rewritability}. Such rule sets may feature non-guarded rules \cite{CaliGP12}; for instance, they may include \emph{concept products} \cite{RudolphKH08,BourhisMP17}, which create a biclique linking instances of two unary predicates, as in 
$
\pred{Elephant}(x) \wedge \pred{Mouse}(y) \to \pred{BiggerThan}(x,y).
$

The above examples demonstrate a crucial weakness of the $\bts$ class: its inability to tolerate universal models exhibiting ``harmless'' unbounded clique-like structures. Opportunely, the graph-theoretic notion of \emph{cliquewidth}~\cite{CourEngBook} overcomes this problem, while retaining most of treewidth's desirable properties. Inspired by this less mainstream, but more powerful concept, we introduce \emph{finite-cliquewidth sets}~($\bcws$) of rules. Our contributions are as follows:
%As the original cliquewidth notion is tailored to finite undirected graphs, some (not entirely straightforward) generalizations are necessary to adapt it to countable instances, while at the same time, preserving its advantageous properties. Our contributions can be summarized as follows:
\vspace{-0.3ex}
\begin{itemize}
    \item We introduce a generic framework for utilizing certain model-theoretic measures to establish decidability of entailment for a comprehensive class of queries (dubbed \emph{datalog/MSO queries}, or \emph{DaMSOQs} for short) that significantly extends conjunctive queries. 
    
    \item Generalizing the eponymous notion from finite graph theory, we introduce the model-the\-o\-re\-tic measure of \emph{cliquewidth} for countable instances over arbitrary signatures. Based on our framework, we show that the derived notion of \emph{finite-cliquewidth sets} %$\fcs$ 
    guarantees decidability of DaMSOQ entailment. In particular, we demonstrate that $\ruleset^\infty_\mathrm{tran}$ is indeed $\fcs$, thus showing that $\fcs$ incorporates rule sets outside $\bts$ and $\fus$.
    
    \item We compare the $\fcs$ and $\bts$ classes, obtaining: (good news) for binary signatures, $\fcs$ subsumes $\bts$, which (bad news) does not hold for higher-arity signatures, but (relieving news) $\fcs$ still ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\begin{itemize}
        %\item[] 
 %       \underline{Good News}: For unary and binary signatures, $\fcs$ subsumes $\bts$;\\
        %\item[] 
 %       \underline{Bad News}: For higher-arity signatures, $\fcs$ does not subsume $\bts$;
        %This inclusion does not generalize to higher arities.\\ 
        %\item[] 
 %       \underline{Relievin}g\underline{ News}: Yet, $\fcs$ ``indirectly subsumes'' higher-arity $\bts$ through reification.
    %\end{itemize}
    \item We compare the $\fcs$ and $\fus$ classes, obtaining: (good news) for sets of single-headed rules over signatures of arity ${\leq}2$, $\fcs$ subsumes $\fus$, which (bad news) does not hold for multi-headed rules, but (relieving news) this could not be any different as there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.
    %\begin{itemize}
        %\item 
  %      \underline{Good News}: For sets of single-headed rules over unary and binary signatures, $\fcs$ subsumes $\fus$;\\
        %\item 
 %       \underline{Bad News}: This inclusion does not hold for multi-headed rules.\\ 
        %\item 
 %       \underline{Relievin}g\underline{ News}: It couldn't be any different, since there are $\fus$ rule sets for which DaMSOQ entailment is undecidable.\\  
    %\end{itemize}
    
%    \item On the negative side, we expose a rule set $\rsgrid$ that is FO-rewritable (and thus admits decidable CQ entailment) but is not $\bcws$---thereby showing that $\bcws$ does not subsume $\fus$, although, this is to be expected as decidability is lost when considering the entailment of more expressive queries from the DaMSOQ family.
%    \item On the positive side, we show that $\bcws$ \emph{does} subsume $\fus$ for all single-head rule sets over binary signatures. The proof of this fact is highly nontrivial, and serves as this paper's deepest result.  
\end{itemize}

%\noindent\textbf{For space reasons, we defer technical details to the appendix.} 


%So called \emph{abstract classes} of existential rule sets have an undecidable membership problem, but they comprise a wide range of rule sets and provide a uniform argument for the decidability of query answering.   



%Existential rules are important <- query entailment is easy <- chase provides universal models. However even the chase fails when existential rules are not constrained. Thus many subclasses that provide decidable query entailment were introduced {\em bounded cliquewidth sets} and FUS/BDD/FO-rewritable covering most of those. With the reasons for the decidablility of query entailment for those classes are well understood it is believed that admitting grid-like universal models lead to undecidability of query entailment. In this paper we show that this is the case for binary signatures --- bcs class subsumes fus --- and surprisingly that it is not true for higher arities.

%Say things about BDD, FUS, FO-rewritability only there.

==> other/binary-ball.tex <==
\section{Results for Binary Signatures}



In this section, we will prove the first of our two main results, \textit{viz.} \cref{thm:binary}. We fix a binary signature $\sig$, a finite unification set $\ruleset$ of single-headed rules over $\sig$, and a database $\database$ over $\sig$ for the remainder of the section. To prove \cref{thm:binary}, it suffices to show that the clique-width of $\sat{\ruleset, \database}$ is bounded, hence, we dedicate this section to establishing the following lemma.

\begin{lemma}\label{lem:binary-main}
%There exists an $n \in \mathbb{N}$ s.t. $\cw{\sat{\ruleset, \database}} \leq n$. 
$\sat{\ruleset, \database}$ has bounded clique-width.
\end{lemma}

Having fixed the rule set $\ruleset$ and the database $\database$, we abbreviate $\sat{\ruleset, \database}$ as $\sa$.

\subsection{Looking Past Datalog}

Let $\se \subseteq \sa$ be the instance containing the existential atoms of $\sa$, that is, the atoms derived via the non-datalog rules of $\ruleset$. We %let the structure of $\se$  be $\struc^{\se} = (\sdom^{\se}, \srel^{\se})$, and 
 note that $\se$ is a crucial building block in the proof of \cref{lem:binary-main} as it satisfies the following observation:


%%%COMMENT%%%
\begin{comment}
\tim{Concerning the sentence: ``If $\sa$ can be derived in multiple ways, we fix a single derivation sequence to determine which atoms are existential.'' which was the second sentence above. Isn't it enough to observe that the atom contains at least one null without consulting a derivation? Since databases only contain constants, we should immediately be able to conclude that any atom with a null was derived via a non-datalog rule. Perhaps we should delete this sentence then, if you agree.}
\piotr{No :) Consider the following rule set $R=$ \begin{itemize}
    \item $A(x) \to \exists{y} E(x,y)$
    \item $A(x) \to \exists{y} F(x,y)$
    \item $E(x,y) \to F(x,y)$
    \item $F(x,y) \to E(x,y)$
\end{itemize}
And the following instance $\set{A(a), E(a,t), F(a, t)} = 
\sat{R, \set{A(a)}}$ there is no way to determine which atom is datalog and which is existential. As a matter of fact, the result of the restricted chase very much depends on the order of rule application. Consider $\set{A(a), E(a, t) F(a, t), E(a, t'), F(a, t')}$. We should discuss that somewhere in the paper as well.
}
\end{comment}
%%%COMMENT%%%



\begin{observation}\label{obs:sate-is-forest}
%Let $\inst = \se \setminus \database$. Then, $\struc^{\inst} = (\sdom^{\inst}, \srel^{\inst})$ is a typed polyforest of bounded degree.
$\se \setminus \database$ is a typed polyforest of bounded degree.
\end{observation}

\begin{proof}
See \cref{appendix} for details.
\end{proof}

From this we can derive the following:

\begin{corollary}\label{cor:skeleton-has-bounded-cw}
%The clique-width of $\struc^{\se}$ is bounded.
 The clique-width of $\se$ is bounded.
\end{corollary}

\begin{proof} %Let $\inst = \se \setminus \db$ and define $\struc^{\inst} = (\sdom^{\inst}, \srel^{\inst})$. 
 By \cref{obs:sate-is-forest}, we know that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest of bounded degree, and by \cref{obs:trees_cw_le3}, we know %$\cw{\struc^{\inst}} \le 2 \cdot |\sig| + 2$
 $\cw{\se \setminus \database} \le 2 \cdot |\sig| + 2$. For some set of typed polytrees in the typed polyforest %$\struc^{\inst}$
 $\se \setminus \database$ (of which there are only finitely many), each has a unique term (which we call a \emph{connection element}) that is connected to a term of $\db$ in %$\struc^{\se}$ 
 $\se$ (which we call a \emph{connection root}). Let $n$ be the number of connection elements in %$\struc^{\inst}$ 
 $\se \setminus \database$ and define the set $\cols_{1} = \{m \in \mathbb{N} \ | \ m \leq n\}$ of colors, which we assume w.l.o.g. to be fresh. Observe that if we additionally extend the set of colors $\cols$ (used in the proof of \cref{obs:trees_cw_le3}) with the set $\cols_{1}$, then we may assume that prior to taking the disjoint union of all typed polytrees in %$\struc^{\inst}$ 
 $\se \setminus \database$ (during the construction process detailed in \cref{obs:trees_cw_le3}) that we have recolored each connection element to a unique color in $\cols_{1}$. We refer to this colored structure as %$(\struc^{\inst},\coloring_{1})$
 $(\se \setminus \database, \coloring_{1})$, and use this fact below to bound the clique-width of $\se$. Note that if we color connection elements in the above way, then $\cw{\se \setminus \db} \le 2 \cdot |\sig| + n + 2 \leq 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, with the last inequality following from the fact that the Skolem chase will only connect connection roots to at most $2 \cdot |\sig|$ typed polytrees. Since $\db$ is a finite graph, we know that $\cw{\db} \leq k$, for $k = |\adom{\db}|$; hence, we may assume that the set of colors used to color the graph of $\db$ is $\cols_{2} = \{t \ | \ t \in \adom{\db}\}$, which we assume to be disjoint from all colors in $\coloring_{1}$. We refer to this colored structure as $(\db,\coloring_{2})$, and define $(\struc, \coloring) = (\se \setminus \db,\coloring_{1}) \disun (\db,\coloring_{2})$. Now, for each typed polytree in $(\se \setminus \db,\coloring_{1})$ that has a connection element with color $l$, we apply either $\add{R,(l,t)}{\struc, \coloring}$ or $\add{R,(t,l)}{\struc, \coloring}$ (depending on if the connection element is connected with an edge typed with the predicate $R$ to the connection root, or away from the connection root, respectively), where $t$ is the color of the connection root in $(\db,\coloring_{2})$. We can therefore see that $\cw{\se} \leq |\adom{\database}| + 2 \cdot |\sig| + 2\cdot|\adom{\db}|\cdot|\sig| + 2$, thus proving the observation.
\end{proof}



In the sequel, we will use $\se$ and the $\mathrm{add}_{R,\vl}$ operation to reconstruct $\sa$ and prove that $\cw{\sa}$ is bounded. However, a specific coloring is required to prove this claim, which is distinct from the coloring used to prove that $\cw{\se}$ is bounded. Thus, we define a new coloring below %that permits us to conclude \cref{thm:binary} 
 by making use of the fact that $\ruleset$ is $\fus$.\footnote{We note that this is not simply a matter of finding the desired coloring, but rather, is a matter of ``recoloring'' in the proper way (see \cref{obs:cross-coloring}).}
 
\subsection{Rewriting Datalog Rules}

Given our rule set $\ruleset$, we re-write the subset of $\ruleset$ containing all datalog rules into a new rule set, which we denote $\rulesetnorm$. Since $\rulesetnorm$ is a finite set and since the body of each rule in $\rulesetnorm$ is a finite conjunction of atomic formulae, we know that a natural number exists that uniformly bounds the diameter of the body of each rule in $\rulesetnorm$.\footnote{See \cref{sec:preliminaries} for the definition of \emph{diameter}.} Moreover, since our signature $\sig$ is assumed to be finite, it follows that only a finite number of finite instances with finite branching can be constructed with a diameter that fits within the natural number bound. Therefore, we can leverage our re-writing to define a finite set of colors---consisting of the aformentioned finite instances---which will play a central role in demonstrating that $\cw{\sa}$ is bounded.

Let us define $\ruleset_{DL}$ to be the subset of $\ruleset$ containing all datalog rules, and note the following useful equation:
\begin{equation}\label{eq:sa-satse}
\sa = \sat{\ruleset_{DL}, \se}.
\end{equation}

For any relational symbol $R \in \sig$, we define the rule set $\rew{R}$ to be the following:\footnote{Recall that in this section $\sig$ is a fixed binary signature.}
$$
\set{\varphi(\vx, y,z) \to R(y,z) \;|\; \exists{\vx} \varphi(\vx, y,z) \in \rewrs{\ruleset}{R(y,z)}}
$$
and
$$
\rulesetnorm = \bigcup_{R \in \sig} \rew{R}.
$$
We now show that the rule set $\rulesetnorm$ admits an important property:

\begin{lemma}\label{lem:trigger-for-each-rewritten-rule}
For any atom $R(t_{1},t_{2}) \in \sa \setminus \se$ there exists a trigger $(\rho, h)$ in $\se$ with $\rho \in \rulesetnorm$ such that applying $(\rho, h)$ adds $R(t_{1},t_{2})$ to $\se$.
\end{lemma}
\begin{proof}
From the fact that $\ruleset$ is $\fus$, we can conclude that for any ordered pair $(t_{1},t_{2})$ of terms from $\se$, there exists a CQ $\exists \vx \phi(\vx,y,z) \in \rewrs{\ruleset}{R(y,z)}$ such that the following holds:
%
$$\sat{\ruleset, \se} \models R(t_{1},t_{2}) \ \ifandonlyif \ \se \models \exists \vx \phi(\vx,t_{1},t_{2}).
$$
%
Thus, we know that the desired trigger exists for some rule of $\rew{R}$ in $\se$.
\end{proof}

From the above lemma and \cref{eq:sa-satse} we can conclude the following:
\begin{equation}\label{eq:skeleton}
\ksat{1}{\rulesetnorm, \se} \;=\; \sa
\end{equation}

The above equation tells us that we can apply all rules of $\rulesetnorm$ within a single step to obtain the same result as $\sa$. Using this fact, we can determine (and provide a bound for) the size of the neighborhood in $\se$ that is needed to apply any given rule from $\rulesetnorm$. Ultimately, this observation will be used to bound the clique-width of $\sa$, which suffices to conclude \cref{thm:binary}.

\begin{definition}\label{def:diameter}
Let us denote twice the maximal diameter of any connected component in any rule body of $\rulesetnorm$ as $\diam$.
\end{definition}

One the basis of \cref{eq:skeleton} above, we may restate \cref{lem:binary-main} in an equivalent manner as:

\begin{lemma}\label{lem:binary-reformulated}
$\ksat{1}{\rulesetnorm, \se}$ has bounded clique-width.
\end{lemma}

We dedicate the remainder of the section to establishing the above lemma, which implies the desired result (\cref{thm:binary}).



\subsection{Searching for a Suitable Coloring}

Now we are almost ready to define the new coloring for $\se$. Consider the following definition:

\medskip \noindent {\bf Neighbourhoods in $\se$.} % Let $\struc^{\se} = (\sdom^{\se},\srel^{\se})$ be the structure obtained from the instance $\se$ as defined in \cref{sec:cliquewidth}. Given a term $t \in \sdom^{\se}$ and a natural number $n$, we define $\ball{n}{t}$ to be the induced subset of $\se$ over the set $\set{t' \in dom(\sdom^{\se}) \;|\; \dist{t,t'} \leq n}$.\footnote{We note that $\dist{t,t'}$ denotes the \emph{distance} between $t$ and $t'$, i.e. the length of the path (not necessarily directed) connecting $t$ and $t'$.} We refer to $t$ as the {\em central term} of $\ball{n}{t}$. We define $\bball{n}{t}$ to be the equivalence class modulo the isomorphism relation of the instance $\ball{n}{t} \cup R(t)$, where $R$ is a fresh unary predicate such that $R \not\in \sig$. We note that the inclusion of $R(t)$ is helpful as it permits us to reconstruct the central term of a neighbourhood from its given equivalence class.
 Given a term $t \in \adom{\se}$ and a natural number $n$, we define $\ball{n}{t}$ to be the induced subset of $\se$ over the set $\set{t' \in \adom{\se} \;|\; \dist{t,t'} \leq n}$.\footnote{We note that $\dist{t,t'}$ denotes the \emph{distance} between $t$ and $t'$, i.e. the length of the path (not necessarily directed) connecting $t$ and $t'$.} We refer to $t$ as the {\em central term} of $\ball{n}{t}$, and define $\bball{n}{t}$ to be the equivalence class modulo the isomorphism relation of the instance $\ball{n}{t} \cup \{ R(t) \}$, where $R$ is a fresh unary predicate such that $R \not\in \sig$. We note that the inclusion of $R(t)$ is helpful as it permits us to reconstruct the central term of a neighbourhood from its given equivalence class.

Enough groundwork has been laid to define the new coloring function $\coloringe$ for $\se$. Given a term $t$ of $\se$, we define:
$$
\coloringe(t) = \bball{\diam}{t}
$$
and argue that the image of $\coloringe$ is finite.

\begin{observation}\label{obs:finite-balls}
For every $n \in \mathbb{N}$ the set $\set{\bball{n}{t} \;|\; t \in \adom{\se}}$ is finite.
\end{observation}


\begin{proof} Since $\se \setminus \database$ is a typed polytree of bounded degree, $\database$ is finite, and $\sig$ is finite, for any given $n \in \mathbb{N}$, only a finite number of $\bball{n}{t}$ exist.
\end{proof}

%Now that we have defined the coloring $\coloringe$, we make use of it to show that another coloring $\prcoloringe$ can be defined such that for some natural number $\ke$, $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$. Toward this end, it suffices to prove the following lemma:

Now that we have defined the coloring $\coloringe$, we make use of it to define another---almost identical---coloring $\prcoloringe$ such that for some natural number $\ke$, $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$. The only feature distinguishing $\prcoloringe$ from $\coloringe$ is that $\codom{\prcoloringe}$ is defined to be a superset of $\codom{\coloringe}$. As argued in the corollary below, expanding the co-domain of $\coloringe$ with a specific number of colors %, while still retaining the its finiteness, 
 ensures that a sufficient, albeit still finite, number of colors are used in bounding $\cw{\se}$. Let us now prove the following corollary:

%From the above lemma, we may conclude the following:


\begin{corollary}
There exists a number $k_\exists \in \mathbb{N}$ such that $(\se, \prcoloringe) \in \mathfrak{L}_{k_\exists}$.
\end{corollary}
\begin{proof}
From \cref{cor:skeleton-has-bounded-cw}, we know that $\cw{\se}$ is bounded. Hence, there exists a $\coloring$ and $k$ such that $(\se, \coloring) \in \mathfrak{L}_{k}$. We define $(\coloring\times\coloringe)(t) = (\coloring(t), \coloringe(t))$ and let $k' = |\codom{\coloringe}| \in \mathbb{N}$, which we know exists by \cref{obs:finite-balls} and the definition of $\coloringe$ above. For every finite induced subinstance $\inst$ of $\se$, we know that $(\inst,\coloring|_{\adom{\inst}}) \in \mathfrak{L}_{k}$ by our assumption that $(\se, \coloring) \in \mathfrak{L}_{k}$. Hence, by \cref{obs:cross-coloring}, we may conclude that $(\inst, (\coloring\times\coloringe)|_{\adom{\inst}}) \in \mathfrak{L}_{k \cdot k'}$. Since this holds for every finite induced subinstance, we may conclude that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$ holds by \cref{def:cw}.

To complete the proof, let us define the set of colors $\cols = \codom{\coloring \times \coloringe} \cup \codom{\coloringe}$ as well as the following coloring:
\begin{center}
$\prcoloringe(t) = \coloringe(t)$
\end{center}
where we assume that $\codom{\prcoloringe} = \cols$. If we let $k_{\exists} = k \cdot k' + k'$, then by the above fact that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$, we may conclude that $(\se, \prcoloringe) \in \mathfrak{L}_{k_{\exists}}$.
%From \cref{cor:skeleton-has-bounded-cw}, we know that $\cw{\se}$ is bounded. Hence, there exists a $\coloring$ and $k$ such that $(\se, \coloring) \in \mathfrak{L}_{k}$. We define $(\coloring\times\coloringe)(t) = (\coloring(t), \coloringe(t))$ and let $k' = |\codom{\coloringe}| \in \mathbb{N}$, which we know exists by \cref{obs:finite-balls} and the definition of $\coloringe$ above. For every finite induced subinstance $\inst$ of $\se$, which is colored by $(\coloring\times\coloringe)|_{\adom{\inst}}$, we know that $(\inst, (\coloring\times\coloringe)|_{\adom{\inst{}}}) \in \mathfrak{L}_{k \cdot k'}$ by \cref{obs:cross-coloring}. Since this holds for every induced subinstance we conclude that $(\se, \coloring\times\coloringe) \in \mathfrak{L}_{k \cdot k'}$ also holds.
%To finish the proof it is enough to project every color of $\coloring\times\coloringe$ onto a second coordinate using $\mathrm{recolor}$ operations. \thomas{To facilitate the projection, we also need to add the $k'$ colors from the image of $\coloringe{}$ to the overall number of used ones. For the numbers of colors this means that we can use up to $k\cdot k' + k'$ many. To be symmetric about it, we might also add the ``original'' ones, amounting to an additional $k'$ colors. Hence $k\cdot k' + k' + k$ does the job as $k_{\exists}$. For better presentability one upper bound would also be $(k+1)\cdot (k'+1)$. Another conservative estimate leaves us at $k_{\exists} = 3\cdot k\cdot k'$.}
\end{proof}

\subsection{From $\se$ to $\so$}

In this section, we show that $(\so, \prcoloringe) \in \mathfrak{L}_{\ke}$, from which we may conclude \cref{lem:binary-reformulated}, and thus, \cref{thm:binary}. More specifically, we show that $(\so, \prcoloringe)$ can be constructed by making use of $(\se, \prcoloringe) \in \mathfrak{L}_{\ke}$ and the $\mathrm{add}_{R, \vl}$ operations. This goal is achieved by introducing the datalog atoms obtained by applying the rules from $\rulesetnorm$ to $\se$. We focus on the case where we consider binary atoms, as the unary case is analogous.

%All we need to do is to introduce to $(\se, \coloringe)$ the datalog atoms derivable by $\rulesetnorm$ in $\se$. We will show this for binary atoms, as the unary case is analogous.

Let $\rho \in \rulesetnorm$ and suppose that $\head(\rho) = R(x,y)$, i.e. the head of $\rho$ is a binary atom. We may assume w.l.o.g. that $\rho$ is of the following form:
%
$$
\rho = \phi_{1}(\vx, x) \land \phi_{2}(\vy, y) \land \phi_{3}(\vz) \to R(x, y)
$$
%
where $\phi_{1}(\vx, x)$ and $\phi_{2}(\vy, y)$ denote the maximal connected components in $\body(\rho)$ containing all occurrences of $x$ and $y$ respectively, and with $\psi(\vz)$ denoting the remaining conjunction of atoms in $\body(\rho)$. We now define the following two sets of colors, which are both assumed to be subsets of $\adom{\se} \times \adom{\se}$:
\begin{flushleft}
$(t,t') \in \cols_{\coloring}$ \ifandonlyif $\ball{\diam}{t} \models \phi_{1}(\vx, t)$, $\ball{\diam}{t'} \models \phi_{2}(\vy, t')$, and $\se \models \phi_{3}(\vz)$;
\end{flushleft}
\begin{flushleft}
$(t,t') \in \cols_{\rho}$ \ifandonlyif $\se \models \phi_{1}(\vx, t) \land \phi_{2}(\vy, t') \land \phi_{3}(\vz)$.
\end{flushleft}
%$$
%\begin{array}{rcl}
%   \cols_\coloring & = & \set{\;(t,t') \in dom(\se)^2 \;|\; \ball{\diam}{t} \models \phi(\vx, t) \;\wedge\\
%    & &  \hspace{3.43cm} \ball{\diam}{t'} \models \phi'(\vx', t') \;\wedge\\
%    & &  \hspace{3.43cm}\se \models \psi(\vz)\;}.\\
%   \cols_\rho & = &  \set{(t,t') \in dom(\se)^2 |\se \models \phi(\vx, t), \phi'(\vx', t'), \psi(\vz)}.
%\end{array}
%$$
%
Both sets $\cols_\coloring$ and $\cols_\rho$ contain pairs of terms $(t,t')$ such that $R(t,t')$ results from applying $\rho$ to $\se$. %The set $\cols_\coloring$ is a subset of $A_\rho$ that contains the pair $(t, t')$ if it can be derived using only a small neighbourhood around $t$ and $t'$ and some general information on $\se$. As it turns out:
 By making use of \cref{def:diameter}, it is straightforward to establish that both sets coincide:

\begin{observation}\label{obs:binary-unary-case-ball}
$\cols_\coloring = \cols_\rho$.
\end{observation}
\begin{proof}
As the inclusion $\cols_\rho \subseteq \cols_\coloring$ follows directly from the definition of each set, we focus on showing the converse, i.e. that $\cols_{\coloring} \subseteq \cols_\rho$. If we assume that $(t,t') \in \cols_{\coloring}$, then we have that $\se \models \phi_{1}(\vx, t) \land \phi_{2}(\vy, t') \land \phi_{3}(\vz)$. By \cref{def:diameter}, we know that $\diam$ is {\em twice the maximal diameter of any connected component in any rule body of $\rulesetnorm$}, which ensures that $\ball{\diam}{t}$ and $\ball{\diam}{t'}$ are sufficiently large enough so that $\ball{\diam}{t} \models \phi_{1}(\vx, t)$ and $\ball{\diam}{t'} \models \phi_{2}(\vy, t')$ (since by our assumption we know that $\se \models \phi_{1}(\vx, t)$ and $\se \models \phi_{2}(\vy, t')$). Since $\se \models \phi_{3}(\vz)$ directly follows from our assumption, we have that $(t,t') \in \cols_{\rho}$, which proves the claim.
\end{proof}

Let us now define the following set, which will be used in the subsequent observation: 
$$
B_\coloring = \set{(\bball{\diam}{t}, \bball{\diam}{t'}) \;|\; (t,t') \in \cols_\coloring}.
$$

\begin{observation}
For each $(l,l') \in B_\coloring$, $\mathrm{add}_{R,(l,l')}(\se, \prcoloringe) = (\se \cup \set{R(t,t') \;|\; (t,t') \in \cols_{\rho}},\; \prcoloringe) \in \mathfrak{L}_{\ke}$.
\end{observation}

\begin{proof} Suppose that $(l,l') \in B_\coloring$. Then, we know that $R(t,t')$ is a fresh atom in $\mathrm{add}_{R,(l,l')}(\se, \prcoloringe)$ \ifandonlyif $\prcoloringe(t) = \bball{\diam}{t} = l$ and $\prcoloringe(t') = \bball{\diam}{t'} = l'$ \ifandonlyif $(t,t') \in \cols_{\coloring}$ (by the definition of $B_\coloring$ above) \ifandonlyif $(t,t') \in \cols_{\rho}$ (by \cref{obs:binary-unary-case-ball} above), thus proving the claim.
\end{proof}

%\begin{proof}
%Follows from \cref{obs:binary-unary-case-ball} and the fact that $\prcoloringe(t) = \bball{\diam}{t}$.
%\end{proof}

Proceeding similarly for the other rules of $\rulesetnorm$, we obtain the following: 
%
$$
(\se \cup \bigcup_{\rho \in \rulesetnorm} \set{R(t,t') \;|\; (t,t') \in \cols_\rho},\;\; \prcoloringe) \in \mathfrak{L}_{\ke}
$$ 
%
Observe that the first component is equal to $\so$. Hence, we may conclude \cref{lem:binary-reformulated}, which entails \cref{thm:binary}.

==> other/boring-comments.tex <==
\piotr{\begin{itemize}
    \item capital Latin letters for predicates
    \item $a,b,c$ for constants
    \item $x,y,z$ for variables
    \item $t,u,v,w$ for terms/nodes/nulls/vertices be careful with instances having constants
    \item $h$ for homomorphisms
    \item $f$ for general functions
    \item mathcal capital Latin $\mathcal{I}$ for instances
    \item mathcal D for databases (only constants allowed) $\mathcal{D}$
    \item $\phi, \psi$ - body and head of ex-rule
    \item $\rho$ for ex-rule
    \item $\alpha, \beta, \gamma$ for atoms of instances and databases
\end{itemize}}

\piotr{\begin{itemize}
    \item We should consider only Boolean queries with constants, as this will make everything easier to process and should not make our results weaker.
\end{itemize}}

\piotr{\begin{itemize}
    \item Instance is a set of Atoms build from terms from constants + nulls over a signature
    \item Database uses only constants
\end{itemize}}

\tim{
\begin{itemize}
    \item Let's us "cliquewidth" as opposed to "clique-width", since it seems (looking through a few papers here) that "treewidth" is usually used rather than "tree-width" (thus, things are kept analogically consistent).
    \item Also, for all classes of existential rules, we should use macros that write the name of the class (an abbreviation) in lower case bold letters; e.g. $\fus$, $\bcws$, etc.
\end{itemize}}

\thomas{\begin{itemize}
    \item Naming convention for our bcs: ``semantic bcs''?
    \item FES vs. $\fes$ resolved in favor of the latter (as is actually the FUS vs. $\fus$ one); use the command
    \item Maybe every equation in a proper equation-environment?
    \item subinstance vs. sub-instance \piotr{I vote for the latter.}
    \item for induced sub<smth>: Should we denote such a relation via $\le$ (to also contrast with $\subseteq$)?
\end{itemize}}

\tim{\begin{itemize}
    \item $A, B, C$ for sets of atoms (make a note that the context will determine when predicates are being used or sets, i.e. allow for ambiguity because easy to differentiate)
    \item We used both $l$ and $i, j$ to denote colors, though in the binary section I have started using $l$ with annotations (e.g. primes, subscripts, etc.). Perhaps we should stick to using this for colors?
    \item Use "rule set" to describe a set of ERs as opposed to "set of existential rules" or "set of ERs" to (i) maintain consistency, and (ii) because it is short and saves space.
    \item We use the abbreviation "ER" now instead of "existential rule" as it saves space.
\end{itemize}}

==> other/cor_skeleton-plus-has-bounded-cw.tex <==
%\subsection{Proof of \cref{cor:skeleton-plus-has-bounded-cw}}\label{sec:cor:skeleton-plus-has-bounded-cw}
\piotr{Proofread this, low priority.}

 %Let $\inst$ be a finite instance, then with its {\em diameter} we will define a following natural number $\max_{t,t' \in \inst}(\ldist{\inst}{t,t'})$.

\begin{customlem}{\ref{cor:skeleton-plus-has-bounded-cw}}
$\ksat{1}{\rulesetnormcon, \se}$ has bounded treewidth.
\end{customlem}
\begin{proof}
Given an instance $\inst$ and two its terms $t, t'$ define the {\em distance} $\ldist{\inst}{t,t'}$ from $t$ to $t'$ in $\inst$ as the minimal length of any path from $t$ to $t'$ treating binary atoms of $\inst$ as undirected edges. Also, let $\db$ denote database fixed in \cref{sec:binary}.

For a null $t$ of $\se$ and a natural number $n$ let {\em neighbourhood} $\neigh{n}{t}$ of $t$ of distance $n$ be a following set of terms $\set{t \in \termset(\se) \;|\; \ldist{\se}{t, t'} \leq n}$. Also let $\neigh{n}{\db} = \set{t \;|\; \exists{c\in\adom{\db}}\;\ldist{\se}{t,c} < n}$

Let $T_n = {V_n, E_n}$ be a following tree decomposition:
\begin{itemize}
    \item $V_n = \set{\neigh{n}{t} \;|\; t \in \nullset(\se) } \cup \set{r}$, where $r = \termset(\db)$.
    \item $E_n = \set{(\neigh{n}{t}, \neigh{n}{t'}) \;|\;  \wedge\exists{R\in\sig}\; \se \models R(t,t') \vee R(t', t)} \;\cup\;\\ \set{(r, \neigh{n}{t}) \;|\;  \exists{c \in \conset(\db)}\; \exists{R\in\sig} \se \models R(t,t') \vee R(t', t)}$.
\end{itemize}

Now we will argue that for every $n > 1$ tree $T_n$ is a tree decomposition of $\se$ as:
\begin{itemize}
    \item $\bigcup_{v\in V_n}v$ is equal to $\termset(\se)$.
    \item Each atom $R(t,t')$ of $\se$ is indeed contained in one of bags of $V_n$, namely $\neigh{n}{t}$, as $n > 1$.
    \item From the definition of neighbourhood, one can note that for each term $t$ in $\se$, the sub-graph of $T_n$ induced by the nodes $v$ of $V$ such that $t \in v$ is connected. 
\end{itemize}

Recall from \cref{obs:sate-is-forest} that $\se$ has a bounded degree. Thus observe that for every $n\in\mathbb{N}$ there exists $k \in \mathbb{N}$ such that for every term $t$ of $\se$ we have $|\neigh{n}{t}| < k$. Thus width of $T_n$ is bounded.

Let $d \in \mathbb{N}$ be such that for every rule $\rho \in \rulesetnormcon$, and its frontier variables $x,y$, the following holds $d \geq \ldist{\body(\rho)}{x,y}$. Note that such a $d$ exists because $x$ and $y$ share the same connected component of $\body(\rho)$. Finally, observe that for every atom $R(t,t')$ of $\ksat{1}{\rulesetnormcon, \se} \setminus \se$ we have that $t,t' \in \neigh{d}{t}$ or $t,t' \in \neigh{d}{\db}$. From this we conclude that $T_d$ is a tree decomposition of $\ksat{1}{\rulesetnormcon, \se}$ of bounded width.

\end{proof}

==> other/fes-and-tbs.tex <==
\section{Finite Unification Sets and Bounded Treewidth Sets}

\begin{definition}[Finite Expansion Set ($\fes$)] A set of existential rules $\calr$ is called a \emph{finite expansion set ($\fes$)} \ifandonlyif for every fact $F$, there exists an integer $k$ such that $F_{k} = \ksat{k}{F,\calr} \equiv \ksat{k+1}{F,\calr} = F_{k+1}$. We refer to $F_{k}$ as a \emph{full derivation} of $F$.
\end{definition}

\piotr{Word theorem should be reserved only to our results.}
\begin{theorem}
If $\calr$ is a $\fes$, then it is BCQ entailment is decidable. 
\end{theorem}

\begin{proof}
See~\cite[\prp~5]{BagLecMugSal11}.
\end{proof}


\thomas{In the preliminaries we define ``fact'' to mean a atomic sentence (i.e. a grounded atom). In the following definition(s!) we use the notion of ``fact'' that is a collection of atomic formulae. There is a clash here that needs to be discussed.}
\piotr{sure, we still need to rewrite this section to fit the rest of the paper.}


==> other/fo-rewritability.tex <==
\medskip \noindent {\bf Rewritings and finite unification sets.}
Given a rule set $\ruleset$ and a CQ $\phi(\vx)$ we say that a UCQ $\psi(\vx)$ is a {\em rewriting} of $\phi(\vx)$ under the rule set $\ruleset$ \ifandonlyif for any database $\database$ and any tuple of its elements $\va$ the following holds:
%
$$\sat{\database,\ruleset} \models \phi(\va) \ \ifandonlyif \ \database \models \psi(\va).$$
%
a rule set $\ruleset$ is a {\em finite unification set} ($\fus$) \iffi for every query there exists a UCQ rewriting \cite{BagLecMugSal11}. This property is also referred to as \emph{first-order rewritability}.
%
If a rule set $\ruleset$ is $\fus$, then for any given CQ $\phi(\vx)$ we denote its rewriting under $\ruleset$ with $\rewrs{\ruleset}{\phi(\vx)}$.




==> other/main-results.tex <==
\section{Main contributions}\label{sect:main-results}
\piotr{Should we merge this section with the introduction?}

Given a rule set $\ruleset$ and a CQ $\phi(\vy)$ we say that a UCQ $\psi(\vy)$ is a {\em rewriting} of $\phi(\vy)$ under the rule set $\ruleset$ \ifandonlyif for any database $\database$ and any tuple of its elements $\va$ the following holds:
%
$$\sat{\ruleset, \database} \models \phi(\va) \ \ifandonlyif \ \database \models \psi(\va).$$
 
Following~\cite{BagLecMugSal11}, we say that a rule set $\ruleset$ has the {\em finite unification set property} (is $\fus$) if for every query there exists a UCQ rewriting. If a rule set $\ruleset$ is $\fus$, then for any given CQ $\phi(\vx)$ we denote its rewriting under $\ruleset$ with $\rewrs{\ruleset}{\phi(\vx)}$.

And so in the case of binary signatures the bounded cliquewidth sets contain FO-rewritable sets:

\begin{theorem}\label{thm:binary}
\tim{
Any FO-rewritable set of single-headed existential rules over a binary signature is a bounded-cliquewidth set.
}
\end{theorem}


Surprisingly this is not the case generally. This constitutes our second main contribution:

\begin{theorem}\label{thm:higher-arity}
There exists a FO-rewritable set of existential rules that is not bounded-cliquewidth set.
\end{theorem}

==> other/obs_cross-coloring.tex <==

\begin{customobs}{\ref{obs:cross-coloring}}
Let $\inst$ be a finite instance. Moreover, let $\coloring : \adom{\inst} \to \{1, \ldots, k\}$ and $\coloring' : \adom{\inst} \to \{1, \ldots, k'\}$ be two colorings with $(\coloring \times \coloring')(t) = (\coloring(t), \coloring'(t))$, for each $t \in \adom{\inst}$. If $\cw{\inst, \coloring} = k$, then $\cw{\inst, \coloring \times \coloring'} = k \cdot k'$.
\end{customobs}

\begin{proof}
Since $\ruleset$ is a set of single-headed rules over a binary signature, and since we only consider non-datalog rules (as $\se \setminus \database$ only contains atoms derived by the non-datalog rules from $\ruleset$), we know that each rule $\rho$ applied during the Skolem chase is of the form $\phi(\vec{x},y) \rightarrow head(\rho)$ with $head(\rho) \in \{\exists z R(y,z), \exists z R(z,y), \exists z \exists z' R(z,z')\}$. That is to say, for each rule $\rho$, $\fr(\rho) = 1$ or $\fr(\rho) = 0$. Observe that if a rule of frontier $1$ is applied during the Skolem chase, then it gives rise to a single edge (typed with the predicate $R$ occurring in the head of the rule) in %$\struc^{\inst}$
 $\se \setminus \database$ that can either be directed toward (if $\head(\rho) = \exists z R(y,z)$) or away from (if $\head(\rho) = \exists \vec{z} R(z,y)$) the frontier term it is attached to. If a rule of frontier $0$ is applied during the Skolem chase, then it creates a disconnected typed edge that corresponds to, and gives rise to, a new typed polytree in %$\struc^{\inst}$. 
 $\se \setminus \database$. Hence, we can see that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest. Moreover, as we are using the Skolem chase and due to the fact that $\ruleset$ is finite, there can only be a finite number of typed edges added to each vertex in the typed polyforest, ensuring that it is of bounded degree.
\end{proof}

\thomas{Proof with new definition}
\begin{proof}
  Let $(\inst, \coloring)$ be a colored instance and $\coloring'\colon\adom{\inst}\to \{ 1, \ldots, k' \}$ another coloring for $\inst$. Furthermore, let $\cw{\inst, \lambda} = k$. Then there exists for a finite set of colors $\cols = \{ 1, \ldots, k \}$ a well $(\cols, Cnst, \Sigma)$-decorated tree $\mathcal{T}$ such that $\inst^{\mathcal{T}}=\inst$ and $\mathit{col}^\mathcal{T} = \coloring$.
  For $\cols' = \{1, \ldots, k \} \times \{ 1, \ldots, k'\}$ we obtain a $(\cols', Cnst, \Sigma)$-decorated tree $\mathcal{T}'$ inductively over the nodes of $\mathcal{T}$ and $\mathcal{T}'$ in the following way:
  
  \textit{Transformations.} Let $s, s'\in \{ 0,1 \}^{\ast}$ and $N_{p} \subseteq (\{ 0,1 \}^{\ast})^{2}$.% We define $\mathcal{T}_{s}$ to be the subtree of $\mathcal{T}$ issued from $s$.
    \begin{enumerate}
        \item\label{item: Transformation1} If $\oplus(s)\in \mathcal{T}_{s}$, then $\oplus(s') \in \mathcal{T}^{s}$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation2} If for $c\in Cnst \cup \{ \ast \}$ and $l\in\cols$ $c_{l}(s)\in \mathcal{T}$, then $c_{(l, \lambda'(s))}(s')\in \mathcal{T}^{s}$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation3} If $\mathrm{Void}(s)\in \mathcal{T}_{s}$, then add $\mathrm{Void}(s')$ to $\mathcal{T}'$ and add to $N_{p}$ the pairs $(s0, s'0)$ and $(s1, s'1)$.% set $s_0 = s0$, $s_1 = s1$, $s'_{0} = s'0$, and $s'_1 = s'1$.
        \item\label{item: Transformation4} If for $R\in\Sigma_1$ and $l\in\cols$ $\mathrm{Add}_{R, l}(s)\in\mathcal{T}_{s}$, then add %\[ \{ \mathrm{Add}_{R, (l, i)}(0^{i-1}), \mathrm{Void}_(0^{j-1}1) \, | \, 1\le i, j \le k'\} \]
        \[ \{ \mathrm{Add}_{R, (l, i)}(0^{i-1}) \, | \, 1\le i, j \le k'\} \]to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i\le k'$ the pairs $(s0, s'0^{i})$ and $(s1, s'0^{i-1}1)$.% and set $s_0 = s0$ and $s'_0 = s'0^{k'}$.
        \item\label{item: Transformation5} If for $R\in\Sigma_2$ and $l_1, l_2\in\cols$ $\mathrm{Add}_{R, l_1, l_2}(s)\in\mathcal{T}_s$, then add %\[ \{ \mathrm{Add}_{R, (l_1, i), (l_2, j)}(0^{i-1 + (j-1)\cdot k'}), \mathrm{Void}(0^{i-1 + (j-1)\cdot k'}1) \, | \, 1\le i, j \le k' \} \]
        \[ \{ \mathrm{Add}_{R, (l_1, i), (l_2, j)}(0^{i-1 + (j-1)\cdot k'}) \, | \, 1\le i, j \le k' \} \] to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i, j\le k'$ the pairs $(s0, s'0^{i + (j-1)\cdot k'})$ and $(s1, s'0^{i-1 + (j-1)\cdot k'}1)$.% set $s_0 = s0$ and $s'_0 = s'0^{k'\cdot k'}$.
        \item\label{item: Transformation6} If for $l_1, l_2\in\cols$ $\mathrm{Recolor}_{l_1 \to l_2}(s)\in\mathcal{T}_{s}$, then add %\[ \{ \mathrm{Recolor}_{(l_1, i) \to (l_2, j)}(0^{i-1 + (j-1)\cdot k'}), \mathrm{Void}(0^{i-1 + (j-1)\cdot k'}1) \, | \, 1\le i,j \le k' \} \]
        \[ \{ \mathrm{Recolor}_{(l_1, i) \to (l_2, j)}(0^{i-1 + (j-1)\cdot k'}) \, | \, 1\le i, j \le k' \} \] to $\mathcal{T}^{s}$ and add to $N_{p}$ for $1\le i, j\le k'$ the pairs $(s0, s'0^{i + (j-1)\cdot k'})$ and $(s1, s'0^{i-1 + (j-1)\cdot k'}1)$.% set $s_0 = s0$ and $s'_0 = s'0^{k'\cdot k'}$.
    \end{enumerate}
  
  \textit{Base case.} Initialize $N_{p} = \{ (\varepsilon, \varepsilon) \}$. Then apply the appropriate transformation for the tuple $(\varepsilon, \varepsilon)$.% $\mathcal{T}_{\epsilon} = \mathcal{T}$ and add the pair(s) $(s_0, s'_0)$ (and $(s_1, s'_1)$) if obtained from the transformation) to the set $N_p$.
    
  \textit{Induction Step.} Suppose $N_p$ already contains more than $(\varepsilon, \varepsilon)$. With $\prec$ we denote the usual prefix order on $\{ 0,1 \}^{\ast}$. We define a partial order on $N_p$ in the following way: \[ (s_1, s_1') < (s_2, s_2') \quad \text{\ifandonlyif} \quad s_1 \prec s_2 \text{ or } s_1 = s_2 \land s_1' \prec s_2' \, . \] Take the tuple $(s,s')\in N_p$ such that $(s,s')$ is a $|s'|$-minimal $<$-maximal element in $N_p$. Then apply the appropriate transformation to $(s,s')$.
  
  Finally, obtain $\mathcal{T}' = \mathcal{T}_{bin}\cup \bigcup_{s\in\mathcal{T}_{bin}}\mathcal{T}^{s}$.
  
  \thomas{\textit{TODO: Properties of $N_p$.}}
    \begin{enumerate}
        \item\label{item: N_property1} If $(s, s')\in N_p$ with $c\in Cnst \cup \{ \ast \}$ and $c_l(s)\in\mathcal{T}$ for some $l\in \cols$, then $c_{(l, \lambda'(s))}(s')\in \mathcal{T}'$ and $s'$ is the unique $s''\in \{ 0, 1\}^{\ast}$ such that $(s,s'')\in N_p$.
            \begin{subproof}
                Let $s\in \{ 0,1 \}^{\ast}$ and for some $l\in \cols$ and $c\in Cnst$ it holds that $c_l(s)\in \mathcal{T}$. Furthermore, suppose that $s', s''\in \{ 0,1 \}^{\ast}$ such that $(s, s'), (s,s'')\in N_p$ with $c_{(l, \lambda'(s))}(s'), c_{(l, \lambda'(s))}(s'')\in \mathcal{T}^{s}$. This can only happen, if there was previously a transformation applied for $r, s''' \in \{ 0,1 \}^{\ast}$ to $(r, s''')\in N_p$ with $\mathrm{Succ}_0(r, s)\in \mathcal{T}$ and $s''' \prec s', s''$ such that either
                \begin{enumerate}
                    \item\label{item: N_property1_a} for $R\in\Sigma_1$ and $m\in\cols$ $\mathrm{Add}_{R, m}(r)\in\mathcal{T}$, or
                    \item\label{item: N_property1_b} for $R\in\Sigma_2$ and $m_1, m_2\in\cols$ $\mathrm{Add}_{R, m_1, m_2}(r)\in\mathcal{T}$, or
                    \item\label{item: N_property1_c} for $m_1, m_2\in\cols$ $\mathrm{Recolor}_{m_1 \to m_2}(r)\in\mathcal{T}$.
                \end{enumerate}
                But then w.l.o.g. (in case \ref{item: N_property1_a}) $s' = s'''0^{i}$ and $s'' = s'''0^{j}$ with $1\le i < j, \le k'$ or (in cases \ref{item: N_property1_b} and \ref{item: N_property1_c}) $s' = s'''0^{i}$ and $s'' = s'''0^{j}$ with $1\le i < j, \le k'\cdot k'$. But then, by the Inductions Step, Transformation \ref{item: Transformation2} is only applied to the tuple $(s, s'''0^{k'})$ (in case \ref{item: N_property1_a}) or $(s, s'''0^{k'\cdot k'})$ (in cases \ref{item: N_property1_b} and \ref{item: N_property1_c}) as this is $<$-maximal for the introduced $N_p$-pairs. Hence $s'''0^{k'\cdot k'} = s' = s''$, showing uniqueness. Furthermore, by Transformation \ref{item: Transformation2} we obtain $c_{(l, \lambda'(s))}(s'), c_{(l, \lambda'(s))}(s'')\in \mathcal{T}^{s}$.
            \end{subproof}
        \item\label{item: N_property2} If $(s, s')\in N_p$ with $\mathrm{Void}(s)\in\mathcal{T}$, then $\mathrm{Void}(s')\in \mathcal{T}'$ and for all $s''\in\{ 0,1 \}^{\ast}$ with $s' \prec s''$ we have $\mathrm{Void}(s'')$.
            \begin{subproof}
                If $(s, s')\in N_p$, application of Transformation \ref{item: Transformation3} yields $\mathrm{Void}(s')\in \mathcal{T}'$. As then $(s0, s'0), (s1, s'1)$ are added to $N_p$, applications of Transformation \ref{item: Transformation3} to both will yield $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\in \mathcal{T}'$. Inductively we obtain for all $s''\in\{ 0,1 \}^{\ast}$ with $s' \prec s''$ we have $\mathrm{Void}(s'')$.
            \end{subproof}
    \end{enumerate}
  
  \thomas{\textit{TODO: Proof}} $\mathcal{T}'$ is a well $(\cols', Cnst, \Sigma)$-decorated tree.
    \begin{itemize}
        \item For every $s\in \{ 0,1 \}^{\ast}$, $Dec(s)\in\mathcal{T}'(s)$ for exactly one $Dec \in Dec(\cols', Cnst, \Sigma)$ by constructions.
        \item Since, by construction, if for $c\in Cnst$, $(l_1, l_2)\in \cols'$ and $s'\in\{ 0,1 \}^{\ast}$ it holds that $c_{(l_1, l_2)}(s')\in\mathcal{T}'$, then there is a $s\in\{ 0,1 \}^{\ast}$ such that $c_{l_1}(s')\in\mathcal{T}$ and $(s, s')\in N_p$. By Property \ref{item: N_property1} $s'$ is unique for $s$. On the other hand, Transformation \ref{item: Transformation2} is only executed, if there is a pair $(s, s')\in N_p$ with $c_{l_1}(s')\in\mathcal{T}$. In conclusion, for every $s'\in \{ 0,1 \}^{\ast}$, $c\in Cnst$, and $l\in\cols'$ there is at most one fact of the form $c_{l}(s')\in\mathcal{T}'$.
        \item If $\mathrm{Void}(s')\in\mathcal{T}'$ or $c_{(l_1, l_2)}(s')\in \mathcal{T}'$, then $\mathrm{Void}(s'0), \mathrm{Void}(s'1)$. In the case of $\mathrm{Void}(s')\in \mathcal{T}'$ this follow immediately from Property \ref{item: N_property2}. If on the other hand $c_{(l_1, l_2)}(s')\in \mathcal{T}'$ we observe that there exists by construction exactly one $s\in\{0,1 \}^{\ast}$ such that $c_{l_1}(s)\in\mathcal{T}$ and $(s, s')\in N_p$. Note that $c_{(l_1, l_2)}(s')$ was then produced by application of Transformation \ref{item: Transformation2} and $(s0, s'0), (s1, s1')$ will have been added to $N_p$. Application of Transformation \ref{item: Transformation3} then has yielded $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\in \mathcal{T}'$ as $\mathrm{Void}(s0), \mathrm{Void}(s1)\in\mathcal{T}$.
        \item If $\oplus(s')\in\mathcal{T}$ then $\mathrm{Void}(s'0), \mathrm{Void}(s'1)\not\in \mathcal{T}'$ follows by construction.
        \item If for $l, l'\in\cols'$ we have $\mathrm{Recolor}_{l\to l'}(s') \in \mathcal{T}'$ or $\mathrm{Add}_{R,l,l'}(s') \in \mathcal{T}'$ or $\mathrm{Add}_{R,l}(s') \in \mathcal{T}'$ then by definition of Transformations \ref{item: Transformation4} - \ref{item: Transformation6} $\mathrm{Void}(s'0)\not\in \mathcal{T}'$ and $\mathrm{Void}(s'1) \in \mathcal{T}'$ hold by construction.
    \end{itemize}
  
  \thomas{\textit{TODO: Proof}} $\mathcal{I}^{\mathcal{T}'} \cong \mathcal{I}^{\mathcal{T}}$ and $\mathrm{col}_{\epsilon}^{\mathcal{T}'} = \coloring \times \coloring'$.
  Obtaining the isomorphism works as follows: By Property \ref{item: N_property1} for every $(s,s')\in N_p$ such that for some $c\in Cnst\cup\{ \ast \}$ and $l\in \cols$ it holds that $c_{l}(s)\in\mathcal{T}$, $s'$ is unique.
  
  --- WORK IN PROGRESS ---
\end{proof}

==> other/obs_sate-is-forest.tex <==
%\subsection{Proof of \cref{obs:sate-is-forest}}\label{sec:obs:sate-is-forest}
\begin{customobs}{\ref{obs:sate-is-forest}}
$\se \setminus \database$ is a typed polyforest of bounded degree.
\end{customobs}

\begin{proof}
Since $\ruleset$ is a set of single-headed rules over a binary signature, and since we only consider non-datalog rules (as $\se \setminus \database$ only contains atoms derived by the non-datalog rules from $\ruleset$), we know that each rule $\rho$ applied during the Skolem chase is of the form $\phi(\vec{x},y) \rightarrow head(\rho)$ with $head(\rho) \in \{\exists z R(y,z), \exists z R(z,y), \exists z \exists z' R(z,z')\}$. That is to say, for each rule $\rho$, $\fr(\rho) = 1$ or $\fr(\rho) = 0$. Observe that if a rule of frontier $1$ is applied during the Skolem chase, then it gives rise to a single edge (typed with the predicate $R$ occurring in the head of the rule) in %$\struc^{\inst}$
 $\se \setminus \database$ that can either be directed toward (if $\head(\rho) = \exists z R(y,z)$) or away from (if $\head(\rho) = \exists \vec{z} R(z,y)$) the frontier term it is attached to. If a rule of frontier $0$ is applied during the Skolem chase, then it creates a disconnected typed edge that corresponds to, and gives rise to, a new typed polytree in %$\struc^{\inst}$. 
 $\se \setminus \database$. Hence, we can see that %$\struc^{\inst}$ 
 $\se \setminus \database$ is a typed polyforest. Moreover, as we are using the Skolem chase and due to the fact that $\ruleset$ is finite, there can only be a finite number of typed edges added to each vertex in the typed polyforest, ensuring that it is of bounded degree.
\end{proof}

==> other/old-clique-width.tex <==

\section{Clique-width and Related Notions}\label{sec:cliquewidth}

\piotr{\begin{itemize}
    \item Discuss clique-width with examples
    \item Introduce bounded clique-width sets
    \item Discuss its importance
    \item Push observations and lemmata which do not contribute to the story to the separate subsection
\end{itemize}}


\medskip \noindent {\bf Cliquewidth.}
We define the notion of clique-width following the formalization provided in \cite[\dfn~15]{GroheT04}.
For a standard definition of a clique-width for graphs one can refer (for example) to \cite[\dfn~2.89]{CourEngBook}.

A {\em structure} is a generalization of an instance that may contain isolated terms (terms that do not appear in any atom). To denote the set of terms of a structure $\struc$ we write $\aadom{\struc}$. Given a finite set of colors $\cols$ a {\em colored structure} is a pair $(\struc, \coloring)$ where $\struc$ is a structure and and $\coloring$ is a function from $\aadom{\struc} \to \cols$.

\tim{
I re-wrote the above paragraph (shown below) to make the definition of structure more explicit. If you find it to be to verbose, feel free to simplify it, or even remove it altogether if you find it unnecessary. I find having the explicit definition is helpful for the reader however as it ensures they have a clear understanding of the meaning of the object being discussed. Also, I've used this notation and terminology in re-writings of the binary section, though it can be amended/easily changed depedning on how we decide to move forward.
}

\tim{
A {\em $\sig$-structure} $\struc$ (which we refer to as a \emph{structure} more simply when the signature $\sig$ is clear from the context) is a pair $(\sdom,\srel)$, where $\sdom$ is a non-empty set of points, referred to as \emph{terms}, and $\srel$ is a family $\{R \ | \ R \in \sig\}$ of relations such that $R \subseteq \sdom^{\arity{R}}$. Observe that structures generalize the notion of an instance as they may contain isolated terms (terms that do not appear in any atom). Hence, every instance $\inst$ can be transformed into a corresponding structure $\struc^{\inst} = (\sdom^{\inst},\srel^{\inst})$, where $\sdom^{\inst} = \aadom{\inst}$, $\srel^{\inst}$ is the set of predicates occurring in $\inst$, and where for any $R \in \srel^{\inst}$, $\vt \in R$ \ifandonlyif $R(\vt) \in \inst$. For a given structure $\struc = (\sdom, \srel)$, we let $\aadom{\struc}$ denote the set of terms in a structure, that is, $\aadom{\struc} = \sdom$. Given a finite set of colors $\cols$ a {\em colored structure} is defined to be a pair $(\struc, \coloring)$ where $\struc$ is a structure and and $\coloring$ is a function from $\aadom{\struc} \to \cols$.
}

\tim{It might be good to note somewhere for the reader that the codomain of colorings is held constant throughout the following construction process.} 

Given a set $\cols$ of $k$ colors a {\em basic $k$-colored finite structure} is a single term or constant $t$ colored with any of colors in $\cols$. We define the set $\mathfrak{L}_k$ of colored finite structures as a minimal set containing basic $k$-colored and closed under following operations:

\begin{itemize}
    \item $\add{A,\vl}{\struc, \coloring}$ adds the following atoms to the colored finite structure $\set{A(\vt) \;|\; \vt \in \aadom{\struc}^{\arity{A}} \wedge \coloring(\vt) = \vl}$, where $A \in \sig$ and \tim{$\vl \in \cols^{\arity{A}}$}.
    \item $\recol{i\to j}{\struc, \coloring}$ recolors $i$-colored terms of $(\struc, \coloring)$ to color~$j$.
    \item $\disun$ takes a disjoint union of the colored finite structures. \thomas{$i, j\in \cols$}
\end{itemize}

\begin{definition}[Clique-width]\label{def:cw}
Given a finite instance $\inst$ we define the {\em clique-width} $\cw{\inst}$ as the smallest $k$ such that there exists a coloring $\coloring$ such that $(\inst, \coloring)$ is in $\mathfrak{L}_k$. \\
\thomas{Given an infinite instance $\inst$ we define its {\em clique-width} $\cw{\inst}$ as the supremum over the clique-widths of all finite induced substructures of $\inst$.}
\end{definition}

\thomas{In the case of finite structures our notion of clique-width coincides with the one from \cite{GroheT04}. The infinite case though diverges from the literature in general as clique-width definitions are usually intricately linked with the terms representing the structures. Those terms lend itself to be extended to infinite ones. Unfortunately this usually does not allow for ``nice'' compactness behavior akin to ``for an infinite structure $\struc{}$ it holds that if every finite induced substructure has clique-width of at most $n$, then so does the structures $\struc{}$ itself''. For more details we refer the reader to e.g. \cite{Cou04}. Luckily, as the cited work shows, boundedness of clique-width does admit a compactness property, i.e. it is true that ``for an infinite structure $\struc{}$ it holds that if there is a {\em uniform} bound $n$ on the clique-width of all finite induced substructures of $\struc{}$ then the clique-width of $\struc{}$ itself is bounded by a number $f(n)$'' where $f$ is a function $\mathbb{N}\to\mathbb{N}$ that is not the identity. TODO, maybe in an observation?}
Now we need to extend our definition to the instances in general not only finite instances.
\piotr{TODO}

\tim{Note: As per our discussion we need to generalize the following to typed polytrees (https://en.wikipedia.org/wiki/Polytree) and also I think we should discuss forests of typed polytrees to make the observation correspond directly to Corollary 8.
}

\begin{observation}\label{obs:trees_cw_le3}
Let $\struc$ be a oriented forest over a finite binary signature\footnote{\thomas{Or should we call this ``edgecolors''? Call it ``edge-colored oriented...'' or something like that?}} $\Sigma$. Then $\cw{\struc} \le 2 \cdot |\Sigma| + 2$.
\end{observation}
\begin{proof}
\thomas{proof sketch for poly forest.} First note that in the case of an infinite oriented forest, every induced finite substructure is an oriented forest as well. Thanks to our definition of clique-width it is thus enough to analyze only the construction of those finite oriented forests. Furthermore, since finite oriented forests are finite, they are the disjoint union of finitely many finite oriented trees. Hence we can concentrate only on finite oriented trees at first. In the construction process, each of those oriented trees will be constructed seperately and in a final step we successively and disjointly unify them. \\
Given a finite oriented tree of a finite binary signature. Then we will define the following set of colors: $\cols{} = \{ E^{+}, E^{-} \, | \, E \in \Sigma \}\cup \{ \texttt{D}, \texttt{R} \}$. Then we construct the oriented tree in the following way:
\begin{enumerate}
    \item leafs will be introduced as the basic structures colored by in the following way: If there is an $E\in\Sigma$-edge ending/starting in the leaf, we will color it by the color $E^{+}$ or $E^{-}$ respectively. Else we will color it with $\texttt{D}$.
    \item If two subtrees of are joined at a node and both subtrees are already constructed, we do the following: We disjointly unify the subtrees. The resulting forest will be disjointly unified with a new basic structure colored with $\texttt{R}$. Then we apply succesively, until we cannot do it any further, the following:
    For each $E \in \Sigma$ such that there is a node of color $E^{+}$ or $E^{-}$:
    \begin{enumerate}
        \item apply the operation $\add{E, (E^{-}, \texttt{R})}{}$ or $\add{E, (\texttt{R}, E^{+})}{}$ depending whether there is a node colored $E^{+}$ or $E^{-}$. If both are the case, apply those operations succesively;
        \item then recolor all nodes of color $E^{+}$ and of color $E^{-}$ to $\texttt{D}$;
        \item and finally recolor all nodes of color $\texttt{R}$ corresponding to whether there is an $F\in\Sigma$-edge incoming (color with $F^{+}$) or outgoing (color with $F^{-}$).
    \end{enumerate}
\end{enumerate}
This process will terminate after finitely many steps, which is easy to see: If a node is not of color $\texttt{D}$, then it is either a leaf node freshly introduced (that has in the oriented tree we want to construct some incoming or outgoing edge), or a root node of an already constructed oriented subtree , or it is a node acting as a ``new root'', merging already constructed oriented subtrees to a bigger oriented subtree. Since we only discuss finite oriented trees, we can only add finitely many leaf nodes or merge finitely many oriented subtrees until we obtain the whole oriented tree we wish to construct.

\end{proof}



==> other/old-higher.tex <==
\section{Results for Higher Arity Signatures}
%Tim: I moved the commands that were here to the MISC section of the "notation" file.

We dedicate this section to the proof of \cref{thm:higher-arity}, i.e. we show that even if we utilize a binary signature, then permitting the use of non-single-headed rules in a given finite unification set can unbound the clique-width of an associated universal model. We let $\sigi = \set{\hpred, \vpred, \origin}$ be a signature where $\hpred$ and $\vpred$ are binary predicates and $\origin$ is a unary predicate. Let us define $\rsgrid$ to be the following rule set over $\sigi$:
$$
\begin{array}{@{}l@{\ \ \ \ \ \ }r@{\ }l@{\ \ \ \ \ \ \ \ }}
\text{(loop)} & \top & \rightarrow \exists x \; (\hpred(x,x) \land \vpred (x,x)) \\[0.5ex]
\text{(grow)} & \top & \rightarrow \exists y \exists y'\; (\hpred(x,y) \land \vpred (x,y')) \\[0.5ex]
\text{(grid)} & \hpred(x,y) \land \vpred(x,x')  & \rightarrow \exists y' \; (\hpred(x',y') \land \vpred(y,y'))
\end{array}
$$

\piotr{Discuss the multi-head higher arity here if necessary, it could be done earlier as well.}

We make use of $\rsgrid$ to establish \cref{thm:higher-arity}, whose proof is split into two parts. First, we provide a database $\dbg$ to form a knowledge base $(\rsg, \dbg)$ for which no universal model of bounded clique-width exists (\cref{lem:no-universal-model-cw}). Second, we show that $\rsg$ is a finite unification set (\cref{lem:rsg-is-fus}). %Hence, taking both of these results together entails \cref{thm:higher-arity}.


\subsection{$\rsgrid$ is not a bounded clique-width set}


We will devote the rest of this section to the proof of the following lemma:



\begin{lemma}\label{lem:no-universal-model-cw}
Let $a$ be a constant and let $\dbg = \set{A(a)}$ be a database then, there is no universal model of $\kbaseg$ with a bounded clique-width.
\end{lemma}


Let $\ginf$ be an instance that is the infinite quarter-grid as depicted on the \cref{fig:ginf}, where all terms other that the constant $a$ are nulls.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/ginf.pdf}
    \caption{ The instance $\ginf$.}
    \label{fig:ginf}
\end{figure}

\begin{observation}\label{obs:ginf-is-universal-model}
The instance $\ginf$ is a universal model of $\kbaseg$.
\end{observation}



%It is well known~\cite{} that all grid like structures have unbounded clique-width. 
%\thomas{The original proof for (undirected!) grids w.r.t. clique-width was done in \cite[\thm~4]{GolumbicRot99}, where grids are considered as (undirected) graphs. We probably(?) should be ``careful'' here since we have two types of edges and are in the directed setting. It's not that it wouldn't work or anything... But we probably should make a short argument why it does hold here.}

It is well known that infinite grids over a signature consisting of single binary relation have unbounded clique-width (see \cite[\thm~4]{GolumbicRot99} for the reference). Consider the following:

\begin{observation}\label{fact:grid-has-unbounded-cw}
The instance $\ginf$ has unbounded clique-width.
\end{observation}
\begin{proof}
    Consider the two following claims:
    \begin{claim}
        Let $\sig$ be a binary signature, $E$ be a binary relational symbol and $\inst$ be any instance over $\sig$. Then the instance $\inst' = \set{E(t,t') | A(t,t') \in \inst, A \in \sig}$ satisfies $\cw{\inst} \geq \cw{\inst'}$.
    \end{claim}
    \begin{subproof}[Proof]
    \todoiftime
    \end{subproof}
    
    \begin{claim}
        Let $\sig$ be a signature consisting of a single binary relational symbol $E$ and $\inst$ be any instance over $\sig$.  Then the instance $\inst' = \set{E(t',t) | E(t,t') \in \inst} \cup \inst$ satisfies $\cw{\inst} \geq \cw{\inst'}$.
    \end{claim}
    \begin{subproof}[Proof]
    \todoiftime
    \end{subproof}
    
    Finally note that adding $\set{A(a^{\arity{A}}) | A \in \sigi}$ to any instance does not lower its clique-width. \thomas{How about $\set{P(a^{\arity{P}}) | P \in \sigi}$ or $R$ instead of $P$? $A$ does not feel well-chosen here, considering that we only have three relations symbols in our signature of which one is called $A$. We could even write it out as $\{ A(a), H(a, a), V(a, a) \}$, because $a^{\arity{A}}$ is also a bit weird.}
\end{proof}

\begin{observation}\label{obs:identity}
If $h: \ginf \to \ginf$ is a homomorphism then $h$ is \thomas{the} identity.
\end{observation}

\piotr{define what is induced sub-instance if we do not do that already.}
\begin{lemma}
Every universal model of $\kbaseg$ contains $\ginf$ as an induced sub-instance.
\end{lemma}
\thomas{Restatement of the lemma:
\begin{lemma}
Every universal model of $\kbaseg$ contains an induced sub-instance isomorphic to $\ginf$.
\end{lemma}
Reason for restatement: Induced sub-instance means we see exactly that structure. But it is easy to see that we could kind of ``rename'' the elements in $\unimod$, such that $\ginf$ is not formally an induced sub-instance.}
\begin{proof}
Take any universal model $\unimod$ of $\kbaseg$. From the fact that $\ginf$ is a universal model as well we conclude the existence of two homomorphisms $h\colon \ginf \to \unimod$ and $h'\colon \unimod \to \ginf$. Consider the homomorphism $h' \circ h$ and note that, from~\cref{obs:identity}, it needs to be an identity. 
\thomas{(Rewriting from last sentence.) Observe that from \cref{obs:identity} the homomorphism $h'\circ h$ has to be the identity on $\ginf$. Hence $h$ has to be injective. Furthermore $h$ is even reflective, hence constitutes an embedding. Let $P\in\sigi$ and $\vt$ be a tuple of length $\arity{P}$ from $\ginf$. If $P(h(\vt))$ holds in $\unimod$ , then $P(h'(h(\vt)))$ holds in $\ginf$. But since $h'\circ h$ is the identity on $\ginf$ we immediately obtain $P(\vt)$. Finally note that the image of $\ginf$ under $h$ is isomorphic to $\ginf$ and hence we obtain the claim.}
\end{proof}

\subsection{$\ruleset_{grid}$ is a finite unification set}


As promised in this section we will prove the following lemma:
\begin{lemma}\label{lem:rsg-is-fus}
$\rsg$ is $\fus$.
\end{lemma}

Clearly, given rule $(loop)$ of $\rsg$, we can see that every BCQ that does not contain constants has a trivial rewriting. Thus, consider the following:

\begin{observation}\label{obs:bcq-no-const-trivial}
Every BCQ that contains no constants is FO-rewritable with respect to $\rsg$.
\end{observation}

\piotr{Here is a link for Xrewrite \url{https://arxiv.org/pdf/1405.2848.pdf}}
Proving that a provided rule set is FO-rewritable is a notoriously difficult task\footnote{This should not be much surprising as FO-rewritability is an undecidable property~\cite{fus-is-undecidable-property}.}. To this end, we hand-tailor a rewriting algorithm to be used only for the proof of~\cref{lem:rsg-is-fus}. However, one can refer to existing rewriting algorithms (XRewrite~\cite{xrewrite} being a notable example) for additional intuitions. Finally, it is important to note that the proof itself is closely following the ideas provided in \cite{hopefully-pods-paper}.

\subsection{Necessary definitions}
As we are considering a binary signature, we will treat queries as graphs with the company of standard graph theoretic notions. \thomas{Does this suffice or would Reviewer 2 state: ``The term \emph{graph} has not been defined. Suggest strong reject.''?}

A {\em marked query} is a pair $(q, M)$ where $q$ is a BCQ and $M$ is a subset of terms (variables and constants) of $q$. Given an instance $\inst$ we say that $\inst \models (q,M)$ if and only if there exists a homomorphism $h: q \to \inst$ such that for every term $t$ of $q$ we have $t \in M$ if and only if $h(t)$ is a constant in $\inst$.

Consider the following:
\begin{observation}\label{obs:buildup-for-properly-marked-chase}
Let $\db$ be any database. Then:
\begin{itemize}
    \item if $H(t,t')$ or $V(t,t')$ is an atom of $\sg$ and $t'\in \adom{\db}$  then $t\in \adom{\db}$,
    \item if there is a cycle $C$ in $\sg$ then $C$ is a subset of $\db$, 
    \item if $E(t_1,t')$ and $E(t_2,t')$ are two atoms in  $\sg$ (where $E\in\{H, V\}$) and $t_1\in  \adom{\db}$ then  also $t_2\in  \adom{\db}$.
    \item if $E(a,t)$ and $E(b,t)$ are two atoms in $\sg$ (where $E\in\{H, V\}$) and $a\neq b$ are constants then $t$ is a constant as well.
\end{itemize}
\end{observation}

Having this observation in mind we define the notion of a {\em properly marked query}.

\begin{definition}\label{def:properly-marked}
A marked query $(q, M)$ is {\em properly marked} when:
\begin{itemize}
    \item if $a$ is a constant of $q$ then $a \in M$,
    \item if $H(t,t')$ or $V(t,t')$ is an atom of $q$ and $t' \in M$ then $t \in M$,
    \item if there is a cycle $C$ in $q$ then terms of $C$ are contained in $M$,
    \item if $E(t_1,t')$ and $E(t_2,t')$ are two atoms in  $q$ (where $E\in\{H, V\}$) and $t_1 \in M$ then $t_2 \in M$.
    \item if $E(a,t)$ and $E(b,t)$ are two atoms in $q$ (where $E\in\{H, V\}$) and $a\neq b$ are constants then $t \in M$.
\end{itemize}
\end{definition}

From \cref{obs:buildup-for-properly-marked-chase} and \cref{def:properly-marked} we immediately conclude the following:

\begin{corollary}
Let $(q, V)$ be a marked query, and $\db$ be any database. If $\sg \models \mq$ then $\mq$ is properly marked.
\end{corollary}

From now on any properly marked query $(q, V)$ such that $V$ is not containing all terms of $q$ will be called {\em alive}. In the case when every term of a properly marked query is marked we will call such a query {\em totally marked}.

To prove~\cref{lem:rsg-is-fus} it is enough to prove the following:

\begin{lemma}\label{lem:rsg-is-fus-reformulated}
For any properly marked query $(q, V)$ there exists a set of totally marked queries $rew(q,V)$ such that for any database $\db$ the following holds: 
$$\sg \models (q,v) \iff \exists{Q' \in rew(q, V)} \db \models Q'.$$
\end{lemma}

\subsection{Rewriting Alive Queries}

Consider the following:

\begin{lemma}\label{lem:exists-maximal}
For every alive query there exists at least one variable with no out-going edges.
\end{lemma}
\begin{proof}
A query is alive if it is properly marked and there exists at least one unmarked variable. From the first we notice that the sub-query induced on the unmarked variables is a directed and acyclic graph. From the second we know that this graph is non-empty.
\end{proof}

Such unmarked variables with no out-going edges will be called {\em maximal}. Those maximal variables will be used as a starting points for the rewriting process. 

\begin{lemma}\label{lem:maximal-cases}
Let $x$ be a maximal variable of a live query $(q, V)$. Then one of the following conditions holds:
\begin{enumerate}
    \item \label{lem:maximal-cases-one} $x$ occurs in exactly one atom  $E(t,x)$, with $E\in \{H,V\}$ for some term $t$ of $q$,
    \item \label{lem:maximal-cases-two} $x$ occurs in exactly two atoms $H(t_H,x)$ and $V(t_V,x)$ for some terms $t_H,t_V$ of $q$,
    \item \label{lem:maximal-cases-three} there exist at least two distinct terms $t\neq t'$ and $E \in \{H,V\}$ such that $E(t,x)$ and $E(t',x)$ are atoms of $q$.
\end{enumerate}
\end{lemma}

Now, in the light~\cref{lem:maximal-cases} we will present four operations that when combined will compute rewritings required by \cref{lem:rsg-is-fus-reformulated}.

\medskip
\noindent
{\bf Five operations}
Given an alive query $(q, V)$ we define:

\begin{definition}[$\cutop$]\label{def:cut}
Let $x$ be a maximal variable of $(q, V)$ such as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-one} then $\cutop((q,V), x) = (q', V)$ where $q'$ is a sub-query of $q$ with the atom containing $x$ removed.
\end{definition}

\begin{definition}[$\reduceop$]\label{def:reduce}
Let $x, t_H, t_V$ be as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-two} then let $q'$ be obtained from $q$ by replacing $H(t_H, x),V(t_V, x)$ with $H(x', t_V), V(x', t_H)$ 
where $x'$ is a fresh variable. Then let $\cutop((q,V), x) = \set{ (q', V), (q', V \cup {x'})}$. \thomas{Shouldn't that be $\reduceop((q,V), x) = \set{ (q', V), (q', V \cup {x'})}$?}
\end{definition}

\begin{definition}[$\mergeop$]\label{def:merge}
Let $x, t, t'$ be as in \cref{lem:maximal-cases} case \ref{lem:maximal-cases-three} then let $q'$ be obtained from $q$ by replacing all occurrences of $t$ in $q$ with $t'$. Then let $\mergeop((q, V), x, t, t') = (q', V)$.
\end{definition}

\begin{observation}[Completeness]\label{obs:high-completeness}
If a query is alive then at least one of above operations can be applied to it.
\end{observation}
\begin{proof}
Follows from~\cref{def:cut,def:reduce,def:merge}, and~\cref{lem:maximal-cases}.
\end{proof}

Now we will prove the soundness for those operations:

\begin{lemma}[Soundness --- $\cutop$]\label{lem:high-soundness-cut}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models \cutop(Q, x)$$
if $x$ is as in \cref{def:cut}.
\end{lemma}
\begin{proof}
TODO
\end{proof}

\begin{lemma}[Soundness --- $\reduceop$]\label{lem:high-soundness-reduce}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models Q' \vee Q''$$
if $x$ is as in \cref{def:reduce} and $\reduceop(Q, x) = \set{Q', Q''}$.

\end{lemma}
\begin{proof}
TODO
\end{proof}

\begin{lemma}[Soundness --- $\mergeop$]\label{lem:high-soundness-merge}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\sg \models Q \iff \sg \models \mergeop(Q, x, t, t')$$
if $x, t, t'$ are as in \cref{def:merge}.
\end{lemma}
\begin{proof}
TODO
\end{proof}

\medskip
\noindent
{\bf Rank of an alive query}

Given a BCQ $Q$ a {\em path} is a finite sequence $P$ such that:

\piotr{cleanup variables $x,y,z,t,u,\ldots$ for consistency with the rest of the paper.} 
 \begin{itemize}
    \item Each of the elements of $P$ is either $E(t,z)$ or $\Em(z,t)$ for some $E(t,z)$ from $q(Q)$, where $E\in\{H,V\}$ 
    \item if $E(s,t)$ and $E'(u,z)$ are two consecutive elements of $P$ then $t=u$ (where $E,E'\in\{H,V,\Hm, \Vm \}$);
    \item No term of $Q$ can be visited in $P$ twice.
 \end{itemize}
 
 We will write $P = P' \cdot E(x,y)$ to denote a path $P$ extends $P'$ with $E(x,y)$. In some cases we write $P = P' \cdot E$ to avoid clutter. Also, by writing $P(x,y)$ we state that $P$ starts in $x$ and ends in $y$.

Given a marked query $Q$ and any path $P$ in $Q$ we define its {\em cost} in the following way:
\begin{itemize}
    \item $\cost{\varepsilon} = |\adom{Q}|$
    \item $\cost{P \cdot E} = \cost{P}$, \hfill for $E \in \set{H, \Hm}$
    \item $\cost{P \cdot V} = \cost{P} + 1$
    \item $\cost{P \cdot \Vm} = \cost{P} - 1$
\end{itemize}

and its {\em rank} as:

\begin{itemize}
    \item $\rank{\varepsilon} = 0$
    \item $\rank{P \cdot E} = \rank{P} + \cost{P \cdot E}$ for $E \in \set{H, \Hm, V, \Vm}$
\end{itemize}

Given a properly marked query\footnote{Recall, that we consider BCQs that contain at least one constant, thus the set of marked variables of any properly marked query cannot be empty.} $\mq$ and any of its unmarked variables $x \in M$ we define the \emph{rank of $x$ in $\mq$}, $\rank{x, \mq}$, as:
$$\rank{x, \mq} = \min(\set{\rank{P(t,x)} | t \in M})$$

And finally, given a properly marked query $\mq$ we define its rank $\rank{\mq}$ as:
$$(|\adom{q}|, \multiset{ \rank{t, \mq} | t \in terms(q) \wedge t \not\in M})$$
with $\multiset{}$ simply denoting a multi-set. For two properly marked queries $Q$ and $Q'$ such that $\rank{Q} = (n, \mathcal{P})$ and $\rank{Q'} = (n', \mathcal{P}')$ we write $\rank{Q} < \rank{Q'}$ if: $n < n'$ or $\mathcal{P}$ is lexicographically smaller than $\mathcal{P}'$ when $\mathcal{P}$ and $\mathcal{P}'$ are treated as ordered lists. It should be clear that the order $<$ on ranks of properly marked queries is well ordered.

\medskip
\noindent
{\bf Termination}
Now we will show that our rewriting process terminates. 

\begin{lemma}[Termination --- $\cutop$]\label{lem:high-termination-cut}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\rank{\cutop(Q, x)} < \rank{Q}$$
if $x$ is as in \cref{def:cut}.
\end{lemma}
\begin{proof}
Note that operation $\cutop$ removes one unmarked variable from $Q$. Thus the active domain of $Q$ is strictly greater than that of $\cutop(Q, x)$.
\end{proof}

\piotr{Be extremely cautious when proofreading this proof}
\begin{lemma}[Termination --- $\reduceop$]\label{lem:high-termination-reduce}
Let $\db$ be any database and let $Q$ be an alive query then:
$$ \rank{Q'} < \rank{Q} \wedge \rank{Q''} < \rank{Q}$$
if $x$ is as in \cref{def:reduce} and $\reduceop(Q, x) = \set{Q_1, Q_2}$.
\end{lemma}
\thomas{The $Q'$ and $Q''$ put me a bit off here. Are those actually $Q_1$ and $Q_2$ respectively, or ..?}
\begin{proof}
Let $Q = \mq$ and let $Q' = (q', M')$ be any of the queries in $\set{Q_1, Q_2}$. Also, let $x$ be the removed variable and let $x'$ be the newly introduced variable.
First we will show the following:
\begin{claim}
Let $y$ be any unmarked variable of $Q$ other than $x$. Then $\rank{x, Q} \geq \rank{x, Q'}$.
\end{claim}
\thomas{Why do you need to introduce the $y$ if you only compare the ranks with respect to $x$ and different queries?}
\begin{subproof}[Proof]
Let $P(t,y)$ be a path of minimal rank from some marked term $t$ of $Q$ to $y$. If $P$ does not visit $x$ then $P$ is a path in $Q'$ as well and so $\rank{y, Q} \geq \rank{y, Q'}$. If $P$ visits $x$ then it is of one of the two following forms: $$P = P_1 \cdot H(t_H, x)\cdot\Vm(x, t_V)\cdot P_2$$ or $$P = P_1' \cdot V(t_V, x)\cdot\Hm(x, t_H) \cdot P_2'.$$ Assume the first case, then $P'(t,y) = P_1 \cdot \Vm(t_H, x)\cdot H(x, t_V) P_2$ is a path from $t$ to $y$ in $Q'$. \thomas{$P'$ does utilize $x$ though. So it is probably not $x$ here?} Observe that the rank of $P'$ is strictly smaller than the rank of $P$. The second case is analogous.
\end{subproof}

Consider:
\begin{observation}
$\rank{x, Q} > \rank{x', Q'}$.
\end{observation}
\thomas{What is $x'$? It's probably the $x'$ from the definition of the $\reduceop$ operation, but I think that should be clarified here. Is it also the same term that will appear in relation to my last comment?}
\begin{subproof}[Proof]
Note that if If $x' \in M'$ then $\rank{x', Q'} = 0$ and thus $\rank{x, Q} > \rank{x', Q'}$ as $x \not\in M$.

Let $P(t,x)$ be a path of minimal rank from some marked term $t$ of $Q$ to $x$. Notice that $P$ is of one of the two following forms: $P = P_1 \cdot H(t_H, x)$ or $P = P_1' \cdot V(t_V, x)$.
Assume that $P = P_1 \cdot H(t_H, x)$. Notice that $P_V = P_1 \cdot \Vm(t_H, x)$ \thomas{Again, is that $x$ or shouldn't it be $x'$ as we now go ``the different'' $V$, though counter the direction of that edge, down.} is a path in $Q'$ and that $\rank{P_V} = \rank{P} - 1$. The second case is analogous.
\end{subproof}

Finally, note that $|\adom{q}| = |\adom{q'}|$. 
\end{proof}

\begin{lemma}[Termination --- $\mergeop$]\label{lem:high-termination-merge}
Let $\db$ be any database and let $Q$ be an alive query then:
$$\rank{\mergeop(Q, x)} < \rank{Q}$$
if $x, t, t'$ are as in \cref{def:merge}.
\end{lemma}
\begin{proof}
Note that operation $\mergeop$ removes one variable from $Q$. Thus the active domain of $Q$ is strictly greater than that of $\mergeop(Q, x)$.
\end{proof}

Finally, from completeness (\cref{obs:high-completeness}), soundness (\cref{lem:high-soundness-cut,lem:high-soundness-reduce,lem:high-soundness-merge}), and termination (\cref{lem:high-termination-cut,lem:high-termination-reduce,lem:high-termination-merge}) we conclude~\cref{lem:rsg-is-fus-reformulated} thus finishing the proof of \cref{lem:rsg-is-fus}.

==> other/old-partition-width.tex <==
\section{Clique-width and Partition-width}

\subsection{New Definition}

\begin{comment}
Let $\cols$ be an infinite set of \emph{colors}. For $C\subseteq \cols$ we define a set $F_{C}$ consisting of the following operation symbols:
\begin{itemize}
	\item For every $n\in C$ let $\unitn$ be a (fresh) constant symbol (i.e. a symbol of rank $0$).
	\item For every predicate $\mathtt{R}\in\sigma$ and tuple $\vc\subseteq C$ of length $\arity{\mathtt{R}}$ let $\add{\mathtt{R}, \vc}{}$ be a unary symbol (rank $1$).
	\item For every two colors $l_1, l_2\in C$ let $\recol{l_1\to l_2}{}$ be a unary symbol (rank $1$).
	\item Let $\oplus$ be a binary symbol (rank $2$).
\end{itemize}
Lastly, we introduce an extended signature $F_{C}^{\mathbf{0}}$, in which we add
\begin{itemize}
	\item a fresh constant-symbol $\mathbf{0}$.
\end{itemize}
\end{comment}
Let $\cols$ be an infinite set of \emph{colors} and $\Sigma = \Sigma_1 \oplus \Sigma_2$ a finite relational signature with unary ($\Sigma_1$) and binary ($\Sigma_2$) relational symbols. As a small technicality, we introduce a fresh unary predicate $\top$ that holds on all terms from $\adom{\inst}$ for a given instance $\inst$.
\begin{definition}
	Let $\Sigma$ be a finite binary relational signature, $\inst$ be an instance. For $C\subseteq\cols$ and $\lambda\colon\adom{\inst} \to C$ we call the tuple $(\inst, \lambda)$ a \emph{$C$-colored instance}, or \emph{colored instance} for short.\\
	Two $C$-colored instances $(\inst_1, \lambda_1)$ and $(\inst_2, \lambda_2)$ are called \emph{isomorphic}, $(\inst_1, \lambda_1) \cong_{\Sigma, C} (\inst_2, \lambda_2)$ iff $\inst_1 \cong_{\Sigma} \inst_2$ with an isomorphism $h\colon \inst_1\to\inst_2$ and there exists a bijection $\kappa\colon \cols \to \cols$ such that $\kappa \circ \lambda_1 = \lambda_2 \circ h$. \\
	For fixed $\Sigma$ and $C$ we call the isomorphy-class of a colored instance $(\inst, \lambda)$ under $\cong_{\Sigma, C}$ an \emph{abstract $C$-colored instance}.
\end{definition}
\begin{definition}
	For $C\subseteq \cols$ we define a set $F_{C}$ consisting of the following operation symbols:
	\begin{itemize}
		\item Let $\bold{0}$ be a instance-construction-constant (\emph{ic-constant} for short) symbol.
		\item For every $n\in C$ and $\mathcal{P}\subseteq \Sigma_{1}$ let $\unit_{n, \mathcal{P}}$ be a ic-constant symbol .
		\item For every $n\in C$, $\mathcal{P}\subseteq \Sigma_{1}$, and $c \in K$ let $c_{n, \mathcal{P}}$ be a ic-constant symbol.
		\item For every binary predicate $\mathtt{R}\in\Sigma$ and pair $(l_1, l_2)\in C^2$ of length $\arity{\mathtt{R}}$ let $\add{\mathtt{R}, (l_1,l_2)}{}$ be a unary ic-symbol.
		\item For every two colors $l_1, l_2\in C$ let $\recol{l_1\to l_2}{}$ be a unary ic-symbol.
		\item Let $\oplus$ be a binary ic-symbol.
	\end{itemize}
	For a given $C\subseteq \cols$ let $T(F_{C})$ denote the set of all terms over $F_{C}$.
\end{definition}
Let $\Sigma$ be some relational signature. To each $t\in F_{C}$ we associate a finite abstract $C$-colored instance\footnote{For simplicity we drop the isomorphism class in the exposition and work with a representant.} $(\inst, \lambda)$ with $\lambda\colon \adom{\inst} \to C$ by defining a \emph{valuation map} $\val{t}$ inductively. First we introduce the interpretations of the ic-symbols on the class of abstract $C$-colored instances over $\Sigma$
\begin{itemize}
	\item $\val{\mathbf{0}}$ is the empty instance colored by $\lambda\colon \emptyset \to C$.
	\item For every $n\in C$ and $\mathcal{P}\subseteq \Sigma_{1}$ let $\val{\unit_{n, \mathcal{P}}}$ be the instance $\{ \top(t) \}\cup \{ R(t) \, | \, R\in \mathcal{P} \}$ colored by $\lambda\colon t \mapsto n$.
	\item For every $n\in C$, $\mathcal{P}\subseteq \Sigma_{1}$, and constant $c\in \mathfrak{C}$ let $\val{c_{n, \mathcal{P}}}$ be the instance $\{ \top(c) \}\cup \{ R(c) \, | \, R\in \mathcal{P} \}$ colored with $\lambda\colon c \mapsto n$.
	\item For every binary predicate $\mathtt{R}\in\sigma$, pair $(l_1,l_2)\in C^2$, and abstract colored instance $(\inst, \lambda)$ let $\add{\mathtt{R}, (l_1,l_2)}{(\inst, \lambda)}$ be the instance $(\inst', \lambda)$, where $\adom{\inst'} = \adom{\inst}$, and \[ \inst' = \inst \cup \{ R(t_1, t_2) \, | \, \lambda((t_1, t_2)) = (l_1,l_2) \} \, .\]
	\item For every two colors $l_1, l_2\in C$ and colored instance $(\inst, \lambda)$ let $\recol{l_1\to l_2}{(\inst, \lambda)} = (\inst, \lambda')$ where $\lambda' = h\circ \lambda$ with $h_{l_1\to l_2} \colon C \to C$ with \[ h(x) := \begin{cases} l_2, \quad \text{if } x = l_1 \\ x, \quad \text{else} \end{cases} \, . \]
	\item For two $C$-colored instances $(\inst_1, \lambda_1), (\inst_2, \lambda_2)$ we let $(\inst_1, \lambda_1) \oplus (\inst_2, \lambda_2) = (\inst', \lambda')$ where with $\adom{\inst_2'}\cap\adom{\inst_1} \subset \mathfrak{C}$, $(\inst_2', \lambda_2') \cong_{\Sigma, C} (\inst_2, \lambda_2)$, $\inst = \inst_1 \cup \inst_2'$, and $\lambda = \lambda_1 \cup\lambda_2'$ the abstract $C$-colored instance $(\inst, \lambda)$ is the disjoint union of both instances.
\end{itemize}
Hence, for every finite \emph{instance-construction-term} (or \emph{ic-term}) $T$ over $F_{C}$, $\val{T}$ is defined inductively as follows:
\begin{itemize}
	\item For every ic-symbol $\mathtt{k}\in F_{C}$ let $\val{\mathtt{k}}$ be as defined above.
	\item For every unary ic-symbol $f\in F_{C}$ and finite ic-term $t\in F_{C}$ let \[ \val{f(t)} = f(\val{t}) \, . \]
	\item For every binary ic-symbol $f\in F_{C}$ and finite ic-terms $t_1, t_2\in F_{C}$ let \[ \val{f(t_1, t_2)} = f(\val{t_{1}}, \val{t_{2}}) \, . \]
\end{itemize}
To describe also countably infinite instances via ic-terms, we need to lift both the ic-terms and there valuation to the infinite case.

%Our first step will be to identify each term with there \emph{syntax-tree}. As our operations are at most of arity $2$, we utilize subtrees of the complete binary tree $2^{< \omega}$ (consisting of all finite sequences over $\{ 0, 1 \}$ with the usual prefix ordering). 
\begin{definition}
	A \emph{syntax-tree over $F_{C}$} of an ic-term is a partial map \[ T \colon 2^{<\omega} \to F_{C} \] with domain $\dom(T)\subseteq 2^{<\omega}$ satisfying the following properties:
	\begin{itemize}
		\item $\dom(T)$ non-empty,
		\item $\dom(T)$ is prefix-closed (i.e. if $\alpha\beta \in 2^{<\omega}$ with $\alpha\beta\in \dom(T)$ then $\alpha\in\dom(t)$)
		\item if $\alpha 1\in\dom(T)$ then $\alpha 0\in\dom(t)$.
		\item Furthermore, for $\alpha\in\dom(T)$ if $t(\alpha) = f$ then for all $i \in\{ 0, 1 \}$ we have $\alpha i\in\dom(T)$ iff $i< \arity{f}$.
	\end{itemize}
	For $T$ a syntax-tree we define as $L_{T}$ the set of all leafs of $T$ (i.e. the set of all $\alpha \in L_{T}$ such that $\alpha 0 \not\in L_{T}$ and $\alpha 1 \not\in L_{T}$) \\
	$T$ is called \emph{well-formed} if there are only finitely many $a\in \mathfrak{C}$ such that there exists exactly one $n\in C$ and exactly one $\alpha\in L_{T}$ such that  $f(\alpha) = a_{n}$. \\
	We define $T^{\infty}(F_{C})$ to consist of all syntax-trees over $F_{C}$.
\end{definition}
We will use ``ic-term'' and ``syntax-tree over $F_{C}$'' interchangably.
\begin{observation}
	Finite syntax-trees over $F_{C}$ correspond one-to-one to terms $t\in F_{C}$.
\end{observation}
In order to lift the valuation-map to infinite ic-terms we will utilize the notion of the \emph{$n$-depth truncation} of a tree.
\begin{definition}
	Let $T\in T^{\infty}(F_{C})$ and $k\in \mathbb{N}$, the \emph{$k$-depth truncation of $T$}, $T^{(k)}$ is defined inductively as follows:
	\begin{itemize}
		\item $T^{(0)} = \mathbf{0}$
	\end{itemize}
	and for $k> 0$
	\begin{itemize}
		\item if $T = T_{1}\oplus T_{2}$ then $T^{(k)} = (T_{1}\oplus T_{2})^{(k)} = T_{1}^{(k-1)}\oplus T_{2}^{(k-1)}$,
		\item for $f\in F_{C}$ unary, $f(T)^{(k)} = f(T^{(k-1)})$,
		\item for $n\in C$, $\unitn^{(k)} = \unitn$,
		\item for $n\in C$ and $a\in\mathfrak{C}$, $a_{n}^{(k)} = a_{n}$,
		\item $\mathbf{0}^{(k)} = \mathbf{0}$.
	\end{itemize}
\end{definition}
Furthermore we define a partial order on the set of syntax-trees):
\begin{definition}
	\begin{itemize}
		\item Let $T, T' \in T(F_{C})$ for some $C\subseteq \cols$. Then $T \prec T'$ iff we have $c\in T(F_{C} \cup \{ u_1, \ldots, u_k \})$ and $T'_{1}, \ldots, T'_{k}\in T(F_{C})$ such that $T = c[\bold{0}, \ldots, \bold{0}]$ and $T' = c[T'_{1}, \ldots, T'_{k}]$.
		\item For $T'\in T^{\infty}(F_{C})$ and $T \in T(F_{C})$, we define $T\prec T'$ to hold iff in the previous setup we have $T', T'_{1}, \ldots, T'_{k}\in T^{\infty}(F_{C})$.
	\end{itemize}
\end{definition}
\begin{observation}
	Note that every ascending chain of finite trees, i.e. $(T_{i})_{i < \omega} \subseteq T(F_{C})$ such that \[ T_{0} \prec T_{1} \prec T_{2} \prec \cdots \] has a least upper bound in $T^{\infty}(F_{C})$. See \cite[Section 2]{Cou78} for approximation of infinite terms by finite ones.
\end{observation}
\begin{comment}
With this partial order defined, we need to introduce one more tool: The \emph{$n$-depth truncation} of a term $t\in T^{\infty}(F_{C})$ which we define inductively:
\begin{itemize}
	\item $t^{(0)} = \bold{0}$
	\item For $n>0$ we set
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(n)} = t_{1}^{(n-1)} \oplus t_{2}^{(n-1)}$
		\item $f(t_{1})^{(n)} = f(t_{1}^{(n)})$ for every unary $f$
		\item $\unit_{1}^{(n)} = \unit_{1}$ and $\bold{0}^{(n)} = \bold{0}$.
	\end{itemize}
\end{itemize}
Note that $t^{(n)}$ for every term $t\in T^{\infty}(F_{C})$ is in fact a finite term over $F_{C}$, i.e. $t^{(n)}\in T(F_{C})$.
\end{comment}

\begin{observation}
	If $T,T'\in T(F_{C})$ with $T\prec T'$ then $\val{T}$ is an induced sub-instances of $\val{T'}$.
\end{observation}
\begin{observation}
	If $T\in T^{\infty}(F_{C})$ then
	\begin{equation*}
		T^{(0)} \prec T^{(1)} \prec \cdots
	\end{equation*}
	which induces an ascending chain of induced sub-instances
	\begin{equation*}
		\val{T^{(0)}} \le \val{T^{(1)}} \le \cdots
	\end{equation*}
\end{observation}
\begin{definition}
	If $T\in T^{\infty}(F_{C})$ is an infinite syntax-tree, then $\val{T} = \bigcup_{i < \omega} \val{T^{(i)}}$.
\end{definition}

\begin{comment}
We extend this idea to all functional signatures $F$ with at most binary function symbols, i.e. $F^{\mathbf{0}}$ will always contain the additional fresh constant-symbol $\mathbf{0}$ if we want to make it obvious that we are now using $\mathbf{0}$.
For a given $C\subseteq \cols$ let $T(F_{C}^{\mathbf{0}})$ denote the set of all terms over $F_{C}^{\mathbf{0}}$.
Let $\Sigma$ be some relational signature. To each $t\in F_{C}^{\mathbf{0}}$ we can associate a(n ismorphism class of a) finite (possibly empty) colored structure\footnote{For simplicity we drop the isomorphism class in the exposition.} $(\mathfrak{A}, \lambda)$ with $\lambda\colon A \to C$ by defining a \emph{valuation map} $\val{t}$ inductively. First we introduce the interpretations of the operation symbols on the class of $C$-colored relational structures over $\Sigma$ and also give already the valuation of the constant symbols
\begin{itemize}
	\item $\val{\mathbf{0}}$ is the empty structure (hence the coloring $\lambda\colon \emptyset \to C$ is the unique map $\emptyset$).
	\item For every $n\in C$ let $\val{\unitn}$ be the structure with one element, no relations holding and the coloring $\lambda$ mapping the unique domain element to $n$.
	\item For every predicate $\mathtt{R}\in\sigma$, tuple $\vc\subseteq C$ of length $\arity{\mathtt{R}}$, and colored relational structure $(\mathfrak{A}, \lambda)$ let $\add{\mathtt{R}, \vc}{(\mathfrak{A}, \lambda)}$ be the structure $(\mathfrak{B}, \lambda)$, where $B = A$, for all constant symbols $\mathtt{c} \in \Sigma$ we have $c^{\mathfrak{B}}= c^{\mathfrak{A}}$, for all $\mathtt{P}\in \Sigma\setminus \{ \mathtt{R} \}$ we have $\mathtt{P}^{\mathfrak{B}} = \mathtt{P}^\mathfrak{A}$ and \[ \mathtt{R}^{\mathfrak{B}} = \mathtt{R}^{\mathfrak{A}} \cup \{ \overline{b} \in B^{\arity{\mathtt{R}}} \, | \, \lambda(\overline{b}) = \vl \} \, .\].
	\item For every two colors $a, b\in C$ and colored relational structure $(\mathfrak{A}, \lambda)$ let \[ \recol{a\to b}{(\mathfrak{A}, \lambda)} = (\mathfrak{A}, \lambda')\] where for $h_{a\to b} \colon C \to C$ with \[ h_{a\to b}(x) := \begin{cases} b, \quad \text{if } x = a \\ x, \quad \text{else} \end{cases} \] we have $\lambda' = h_{a\to b}\circ \lambda$.
	\item For two $C$-colored structures $(\mathfrak{A}, \lambda_1), (\mathfrak{B}, \lambda_2)$ we let $(\mathfrak{A}, \lambda_1) \oplus (\mathfrak{B}, \lambda_2)$ be the disjoint union of both structures.
\end{itemize}
We now lift the valuation map from the constant symbols to finite terms in the natural way:
\begin{itemize}
	\item For every constant-symbol $\mathtt{k}\in F_{C}^{\mathbf{0}}$ let $\val{\mathtt{k}}$ be as defined above.
	\item For every unary operation-symbol $f\in F_{C}$ and finite term $t\in F_{C}$ let \[ \val{f(t)} = f(\val{t}) \, . \]
	\item For every binary operation-symbol $f\in F_{C}$ and finite terms $t_1, t_2\in F_{C}$ let \[ \val{f(t_1, t_2)} = f(\val{t_{1}}, \val{t_{2}}) \, . \]
\end{itemize}
\begin{observation}
    Obviously, restricting $F_{C}^{\mathbf{0}}$ to $F_{C}$ yields a valid valuation map, too.
\end{observation}
Until now we only deal with finite terms and hence can describe only finite colored structures with those. As we are interested to also describe countably infinite colored structures, our next goal will be to introduce infinite terms and then extend the valuation map to those.

Our first step will be to identify each term with its \emph{syntax-tree}. We define this in the general setting with $F$ being an algebraic signature containing function symbols up to arity $2$. As our operations are at most of arity $2$, we utilize subtrees of the complete binary tree $2^{< \omega}$ (consisting of all finite sequences over $\{ 0, 1 \}$ with the usual prefix ordering). 
\begin{definition}
	A \emph{syntax-tree over $F$} is a partial map \[ t \colon 2^{<\omega} \to F \] with domain $\dom(t)\subseteq 2^{<\omega}$ satisfying the following properties:
	\begin{itemize}
		\item $\dom(t)$ non-empty,
		\item $\dom(t)$ is prefix-closed (i.e. if $\alpha\beta \in 2^{<\omega}$ with $\alpha\beta\in \dom(t)$ then $\alpha\in\dom(t)$)
		\item if $\alpha 1\in\dom(t)$ then $\alpha 0\in\dom(t)$.
		\item Furthermore, for $\alpha\in\dom(t)$ if $t(\alpha) = f$ then for all $i \in\{ 0, 1 \}$ we have $\alpha i\in\dom(t)$ iff $i< \arity{f}$.
	\end{itemize}
	For $t$ a syntax-tree we define as $L_{t}$ the set of all leafs of $t$ (i.e. the set of all $\alpha \in \dom(t)$ such that $\alpha 0 \not\in \dom(t)$ and $\alpha 1 \not\in \dom(t)$)
\end{definition}
\begin{observation}
	Finite syntax-trees over $F_{C}$ correspond one-to-one to terms $t\in F_{C}$.
\end{observation}
We define $T^{\infty}(F)$ to consist of all syntax-trees over $F$.

We will now lift the valuation-map to infinite terms (which are infinite syntax-trees). For this we will utilize the notion of the \emph{$n$-depth truncation} of a tree.
\begin{definition}
	 For an arbitrary algebraic signature $F$ with arity at most $2$, let $t\in T^{\infty}(F)$ and $k\in \mathbb{N}$. The \emph{$k$-depth truncation of $t$} is the finite term $t^{(k)}\in T(F^{\bold{0}})$ defined inductively as follows:
	\begin{itemize}
		\item $t^{(0)} = \bold{0}$
	\end{itemize}
	and for $k> 0$
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(k)} = t_{1}^{(k-1)}\oplus t_{2}^{(k-1)}$,
		\item for $f\in F$ unary, $f(t)^{(k)} = f(t^{(k-1)})$,
		\item for $n\in C$, $\unitn^{(k)} = \unitn$,
%		\item $\bold{0}^{(k)} = \bold{0}$.
	\end{itemize}
\end{definition}
We can define a partial order on the set of syntax-trees in the following way (note that adding variable symbols to the signature corresponds to having the ability to substitute terms for those variable symbols):
\begin{itemize}
	\item Let $t, t' \in T(F_{C})$ for some $C\subseteq \cols$. Then $t \prec t'$ iff we have $c\in T(F_{C} \cup \{ u_1, \ldots, u_k \})$ and $t'_{1}, \ldots, t'_{k}\in T(F_{C})$ such that $t = c[\bold{0}, \ldots, \bold{0}]$ and $t' = c[t'_{1}, \ldots, t'_{k}]$.
	\item Furthermore, for $t'\in T^{\infty}(F_{C})$ and $t \in T(F_{C})$, we define $t \prec t'$ to hold iff in the previous setup we have $t', t'_{1}, \ldots, t'_{k}\in T^{\infty}(F_{C})$.
\end{itemize}
\begin{observation}
	Note that every ascending chain of finite trees, i.e. $(t_{i})_{i < \omega} \subseteq T(F_{C})$ such that \[ t_{0} \prec t_{1} \prec t_{2} \prec \cdots \] has a least upper bound in $T^{\infty}(F_{C})$. (Quote 3, Section 2 of Courcelle Paper).
\end{observation}
With this partial order defined, we need to introduce one last tool: The \emph{$n$-depth truncation} of a term $t\in T^{\infty}(F_{C})$ which we define inductively:
\begin{itemize}
	\item $t^{(0)} = \bold{0}$
	\item For $n>0$ we set
	\begin{itemize}
		\item $(t_{1}\oplus t_{2})^{(n)} = t_{1}^{(n-1)} \oplus t_{2}^{(n-1)}$
		\item $f(t_{1})^{(n)} = f(t_{1}^{(n)})$ for every unary $f$
		\item $\unit_{1}^{(n)} = \unit_{1}$ and $\bold{0}^{(n)} = \bold{0}$.
	\end{itemize}
\end{itemize}
Note that $t^{(n)}$ for every term $t\in T^{\infty}(F_{C})$ is in fact a finite term over $F_{C}$, i.e. $t^{(n)}\in T(F_{C})$.
\begin{observation}
	If $t,t'\in T(F_{C})$ then $\val{t}$ is an induced substructure of $\val{t'}$.
\end{observation}
\begin{observation}
	If $t\in T^{\infty}(F_{C})$ then
	\begin{equation*}
		t^{(0)} \prec t^{(1)} \prec \cdots
	\end{equation*}
	which induces an ascending chain of induced substructures
	\begin{equation*}
		\val{t^{(0)}} \le \val{t^{(1)}} \le \cdots
	\end{equation*}
\end{observation}
With this we can finally define a valuation-function that maps each syntax-tree $t\in T^{\infty}(F_{C})$ to a colored structure in the following way:
\begin{itemize}
	\item If $t\in T(F_{C})$, then $\val{t}$ is as previously defined.
	\item If $t\in T^{\infty}(F_{C})$ is an infinite syntax-tree, then $\val{t} = \bigcup_{i < \omega} \val{t^{(i)}}$.
\end{itemize}
With this we can finally define cliquewidth.
\end{comment}
\begin{definition}
	Let $\inst$ be a countable instance over $\Sigma$. We define its \emph{cliquewidth} as the minimal $k\in \mathbb{N}$ ($\cw{\inst}=k$ for short) such that there exist a $C\subseteq \cols$ with $|C|=k$, a map $\lambda \colon A \to C$ and a term $t\in T^{\infty}(F_{C})$ such that $\val{t} = (\inst, \lambda)$. If there is no such $n\in \mathbb{N}$, we set $\cw{\inst}= \infty$. \piotr{Moreover, for a map $\coloring$ we will write $\cw{\inst, \coloring}$ = k if the co-domain of $\coloring$ is of size $k$ and there exists a term $t$ such that $\val{t} = (\inst, \coloring)$.}
\end{definition}
\piotr{We will use $\mathrm{add}_{R,(l,l')}(\instance, \coloring)$ as a shorthand for\\ $\val{\mathrm{add}_{R,(l,l')}(t)}$ where $t$ is such that $\val{t} = (\instance, \coloring)$.}

\begin{comment}
As another tool we introduce several formula talking about finite syntax-trees over $F_{C}$. The main idea behind those is that they track first, whether a tuple of elements will be put into a relation while evaluating the term and second, which color individual elements will have. Let $t\in T(F_{C})$ (note: a finite term!) and $\mathtt{R}\in\Sigma$ a relational symbol.
\begin{itemize}
	\item Let $\psi_{C}(t, x, i)$ with $x\in L_{t}$ and $i\in C$ denote the sentence saying that $x$ will have the color $i$ at the root of $t$.
	\item We denote by $\phi_{\mathtt{R}}(t, \overline{x})$ the sentence saying the following: For a tuple $\overline{x}\in L_{t}^{\arity{\mathtt{R}}}$ if there is a node $u$ in $t$ such that all $\overline{x}_{i}$ have $u$ as an ancestor, $t(u) = \add{R, \vl}{}$ and for all $0\le i\le \arity{\mathtt{R}}$ it holds that $\psi_{C}(t/u, \overline{x}_i, \vl_{i})$.
\end{itemize}
\begin{observation}
	As long as $x, y$ are both of depth $\le n-1$ we have $\psi_{C}(t, x, i)$ iff $\psi_{C}(t^{(n)}, x, i)$ and $\phi_{\mathtt{R}}(t, \overline{x})$ iff $\phi_{\mathtt{R}}(t^{(n)}, \overline{x})$.
\end{observation}
We use this observation in order to extend the valuation map in the following way:
\begin{definition}
	Let $t\in T^{\infty}(F_{C})$ be a term over $F_{C}$. Then $\val{t} = (\mathfrak{A}, \lambda)$ with
	\begin{itemize}
		\item $A = L_{t}$,
		\item \thomas{\textbf{TODO: Constants!}}
		\item for every $\mathtt{R}\in\Sigma$ and $\overline{a}\in A^{\arity{\mathtt{R}}}$ it holds that $\overline{a}\in \mathtt{R}^{\mathfrak{A}}$ iff there exists a $k\in\mathbb{N}$ such that $\phi_{\mathtt{R}}(t^{(n)}, \overline{a})$ holds.
		\item for all $a\in A$ we define $\lambda(a) = i$ iff there exists $n\in \mathbb{N}$ such that $\psi_{C}(t^{(n)}, a, i)$.
	\end{itemize}
\end{definition}
\begin{lemma}
	On finite terms, this valuation is equivalent to our former definition.
\end{lemma}
\end{comment}

\subsection{Clique-width terms are partition-width terms}

Hence, given the MSO-decidability, we only have to discuss the translation of a term for clique-width to a corresponding/equivalent ``partition-width'' term. For this, let us introduce those terms:

Firstly, a \emph{graded set of colors} is a set $C$ that is partitioned into finite and nonempty sets $C_{n}$ for $n<\omega$. We call colors $c\in C_{n}$ \emph{colors of arity $n$}. Naturally we define a \emph{$C$-coloring} $\chi$ on a structure $\mathfrak{M}$ as a map associating to each tuple $\bold{a}\in M^{n}$ a $n$-ary color, i.e. $\chi(\bold{a})\in C_{n}$.

We will now define update-instructions and associated operations in a signature $\mathcal{Y}_{C, \Sigma}$ where $\Sigma$ is our signature. Note that we will only define a reduced form to make it fit nice and snuggly.

An \emph{update instruction} is a tuple $(n, 2, \overline{I}, \overline{c}, d, S)$ where:
\begin{itemize}
	\item $n < \omega$,
	\item $\overline{I}$ is a partition $\oplus_{i<2}I_{i} = [n]$ of $[n]$ into $2$ classes,
	\item $\overline{c}\in C^{2}$ is a sequence of $2$ colors such that the arity of $c_i$ is $|I_{i}|$,
	\item $d\in C_{n}$ is a color of arity $n$; and
	\item $S\subseteq \Sigma$ is a set of $n$-ary relational symbols.
\end{itemize}
The number $n$ is the arity of the instruction.

Which leads us the definition of an \emph{ordered $2$-update}, which is a set $\Theta$ of update instructions such that it contains for every $n, \overline{I}, \overline{c}$ exactly one update instruction $(n, 2, \overline{I}, \overline{c}, d, S)$. Because of demanding the uniqueness of the update instructions for every $n, \overline{I}, \overline{c}$ we can introduce the notation for the ordered $2$-update as a familiy of functions \[ \Theta_{n}(\overline{I}; \overline{c}) = (d, S)  \text{ iff } (n, 2, \overline{I}, \overline{c}, d, S) \in \Theta \, . \]

With all that said, we will now define the \emph{ordered sum} associated with an ordered $2$-update as follows: For two $C$-colored structures $(\mathfrak{M}_{0}, \chi_{0})$ and $(\mathfrak{M}_{1}, \chi_{1})$ and an ordered $2$-update $\theta$ the ordered sum $(\mathfrak{M}_{0}, \chi_{0}) \oplus_{\Theta}(\mathfrak{M}_{1}, \chi_{1})$ is defined as the $C$-colored structure $(\mathfrak{N}, \eta)$ such that
\begin{itemize}
	\item $\mathfrak{N}$ is the disjoint union of $\mathfrak{M}_{0}$ and $\mathfrak{M}_{1}$,
	\item and the additional application of the following operation afterwards: For every tuple $\bold{a} \in N^{n}$ with $n<\omega$, if $\Theta_{n}(\overline{I}; \overline{c}) = (d, S)$ where \[ I_{i} := \{ k < n \, | \, a_k \in M_{i} \} \quad \text{and} \quad c_{i} := \chi_{i}(\bold{a}|_{I_{i}}) \quad \text{for } i\in \{ 0, 1 \} \] we add $\bold{a}$ to all relations $R\in S$ and set the new color to $\eta(\bold{a})$.
\end{itemize}
Lastly, we introduce our basic $C$-colored structures, acting as our ground terms from the term point-of-view: Let $c_{n}\in C_{n}$ be a sequence of $C$-colors, then we denote by $\overline{c}$ the $C$-colored structure $(\mathfrak{D}, \zeta)$ whith the universe $D := \{ 0 \}$, empty relations $R^{\mathfrak{D}} = \emptyset$ and the unique $n$-tuple in $\mathfrak{D}$ being colored by $c_{n}$ for every $n<\omega$.

We introduce the signature $\mathcal{Y}^{<, 2}_{C, \tau}$ for a graded set of colors $C$ and a signature $\tau$ consisting of all operations of the form $\oplus_{\Theta}$ and $\overline{c}$.
We now can build terms over this signature that evaluate in the obvious way to $C$-colored structures.

As a last but very important preparation, we want to show, that our ``clique-width operations'' can be expressed by the operations of the signature $\mathcal{Y}^{2, <}_{C, \tau}$. For this we note several things: First our clique-width notion (and every clique-width notion in general) just utilizes unary colors, whereas terms from $\mathcal{Y}^{2, <}_{C, \tau}$ uses a range of multi-arity colors. This will not make much difference; intuitively we introduce just one ``dummy color'' for tuples of length bigger then $1$ and only properly utilize the unary ones.

First note, that clique-width terms consist of basic colored structures, disjoint unions, and, at least in the finite case, ``between'' two disjoint unions a finite sequence of the  unary ``add'' and ``recolor'' operations, i.e., given two graphs or colored structures $\mathfrak{M}_{0}, \mathfrak{M}_{1}$ we have something along the lines of \[ f_n ( f_{n-1} (\cdots f_1(\mathfrak{M}_{0}\oplus \mathfrak{M}_{1}))) \, , \] where $f_{1}, \ldots, f_{n}$ are among the unary operations $\recol{a\to b}{}$ and $\add{R, \vl}{}$ with $a, b$ colors, $\vl$ a tuple of colors of length $\arity{R}$ sucht that the given term is now a subterm issued from another disjoint union. Intuitively, we want to roll all those operations (the disjoint union $\mathfrak{M}_{0}\oplus \mathfrak{M}_{1}$ together with $f_n ( f_{n-1} (\cdots f_1()))$ into one operation via the updates). Lastly, note that even an infinite chain of unary operations here should be fine \thomas{(but this is subject to discussion, as it is not strictly needed!)}.

For a relational signature $\tau$ with maximal arity $m$ (if it is infinite we set $m=\omega$) and a finite(!) set of colors $K\subseteq \cols$ (for clique-width!), we define $C$ as a set of graded colors to be the (disjoint) union of the following sets:
\begin{itemize}
	\item $C_{0} = \{ \mathtt{d}_{0} \}$,
	\item $C_{1} = K$,
	\item $C_{i} = K^{i}$ for every $1 < i \le m$ (if $m$ is finite, else $i< m$)
	\item $C_{i} = \{ \mathtt{d}_{i} \}$ for every $m < i < \omega$ if $m$ is finite.
\end{itemize}
The only thing the $C_{i}$ for $i > 1$ do is to keep track of the individual color in the tuples. Nothing more.

\thomas{\textbf{Maybe this should be moved?} In the next step we ``translate'' our constant-symbols/basic-structures: $\unitn$: The associated coloring sequence $\overline{c}$ will consist of the following colors: $c_{0} = \mathtt{d}_{0}$, for $1< i \le m$ we have $c_{i} = (n, \ldots, n)$ and for $m < i$ we have $c_{i} = \mathtt{d}_{i}$. The associated basic-structure (hence the valuation on atomic terms) is obvious to define with the previous definitions.}

\textbf{The subsequent translation will not be that straight forward.}
We collect for the sequence $(f_i)_i$ in the set \[ ADD := \{ i < \omega \, | \, f_i = \add{R, \vl}{} \text{ for some } R\in\tau \text{ and } \vl\in C_{1}^{\arity{R}} \} \] all indices where an add-operation appears. Analogous, for the recoloring operations, let \[ REC := \{ i < \omega \, | \, f_i = \recol{a\to b}{} \text{ for some } a, b \in C_{1}^{\arity{R}} \} \, . \] 

For every $k\in ADD$ we define a binary relation $RT_{k}\subseteq C_{1}\times C_{1}$ called the \emph{recolor-trace} of the $k$-th operation and a set $CS_{k} \subseteq C_{1}\times C_{1}$ called the \emph{color-subsumption relation} of the $k$-th operation (which is an add-operation!) in the following way: Let $REC_{< k}$ be the set of all indices from $REC$ that are smaller then $k$. Let \[ a \to_{REC, <k} b \text{ iff } \exists i\in REC_{< k}. f_{i} = \recol{a\to b}{} \, .  \] 
Let $RT_{k}$ be defined as follows: $(a, b)\in RT_{k}$ iff there exists a maximal $\to_{REC, <k}$ path from $a$ to $b$ \textbf{or} $a = b$.
Hence $RT_{k}$ traces the complete color-changes that happen via recoloring operations until up to the $k$-th operation.
\begin{observation}
	$RT_{k}$ is  a functional binary relation, i.e. for every $a\in C_{1}$ there exists exactly one $b\in C_{1}$ such that $(a,b)\in RT_{k}$.
\end{observation}
\begin{proof}
	trivial.
\end{proof}
Note that we thus can also view $RT_{k}$ as a map $RT_{k}\colon C_{1} \to C_{1}$. This abuse of notation will be used in the future, so we say here that
\[ (a,b)\in RT_{k} \quad \text{iff} \quad RT_{k}(a) = b \] and the previous observation justifies this.
\begin{comment}
Then $RT_{k}$ is the transitive closure of $<_{rec}$. $RT_{k}$ thus collects all the pairs $(a,b)$ up until (and excluding) the $k$-th operation in the sequence, such that every $a$-colored element will be $b$-colored eventually during all the recoloring-operations appearing in the operations-sequence before the $k$-th operation.
\end{comment}
Suppose $f_{k} = \add{R, \vl}{}$, then \[ CS_{k} := \{ (c, l) \in RT_{k} \, | \, \exists i. l = \vl_i \} \, .\]
Now we have every tool together, to define some preliminary updates $\Theta^{(k)}$. The update-instructions come in several flavors.

\textbf{The case $n=0$ is trivial:} We only have $\overline{I} = (\emptyset, \emptyset)$, $\overline{c} = (\mathtt{d}_{0}, \mathtt{d}_{0})$ as arguments available. Hence:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{0}(\overline{I}; \overline{c}) &= (\mathtt{d}_{0}, \emptyset)
	\end{split}
\end{equation*}

\textbf{We now start properly with $n = 1$.} The arguments of $\Theta^{(k)}_{1}(\overline{I}; \overline{c})$ can only have the following forms:
\begin{itemize}
	\item Then $\overline{I} = ({0}, \emptyset)$ or $\overline{I} = (\emptyset, {0})$ and
	\item $\overline{c} = (c, \mathtt{d}_{0})$ or $\overline{c} = (\mathtt{d}_{0}, c)$ respectively with $c\in C_{1}$.
\end{itemize}
So we have to define the $(d,S)$ for $\Theta^{(k)}_{1}(\overline{I}; \overline{c}) = (d,S)$. This we do in the following fashion for which we have two cases:

\textbf{Case 1:} Suppose $R$ is unary. Then $\vl$ is actually a one-tuple $\vl = l\in C_{1}$. Then:
\begin{equation*}
	\begin{split}
	\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \{ R \}) \text{ iff } (c,d)\in RT_{k} \text{ and } d = l \\
	\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \text{ and } d \neq l \\
	\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \{ R \}) \text{ iff } (c,d)\in RT_{k} \text{ and } d = l \\
	\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \text{ and } d \neq l
	\end{split}
\end{equation*}
Those update-instructions do two things simultaneously: First we recolor all elements in one step to the color after every recoloring in our clique-width operation setup until step $k$ is done and secondly, we add at every node that was colored $l$ (either originally or after the previous recolorings) the unary relation $R$.

\textbf{Case 2:} Suppose $R$ is not unary. Then:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{1}((\{ 0 \}, \emptyset); (c, \mathtt{d}_{0})) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k} \\
		\Theta^{(k)}_{1}((\emptyset, \{ 0 \}); (\mathtt{d}_{0}, c)) &= (d, \emptyset) \text{ iff } (c,d)\in RT_{k}
	\end{split}
\end{equation*}
Here we just recolor.

\textbf{Suppose now that $m \ge n> 1$.} %Since we do not color tuples or length bigger then $1$, we simulate this by using a ``dead'' color $\mathtt{d}_{n}$. For every update-instruction we will now have $\Theta^{(k)}_{n}(\overline{I}, \overline{c}) = (\mathtt{d}_{n}, S)$, where we only need to concern ourselves with the definition of $S$ for each $n, \overline{I}, \overline{c}$.
Then for every $\overline{I}, \overline{c}$ we do the following: As we only have $2$-partitions of $[n]$, we only need to worry about $\overline{I} = (I_{0}, I_{1})$ and $\overline{c} = (c_{0}, c_{1})$ with $c_{i} \in C_{|I_{i}|}$. We will now define a color $c\in C_{n}$ that aims at ``shuffling" $c_{0}$ and $c_{1}$ together, so that the restriction on the indices in $|I_{0}|$ and $|I_{1}|$ respectively yield the colors $c_{0}$ and $c_{1}$ again, again respectively.For this, we will at first order naturally the numbers in $I_{0}$ and $I_{1}$ respectively by the relation $\prec_{0}$ and $\prec_{1}$. Then we bijectively map $(I_{i}, \prec_{i})$ to the unique initial segment of $(\omega, <)$ via $f_{i}$. $f_{i}$ will also be an order isomorphism. Lastly, interpreting the $c_{i}$ as maps themselves, we note, that their domain is the exact unique initial segment of $(\omega, <)$ that is isomorphic to $(I_{i}, \prec_{i})$. Hence we obtain in the first step two maps $h_{i} := c_{i} \circ f_{i}$ for $i\in \{ 0, 1 \}$ that associate to each number $i\in [n]$ seen as a position the corresponding unary color, which we implicitly keep track of in the case of colors of arity bigger then $1$. By taking the union of those maps (as there domains are disjoint, this is a unique extension of $h_{0}$ by $h_{1}$) we obtain a map $h_{\overline{I}; \overline{c}}$ that maps each ``position'' $i\in [n]$ to its corresponding color. Furthermore, this map gives as the ``shuffling'' we were so intent on looking for. Lastly, we can interpret $h_{\overline{I}; \overline{c}}$ itself as a $n$-tuple and hence by construction $h_{\overline{I}; \overline{c}}\in C_{n}$.

For the following note that after the previous discussion, we can obtain another $n$-tuple of colors from $h_{c}$ by ``applying'' the functional relation $RT_{k}$: $d = RT_{k}(h_{c}) = RT_{k} \circ h_{c}$. This will be our shorthand of describing the state of the individual $1$-colors being tracked by the $n$-color $h_{c}$ after all recoloring operations until the $k$-th operation in our sequence have been applied.
With this we now have only two cases to consider.

\textbf{Case 1:} $R$ is of arity $n$. Then $\vl$ is also a $n$-tuple, more precisely $\vl\in C_{n}$ by definition. Then for every $\overline{I}, \overline{c}$:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (RT_{k}(h_{\overline{I}; \overline{c}}), \{ R \}) \text{ iff }  RT_{k}(h_{\overline{I}; \overline{c}}) = \vl \\
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (d, \emptyset) \text{ iff }  RT_{k}(h_{\overline{I}; \overline{c}}) \neq l
	\end{split}
\end{equation*}

\textbf{Case 2:} $R$ is not of arity $n$. Then for every $\overline{I}, \overline{c}$:
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (d, \emptyset)
	\end{split}
\end{equation*}


\textbf{Lastly, for $n> m$}, the update instructions are even simpler. As we do not have any relational symbols of arity $n$ in this case, every update-instruction will give $\emptyset$ for the second component and $\mathtt{d}_{n}$ for the colorings. Formally, for every $\overline{I}, \overline{c}$ we have
\begin{equation*}
	\begin{split}
		\Theta^{(k)}_{n}(\overline{I}; \overline{c}) &= (\mathtt{d}_{n}, \emptyset)
	\end{split}
\end{equation*}

All in all this defines an ordered update $\Theta^{(k)} = \bigcup_{i<\omega}\Theta^{(k)}_{i}$. Unfortunately we are not done yet, since we define for every $k\in ADD$ such an ordered update, but our goal is to define it for the whole sequence. So here our definition will be:
\[ \Theta_{n}(\overline{I}, \overline{c}) := (d, S) \] where
\begin{itemize}
	\item $d = d^{(j)}$ for the smallest $j< \omega$ such that $\Theta^{(j)}_{n}(\overline{I}, \overline{c}) = (d^{(j)}, S_{j})$ and for every $i> k$ we have $\Theta^{(i)}_{n}(\overline{I}, \overline{c}) = (d^{(i)}, S_{i})$ with $d^{(j)} = d^{(i)}$ (in the finite case this is trivial, but in the infinite it is not much more difficult!\footnote{Every $n$-ary color depends on the finitely many colors in $C_{1}$. And the recolor-operations, when only sued for this finite set, can only make finitely many changes to the tuples until they have to stabilize!})
	\item $S = \bigcup_{i< \omega}S_{i}$ where $\Theta^{(i)}_{n}(\overline{I}, \overline{c}) = (d^{(i)}, S_{i})$.
\end{itemize}


Hence:
\begin{proposition}
	Clique-width terms (finite or infinite), can be expressed via the $\mathcal{Y}^{<, 2}_{C, \tau}$-terms.
\end{proposition}
\begin{proof}
	The definition of the valuation for partition-width terms is coincides with ours for the clique-width terms.
\end{proof}


\begin{lemma}
	Every countable structure $\mathfrak{M}$ with a bounded clique-width of $k$ has a bounded partition width.
\end{lemma}
\begin{proof}
	First we translate a clique-width term into a ``partition-width term''. Then we use the number of colors in our translation to obtain bounds on the partition-width via established results.
\end{proof}

\begin{theorem}
	\thomas{$\cw$ is an MSO-friendly width measure.}%Then the MSO-Theory of the class of all countable structures $\mathfrak{A}$ with $\cw{\mathfrak{A}}\le k$ is decidable.
\end{theorem}
\begin{proof}
	Use the result for partition-width with the previous lemma.
	\sebastian{Needs to be made more precise.}
\end{proof}

\begin{comment}
\subsection{Compactness: The countable case}

\thomas{\textbf{TODO:} We want to show the compactness for our clique-width definition in order to lift the more colloquial formulation as used by Grohe-Turan. For this we do in fact need the partition-width. Then we addapt the Courcelle-Compactness prove for partition-width over $2^{< \omega}$}

\thomas{\textbf{Proper TODO:}
\begin{itemize}
	\item Lift notion of syntax-tree to partition-width terms (i.e. $T(\mathcal{Y}^{<, 2}_{C, \tau})$ and $T^{\infty}(\mathcal{Y}^{<, 2}_{C, \tau})$)
	\item introduce order on syntax-trees
	\item show the ascending-chain-interpretation property for partition-width-terms
	\item need layouts
	\item flipping of number of types. Maybe we can use here results from Achim.
\end{itemize}}
\end{comment}

==> other/old-prelims.tex <==

\subsection{Logical Preliminaries}

\thomas{Question: Considering, that we have our ``meta-algebra'' over which we not only have the terms but also a algebra of structures, shouldn't we also kind of make a note on that somewhere? Technically we \textbf{do} work with functional signatures there.}
We make use of a first-order language that employs constant symbols, but no other function symbols. We let  $\conset := \{a,b,c,\ldots\}$ be a set of \emph{constants}, $\varset := \{x, y, z, \ldots\}$ be a set of \emph{variables}, and define a \emph{term} to be either a constant or variable. We use $t$, $s$, \etc (possibly annotated) to denote terms and define the set of terms $\termset := \conset \cup \varset$. Moreover, we let $\predset := \{p, q, r, \ldots\}$ be a set of \emph{predicates} containing infinitely many predicates for each arity $k \in \mathbb{N}$, using $\arity{p}$ to denote the arity of a predicate $p$, and refer to a formula of the form $p(t_{1}, \ldots, t_{k})$ (for $p$ a predicate of arity $k$ and $t_{1}, \ldots, t_{k}$ terms) as an \emph{atom}. Our first-order language is defined accordingly.


\begin{definition}[The Language $\lang$] We define the first-order \emph{language} $\lang$ to be the set of formulae generated via the BNF grammar shown below:
$$
A ::= p(t_{1}, \ldots, t_{n}) \ | \ \bot \ | \ A \land A \ | \ A \rightarrow A \ | \ \exists x A \ | \ \forall x A
$$
where $t_{i} \in \conset \cup \varset$ for each $i \in \{1, \ldots, n\}$, $x \in \varset$, and $p \in \predset$ is a predicate symbol such that $\arity{p} = k$.
\end{definition}
\thomas{Do we want to use capital-latin for formulae/sentences? Some prefer to use big-greek (more precisely $\Phi$ and $\Psi$) for sentences and small-greek (i.e. $\varphi$ and $\psi$) for non-sentence formulae (though I personally prefer the small-greek ones across the board for formulae!). This decision might have also an impact on naming rules, where $\varrho$ would be a naturally choice in the ``small-greek'' setting.}
\piotr{I think capital for sentences and small for other is quite clear. It is also nice to use capital letters for queries without explicitly naming free variables. For example $Q$ and $q(\vx)$}
We use $A$, $B$, $C$, $\ldots$ (possibly annotated) to denote formulae from our language and use $A(t/x)$ to denote the formula obtained by substituting the term $t$ for the each free occurrence of $x$ in $A$. Note, we assume that the reader is familiar with the concept of a free variable, bound variable, and occurrences thereof. Given a set of formulae $\formset \subseteq \lang$, we define $\conset(\formset)$, $\varset(\formset)$, $\termset(\formset)$, and $\predset(\formset)$ to be the set of constants, variables, terms, and predicates occurring in the formulae of $\formset$, respectively. When $\formset$ is a singleton $\{A\}$, we simply write $\conset(A)$, $\varset(A)$, $\termset(A)$, and $\predset(A)$, omitting the set brackets.





\begin{definition}[Structure, Environment, Model] We define a \emph{structure} to be an ordered pair $\struc := (\dom,\inter)$, where $\dom$ is a non-empty set called the \emph{domain} and $\inter$ is an \emph{assignment} such that 


\begin{itemize}

\item[(i)] for each constant symbol $c$, $\inter(c) \in \dom$;

\item[(ii)] for each predicate symbol $p$ with $\arity{p} = k$, $\inter(p) \subseteq \dom^{k}$.

\end{itemize}

An \emph{environment} $\env$ is a function such that for each variable $x$, $\env(x) \in \dom$ and we write $\env[d/x]$ to mean the environment $\env$ but where the variable $x$ is mapped to the element $d \in \dom$. Last, we define a \emph{model} to be an ordered pair $\model := (\struc, \env)$, where $\struc$ is a structure and $\env$ is an environment.

\end{definition}


\begin{definition}[Term Assignment] Let  $\model := (\struc, \env)$ be a model with $\struc := (\dom,\inter)$. We define the \emph{assignment} of a term $t$, written $\assign{t}^{\struc}_{\env}$, to be a function $\assign{\cdot}^{\struc}_{\env} : \conset \cup \varset \mapsto \dom$ defined as follows: 

\begin{itemize}

\item[(i)] if $t \in \conset$, then $\assign{t}^{\struc}_{\env} := \inter(t)$;

\item[(ii)] if $t \in \varset$, then $\assign{t}^{\struc}_{\env} := \env(t)$.

\end{itemize}
\end{definition}




\begin{definition}[Semantics] Let $\model := (\struc, \env)$ be a model with $\struc := (\dom, \inter)$.

\begin{itemize}

\item $\model \models p(t_{1}, \ldots, t_{n})$ \ifandonlyif $(\assign{t_{1}}^{\struc}_{\env}, \ldots, \assign{t_{n}}^{\struc}_{\env}) \in \inter(p)$;

\item $\model \not\models\bot$;

\item $\model \models A \land B$ \ifandonlyif $\model \models A$ and $\model \models B$;

\item $\model \models A \rightarrow B$ \ifandonlyif if $\model \models A$, then $\model \models B$;

\item $\model \models \exists x A$ \ifandonlyif there exists an element $d \in \dom$ such that $(\struc,\env[d/x]) \models A$.

\item $\model \models \forall x A$ \ifandonlyif for each element $d \in \dom$, $(\struc,\env[d/x]) \models A$.

\end{itemize}

We say that a formula $A$ is \emph{valid} \ifandonlyif for all models $\model$, $\model \models A$. We say that a multiset $\formset$ of formulae \emph{entails} a multiset $\formsetii$, written $\formset \models \formsetii$, \ifandonlyif for all models $\model$, if $\model \models A$ for all $A \in \formset$, there exists a formula $B \in \formsetii$ such that $\model \models B$.
\end{definition}



\subsection{Existential Rule Preliminaries}

We define a \emph{conjunct} $C(\vec{x})$ to be a conjunction of atoms, where $\vec{x}$ represents the set of all variables $x_{1}, \ldots, x_{n}$ occurring in $C$. Also, we define a \emph{fact} and a \emph{Boolean conjunctive query (BCQ)} to be an existentially closed conjunct, and so, although facts are used to model data and BCQs are used to model queries, both have the same logical form. In the following, we will often view conjuncts, facts, and BCQs as sets of atoms, and will use $C$, $F$, and $Q$ (possibly annotated) to denote each type of entity, respectively.

\begin{definition}[Existential Rule] We define an \emph{existential rule (ER)} to be a formula of the form $R := \forall \vec{x} \forall \vec{y} (B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}))$ where $B := \body(R)$ and $H := \head(R)$ are conjuncts, referred to as the \emph{head} and the \emph{body} of $R$, respectively. The \emph{frontier} of $R$, written $\fr(R)$, is the set of variables $\varset(H) \cap \varset(B) = \vec{y}$.
\end{definition}

In practice, we will omit the universal quantifiers when writing existential rules, i.e. instead of writing $\forall \vec{x} \forall \vec{y} (B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}))$ we will write $B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})$.

\begin{definition}[Substitution, Homomorphism] Given a set of variables $V$ and a set of terms $T$, a \emph{substitution} $\hism$ is a mapping $\hism : V \mapsto T$, and given a formula $A$, $\hism(A)$ is the formula obtained by replacing each occurrence of a free variable $x \in V$ in $A$ with $\hism(x)$.

A \emph{safe substitution} is a bijection from a set of variables $V$ to a set of fresh variables, that is, to a set of variables that do not occur within the formulae one is considering.

Given two facts $F$ and $Q$, a \emph{homomorphism} from $Q$ to $F$ is a substitution $\hism : \varset(Q) \mapsto \termset(F)$ such that $\hism(Q) \subseteq F$. We say that $Q$ \emph{maps to} $F$ \ifandonlyif there exists a homomorphism from $Q$ to $F$.
\end{definition}



\begin{definition}[Forward Chaining Terminology]
\piotr{We need a way to refer to elements of $\sat{R, A}$, I propose to call them {\em atoms}}

\piotr{We need to define what a Datalog rule is.}

\piotr{Make sure that restricted chase vs oblivious chase is explained somewhere.}

\piotr{Make sure that we use restricted chase.}

We say that an existential rule $R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})$ is \emph{applicable} to a fact $F$ \ifandonlyif there is a homomorphism $\hism$ mapping $B(\vec{x},\vec{y})$ to $F$. The \emph{application of $R$ to $F$ according to $\hism$} yields the fact $\fchain{F,R,\hism} = F \cup \hism(\hism'(H(\vec{y},\vec{z})))$, where $\hism'$ is a safe substitution on the variables $\vec{z}$. (NB. We often use $\hism^{\safe}$ to denote the composition $\hism \circ \hism'$.) An application of $R$ to $F$ according to $\hism$ is \emph{redundant} \ifandonlyif $\fchain{F,R,\hism} \equiv F$. 

An \emph{$\calr$-derivation} is a sequence $(F = F_{0}), (R_{0},\hism_{0},F_{1}), \ldots, (R_{n-1},\hism_{n-1},F_{n})$ such that for all $i \in \{0, \ldots, n-1\}$, $R_{i} \in \calr$ and $\pi_{i}$ is a homomorphism from $\body(R_{i})$ to $F_{i}$ such that $F_{i+1} = \fchain{F_{i}, R_{i}, \hism_{i}}$. We say that a fact $F'$ is \emph{$\calr$-derivable} from a fact $F$ \ifandonlyif there exists a derivation sequence starting with $F$ and ending with $F'$.
\end{definition}


\begin{definition}[$k$-Saturation~\cite{BagLecMugSal11}] Let $F$ be a fact with $\calr$ a set of ERs. We define:
$$
\Pi(\calr,F) := \{(R,\hism) \ | \ R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z}) \text{ and }
$$
$$
\hism \text{ is a homomorphism from $B$ to $F$.} \}
$$
We define the \emph{direct saturation} of $F$ with $\calr$ to be:
$$
\fchain{F,\calr} := F \cup \bigcup_{(R,\hism) \in \Pi(\calr,F)} \hism^{\safe}(H(\vec{y},\vec{z})) \text{ with } R = B(\vec{x},\vec{y}) \rightarrow \exists \vec{z} H(\vec{y},\vec{z})
$$
We define the \emph{$k$-saturation} of $F$ with $\calr$ to be $\ksat{k}{F,\calr}$, which is inductively defined as follows:
$$
\ksat{0}{F,\calr} = F \text{ and, for $i > 0$, } \ksat{i}{F,\calr} = \fchain{\ksat{i-1}{F,\calr},\calr}
$$
Last, we define $\ksat{\infty}{F,\calr} := \bigcup_{k \in \mathbb{N}} \ksat{k}{F,\calr}$.
\end{definition}

A \emph{knowledge base (KB)} $\kb := (F,\calr)$ is an ordered pair composed of a fact $F$ and a finite set of existential rules $\calr$. We use the notation $\kb \models Q$ as shorthand for $F,\calr \models Q$. The \emph{BCQ entailment} problem is the following: given a KB $\kb$ and a BCQ $Q$, is it the case that $\kb \models Q$?









==> other/tree-width.tex <==
\medskip \noindent {\bf Treewidth and bounded treewidth sets.}
Let $\inst$ be an instance. A \emph{tree decomposition} of $\inst$ is a (potentially infinite) tree $\tree = (V,E)$ with $V \subseteq 2^{\adom{\inst}}$, where:
\begin{itemize}

\item each $X \in V$ is a set of terms of $\inst$ with $\bigcup_{X \in V} X = \adom{\inst}$;

\item for each atom $p(t_{1}, \ldots,t_{n})$ in $\inst$, there is an $X \in V$ such that $\{t_{1}, \ldots,t_{n}\} \subseteq X$;

\item for each term $t$ in $\inst$, the subgraph of $T$ induced by the nodes $X$ with $t \in X$ is connected.
\end{itemize}

We define the \emph{width} of a tree decomposition to be equal to the largest node minus 1. Last, we define the \emph{treewidth} of an instance $\inst$ to be the minimal width among all of its tree decompositions, and denote the treewidth of $\inst$ as $\treewidth{\inst}$.


%\thomas{``semantic $\bts$?''}
%\begin{definition}[Bounded-treewidth set]

We define a set of existential rules $\ruleset$ to be a \emph{bounded-treewidth set ($\bts$)} \ifandonlyif for any database $\database$, there is a universal model for $\database$ and $\ruleset$ of finite treewidth.\footnote{We note that the term ``\emph{finite} treewidth set'' might be more appropriate and coherent with our terminology, but we stick to the established name. Also, the $\bts$ notion is not used entirely consistently in the literature; it sometimes also refers to structural properties of a specific type of chase. The ``semantic $\bts$'' notion adopted here subsumes all the others.}
%\end{definition}

==> other/very-old-clique-width.tex <==
\section{Clique-width and Related Notions}\label{sec:cliquewidth}


\thomas{One thing to think about: I would lobby for following Courcelle and look at \emph{isomorphy-classes} of colored structures! This should also help us make our algebra of colored structures work the way we actually want to.}
We define a \emph{signature} $\sig$ to be a pair $(P,ar)$ such that $P \subseteq \predset$ and $ar$ is the arity function restricted to $P$. When $\sig = (P,ar)$, we write $p \in \sig$ to mean $p \in P$. Moreover, we let $\langsig$ denote the restriction of our language $\lang$ to the use of predicates from the signature $\sig$.

\begin{definition}[Colored Relational Structure] Let $\sig$ be a signature. We define a \emph{relational structure} $\relstr$ to be a pair $(V,\{E_{p} \ | \ p \in \sig\})$ where $V$ is a non-empty set of points called \emph{vertices} and for each $p \in \sig$, $E_{p} \subseteq V^{\arity{p}}$. We define a \emph{colored relational structure} $\crelstr$ to be a pair $(\relstr, \coloring)$ such that $\relstr = (V,\{E_{p} \ | \ p \in \sig\})$ is a relational structure and $\coloring : V \to \mathbb{L}$ is a \emph{coloring} mapping each vertex $V$ to an element of some countably infinite set of colors $\cols$. The set of all finite relational structures over signature $\sig$ and the set of colors $\cols$ will be denoted with $\colstructs$.
\end{definition}

\thomas{A note on ``expressivity'' of ``our'' clique-width notion in relation to partition width: Take an infinite linear order (for example $(\mathbb{Q}, <)$ with the usual ordering). Then add the following inbetweenness relation $R$ to the structure with \[ R = \{ (x,y,z) \, | \, x < y < z \} \]. Then the structure $(\mathbb{Q}, <, R)$ has infinite ``unitarily colored'' width (i.e., our clique-width for example) and finite partition-width. This proofs that partition width is strictly more expressive (or more precisely that \emph{bounded} partition-width captures more structures). I admit, that at the top of my head I do not see a partition-refinement, that might help with getting a finite partition-width here (I am probably just dense and thus see the fact that $\mathbb{Q}$ is dense too as a problem...).}

\begin{definition}[Number of Colors] Let $\crelstr = (\relstr, \coloring)$ be a colored relational structure. The \emph{number of colors} of $\crelstr$ is defined to be $\numcolors{\crelstr} := |image(\coloring)|$.
\end{definition}

Let us now describe how colored relational structures are built from atomic graphs (referred to as \emph{units}) by making use of special operations. We define the \emph{n-unit} colored relational structure as follows:
\thomas{Is ``n-unit colored...'' good? Because we actually color that unit-structure with the color $n$.}
\piotr{I do not understand this comment :/}
\thomas{It sounds like the $n$ is part of the ``unit'' and not associated with the ``colored'' part. I am not sure about a change like saying ``unit $n$-colored'' structure, but that would at least communicate way I felt to make the comment in the first place. The problem with this ``new'' option is however, that now the $n$ seems more rigid then in the proposed version (where having it in front of the unit makes it ``feel'' more dynamic). Still... ``$n$-unit colored'' kind of throws me off a bit.}
\piotr{ok, I would not worry about that, n-unit colored is fine}
\thomas{probably yes. Kind of funny to observe other authors write their texts in real time.}
\piotr{:D}
\piotr{I am going to use your idea from the very long green comment, and this part is going into prelims}\piotr{I am taking it back, I will use what Tim wrote, adjust it and put into preliminaries. The thing is, that we need an "easy to understand" definition rather than "beautiful"}
$$
\unitn := (V,\{E_{p} \ | \ p \in \sig\},\coloring)
$$
where $V = \{\unit\}$, $E_{p} = \emptyset$ for each $p \in \sig$, and $\coloring(\unit) = n$. Furthermore, while constructing colored relational structures, we will use the \emph{disjoint union} $\disun$ of two colored relational structures $\crelstr = (V,\{E_{p} \ | \ p \in \sig\}, \coloring)$ and $\crelstr' = (V',\{E_{p}' \ | \ p \in \sig\}, \coloring')$, defined as follows:
$$
\crelstr \disun \crelstr' = (V \cup V', \{E_{p} \cup E_{p}' \ | \ p \in \sig\}, \coloring \cup \coloring')
$$
where we assume that $V \cap V' = \emptyset$.

The \emph{add} operation, which adds hyper-edges to a colored relational structure given that such hyper-edges satisfy a certain coloring of vertices, requires the use of sequences of natural numbers from $\mathbb{N}^{k}$. We will often use $\vec{n}$ as shorthand for a sequence $(n_{1}, \ldots, n_{k})$ and let $\length{\vec{n}}$ denote the length of the sequence, i.e. for $\vec{n} = (n_{1}, \ldots, n_{k})$, $\length{\vec{n}} = k$. Similarly, we use $\vec{v}$ to represent a sequence of vertices $(v_{1}, \ldots, v_{k})$ from a given (colored) relational structure, and for a coloring $\coloring$, we define $\coloring(\vec{v}) = (\coloring(v_{1}), \ldots, \coloring(v_{k}))$ to be the coloring applied componentwise. We now define the add operation
$$
\add{p}{(V,\{E_{p} \ | \ p \in \sig\},\coloring),\vec{n}} = (V,\{E_{p}' \ | \ p \in \sig\},\coloring)
$$
where $\length{\vec{n}} = \arity{p}$ and
\[
  E_{\relstr}' =
  \begin{cases}
       E_{\relstr} & \text{if $r \in \sig \setminus \{p\}$} \\
       E_{p} \cup \{\vec{v} \in V^{\arity{p}} \ |\ \coloring(\vec{v}) = \vec{n} \} & \text{otherwise.}
  \end{cases}
\]

Last, we define the \emph{recolor} operation which takes a function $h : \mathbb{N} \to \mathbb{N}$ such that $|\{n \in \mathbb{N} \ | \ h(n) \neq n\}|$ is finite and applies it to the coloring of a given colored relational structure:
$$
\recol{h}{(\relstr,\coloring)} = (\relstr,h \fcomp \coloring)
$$

\thomas{In the following block I might have a completely different idea. First of all, if we are talking about terms and the term-algebra it would be a better idea to not bring up any interpretation of the symbols, as terms in the term-algebra are purely syntactic objects devoid of meaning (looking at ``$\unitn$ is among the set...''). We thus have to do the following:
\begin{enumerate}
    \item disambiguate between the \emph{syntactic object} $\unitn$ which is ``just a symbol'' and
    \item its interpretation in the algebra of structures by means of the \emph{structure} $\unitn$.
\end{enumerate}
Then there is the nice property, that the term-algebra (over the generating set described by the constant symbols, which are the ``syntactic'' $\unitn$) is actually \emph{the} free algebra over that generating set (up to isomorphism). This entails that every map from the generating set into every algebra with the same signature (that map has to be the one sending syntactic-$\unitn$ to the structure (or ``semantic'') $\unitn$ to ensure what I will now say about homomorphisms) can be \emph{uniquely} extended to a homomorphism from the term-algebra into and onto our algebra of structures (we assume every structure to be constructible by our operations which they are, especially the finite ones). In fact that very homomorphism \emph{is} our valuation map. The recursive definition is baked into the fact that we work with the term-algebra which is the free-algebra in our setting. Note:
\begin{enumerate}
    \item The term-algebra used here does \emph{not} make use of variable symbols! We are only working on grounded terms.
    \item This might be a hurdle for infinite structures!
    \item Maybe use superscripts to signify interpretations of symbols in a specific structure.
\end{enumerate}
\textbf{Bonus remark:} Refers actually to the Definition of Environment, Model and to some extend Term Assignments. Do we really want to have the environments in the definition of models? They seem to assign to each variable symbol a domain element. This feels like a ``very dynamic'' way to define a model to be a bit euphemistic. On the other hand, $\xi[d/x]$ seems weird, because one could possibly think about $x$ being substituted by $d$ (and some authors use that even the other way round!). And that would not make much sense as $\xi$ is a map with domain the variables!}
Let us now introduce \emph{colored relational structure terms (CRS-terms)}, which will be evaluated over the class of colored relational structures. Such terms are crucial for defining the clique-width of relational structures. Such terms are defined via the following grammar in BNF:
$$
\term ::= \unitn \ | \ \term \disun \term \ | \ \add{p,\vec{n}}{T} \ | \ \recol{h}{T}
$$
where $\unitn$ is among the set $\{\unitn \ | \ n \in \mathbb{N}\}$, $p \in \sig$, $\vec{n}$ is among the finite sequences of natural numbers \thomas{$\vec{n}$ is a sequence of natrual numbers of length arity of $p$!}, and $h$ is a name from a countable set of names (disjoint from all previously mentioned symbols). The value of a term is defined as follows:

\begin{definition}[Value] We define the \emph{value} $\val{\term}$ of a CRS-term $\term$ recursively on the structure of the term such that $\val{\unitn} = \unitn$, $\val{\term \disun \term'} = \val{\term} \disun \val{\term'}$, $\val{\add{p,\vec{n}}{\term}} = \add{p,\vec{n}}{\val{\term}}$, and $\val{\recol{h}{\term}} = \recol{h}{\val{\term}}$.
\end{definition}

We use $\term \sqsubseteq \term'$ to indicate that $\term$ is a sub-term of $\term'$.

\begin{definition}[Clique-width] We define the \emph{clique-width of a CRS-term} as
$$
\cw{\term} = \sup\{\numcolors{\val{\term}} \ | \ \term' \subterm \term \}.
$$
The \emph{clique-width of a relational structure} is defined as
$$
\cw{\relstr} = \inf\{n \in \mathbb{N} \ | \ \exists \term, \exists \coloring (\val{\term} = (\relstr,\coloring) \text{ and } \cw{T} = n)\}.
$$
\end{definition}

\thomas{Though I think that, considered the ``boundedness behavior'' our clique-width definition is equivalent to the one by Courcelle, we probably should still at least note or, even better, proof that they relate ``close enough''. My initial guess is probably again a upper bound of twice ``our'' clique-width and a lower bound of ``our'' clique-width for the ``Courcelle clique-width''. Still we introduce a ``new'' notion of clique-width and it would be good to have that covered.}

\begin{observation}\label{obs:cross-coloring}
Let $\struc$ be a relational structure, let $\coloring : dom(\struc) \to \cols$ and $\coloring' : dom(\struc) \to \cols'$ be two coloring functions, where $\cols$ and $\cols'$ are some sets of colors. If $\cw{\struc, \coloring} = k$ and $\cw{\struc, \coloring'} = k'$ then $\cw{\struc, \coloring^{\times}} \leq k \cdot k'$ where $\coloring^{\times}(a) = (\coloring(a), \coloring'(a))$.
\end{observation}
\begin{proof}
\piotr{easy, TODO}
\end{proof}

\begin{observation}\label{obs:trees_cw_le3}
Let $\struc$ be a (rooted and directed) tree. Then $\cw{\struc} \le 3$.
\end{observation}
\begin{proof}
\thomas{easy, sketched in the following:} Construct the tree in a bottom up fashion. Introduce the leafs as a specific color (let's say \textcolor{blue}{blue}). Then add those nodes in \textcolor{red}{red} that are ``complete parent nodes'' of already ``existing'' nodes (i.e. we want to have subtrees of the whole tree with height $1$ (or $2$ depending on the readers fancy of defining tree-height)). Connect \textcolor{red}{red} to \textcolor{blue}{blue}.
Now do recursively/inductively the following: Add the nest layer of ``complete parents'' in \textcolor{thomas}{green}, connect \textcolor{thomas}{green} to \textcolor{red}{red} and recolor \textcolor{red}{red} to \textcolor{blue}{blue} and \textcolor{thomas}{green} to \textcolor{red}{red}. We are done, when the root of the (directed) tree is added.
All in all we only use $3$ colors and hence have clique-width $\le 3$.
\textbf{Very important note:} The tree structure of the given tree has to be essentially completely copied for the syntax-tree of the clique-width term! This means, we do those iterations on specific disjoint parts of the tree kind of ``in parallel''. The clique-width term will be, written as its syntax tree, only the same tree as the original one if one ``ignores'' the recoloring operations (they just add very short paths between nodes of the tree). That's why it also is just a sketch (because one could get the idea, that all leaves will be connected to one parent note in the first step and the rest would be superfluous drivel).
\end{proof}
\thomas{As a side-note: In the undirected case one could use a result from Courcelle (findable in ``The Book'') which states in that case that the clique-width is bounded on the upper side by $3\cdot 2^{\treewidth{\struc} - 1}$. Then use that the tree-width of a tree is $1$. In general this does not hold for the directed case, but as seen in the sketch, it should work with directed/rooted trees just fine.}
